Effect of Contact Inhibition Locomotion on confined cellular organization

Experiments performed using micro-patterned one dimensional collision assays have allowed a precise quantitative analysis of the collective manifestation of contact inhibition locomotion (CIL) wherein, individual migrating cells reorient their direction of motion when they come in contact with other cells. Inspired by these experiments, we present a discrete, minimal 1D Active spin model that mimics the CIL interaction between cells in one dimensional channels. We analyze the emergent collective behaviour of migrating cells in such confined geometries, as well as the sensitivity of the emergent patterns to driving forces that couple to cell motion. In the absence of vacancies, akin to dense cell packing, the translation dynamics is arrested and the model reduces to an equilibrium spin model which can be solved exactly. In the presence of vacancies, the interplay of activity-driven translation, cell polarity switching, and CIL results in an exponential steady cluster size distribution. We define a dimensionless P\'eclet number Q - the ratio of the translation rate and directional switching rate of particles in the absence of CIL. While the average cluster size increases monotonically as a function of Q, it exhibits a non-monotonic dependence on CIL strength, when the Q is sufficiently high. In the high Q limit, an analytical form of average cluster size can be obtained approximately by effectively mapping the system to an equivalent equilibrium process involving clusters of different sizes wherein the cluster size distribution is obtained by minimizing an effective Helmholtz free energy for the system. The resultant prediction of exponential dependence on CIL strength of the average cluster size and Q^{1/2} dependence of the average cluster size is borne out to reasonable accuracy as long as the CIL strength is not very large.

==> jabbrv-ltwa-all.ldf.tex <==
%% Copyright 2010-2019 Erich E. Hoover
%% E-mail: erich.e.hoover@gmail.com
%% 
%% =============================================
%% IMPORTANT NOTICE:
%% 
%% This work may be distributed and/or modified under the conditions
%% of the LaTeX Project Public License, either version 1.3c of this
%% license or (at your option) any later version.
%% The latest version of this license is available at
%%   http://www.latex-project.org/lppl.txt
%% =============================================
%% The List of Title Word Abbreviations below is automatically
%% generated from the ISSN LTWA database, publicly accessible from
%% their website:
%%   http://www.issn.org/2-22660-LTWA.php

\DefineJournalPartialAbbreviation{Abhor}{Abhor}
\DefineJournalAbbreviation{Abolition}{Abolit}
\DefineJournalWordException{Abscence}{Abscence}
\DefineJournalPartialAbbreviation{Absol\^ut}{Absol}
\DefineJournalPartialAbbreviation{Accent}{Accent}
\DefineJournalPartialAbbreviation{Accessib}{Access}
\DefineJournalPartialAbbreviation{Accompl}{Accompl}
\DefineJournalAbbreviation{Accumulation}{Accumul}
\DefineJournalWordException{A\c cores}{A\c cores}
\DefineJournalWordException{Actinidia}{Actinidia}
\DefineJournalAbbreviation{Adjacent}{Adjac}
\DefineJournalPartialAbbreviation{Administr}{Adm}
\DefineJournalPartialAbbreviation{Admit}{Admit}
\DefineJournalWordException{Adonis}{Adonis}
\DefineJournalPartialAbbreviation{Adopt}{Adopt}
\DefineJournalPartialAbbreviation{Adress}{Adress}
\DefineJournalPartialAbbreviation{Adriatic}{Adriat}
\DefineJournalPartialAbbreviation{Advokat}{Advok}
\DefineJournalPartialAbbreviation{Aerodynam}{Aerodyn}
\DefineJournalPartialAbbreviation{A\`erolog}{Aerol}
\DefineJournalPartialAbbreviation{Aeronauti}{Aeronaut}
\DefineJournalPartialAbbreviation{Aeronom}{Aeron}
\DefineJournalPartialAbbreviation{Aerophotograph}{Aerophotogr}
\DefineJournalPartialAbbreviation{Aeroport}{Aeropt}
\DefineJournalPartialAbbreviation{Aerotechni}{Aerotech}
\DefineJournalPartialAbbreviation{Aftos}{Aft}
\DefineJournalPartialAbbreviation{Agil}{Agil}
\DefineJournalPartialAbbreviation{Agressolog}{Agressol}
\DefineJournalPartialAbbreviation{Agrobiolog}{Agrobiol}
\DefineJournalPartialAbbreviation{Agrobotan}{Agrobot}
\DefineJournalPartialAbbreviation{Agrogeolog}{Agrogeol}
\DefineJournalPartialAbbreviation{Agrolog}{Agrol}
\DefineJournalPartialAbbreviation{Agromeliora}{Agromelior}
\DefineJournalPartialAbbreviation{Agronom}{Agron}
\DefineJournalPartialAbbreviation{Agrotechni}{Agrotech}
\DefineJournalWordException{Ahmadu}{Ahmadu}
\DefineJournalWordException{A\"ikido}{A\"ikido}
\DefineJournalPartialAbbreviation{Aktual}{Aktual}
\DefineJournalAbbreviation{Akutan}{Akut}
\DefineJournalAbbreviation{Alaska}{Alsk}
\DefineJournalWordException{Albatros}{Albatros}
\DefineJournalWordException{Albedo}{Albedo}
\DefineJournalWordException{Albert}{Albert}
\DefineJournalPartialAbbreviation{Alcover}{Alcover}
\DefineJournalWordException{Alcuin}{Alcuin}
\DefineJournalAbbreviation{Alexandria}{Alex}
\DefineJournalWordException{Alfalfa}{Alfalfa}
\DefineJournalPartialAbbreviation{\'Algebr}{Algebr}
\DefineJournalPartialAbbreviation{Al'golog}{Algol}
\DefineJournalPartialAbbreviation{Algoritm}{Algoritm}
\DefineJournalPartialAbbreviation{Aliment}{Aliment}
\DefineJournalPartialAbbreviation{Allergolog}{Allergol}
\DefineJournalWordException{Almamater}{Almamater}
\DefineJournalWordException{Alzheimer}{Alzheimer}
\DefineJournalAbbreviation{\"Ambetsmannakommitt\'en}{\"Ambetsmannakomm}
\DefineJournalPartialAbbreviation{Amelior}{Amelior}
\DefineJournalPartialAbbreviation{Amerik}{Am}
\DefineJournalPartialAbbreviation{Amfib}{Amfib}
\DefineJournalWordException{Amoeba}{Amoeba}
\DefineJournalPartialAbbreviation{Ampelolog}{Ampelol}
\DefineJournalPartialAbbreviation{Amphibi}{Amphib}
%\DefineJournalPartialWordException{Amput}{Amput-}
\DefineJournalPartialAbbreviation{Anabaptis}{Anabapt}
\DefineJournalPartialAbbreviation{Analges}{Analg}
\DefineJournalPartialAbbreviation{Analog}{Analog}
\DefineJournalPartialAbbreviation{Analys}{Anal}
\DefineJournalPartialAbbreviation{Anamnes}{Anamn}
\DefineJournalPartialAbbreviation{Anatomi}{Anat}
\DefineJournalWordException{Ancestral}{Ancestral}
\DefineJournalWordException{Andes}{Andes}
\DefineJournalPartialAbbreviation{Angeiolog}{Angeiol}
\DefineJournalPartialAbbreviation{Angiolog}{Angiol}
\DefineJournalAbbreviation{Anglia}{Angl}
\DefineJournalWordException{Angora}{Angora}
\DefineJournalPartialAbbreviation{Annex}{Annex}
\DefineJournalPartialAbbreviation{Anorgani}{Anorg}
\DefineJournalPartialAbbreviation{Antagonism}{Antagon}
%\DefineJournalPartialWordException{Antananariv}{Antananariv-}
\DefineJournalPartialAbbreviation{Antholog}{Anthol}
\DefineJournalPartialAbbreviation{Anthropolog}{Anthropol}
\DefineJournalPartialAbbreviation{Anthroposophisch}{Anthropos}
\DefineJournalPartialAbbreviation{Antiandrogen}{Antiandrog}
\DefineJournalPartialAbbreviation{Antibioti}{Antibiot}
\DefineJournalPartialAbbreviation{Anticoncept}{Anticoncept}
\DefineJournalPartialAbbreviation{Antimetaboli}{Antimetab}
\DefineJournalPartialAbbreviation{Antiparasit}{Antiparasit}
\DefineJournalPartialAbbreviation{Antitermit}{Antitermit}
\DefineJournalPartialAbbreviation{Aphidol}{Aphidol}
\DefineJournalPartialAbbreviation{Appendi}{Append}
\DefineJournalPartialAbbreviation{Aquisi}{Aquis}
\DefineJournalPartialAbbreviation{Arab}{Arab}
\DefineJournalPartialAbbreviation{Arachnolog}{Arachnol}
\DefineJournalPartialAbbreviation{Arbitra}{Arbitr}
\DefineJournalPartialAbbreviation{Archiv}{Arch}
\DefineJournalWordException{Arena}{Arena}
\DefineJournalPartialAbbreviation{Argentin}{Argent}
\DefineJournalAbbreviation{Argus}{Arg}
\DefineJournalWordException{Ariadne}{Ariadne}
\DefineJournalPartialAbbreviation{Aromati}{Aromat}
\DefineJournalAbbreviation{Arsenic}{Arsen}
\DefineJournalPartialAbbreviation{Arteri}{Arter}
\DefineJournalAbbreviation{Articole}{Artic}
\DefineJournalPartialAbbreviation{Artik}{Artik}
\DefineJournalPartialAbbreviation{Artist}{Artist}
\DefineJournalPartialAbbreviation{Ascens}{Ascens}
\DefineJournalPartialAbbreviation{Asceti}{Ascet}
\DefineJournalPartialAbbreviation{Asphalt}{Asph}
\DefineJournalPartialAbbreviation{Aspirant}{Aspir}
\DefineJournalPartialAbbreviation{Assist}{Assist}
\DefineJournalWordException{Astra}{Astra}
\DefineJournalPartialAbbreviation{Astrobotan}{Astrobot}
\DefineJournalPartialAbbreviation{Astrolog}{Astrol}
\DefineJournalPartialAbbreviation{Astronaut}{Astronaut}
\DefineJournalPartialAbbreviation{Astronom}{Astron}
\DefineJournalPartialAbbreviation{Astrophys}{Astrophys}
\DefineJournalWordException{Atlantis}{Atlantis}
\DefineJournalPartialAbbreviation{Atomapsorbtion}{Atomapsorbt}
\DefineJournalPartialAbbreviation{Atomi}{At}
\DefineJournalPartialAbbreviation{Atomo}{At}
\DefineJournalPartialAbbreviation{Attrib}{Attrib}
\DefineJournalPartialAbbreviation{Audiolog}{Audiol}
\DefineJournalPartialAbbreviation{Augment}{Augment}
\DefineJournalWordException{Aurore}{Aurore}
\DefineJournalPartialAbbreviation{Australi}{Aust}
\DefineJournalWordException{Autisme}{Autisme}
%\DefineJournalPartialWordException{Autobus}{Autobus-}
\DefineJournalPartialAbbreviation{Automat}{Autom}
\DefineJournalPartialAbbreviation{Autonom}{Auton}
\DefineJournalPartialAbbreviation{Autoradiograph}{Autoradiogr}
\DefineJournalPartialAbbreviation{Autoris}{Aut}
\DefineJournalPartialAbbreviation{Autotransp}{Autotransp}
\DefineJournalPartialAbbreviation{Auxolog}{Auxol}
\DefineJournalWordException{Avalanche}{Avalanche}
\DefineJournalWordException{Avatar}{Avatar}
\DefineJournalWordException{Avesta}{Avesta}
\DefineJournalPartialAbbreviation{Avicult}{Avic}
\DefineJournalWordException{Azania}{Azania}
\DefineJournalPartialAbbreviation{Azur}{Azur}
\DefineJournalWordException{Bahrein}{Bahrein}
\DefineJournalPartialAbbreviation{Balan\c c}{Balanc}
\DefineJournalPartialAbbreviation{Ballot}{Ballot}
\DefineJournalWordException{Balsa}{Balsa}
\DefineJournalPartialAbbreviation{Balti}{Balt}
\DefineJournalWordException{Banane}{Banane}
\DefineJournalAbbreviation{Bangkok}{Bangk}
\DefineJournalWordException{Bangladesh}{Bangladesh}
\DefineJournalPartialAbbreviation{Baromet}{Barom}
\DefineJournalWordException{Basico}{Basico}
\DefineJournalWordException{Basket}{Basket}
\DefineJournalWordException{Battelle}{Battelle}
\DefineJournalWordException{Belize}{Belize}
\DefineJournalWordException{Belleville}{Belleville}
\DefineJournalPartialAbbreviation{Benedict}{Benedict}
\DefineJournalWordException{Benelux}{Benelux}
\DefineJournalWordException{Bhagavadgita}{Bhagavadgita}
\DefineJournalWordException{Biathlon}{Biathlon}
\DefineJournalWordException{Bible}{Bible}
\DefineJournalPartialAbbreviation{Bibliograph}{Bibliogr}
\DefineJournalAbbreviation{Bifurcation}{Bifurc}
\DefineJournalWordException{Billion}{Billion}
\DefineJournalPartialAbbreviation{Biochronometr}{Biochronom}
\DefineJournalPartialAbbreviation{Biocoordinat}{Biocoord}
\DefineJournalPartialAbbreviation{Bioenerget}{Bioenerg}
\DefineJournalPartialAbbreviation{Bioepistemolog}{Bioepistemol}
\DefineJournalPartialAbbreviation{Biogen}{Biog}
\DefineJournalPartialAbbreviation{Biogeograph}{Biogeogr}
\DefineJournalPartialAbbreviation{Biograph}{Biogr}
\DefineJournalPartialAbbreviation{B\`iolog}{Biol}
\DefineJournalPartialAbbreviation{Biomaterial}{Biomater}
\DefineJournalPartialAbbreviation{Biomathemat}{Biomath}
\DefineJournalPartialAbbreviation{Biomechani}{Biomech}
\DefineJournalPartialAbbreviation{Biometeorolog}{Biometeorol}
\DefineJournalPartialAbbreviation{Biometri}{Biom}
\DefineJournalPartialAbbreviation{Biomineral}{Biominer}
\DefineJournalPartialAbbreviation{Biophysi}{Biophys}
\DefineJournalPartialAbbreviation{Biopolymer}{Biopolym}
\DefineJournalPartialAbbreviation{Biorheolog}{Biorheol}
\DefineJournalPartialAbbreviation{Biotechni}{Biotech}
\DefineJournalPartialAbbreviation{Biotechnolog}{Biotechnol}
\DefineJournalPartialAbbreviation{Biotheoreti}{Biotheor}
\DefineJournalAbbreviation{Biznis}{Bizn}
\DefineJournalWordException{Blessure}{Blessure}
\DefineJournalWordException{Blonde}{Blonde}
\DefineJournalWordException{Blues}{Blues}
\DefineJournalPartialAbbreviation{Boliv}{Boliv}
\DefineJournalWordException{Bonanza}{Bonanza}
\DefineJournalPartialAbbreviation{Botan}{Bot}
\DefineJournalWordException{Bravo}{Bravo}
\DefineJournalPartialAbbreviation{Brevet}{Brev}
\DefineJournalPartialAbbreviation{Bromatolog}{Bromatol}
\DefineJournalPartialAbbreviation{Bronchoesophagolog}{Bronchoesophagol}
\DefineJournalPartialAbbreviation{Brucellos}{Brucell}
\DefineJournalPartialAbbreviation{Bryolog}{Bryol}
\DefineJournalPartialAbbreviation{Bryophyt}{Bryophyt}
\DefineJournalAbbreviation{Bulimia}{Bulim}
\DefineJournalPartialAbbreviation{Bulletin}{Bull}
\DefineJournalWordException{Cable}{Cable}
\DefineJournalWordException{Cabled}{Cabled}
\DefineJournalWordException{Cadence}{Cadence}
\DefineJournalPartialAbbreviation{Calabr}{Calabr}
\DefineJournalWordException{Calcium}{Calcium}
\DefineJournalAbbreviation{Calorie}{Calor}
\DefineJournalPartialAbbreviation{Calvinist}{Calvin}
\DefineJournalWordException{Calypso}{Calypso}
\DefineJournalWordException{Cannabis}{Cannabis}
\DefineJournalWordException{Canton}{Canton}
\DefineJournalWordException{Caracas}{Caracas}
\DefineJournalPartialAbbreviation{Caravan}{Caravan}
\DefineJournalWordException{Carbon}{Carbon}
\DefineJournalWordException{Carcajou}{Carcajou}
\DefineJournalPartialAbbreviation{Carsk}{Carsk}
\DefineJournalWordException{Casablanca}{Casablanca}
\DefineJournalWordException{Casino}{Casino}
\DefineJournalWordException{Catamaran}{Catamaran}
\DefineJournalPartialAbbreviation{Cataract}{Cataract}
\DefineJournalWordException{Cathay}{Cathay}
\DefineJournalWordException{Cathedra}{Cathedra}
\DefineJournalWordException{Cathode}{Cathode}
\DefineJournalAbbreviation{Cavalcade}{Cavalc}
\DefineJournalWordException{Cavali\`ere}{Cavali\`ere}
\DefineJournalPartialAbbreviation{Celti}{Celt}
\DefineJournalWordException{Centaure}{Centaure}
\DefineJournalPartialAbbreviation{Centr\=al}{Cent}
\DefineJournalAbbreviation{Centrum}{Cent}
\DefineJournalWordException{Chalet}{Chalet}
\DefineJournalWordException{Chance}{Chance}
\DefineJournalPartialAbbreviation{Chang}{Chang}
\DefineJournalPartialAbbreviation{Charg}{Charg}
\DefineJournalPartialAbbreviation{Charism}{Charism}
\DefineJournalPartialAbbreviation{Charitab}{Charit}
\DefineJournalWordException{Charleroi}{Charleroi}
\DefineJournalWordException{Chart}{Chart}
\DefineJournalWordException{Chassis}{Chassis}
\DefineJournalWordException{Chinchilla}{Chinchilla}
\DefineJournalWordException{Cholera}{Cholera}
\DefineJournalAbbreviation{Cholesterol}{Cholest}
\DefineJournalWordException{Choral}{Choral}
\DefineJournalPartialAbbreviation{Choral}{Choral}
\DefineJournalPartialAbbreviation{Christian}{Christ}
\DefineJournalPartialAbbreviation{Chromosom}{Chromosom}
\DefineJournalPartialAbbreviation{Chronobiolog}{Chronobiol}
\DefineJournalPartialAbbreviation{Chronolog}{Chronol}
\DefineJournalWordException{Chrysop\oe ia}{Chrysop\oe ia}
\DefineJournalAbbreviation{Cigarette}{Cigar}
\DefineJournalWordException{Cinderella}{Cinderella}
\DefineJournalPartialAbbreviation{Circul}{Circ}
\DefineJournalAbbreviation{Clar\'inet}{Clar}
\DefineJournalWordException{Clique}{Clique}
\DefineJournalWordException{Cloche}{Cloche}
\DefineJournalWordException{Coaticook}{Coaticook}
\DefineJournalWordException{Codex}{Codex}
\DefineJournalPartialAbbreviation{Codif}{Codif}
\DefineJournalWordException{Coenzyme}{Coenzyme}
\DefineJournalPartialAbbreviation{Cognit}{Cogn}
\DefineJournalWordException{Coitus}{Coitus}
\DefineJournalAbbreviation{Coloproctolog\'ia}{Coloproctol}
\DefineJournalPartialAbbreviation{Color}{Color}
\DefineJournalPartialAbbreviation{Com\'ed}{Comed}
\DefineJournalWordException{Comer\J@C t}{Comer\J@C t}
\DefineJournalAbbreviation{Comestible}{Comest}
\DefineJournalPartialAbbreviation{Command}{Command}
\DefineJournalWordException{Commando}{Commando}
\DefineJournalWordException{Communist}{Communist}
\DefineJournalWordException{Comores}{Comores}
\DefineJournalWordException{Compassion}{Compassion}
%\DefineJournalPartialWordException{Compostel}{Compostel-}
%\DefineJournalPartialWordException{Comunal}{Comunal-}
\DefineJournalPartialAbbreviation{Concert}{Concert}
\DefineJournalPartialAbbreviation{Concurr}{Concurr}
\DefineJournalPartialAbbreviation{Conduct}{Conduct}
\DefineJournalPartialAbbreviation{Confin}{Confin}
\DefineJournalPartialAbbreviation{Congest}{Congest}
\DefineJournalPartialAbbreviation{Connect}{Connect}
\DefineJournalAbbreviation{Consensus}{Consens}
\DefineJournalPartialAbbreviation{Conserv}{Conserv}
\DefineJournalAbbreviation{Consolation}{Consolat}
\DefineJournalPartialAbbreviation{Context}{Context}
\DefineJournalPartialAbbreviation{Contradict}{Contradict}
\DefineJournalPartialAbbreviation{Conven}{Conv}
\DefineJournalPartialAbbreviation{Convoca}{Convoc}
\DefineJournalPartialAbbreviation{Convuls}{Convuls}
\DefineJournalPartialAbbreviation{Coordin}{Coord}
\DefineJournalPartialAbbreviation{Cosmi}{Cosm}
\DefineJournalPartialAbbreviation{Cosmonaut}{Cosmonaut}
\DefineJournalPartialAbbreviation{Cosmopolit}{Cosmop}
\DefineJournalWordException{Cowansville}{Cowansville}
\DefineJournalPartialAbbreviation{Cr\'eat}{Creat}
\DefineJournalPartialAbbreviation{Credit}{Cr\'edit}
%\DefineJournalPartialWordException{Criter}{Criter-}
\DefineJournalPartialAbbreviation{Critica}{Crit}
\DefineJournalAbbreviation{Crochet}{Croch}
\DefineJournalPartialAbbreviation{Crucif}{Crucif}
\DefineJournalPartialAbbreviation{Crustac}{Crustac}
\DefineJournalWordException{Cudzie}{Cudzie}
\DefineJournalWordException{Cura\c cao}{Cura\c cao}
%\DefineJournalPartialWordException{Curios}{Curios-}
\DefineJournalWordException{Cyber}{Cyber}
\DefineJournalAbbreviation{Cynosure}{Cynos}
\DefineJournalPartialAbbreviation{Dacoroman}{Dacorom}
\DefineJournalWordException{Dahlia}{Dahlia}
\DefineJournalWordException{Danse}{Danse}
\DefineJournalPartialAbbreviation{Danub}{Danub}
\DefineJournalWordException{Dar es Salaam}{Dar es Salaam}
\DefineJournalPartialAbbreviation{Decod}{Decod}
\DefineJournalPartialAbbreviation{Deform}{Deform}
\DefineJournalPartialAbbreviation{Delect}{Delect}
\DefineJournalPartialAbbreviation{Deleg}{Deleg}
\DefineJournalAbbreviation{Delphinium}{Delphin}
\DefineJournalWordException{Deltaplan}{Deltaplan}
\DefineJournalPartialAbbreviation{Demograph}{Demogr}
\DefineJournalPartialAbbreviation{Demonstrat}{Demonstr}
\DefineJournalPartialAbbreviation{Dendrolog}{Dendrol}
\DefineJournalPartialAbbreviation{Dentrolog}{Dentrol}
\DefineJournalPartialAbbreviation{Deontolog}{Deontol}
\DefineJournalPartialAbbreviation{Deport}{Deport}
\DefineJournalPartialAbbreviation{Deputat}{Deput}
\DefineJournalAbbreviation{Dermato}{Derm}
\DefineJournalPartialAbbreviation{Dermatolog}{Dermatol}
\DefineJournalPartialAbbreviation{Dermatovenerolog}{Dermatovenerol}
\DefineJournalPartialAbbreviation{Dermosifiliograf}{Dermosifiliogr}
\DefineJournalPartialAbbreviation{Desintoxic}{Desintox}
\DefineJournalWordException{Dessert}{Dessert}
\DefineJournalWordException{Diabete}{Diabete}
\DefineJournalPartialAbbreviation{Diabetolog}{Diabetol}
\DefineJournalPartialAbbreviation{Diagnos}{Diagn}
\DefineJournalPartialAbbreviation{Dialekti}{Dialekt}
\DefineJournalPartialAbbreviation{Dialektolog}{Dialektol}
\DefineJournalPartialAbbreviation{Dialys}{Dial}
\DefineJournalWordException{Diaspora}{Diaspora}
\DefineJournalPartialAbbreviation{Didaskal}{Didask}
\DefineJournalPartialAbbreviation{Dietet}{Diet}
\DefineJournalPartialAbbreviation{Dietolog}{Dietol}
\DefineJournalPartialAbbreviation{Digit}{Digit}
\DefineJournalWordException{Dilema}{Dilema}
\DefineJournalWordException{D\'inamo}{D\'inamo}
\DefineJournalWordException{Dioxide}{Dioxide}
\DefineJournalPartialAbbreviation{Diplomat}{Dipl}
\DefineJournalWordException{Direct}{Direct}
\DefineJournalPartialAbbreviation{Discrimin}{Discrim}
\DefineJournalWordException{Diskette}{Diskette}
\DefineJournalAbbreviation{Dispersion}{Dispers}
\DefineJournalAbbreviation{Disposable}{Dispos}
\DefineJournalPartialAbbreviation{Disput}{Disput}
\DefineJournalWordException{Djakarta}{Djakarta}
\DefineJournalWordException{Dollar}{Dollar}
\DefineJournalWordException{Dolmen}{Dolmen}
\DefineJournalWordException{Domino}{Domino}
\DefineJournalPartialAbbreviation{Dosimetr}{Dosim}
\DefineJournalPartialAbbreviation{Droforskn}{Droforsk}
\DefineJournalPartialAbbreviation{Drogforskn}{Drogforsk}
\DefineJournalPartialAbbreviation{Droguer}{Drog}
\DefineJournalPartialAbbreviation{Duoden}{Duoden}
\DefineJournalPartialAbbreviation{Duplicat}{Duplic}
\DefineJournalWordException{Dynamite}{Dynamite}
\DefineJournalPartialAbbreviation{Dynasti}{Dynast}
\DefineJournalPartialAbbreviation{Econometri}{\'Econom}
\DefineJournalPartialAbbreviation{\`Ekolog}{Ekol}
\DefineJournalPartialAbbreviation{Ekonom}{\`Ekon}
\DefineJournalPartialAbbreviation{\'Elabor}{Elabor}
\DefineJournalPartialAbbreviation{Elastoplasti}{Elastoplast}
\DefineJournalWordException{Electrode}{Electrode}
\DefineJournalPartialAbbreviation{Electrofisiolog}{Electrofisiol}
\DefineJournalPartialAbbreviation{Electroimmunochemi}{Eletroimmunochem}
\DefineJournalPartialAbbreviation{Elementoorgani}{Elementoorg}
\DefineJournalWordException{Email}{Email}
\DefineJournalWordException{Embargo}{Embargo}
\DefineJournalPartialAbbreviation{Embryolog}{Embryol}
\DefineJournalPartialAbbreviation{Emigr}{Emigr}
\DefineJournalWordException{Emmaus}{Emmaus}
\DefineJournalWordException{Emporium}{Emporium}
\DefineJournalPartialAbbreviation{Emuls}{Emuls}
\DefineJournalPartialAbbreviation{Encourag}{Encourag}
\DefineJournalPartialAbbreviation{Endemi}{Endem}
\DefineJournalPartialAbbreviation{Endogen}{Endog}
\DefineJournalPartialAbbreviation{Endothel}{Endothel}
\DefineJournalPartialAbbreviation{Endourolog}{Endourol}
\DefineJournalPartialAbbreviation{Endur}{Endur}
\DefineJournalPartialAbbreviation{\`Energet}{Energ}
\DefineJournalAbbreviation{Energistatistik}{Energistat}
\DefineJournalPartialAbbreviation{Enterolog}{Enterol}
\DefineJournalPartialAbbreviation{Entomolog}{\`Entomol}
\DefineJournalPartialAbbreviation{Envelop}{Envel}
\DefineJournalPartialAbbreviation{Enzymolog}{Enzymol}
\DefineJournalPartialAbbreviation{\`Epidemiolog}{Epidemiol}
\DefineJournalPartialAbbreviation{Epigraph}{Epigr}
\DefineJournalPartialAbbreviation{Epileptolog}{Epileptol}
\DefineJournalPartialAbbreviation{Epiphyti}{Epiphyt}
\DefineJournalPartialAbbreviation{Epizooti}{Epizoot}
\DefineJournalPartialAbbreviation{Epizootolog}{Epizootol}
\DefineJournalWordException{Erato}{Erato}
\DefineJournalPartialAbbreviation{Ergonom}{Ergon}
\DefineJournalAbbreviation{Erotika}{Erot}
\DefineJournalPartialAbbreviation{Erythropoiet}{Erythrop}
\DefineJournalPartialAbbreviation{Eslastom}{Eslastom}
\DefineJournalPartialAbbreviation{Esophagolog}{\'Esophagol}
\DefineJournalPartialAbbreviation{Esoteri}{Esoter}
\DefineJournalPartialAbbreviation{Espac}{Espa\c c}
\DefineJournalAbbreviation{Esterior}{Ester}
\DefineJournalPartialAbbreviation{Estheti}{Esthet}
\DefineJournalPartialAbbreviation{Ethnograph}{Ethnogr}
\DefineJournalPartialAbbreviation{Ethnolog}{Ethnol}
\DefineJournalPartialAbbreviation{Ethnomusicolog}{Ethnomusicol}
\DefineJournalPartialAbbreviation{Ethopharmacolog}{Ethopharmacol}
\DefineJournalPartialAbbreviation{Etiolog}{Etiol}
%\DefineJournalPartialWordException{Euphorbiac}{Euphorbiac-}
\DefineJournalWordException{Eureka}{Eureka}
\DefineJournalWordException{Eurocard}{Eurocard}
\DefineJournalPartialAbbreviation{Europ}{Eur}
\DefineJournalAbbreviation{Euroregion}{Euroreg}
\DefineJournalAbbreviation{Eurostandard}{Eurostand}
\DefineJournalWordException{Eurostat}{Eurostat}
\DefineJournalPartialAbbreviation{Eurostat}{Eurostat}
\DefineJournalAbbreviation{Eurovision}{Eurovis}
\DefineJournalPartialAbbreviation{Euthanas}{Euthan}
\DefineJournalWordException{Everest}{Everest}
\DefineJournalPartialAbbreviation{Except}{Except}
\DefineJournalAbbreviation{Excipient}{Excip}
\DefineJournalPartialAbbreviation{Exclusiv}{Exclus}
\DefineJournalPartialAbbreviation{Exempl}{Ex}
\DefineJournalPartialAbbreviation{Exig}{Exig}
\DefineJournalPartialAbbreviation{Exist}{Exist}
\DefineJournalPartialAbbreviation{Expans}{Expans}
\DefineJournalPartialAbbreviation{Expatr}{Expatr}
\DefineJournalPartialAbbreviation{Expecta}{Expect}
\DefineJournalWordException{Expert}{Expert}
\DefineJournalPartialAbbreviation{Expert}{Expert}
\DefineJournalWordException{Extra}{Extra}
\DefineJournalWordException{Factum}{Factum}
\DefineJournalPartialAbbreviation{Fakult}{Fak}
\DefineJournalWordException{Fanfare}{Fanfare}
\DefineJournalPartialAbbreviation{Fantast}{Fantast}
\DefineJournalWordException{Fascisme}{Fascisme}
\DefineJournalPartialAbbreviation{Fatal}{Fatal}
\DefineJournalPartialAbbreviation{Femin}{Fem}
\DefineJournalPartialAbbreviation{Fenomen}{Fenom}
\DefineJournalWordException{Ferret}{Ferret}
\DefineJournalPartialAbbreviation{Fertili}{Fertil}
\DefineJournalPartialAbbreviation{Filateli}{Filat}
\DefineJournalWordException{Filia}{Filia}
\DefineJournalWordException{Filmforum}{Filmforum}
\DefineJournalPartialAbbreviation{Filmogr}{Filmogr}
\DefineJournalPartialAbbreviation{Filmologic}{Filmol}
\DefineJournalPartialAbbreviation{Filosof}{Filos}
%\DefineJournalPartialWordException{Firmament}{Firmament-}
\DefineJournalWordException{Fjordane}{Fjordane}
\DefineJournalPartialAbbreviation{Flagrant}{Flagr}
\DefineJournalAbbreviation{Flexible}{Flex}
\DefineJournalWordException{Fluor}{Fluor}
\DefineJournalPartialAbbreviation{Fluviometr}{Fluviom}
\DefineJournalWordException{Folio}{Folio}
\DefineJournalWordException{Forfait}{Forfait}
\DefineJournalWordException{Format}{Format}
\DefineJournalPartialAbbreviation{Formular}{Formul}
\DefineJournalPartialAbbreviation{Formulat}{Formul}
\DefineJournalPartialAbbreviation{Fortifi}{Fortif}
\DefineJournalPartialAbbreviation{Fossil}{Foss}
\DefineJournalPartialAbbreviation{Fotograph}{Fotogr}
\DefineJournalPartialAbbreviation{Fotointerpret}{Fotointerpret}
\DefineJournalWordException{Francfort}{Francfort}
\DefineJournalPartialAbbreviation{Fruct}{Fruct}
\DefineJournalWordException{Fuchsia}{Fuchsia}
\DefineJournalWordException{Fusion}{Fusion}
\DefineJournalPartialAbbreviation{Galacti}{Galact}
\DefineJournalPartialAbbreviation{Galeni}{Galen}
\DefineJournalWordException{Galerie}{Galerie}
\DefineJournalWordException{Galicien}{Galicien}
\DefineJournalAbbreviation{Gallia}{Gall}
\DefineJournalPartialAbbreviation{Galvanotechni}{Galvanotech}
\DefineJournalPartialAbbreviation{Gambi}{Gamb}
\DefineJournalWordException{Gamma}{Gamma}
\DefineJournalWordException{Ganganatha}{Ganganatha}
\DefineJournalWordException{Garage}{Garage}
\DefineJournalPartialAbbreviation{Gastroenterolog}{Gastroenterol}
\DefineJournalPartialAbbreviation{Gemellolog}{Gemellol}
\DefineJournalPartialAbbreviation{Gemmolog}{Gemmol}
\DefineJournalAbbreviation{Genagogue}{Genagog}
\DefineJournalPartialAbbreviation{Genealog}{Geneal}
\DefineJournalPartialAbbreviation{Generat}{Gener}
\DefineJournalAbbreviation{Genesis}{Genes}
\DefineJournalPartialAbbreviation{Genesung}{Genes}
\DefineJournalPartialAbbreviation{Genet}{Genet}
\DefineJournalWordException{Genocide}{Genocide}
\DefineJournalPartialAbbreviation{Geobotan}{Geobot}
\DefineJournalPartialAbbreviation{G\'eod\'es}{G\'eod}
\DefineJournalPartialAbbreviation{Geodet}{G\'eod}
\DefineJournalAbbreviation{Geoindustria}{Geoind}
\DefineJournalPartialAbbreviation{Geolog}{Geol}
\DefineJournalPartialAbbreviation{Geomagneti}{Geomagn}
\DefineJournalAbbreviation{Geomathematic}{Geomath}
\DefineJournalPartialAbbreviation{Geomechani}{G\'eom\'ech}
\DefineJournalPartialAbbreviation{Geometr}{Geom}
\DefineJournalPartialAbbreviation{Geoscien}{Geosci}
\DefineJournalAbbreviation{Geosphaera}{Geosph}
\DefineJournalPartialAbbreviation{Geostatisti}{Geostat}
\DefineJournalPartialAbbreviation{Geotechni}{Geotech}
\DefineJournalPartialAbbreviation{Geriatri}{Geriatr}
\DefineJournalPartialAbbreviation{Gerontolog}{Gerontol}
\DefineJournalWordException{Gilde}{Gilde}
\DefineJournalWordException{Ginseng}{Ginseng}
\DefineJournalPartialAbbreviation{Global}{Glob}
\DefineJournalPartialAbbreviation{Glorif}{Glorif}
\DefineJournalWordException{Glucose}{Glucose}
\DefineJournalPartialAbbreviation{Gnatholog}{Gnathol}
\DefineJournalPartialAbbreviation{Gnotobiolog}{Gnotobiol}
\DefineJournalWordException{G\oe the}{G\oe the}
\DefineJournalWordException{Gondwana}{Gondwana}
\DefineJournalPartialAbbreviation{Grafi}{Graf}
\DefineJournalWordException{Grange}{Grange}
\DefineJournalPartialAbbreviation{Grapholog}{Graphol}
\DefineJournalWordException{Gratis}{Gratis}
\DefineJournalAbbreviation{Graveur}{Grav}
\DefineJournalPartialAbbreviation{Gravimetr}{Gravim}
\DefineJournalWordException{Guerrilla}{Guerrilla}
\DefineJournalAbbreviation{Guinea-Bissau}{Guin-Bissau}
\DefineJournalPartialAbbreviation{Guitar}{Guitar}
\DefineJournalPartialAbbreviation{Habilitat}{Habilit}
\DefineJournalWordException{Hammadi}{Hammadi}
\DefineJournalPartialAbbreviation{Handelsstatisti}{Handelsstat}
\DefineJournalWordException{Hanover}{Hanover}
\DefineJournalWordException{Harappa}{Harappa}
\DefineJournalAbbreviation{Hebraic}{Hebr}
\DefineJournalWordException{Hectare}{Hectare}
\DefineJournalWordException{Helicon}{Helicon}
\DefineJournalPartialAbbreviation{Hematolog}{Hematol}
\DefineJournalPartialAbbreviation{Hemophil}{Hemoph}
\DefineJournalPartialAbbreviation{Hepatolog}{Hepatol}
\DefineJournalPartialAbbreviation{Hepatosplenolog}{Hepatosplenol}
\DefineJournalPartialAbbreviation{Herbivor}{Herbiv}
\DefineJournalWordException{Hermes}{Hermes}
\DefineJournalPartialAbbreviation{Herpetolog}{Herpetol}
\DefineJournalPartialAbbreviation{Heterogen}{Heterog}
\DefineJournalPartialAbbreviation{Hexachord}{Hexachord}
\DefineJournalPartialAbbreviation{Hipertens}{Hipertens}
\DefineJournalPartialAbbreviation{Histolog}{Histol}
\DefineJournalPartialAbbreviation{Histophysiolog}{Histophysiol}
\DefineJournalPartialAbbreviation{Holograph}{Hologr}
\DefineJournalPartialAbbreviation{Homeopat}{Homeopat}
\DefineJournalWordException{Homicide}{Homicide}
\DefineJournalAbbreviation{Honolulu}{Honol}
\DefineJournalPartialAbbreviation{Honor}{Honor}
\DefineJournalPartialAbbreviation{Hormon}{Horm}
\DefineJournalPartialAbbreviation{Hormonolog}{Hormonol}
\DefineJournalPartialAbbreviation{Horolog}{Horol}
\DefineJournalPartialAbbreviation{Hostel}{Hostel}
\DefineJournalWordException{Humus}{Humus}
\DefineJournalPartialAbbreviation{Husserl}{Husserl}
\DefineJournalPartialAbbreviation{Hydraul}{Hydraul}
\DefineJournalPartialAbbreviation{Hydrobiolog}{Hydrobiol}
\DefineJournalPartialAbbreviation{Hydrodynam}{Hydrodyn}
\DefineJournalPartialAbbreviation{Hydrogeolog}{Hydrogeol}
\DefineJournalPartialAbbreviation{Hydrograph}{Hydrogr}
\DefineJournalPartialAbbreviation{Hydrolog}{Hydrol}
\DefineJournalPartialAbbreviation{Hyperact}{Hyperact}
\DefineJournalPartialAbbreviation{Hyperbar}{Hyperb}
\DefineJournalPartialAbbreviation{Hypothalam}{Hypothal}
\DefineJournalPartialAbbreviation{Ichthyolog}{Ichthyol}
\DefineJournalPartialAbbreviation{Ictiolog}{Ictiol}
\DefineJournalAbbreviation{Id\'efemina}{Id\'efem}
\DefineJournalWordException{Idiot}{Idiot}
\DefineJournalAbbreviation{Ikorodu}{Ikor}
\DefineJournalPartialAbbreviation{Illicit}{Illicit}
\DefineJournalPartialAbbreviation{Illusion}{Illusion}
\DefineJournalPartialAbbreviation{Immacul}{Immacul}
\DefineJournalPartialAbbreviation{Immediat}{Immed}
\DefineJournalPartialAbbreviation{Immortal}{Immortal}
%\DefineJournalPartialWordException{Impass}{Impass-}
\DefineJournalPartialAbbreviation{Imperia}{Imp}
\DefineJournalPartialAbbreviation{Implantolog}{Implantol}
\DefineJournalAbbreviation{Impregnation}{Impregn}
\DefineJournalAbbreviation{Inali\'enable}{Inalien}
\DefineJournalPartialAbbreviation{Incendi}{Incend}
\DefineJournalPartialAbbreviation{Indemnit}{Indemn}
\DefineJournalWordException{India}{India}
\DefineJournalWordException{Indigo}{Indigo}
\DefineJournalPartialAbbreviation{Individ}{Individ}
\DefineJournalPartialAbbreviation{Indoeurop}{Indoeur}
\DefineJournalPartialAbbreviation{Industr}{Ind}
\DefineJournalPartialAbbreviation{Infinit}{Infin}
\DefineJournalAbbreviation{Infobulletin}{Infobull}
\DefineJournalAbbreviation{Information}{Inf}
\DefineJournalAbbreviation{Infraction}{Infract}
\DefineJournalAbbreviation{Infusion}{Infus}
\DefineJournalPartialAbbreviation{Inhibit}{Inhib}
\DefineJournalPartialAbbreviation{Innovat}{Innov}
\DefineJournalPartialAbbreviation{Inox}{Inox}
\DefineJournalWordException{Input}{Input}
\DefineJournalPartialAbbreviation{Inser}{Inser}
\DefineJournalAbbreviation{Institut}{Inst}
\DefineJournalAbbreviation{Institution}{Inst}
\DefineJournalAbbreviation{Integration}{Integr}
\DefineJournalPartialAbbreviation{Intelektual}{Intelekt}
\DefineJournalAbbreviation{Intelligent}{Intell}
\DefineJournalWordException{Inter}{Inter}
\DefineJournalPartialAbbreviation{Interchang}{Interchang}
\DefineJournalWordException{Intercine}{Intercine}
\DefineJournalWordException{Interferon}{Interferon}
\DefineJournalAbbreviation{Interlingua}{Interling}
\DefineJournalWordException{Interlude}{Interlude}
\DefineJournalAbbreviation{Internat}{Intern}
\DefineJournalAbbreviation{Interpanorama}{Interpanor}
\DefineJournalWordException{Interpress}{Interpress}
\DefineJournalPartialAbbreviation{Interpr\`et}{Interpret}
\DefineJournalWordException{Interracial}{Interracial}
\DefineJournalWordException{Interrail}{Interrail}
\DefineJournalPartialAbbreviation{Intersection}{Intersect}
\DefineJournalPartialAbbreviation{Interven}{Interv}
\DefineJournalWordException{Intrusion}{Intrusion}
\DefineJournalPartialAbbreviation{Investiga}{Investig}
\DefineJournalWordException{Invincible}{Invincible}
\DefineJournalAbbreviation{Ionic}{Ion}
\DefineJournalPartialAbbreviation{Irani}{Iran}
\DefineJournalWordException{Islam}{Islam}
\DefineJournalPartialAbbreviation{Islam}{Islam}
\DefineJournalWordException{Islamabad}{Islamabad}
\DefineJournalPartialAbbreviation{Isotop}{Isot}
\DefineJournalPartialAbbreviation{Israel}{Isr}
\DefineJournalPartialAbbreviation{Izolant}{Izol}
\DefineJournalAbbreviation{Jargon}{Jarg}
\DefineJournalPartialAbbreviation{Jedin}{Jedin}
\DefineJournalWordException{Jehova}{Jehova}
\DefineJournalPartialAbbreviation{Jesuit}{Jesuit}
\DefineJournalPartialAbbreviation{Jubil}{Jubil}
\DefineJournalWordException{Judoka}{Judoka}
\DefineJournalAbbreviation{Jurnal}{J}
\DefineJournalAbbreviation{Kalahari}{Kalah}
\DefineJournalAbbreviation{Kaleidoscope}{Kaleidosc}
\DefineJournalWordException{Kalinka}{Kalinka}
\DefineJournalAbbreviation{Kampuchea}{Kampuch}
\DefineJournalWordException{Karate}{Karate}
\DefineJournalWordException{Kashim}{Kashim}
\DefineJournalWordException{Kendriya}{Kendriya}
\DefineJournalWordException{Kinder}{Kinder}
\DefineJournalPartialAbbreviation{Kinematogr}{Kinematogr}
\DefineJournalAbbreviation{Kombatant}{Kombat}
\DefineJournalPartialAbbreviation{Komunist}{Komunist}
\DefineJournalWordException{Konsument}{Konsument}
\DefineJournalPartialAbbreviation{Kosmonaut}{Kosmonaut}
\DefineJournalPartialAbbreviation{Kosov}{Kos}
\DefineJournalPartialAbbreviation{Kreat}{Kreat}
\DefineJournalWordException{Krokodil}{Krokodil}
\DefineJournalWordException{Kuala Lumpur}{Kuala Lumpur}
\DefineJournalWordException{Kung-fu}{Kung-fu}
\DefineJournalPartialAbbreviation{Kurat}{Kurat}
\DefineJournalAbbreviation{Kurdistan}{Kurd}
\DefineJournalWordException{Labor}{Labor}
\DefineJournalWordException{Labor (work)}{Labor (work)}
\DefineJournalPartialAbbreviation{Laborator}{Lab}
\DefineJournalWordException{Lac Megantic}{Lac Megantic}
\DefineJournalWordException{Lambarene}{Lambarene}
\DefineJournalWordException{Lambda}{Lambda}
\DefineJournalPartialAbbreviation{Laryngolog}{Laryngol}
\DefineJournalWordException{Laser}{Laser}
\DefineJournalAbbreviation{Lector}{Lect}
\DefineJournalPartialAbbreviation{Legum}{Legum}
\DefineJournalAbbreviation{Leningrad}{Leningr}
\DefineJournalPartialAbbreviation{Leninist}{Lenin}
%\DefineJournalPartialWordException{Lentil}{Lentil-}
%\DefineJournalPartialWordException{Leon}{Leon-}
\DefineJournalPartialAbbreviation{Leprolog}{Leprol}
\DefineJournalWordException{Letridiidae}{Letridiidae}
\DefineJournalPartialAbbreviation{Leukemi}{Leuk}
\DefineJournalPartialAbbreviation{Lichenolog}{Lichenol}
\DefineJournalAbbreviation{Licitation}{Licit}
\DefineJournalWordException{Lilliput}{Lilliput}
\DefineJournalPartialAbbreviation{Limnolog}{Limnol}
\DefineJournalPartialAbbreviation{Ling\"u\'ist}{Linguist}
\DefineJournalPartialAbbreviation{Literat}{Lit}
\DefineJournalPartialAbbreviation{Lithograph}{Lithogr}
\DefineJournalPartialAbbreviation{Litholog}{Lithol}
\DefineJournalPartialAbbreviation{Lithuani}{Lith}
\DefineJournalPartialAbbreviation{Litolog}{Litol}
\DefineJournalWordException{Livigno}{Livigno}
\DefineJournalAbbreviation{Localisation}{Localis}
\DefineJournalPartialAbbreviation{Locomoti}{Locomot}
\DefineJournalPartialAbbreviation{Logoped}{Logop}
\DefineJournalWordException{Logos}{Logos}
\DefineJournalWordException{Luzerne}{Luzerne}
\DefineJournalAbbreviation{Lymphocyte}{Lymph}
\DefineJournalPartialAbbreviation{Macedoni}{Maced}
\DefineJournalAbbreviation{Macroperspective}{Macroperspect}
\DefineJournalAbbreviation{Madagascar}{Madag}
\DefineJournalWordException{Magister}{Magister}
\DefineJournalPartialAbbreviation{Magmati}{Magmat}
\DefineJournalAbbreviation{Magnesium}{Magnes}
\DefineJournalPartialAbbreviation{Magneti}{Magn}
\DefineJournalPartialAbbreviation{Magnetohydrodynami}{Magn\'etohydrodyn}
\DefineJournalPartialAbbreviation{Magnetoplasmadynami}{Magn\'etoplasmadyn}
\DefineJournalWordException{Magnolia}{Magnolia}
\DefineJournalPartialAbbreviation{Maket}{Maket}
\DefineJournalWordException{Malagasy}{Malagasy}
\DefineJournalPartialAbbreviation{Malariolog}{Malariol}
\DefineJournalWordException{Malawi}{Malawi}
\DefineJournalWordException{Malta}{Malta}
\DefineJournalPartialAbbreviation{Manag}{Manag}
\DefineJournalWordException{Manga}{Manga}
\DefineJournalWordException{Maniwaki}{Maniwaki}
\DefineJournalWordException{Marathon}{Marathon}
\DefineJournalWordException{Mariposa}{Mariposa}
\DefineJournalPartialAbbreviation{Marx}{Marx}
%\DefineJournalPartialWordException{Mascot}{Mascot-}
\DefineJournalPartialAbbreviation{Matern}{Matern}
\DefineJournalWordException{Media}{Media}
\DefineJournalPartialAbbreviation{Medicament}{Medicam}
\DefineJournalPartialAbbreviation{Medic\=in}{Med}
\DefineJournalAbbreviation{M\'editation}{Medit}
\DefineJournalWordException{Medium}{Medium}
\DefineJournalPartialAbbreviation{Mekani}{Mek}
\DefineJournalPartialAbbreviation{Melanes}{Melanes}
\DefineJournalWordException{Melita}{Melita}
\DefineJournalPartialAbbreviation{Mercat}{Mercat}
\DefineJournalPartialAbbreviation{Mercena}{Mercen}
\DefineJournalAbbreviation{Meridional}{Merid}
\DefineJournalPartialAbbreviation{Mesolith}{Mesolith}
\DefineJournalPartialAbbreviation{Messag}{Messag}
\DefineJournalWordException{Messe}{Messe}
\DefineJournalPartialAbbreviation{Messin}{Messin}
\DefineJournalPartialAbbreviation{Metaboli}{Metab}
\DefineJournalPartialAbbreviation{Metabolog}{Metabol}
\DefineJournalPartialAbbreviation{Metal}{Met}
\DefineJournalPartialAbbreviation{Metallogen}{Metallog}
\DefineJournalPartialAbbreviation{Metallurg}{Metall}
\DefineJournalPartialAbbreviation{Meteorolog}{Meteorol}
\DefineJournalPartialAbbreviation{Metrolog}{Metrol}
\DefineJournalPartialAbbreviation{Metropolitan}{Metrop}
\DefineJournalWordException{Microcircuit}{Microcircuit}
\DefineJournalPartialAbbreviation{Microecolog}{Microecol}
\DefineJournalPartialAbbreviation{Microfich}{Microfich}
\DefineJournalPartialAbbreviation{Microfilm}{Microfilm}
\DefineJournalPartialAbbreviation{Migrator}{Migr}
\DefineJournalWordException{Militia}{Militia}
\DefineJournalAbbreviation{Mill\'esime}{Mill\'es}
\DefineJournalPartialAbbreviation{Mimeograph}{Mimeogr}
\DefineJournalWordException{Mimesis}{Mimesis}
\DefineJournalWordException{Mindanao}{Mindanao}
\DefineJournalPartialAbbreviation{Mineral}{Miner}
\DefineJournalPartialAbbreviation{Mineralog}{Mineral}
\DefineJournalWordException{Minigolf}{Minigolf}
\DefineJournalPartialAbbreviation{Ministr}{Minist}
\DefineJournalPartialAbbreviation{Minor}{Minor}
\DefineJournalWordException{Minuses}{Minuses}
\DefineJournalWordException{Miracle}{Miracle}
\DefineJournalWordException{Mirage}{Mirage}
\DefineJournalPartialAbbreviation{Mission}{Mission}
\DefineJournalWordException{Missive}{Missive}
\DefineJournalPartialAbbreviation{Mitropol}{Mitrop}
\DefineJournalWordException{Mnemosyne}{Mnemosyne}
\DefineJournalAbbreviation{Mobilo}{Mob}
\DefineJournalPartialAbbreviation{Modifi}{Modif}
\DefineJournalWordException{Mohair}{Mohair}
\DefineJournalPartialAbbreviation{Monarch}{Monarch}
\DefineJournalPartialAbbreviation{Mon\'et}{Monet}
\DefineJournalPartialAbbreviation{Monolith}{Monolith}
\DefineJournalAbbreviation{Monologue}{Monolog}
\DefineJournalPartialAbbreviation{Monopol}{Monop}
\DefineJournalAbbreviation{Montenegro}{Monten}
\DefineJournalPartialAbbreviation{Morbid}{Morb}
\DefineJournalPartialAbbreviation{Motiv}{Motiv}
\DefineJournalPartialAbbreviation{Multicultur}{Multicult}
\DefineJournalPartialAbbreviation{Multidimension}{Multidimens}
\DefineJournalPartialAbbreviation{Multiethnic}{Multiethn}
\DefineJournalPartialAbbreviation{Multietn}{Multietn}
\DefineJournalAbbreviation{Multim\'edia}{Multimed}
\DefineJournalAbbreviation{Multiprint}{Multipr}
\DefineJournalWordException{Mural}{Mural}
\DefineJournalWordException{Murale}{Murale}
\DefineJournalPartialAbbreviation{Museolog}{Museol}
\DefineJournalAbbreviation{Musette}{Muset}
\DefineJournalWordException{Mutant}{Mutant}
\DefineJournalAbbreviation{Myocardium}{Myocard}
\DefineJournalPartialAbbreviation{Myograph}{Myogr}
\DefineJournalPartialAbbreviation{Myolog}{Myol}
\DefineJournalPartialAbbreviation{Myth}{Myth}
\DefineJournalPartialAbbreviation{Myxomycet}{Myxomyc}
\DefineJournalPartialAbbreviation{Nacion}{Nac}
\DefineJournalWordException{Nanjing}{Nanjing}
\DefineJournalPartialAbbreviation{Narkot}{Nark}
\DefineJournalWordException{Nation}{Nation}
\DefineJournalPartialAbbreviation{Naviga}{Navig}
\DefineJournalPartialAbbreviation{Necrolog}{Necrol}
\DefineJournalPartialAbbreviation{Nematolog}{Nematol}
\DefineJournalPartialAbbreviation{Neohelleni}{Neohell}
\DefineJournalPartialAbbreviation{Neolit}{Neolit}
\DefineJournalPartialAbbreviation{Neotestament}{Neotestam}
\DefineJournalAbbreviation{Neozelandesa}{Neozel}
\DefineJournalWordException{Nepal}{Nepal}
\DefineJournalAbbreviation{Nervosa}{Nerv}
\DefineJournalPartialAbbreviation{Neuroanatom}{Neuroanat}
\DefineJournalPartialAbbreviation{Neurobiolog}{Neurobiol}
\DefineJournalPartialAbbreviation{Neuroendocrin}{Neuroendocr}
\DefineJournalPartialAbbreviation{Neurogerontolog}{Neurogerontol}
\DefineJournalPartialAbbreviation{Neuroleptanalges}{Neuroleptanalg}
\DefineJournalPartialAbbreviation{Neurolog}{Neurol}
\DefineJournalPartialAbbreviation{Neurometaboli}{Neurometab}
\DefineJournalPartialAbbreviation{Neuroontogen}{Neuroontog}
\DefineJournalPartialAbbreviation{Neuropatholog}{Neuropathol}
\DefineJournalPartialAbbreviation{Neurophysiolog}{Neurophysiol}
\DefineJournalPartialAbbreviation{Neuropsychiatri}{Neuropsychiatr}
\DefineJournalPartialAbbreviation{Neuropsycholog}{Neuropsychol}
\DefineJournalPartialAbbreviation{Neurovegetativ}{Neuroveg}
\DefineJournalWordException{Nifedipina}{Nifedipina}
\DefineJournalPartialAbbreviation{Nihil}{Nihil}
\DefineJournalPartialAbbreviation{Nipiolog}{Nipiol}
\DefineJournalPartialAbbreviation{Nippon}{Nippon}
\DefineJournalPartialAbbreviation{Nocturn}{Noct}
\DefineJournalWordException{Nominal}{Nominal}
\DefineJournalAbbreviation{Nonviolent}{Nonviol}
\DefineJournalPartialAbbreviation{Nord}{Nord}
\DefineJournalPartialAbbreviation{Normal}{Norm}
\DefineJournalPartialAbbreviation{Nostalg}{Nostalg}
\DefineJournalAbbreviation{Notation}{Not}
\DefineJournalAbbreviation{November}{Novemb}
\DefineJournalWordException{Novice}{Novice}
\DefineJournalWordException{Nubica}{Nubica}
\DefineJournalAbbreviation{Nukleus}{Nukl}
\DefineJournalPartialAbbreviation{Numismati}{Numis}
\DefineJournalWordException{Nunavut}{Nunavut}
\DefineJournalPartialAbbreviation{Nutri}{Nutr}
\DefineJournalPartialAbbreviation{Objecti}{Object}
\DefineJournalWordException{Obokun}{Obokun}
\DefineJournalWordException{Obscura}{Obscura}
\DefineJournalPartialAbbreviation{Observ}{Obs}
\DefineJournalPartialAbbreviation{Obstetri}{Obstet}
\DefineJournalPartialAbbreviation{Oc\'ean}{Ocean}
\DefineJournalWordException{Octane}{Octane}
%\DefineJournalPartialWordException{Octav}{Octav-}
\DefineJournalWordException{Ocultism}{Ocultism}
\DefineJournalAbbreviation{Odalisque}{Odal}
\DefineJournalPartialAbbreviation{Odbor}{Odbor}
\DefineJournalWordException{Odd-Fellow}{Odd-Fellow}
\DefineJournalPartialAbbreviation{Odontoiatri}{Odontoiatr}
\DefineJournalPartialAbbreviation{Odontolog}{Odontol}
\DefineJournalPartialAbbreviation{Odontostomatolog}{Odontostomatol}
\DefineJournalPartialAbbreviation{Offic}{Off}
\DefineJournalPartialAbbreviation{Oftalmolog}{Oftalmol}
\DefineJournalPartialAbbreviation{Olisip}{Olisip}
\DefineJournalWordException{Omega}{Omega}
\DefineJournalPartialAbbreviation{Onomast}{Onomast}
\DefineJournalPartialAbbreviation{Ontogen}{Ontog}
\DefineJournalPartialAbbreviation{Operat}{Oper}
\DefineJournalAbbreviation{Optimum}{Optim}
\DefineJournalPartialAbbreviation{Optometr}{Optom}
\DefineJournalWordException{Orange}{Orange}
\DefineJournalWordException{Orangerie}{Orangerie}
\DefineJournalPartialAbbreviation{Orchid}{Orchid}
\DefineJournalWordException{Organ}{Organ}
\DefineJournalPartialAbbreviation{Organiza}{Organ}
\DefineJournalPartialAbbreviation{Organologi}{Organol}
%\DefineJournalPartialWordException{Orgasm}{Orgasm-}
\DefineJournalWordException{Orient}{Orient}
\DefineJournalWordException{Origami}{Origami}
\DefineJournalPartialAbbreviation{Orthodox}{Orthodox}
\DefineJournalPartialAbbreviation{Orthognath}{Orthognath}
\DefineJournalPartialAbbreviation{Oscil}{Oscil}
\DefineJournalPartialAbbreviation{Osteoarticul}{Osteoartic}
\DefineJournalPartialAbbreviation{Otolaryngolog}{Otolaryngol}
\DefineJournalPartialAbbreviation{Otolog}{Otol}
\DefineJournalPartialAbbreviation{Otoophthalmolog}{Otoophthalmol}
\DefineJournalPartialAbbreviation{Otorhinolaryngolog}{Otorhinolaryngol}
\DefineJournalWordException{Ovation}{Ovation}
\DefineJournalWordException{Overdose}{Overdose}
%\DefineJournalPartialWordException{Ovin}{Ovin-}
\DefineJournalWordException{Ozone}{Ozone}
\DefineJournalPartialAbbreviation{Pacifist}{Pacif}
\DefineJournalPartialAbbreviation{Paleodont}{Paleodont}
\DefineJournalPartialAbbreviation{Paleontograph}{Pal\'eontogr}
\DefineJournalPartialAbbreviation{Paleontolog}{Pal\'eontol}
\DefineJournalPartialAbbreviation{Paleotectonic}{Paleotecton}
\DefineJournalPartialAbbreviation{Palestin}{Palest}
\DefineJournalPartialAbbreviation{Palmyr}{Palmyr}
\DefineJournalPartialAbbreviation{Paludism}{Palud}
\DefineJournalPartialAbbreviation{Palynolog}{Palynol}
\DefineJournalPartialAbbreviation{Pamiat}{Pamiat}
\DefineJournalWordException{Panchayat}{Panchayat}
\DefineJournalWordException{Pandemonia}{Pandemonia}
\DefineJournalAbbreviation{Panorama}{Panor}
\DefineJournalPartialAbbreviation{Pantograph}{Pantogr}
\DefineJournalWordException{Papillon}{Papillon}
\DefineJournalAbbreviation{Papirforedling}{Papirforedl}
\DefineJournalPartialAbbreviation{Parabol}{Parabol}
\DefineJournalPartialAbbreviation{Parachut}{Parachut}
\DefineJournalPartialAbbreviation{Paralis}{Paralis}
\DefineJournalPartialAbbreviation{Paramagn}{Paramagn}
\DefineJournalPartialAbbreviation{Param\'edic}{Paramed}
\DefineJournalPartialAbbreviation{Parametr}{Parametr}
\DefineJournalAbbreviation{Paranormal}{Paranorm}
\DefineJournalPartialAbbreviation{Parapsycholog}{Parapsychol}
\DefineJournalPartialAbbreviation{Parapsykol}{Parapsykol}
\DefineJournalWordException{Parishads}{Parishads}
\DefineJournalPartialAbbreviation{Parit}{Parit}
\DefineJournalPartialAbbreviation{Parnas}{Parnas}
\DefineJournalPartialAbbreviation{Parodontolog}{Parodontol}
\DefineJournalPartialAbbreviation{Particip}{Particip}
\DefineJournalWordException{Passant}{Passant}
\DefineJournalWordException{Pastiche}{Pastiche}
\DefineJournalAbbreviation{Pataphysica}{Pataphys}
\DefineJournalPartialAbbreviation{Pathobiolog}{Pathobiol}
\DefineJournalPartialAbbreviation{Pathogen}{Pathog}
\DefineJournalPartialAbbreviation{Patholog}{Pathol}
\DefineJournalPartialAbbreviation{Pedagog}{Pedagog}
\DefineJournalPartialAbbreviation{Pediatri}{Pediatr}
\DefineJournalPartialAbbreviation{Pedolog}{Pedol}
\DefineJournalPartialAbbreviation{Pendul}{Pendul}
\DefineJournalPartialAbbreviation{Peptid}{Pept}
\DefineJournalPartialAbbreviation{Percuss}{Percuss}
\DefineJournalPartialAbbreviation{Perfus}{Perfus}
\DefineJournalPartialAbbreviation{Perinatolog}{Perinatol}
\DefineJournalPartialAbbreviation{Periodi}{Period}
\DefineJournalPartialAbbreviation{Periodontolog}{Periodontol}
\DefineJournalAbbreviation{Permaculture}{Permac}
\DefineJournalPartialAbbreviation{Person}{Pers}
\DefineJournalPartialAbbreviation{Perspectiv}{Perspect}
\DefineJournalPartialAbbreviation{Petrolog}{Petrol}
\DefineJournalPartialAbbreviation{Pharmacodynam}{Pharmacodyn}
\DefineJournalPartialAbbreviation{Phenomenolog}{Phenomenol}
\DefineJournalPartialAbbreviation{Philanthrop}{Philanthr}
\DefineJournalPartialAbbreviation{Philharmoni}{Philharm}
\DefineJournalPartialAbbreviation{Philomathi}{Philomath}
\DefineJournalPartialAbbreviation{Philosoph}{Philos}
\DefineJournalPartialAbbreviation{Phlebolog}{Phlebol}
\DefineJournalPartialAbbreviation{Phoniatri}{Phoniatr}
\DefineJournalPartialAbbreviation{Phonolog}{Phonol}
\DefineJournalWordException{Phosphate}{Phosphate}
\DefineJournalWordException{Photo}{Photo}
\DefineJournalPartialAbbreviation{Photobiolog}{Photobiol}
\DefineJournalPartialAbbreviation{Photocop}{Photocop}
\DefineJournalPartialAbbreviation{Photogrammetr}{Photogramm}
\DefineJournalPartialAbbreviation{Photograph}{Photogr}
\DefineJournalPartialAbbreviation{Photojournal}{Photoj}
\DefineJournalPartialAbbreviation{Photometr}{Photom}
\DefineJournalPartialAbbreviation{Photophysiolog}{Photophysiol}
\DefineJournalPartialAbbreviation{Photoreact}{Photoreact}
\DefineJournalPartialAbbreviation{Physiatri}{Physiatr}
\DefineJournalPartialAbbreviation{Physich}{Phys}
\DefineJournalPartialAbbreviation{Physiogn}{Physiogn}
\DefineJournalPartialAbbreviation{Physiograph}{Physiogr}
\DefineJournalPartialAbbreviation{Physiolog}{Physiol}
\DefineJournalPartialAbbreviation{Physiopatholog}{Physiopathol}
\DefineJournalPartialAbbreviation{Physiotherap}{Physiother}
\DefineJournalPartialAbbreviation{Phytiatr}{Phytiatr}
\DefineJournalPartialAbbreviation{Phytochem}{Phytochem}
\DefineJournalAbbreviation{Phytocoenosis}{Phytocoen}
\DefineJournalPartialAbbreviation{Phytogenet}{Phytogenet}
\DefineJournalPartialAbbreviation{Phytogeograph}{Phytogeogr}
\DefineJournalPartialAbbreviation{Phytolog}{Phytol}
\DefineJournalPartialAbbreviation{Phytoparasit}{Phytoparasit}
\DefineJournalPartialAbbreviation{Phytopatholog}{Phytopathol}
\DefineJournalPartialAbbreviation{Phytotaxonom}{Phytotaxon}
\DefineJournalPartialAbbreviation{Phytoth\'erap}{Phytother}
\DefineJournalWordException{Piano}{Piano}
\DefineJournalWordException{Pianola}{Pianola}
\DefineJournalWordException{Pigeon}{Pigeon}
\DefineJournalPartialAbbreviation{Pigment}{Pigment}
\DefineJournalPartialAbbreviation{Pilot}{Pilot}
\DefineJournalPartialAbbreviation{Pinta}{Pint}
\DefineJournalWordException{Placenta}{Placenta}
\DefineJournalWordException{Plafond}{Plafond}
\DefineJournalPartialAbbreviation{Plakat}{Plakat}
\DefineJournalPartialAbbreviation{Planif}{Planif}
\DefineJournalWordException{Plantain}{Plantain}
\DefineJournalWordException{Plasma}{Plasma}
\DefineJournalPartialAbbreviation{Plasti}{Plast}
\DefineJournalWordException{Plateau}{Plateau}
\DefineJournalWordException{Platin}{Platin}
\DefineJournalAbbreviation{Plexus}{Plex}
\DefineJournalPartialAbbreviation{Plural}{Plur}
\DefineJournalWordException{Pluses}{Pluses}
\DefineJournalPartialAbbreviation{Pneumati}{Pneum}
\DefineJournalPartialAbbreviation{Pneumolog}{Pneumol}
\DefineJournalPartialAbbreviation{Pneumonolog}{Pneumonol}
\DefineJournalPartialAbbreviation{Podol}{Podol}
\DefineJournalPartialAbbreviation{Poet}{Poet}
\DefineJournalWordException{Point}{Point}
\DefineJournalPartialAbbreviation{Polarograph}{Polarogr}
\DefineJournalAbbreviation{Polen}{Pol}
\DefineJournalWordException{Polio}{Polio}
%\DefineJournalPartialWordException{Politi}{Politi-}
\DefineJournalPartialAbbreviation{Polycondensat}{Polycondens}
\DefineJournalAbbreviation{Polysaccharide}{Polysacch}
\DefineJournalPartialAbbreviation{Pontifi}{Pontif}
\DefineJournalWordException{Popstar}{Popstar}
\DefineJournalPartialAbbreviation{Popular}{Pop}
\DefineJournalPartialAbbreviation{Pornograph}{Pornogr}
\DefineJournalWordException{Portion}{Portion}
\DefineJournalWordException{Posterior}{Posterior}
\DefineJournalPartialAbbreviation{Postmagmati}{Postmagmat}
\DefineJournalWordException{Potassium}{Potassium}
\DefineJournalWordException{Potion}{Potion}
\DefineJournalWordException{Prague}{Prague}
\DefineJournalPartialAbbreviation{Prakt}{Prakt}
\DefineJournalPartialAbbreviation{Praximetr}{Praxim}
\DefineJournalAbbreviation{Praxis}{Prax}
\DefineJournalPartialAbbreviation{Prefabric}{Prefabr}
\DefineJournalPartialAbbreviation{Pr\'efac}{Pref}
\DefineJournalWordException{Pressefoto}{Pressefoto}
\DefineJournalAbbreviation{Pression}{Press}
\DefineJournalPartialAbbreviation{Prestig}{Prestig}
\DefineJournalPartialAbbreviation{Primatolog}{Primatol}
\DefineJournalPartialAbbreviation{Prirodoslovn}{Prirodosl}
\DefineJournalWordException{Probable}{Probable}
\DefineJournalPartialAbbreviation{Problem}{Probl}
\DefineJournalPartialAbbreviation{Professor}{Profr}
\DefineJournalWordException{Profil}{Profil}
\DefineJournalPartialAbbreviation{Profitab}{Profitab}
\DefineJournalPartialAbbreviation{Prognos}{Progn}
\DefineJournalWordException{Program}{Program}
\DefineJournalPartialAbbreviation{Proizvod}{Proizv}
\DefineJournalPartialAbbreviation{Prokur}{Prokur}
\DefineJournalPartialAbbreviation{Prophylax}{Prophyl}
\DefineJournalWordException{Prosa}{Prosa}
\DefineJournalWordException{Prostate}{Prostate}
\DefineJournalAbbreviation{Protestation}{Protest}
\DefineJournalPartialAbbreviation{Protistolog}{Protistol}
\DefineJournalPartialAbbreviation{Protozoolog}{Protozool}
\DefineJournalPartialAbbreviation{Provid}{Provid}
\DefineJournalPartialAbbreviation{Provocat}{Provocat}
\DefineJournalPartialAbbreviation{Proxim}{Prox}
\DefineJournalPartialAbbreviation{Pseudonym}{Pseud}
\DefineJournalPartialAbbreviation{Psicopedag}{Psicopedag}
\DefineJournalWordException{Psoriasis}{Psoriasis}
\DefineJournalPartialAbbreviation{Psychiatri}{Psychiatr}
\DefineJournalPartialAbbreviation{Psychobiolog}{Psychobiol}
\DefineJournalPartialAbbreviation{Psycholog}{Psychol}
\DefineJournalPartialAbbreviation{Psychometr}{Psychom}
\DefineJournalPartialAbbreviation{Psychoneurolog}{Psychoneurol}
\DefineJournalPartialAbbreviation{Psychonom}{Psychon}
\DefineJournalPartialAbbreviation{Psychosomat}{Psychosom}
\DefineJournalPartialAbbreviation{Psychotechni}{Psychotech}
\DefineJournalPartialAbbreviation{Psychoterap}{Psychoter}
\DefineJournalPartialAbbreviation{Psychotherap}{Psychother}
\DefineJournalPartialAbbreviation{Psychotrop}{Psychotr}
\DefineJournalWordException{Pyramide}{Pyramide}
\DefineJournalPartialAbbreviation{Pyrometr}{Pyrom}
\DefineJournalPartialAbbreviation{Quantit}{Quant}
\DefineJournalWordException{Quatuor}{Quatuor}
\DefineJournalWordException{Racismo}{Racismo}
\DefineJournalWordException{R\'adi\'o}{R\'adi\'o}
\DefineJournalPartialAbbreviation{R\'adi\'oamat}{Radioamat}
\DefineJournalPartialAbbreviation{Radioanaly}{Radioanal}
\DefineJournalPartialAbbreviation{Radioastronom}{Radioastron}
\DefineJournalPartialAbbreviation{Radiobiolog}{Radiobiol}
\DefineJournalPartialAbbreviation{Radiocommunic}{Radiocommun}
\DefineJournalWordException{Radiocontrol}{Radiocontrol}
\DefineJournalPartialAbbreviation{Radioelement}{Radioelem}
\DefineJournalPartialAbbreviation{Radiogeolog}{Radiogeol}
\DefineJournalPartialAbbreviation{Radiograph}{Radiogr}
\DefineJournalPartialAbbreviation{Radioindustri}{Radioind}
\DefineJournalPartialAbbreviation{Radioisotop}{Radioisot}
\DefineJournalPartialAbbreviation{Radiolaborat}{Radiolab}
\DefineJournalPartialAbbreviation{Radiolog}{Radiol}
\DefineJournalPartialAbbreviation{Radiometr}{Radiom}
\DefineJournalPartialAbbreviation{Radiophysiolog}{Radiophysiol}
\DefineJournalPartialAbbreviation{Radiotelemetr}{Radiotelem}
\DefineJournalPartialAbbreviation{Radiotelev}{Radiotelev}
\DefineJournalPartialAbbreviation{Radiotherap}{Radiother}
\DefineJournalWordException{Rallycross}{Rallycross}
\DefineJournalAbbreviation{Ramification}{Ramif}
\DefineJournalAbbreviation{Raphaelite}{Raphael}
\DefineJournalWordException{Ratable}{Ratable}
\DefineJournalPartialAbbreviation{Razveden}{Razved}
\DefineJournalPartialAbbreviation{Razvit}{Razvit}
\DefineJournalPartialAbbreviation{Realiz}{Realiz}
\DefineJournalPartialAbbreviation{Reanimatolog}{Reanimatol}
\DefineJournalPartialAbbreviation{Referenc}{Ref}
\DefineJournalWordException{Reflex}{Reflex}
\DefineJournalPartialAbbreviation{Refus}{Refus}
\DefineJournalAbbreviation{Regio}{Reg}
\DefineJournalPartialAbbreviation{Region}{Reg}
\DefineJournalPartialAbbreviation{Regist}{Regist}
\DefineJournalPartialAbbreviation{Regulament}{Regulam}
\DefineJournalPartialAbbreviation{R\'ehabilitat}{Rehabil}
\DefineJournalPartialAbbreviation{Relev}{Relev}
\DefineJournalAbbreviation{Renaissance}{Renaiss}
\DefineJournalAbbreviation{Rendement}{Rend}
\DefineJournalPartialAbbreviation{Replace}{Replace}
\DefineJournalPartialAbbreviation{Reptil}{Reptil}
\DefineJournalPartialAbbreviation{Republik}{Repub}
\DefineJournalPartialAbbreviation{Reserv}{Reserv}
\DefineJournalPartialAbbreviation{Residenc}{Resid}
\DefineJournalWordException{Respekt}{Respekt}
\DefineJournalPartialAbbreviation{Responsab}{Responsab}
\DefineJournalPartialAbbreviation{Restaurant}{Restaur}
\DefineJournalPartialAbbreviation{Retard}{Retard}
\DefineJournalAbbreviation{Retrovirus}{Retrovir}
\DefineJournalAbbreviation{Revendication}{Revendic}
\DefineJournalPartialAbbreviation{Rhapsod}{Rhaps}
\DefineJournalPartialAbbreviation{Rhenan}{Rhenan}
\DefineJournalPartialAbbreviation{Rheolog}{Rheol}
\DefineJournalPartialAbbreviation{Rheumati}{Rheum}
\DefineJournalPartialAbbreviation{Rheumatolog}{Rheumatol}
\DefineJournalPartialAbbreviation{Rhinolog}{Rhinol}
\DefineJournalAbbreviation{Risalah}{Risal}
\DefineJournalAbbreviation{Romance}{Roman}
\DefineJournalWordException{Rondeau}{Rondeau}
\DefineJournalPartialAbbreviation{Rosenthalian}{Rosenthal}
\DefineJournalWordException{Rotary}{Rotary}
\DefineJournalAbbreviation{Rotisserie}{Rotiss}
\DefineJournalWordException{Rotterdam}{Rotterdam}
\DefineJournalWordException{Roulotte}{Roulotte}
%\DefineJournalPartialWordException{Ruch}{Ruch-}
\DefineJournalAbbreviation{Ruminant}{Rumin}
\DefineJournalWordException{Rupestre}{Rupestre}
\DefineJournalPartialAbbreviation{Rural}{Rural}
\DefineJournalAbbreviation{Saccharide}{Sacch}
\DefineJournalPartialAbbreviation{Sacrific}{Sacrif}
\DefineJournalWordException{Safari}{Safari}
\DefineJournalWordException{Sahel}{Sahel}
\DefineJournalWordException{Salon}{Salon}
\DefineJournalWordException{Saloon}{Saloon}
\DefineJournalWordException{Samitis}{Samitis}
\DefineJournalAbbreviation{Sammenslutning}{Sammenslut}
\DefineJournalAbbreviation{San Francisco}{San Franc}
\DefineJournalAbbreviation{Sanctus}{St}
\DefineJournalWordException{Sarasvati}{Sarasvati}
%\DefineJournalPartialWordException{Sarmat}{Sarmat-}
\DefineJournalPartialAbbreviation{Satisf}{Satisf}
\DefineJournalWordException{Sauna}{Sauna}
\DefineJournalWordException{Savans}{Savans}
\DefineJournalWordException{Scanair}{Scanair}
\DefineJournalPartialAbbreviation{Scandic}{Scand}
\DefineJournalWordException{Sceptre}{Sceptre}
\DefineJournalPartialAbbreviation{Schizophren}{Schizophr}
\DefineJournalPartialAbbreviation{Sedimentolog}{Sedimentol}
\DefineJournalAbbreviation{Segment}{Segm}
\DefineJournalPartialAbbreviation{Seism}{Seism}
\DefineJournalPartialAbbreviation{Sektor}{Sekt}
\DefineJournalPartialAbbreviation{Seminar}{Semin}
\DefineJournalPartialAbbreviation{Semioti}{Semiot}
\DefineJournalAbbreviation{Senile}{Sen}
\DefineJournalPartialAbbreviation{Senolog}{Senol}
\DefineJournalPartialAbbreviation{Sensibil}{Sensib}
\DefineJournalAbbreviation{Sensible}{Sensib}
\DefineJournalPartialAbbreviation{Septentrional}{Septentr}
\DefineJournalPartialAbbreviation{Sequen}{Seq}
\DefineJournalAbbreviation{Serie}{Ser}
\DefineJournalPartialAbbreviation{Seriolog}{Seriol}
\DefineJournalPartialAbbreviation{Serolog}{Serol}
\DefineJournalPartialAbbreviation{Serotaxonom}{Serotaxon}
\DefineJournalWordException{Sesame}{Sesame}
\DefineJournalPartialAbbreviation{Sexolog}{Sexol}
\DefineJournalWordException{Seychelles}{Seychelles}
\DefineJournalWordException{Shanghai}{Shanghai}
\DefineJournalPartialAbbreviation{Siderurgi}{Sider}
\DefineJournalPartialAbbreviation{Sifiliograf}{Sifiliogr}
\DefineJournalPartialAbbreviation{Sifilograph}{Sifilogr}
\DefineJournalWordException{Sigle}{Sigle}
\DefineJournalPartialAbbreviation{Silent}{Silent}
\DefineJournalPartialAbbreviation{Singul}{Singul}
\DefineJournalPartialAbbreviation{Sinolog}{Sinol}
\DefineJournalPartialAbbreviation{\v Skol}{Sk}
\DefineJournalPartialAbbreviation{Slovakist}{Slovak}
\DefineJournalPartialAbbreviation{Sociocultur}{Sociocult}
\DefineJournalWordException{Sodium}{Sodium}
\DefineJournalPartialAbbreviation{Sonor}{Son}
\DefineJournalPartialAbbreviation{Sophistic}{Sophistic}
\DefineJournalPartialAbbreviation{Soviet}{Sov}
\DefineJournalPartialAbbreviation{Speculation}{Specul}
\DefineJournalPartialAbbreviation{Speleolog}{Speleol}
\DefineJournalPartialAbbreviation{Spermatolog}{Spermatol}
\DefineJournalWordException{Sphinx}{Sphinx}
\DefineJournalPartialAbbreviation{Splenolog}{Splenol}
\DefineJournalWordException{Spore}{Spore}
\DefineJournalWordException{Sport}{Sport}
\DefineJournalAbbreviation{Square}{Sq}
\DefineJournalAbbreviation{Stalinism- }{Stalin}
\DefineJournalPartialAbbreviation{Statist}{Stat}
\DefineJournalWordException{Stellenbosch}{Stellenbosch}
\DefineJournalWordException{Stencil}{Stencil}
\DefineJournalPartialAbbreviation{Stereolog}{Stereol}
\DefineJournalPartialAbbreviation{Stereophon}{Stereoph}
\DefineJournalPartialAbbreviation{Stipend}{Stipend}
\DefineJournalAbbreviation{Stipulation}{Stipul}
\DefineJournalPartialAbbreviation{Stomatolog}{Stomatol}
\DefineJournalPartialAbbreviation{Strateg}{Strateg}
\DefineJournalPartialAbbreviation{Stress}{Stress}
\DefineJournalPartialAbbreviation{Student}{Stud}
\DefineJournalWordException{St\'udi\'o}{St\'udi\'o}
\DefineJournalPartialAbbreviation{Subalpin}{Subalp}
\DefineJournalPartialAbbreviation{Submerg}{Submerg}
\DefineJournalPartialAbbreviation{Subnorm}{Subnorm}
\DefineJournalPartialAbbreviation{Subsid}{Subsid}
\DefineJournalAbbreviation{Substrat}{Substr}
\DefineJournalPartialAbbreviation{Subtrop}{Subtrop}
\DefineJournalPartialAbbreviation{Subvers}{Subvers}
\DefineJournalWordException{Succesromanen}{Succesromanen}
\DefineJournalPartialAbbreviation{Suicidolog}{Suicidol}
\DefineJournalWordException{Supercross}{Supercross}
\DefineJournalWordException{Supermoto}{Supermoto}
\DefineJournalWordException{Support}{Support}
\DefineJournalPartialAbbreviation{Support}{Support}
\DefineJournalAbbreviation{Surplus}{Surpl}
\DefineJournalPartialAbbreviation{Suspens}{Suspens}
\DefineJournalWordException{Sutra}{Sutra}
\DefineJournalWordException{Swahili}{Swahili}
\DefineJournalPartialAbbreviation{Symbol}{Symb}
\DefineJournalWordException{Sympathie}{Sympathie}
\DefineJournalPartialAbbreviation{Sympos}{Symp}
\DefineJournalPartialAbbreviation{Sympoz}{Symp}
\DefineJournalAbbreviation{Synapse}{Synap}
\DefineJournalPartialAbbreviation{Syndrom}{Syndr}
\DefineJournalPartialAbbreviation{Synopt}{Synop}
\DefineJournalPartialAbbreviation{Synthes}{Synth}
\DefineJournalPartialAbbreviation{Synthet}{Synth}
\DefineJournalPartialAbbreviation{Syphiligraph}{Syphiligr}
\DefineJournalAbbreviation{Syphilis}{Syph}
\DefineJournalPartialAbbreviation{Syphiliti}{Syph}
\DefineJournalPartialAbbreviation{Syphilolog}{Syphilol}
\DefineJournalWordException{Syracuse}{Syracuse}
\DefineJournalPartialAbbreviation{Syri}{Syr}
\DefineJournalWordException{Taekwondo}{Taekwondo}
\DefineJournalWordException{Taisce}{Taisce}
\DefineJournalWordException{Taiwan}{Taiwan}
\DefineJournalWordException{Tantra}{Tantra}
\DefineJournalWordException{Tantum}{Tantum}
\DefineJournalPartialAbbreviation{Tarif}{Tarif}
\DefineJournalWordException{Tautos}{Tautos}
\DefineJournalPartialAbbreviation{Taxonom}{Taxon}
\DefineJournalWordException{Tchernobyl}{Tchernobyl}
\DefineJournalPartialAbbreviation{Teatr}{Teatr}
\DefineJournalPartialAbbreviation{Techni}{Tech}
\DefineJournalPartialAbbreviation{Technolog}{Technol}
\DefineJournalPartialAbbreviation{Tekni}{Tek}
\DefineJournalWordException{Telecom}{Telecom}
\DefineJournalWordException{Telefax}{Telefax}
\DefineJournalPartialAbbreviation{Telefon}{Telef}
\DefineJournalPartialAbbreviation{Telegraph}{Telegr}
\DefineJournalPartialAbbreviation{Telemechani}{Telemech}
\DefineJournalPartialAbbreviation{Telesympos}{Telesymp}
\DefineJournalWordException{Tenerife}{Tenerife}
\DefineJournalPartialAbbreviation{Teoreti}{Teor}
\DefineJournalPartialAbbreviation{Termal}{Termal}
\DefineJournalPartialAbbreviation{Terminolog}{Terminol}
\DefineJournalPartialAbbreviation{Termoidraulic}{Termoidraul}
\DefineJournalPartialAbbreviation{Thalass}{Thalass}
\DefineJournalPartialAbbreviation{Thanatolog}{Thanatol}
\DefineJournalAbbreviation{Theknos}{Thek}
\DefineJournalPartialAbbreviation{Theriolog}{Th\'eriol}
\DefineJournalPartialAbbreviation{Thermobiolog}{Thermobiol}
\DefineJournalPartialAbbreviation{Thermograph}{Thermogr}
\DefineJournalPartialAbbreviation{Thermolog}{Thermol}
\DefineJournalPartialAbbreviation{Thermometr}{Thermom}
\DefineJournalPartialAbbreviation{Thermoregulat}{Thermor\'egul}
\DefineJournalWordException{Thesaurus}{Thesaurus}
\DefineJournalWordException{Thinktank}{Thinktank}
\DefineJournalWordException{Thorax}{Thorax}
\DefineJournalPartialAbbreviation{Thrombos}{Thromb}
\DefineJournalWordException{Thule}{Thule}
\DefineJournalPartialAbbreviation{Thyroid}{Thyroid}
\DefineJournalPartialAbbreviation{Tibet}{Tibet}
\DefineJournalWordException{Tirage}{Tirage}
\DefineJournalWordException{Titan}{Titan}
\DefineJournalWordException{Toboggan}{Toboggan}
\DefineJournalWordException{Tonus}{Tonus}
\DefineJournalPartialAbbreviation{Topograph}{Topogr}
\DefineJournalPartialAbbreviation{Topometr}{Topom}
\DefineJournalAbbreviation{Touring}{Tour}
\DefineJournalPartialAbbreviation{Toxicom}{Toxicom}
\DefineJournalWordException{Trace}{Trace}
\DefineJournalWordException{Tracer}{Tracer}
\DefineJournalPartialAbbreviation{Trachom}{Trach}
\DefineJournalPartialAbbreviation{Tradition}{Tradit}
%\DefineJournalPartialWordException{Trafic}{Trafic-}
\DefineJournalPartialAbbreviation{Transact}{Trans}
\DefineJournalPartialAbbreviation{Transform}{Transform}
\DefineJournalPartialAbbreviation{Transfront}{Transfront}
\DefineJournalWordException{Transvaal}{Transvaal}
\DefineJournalPartialAbbreviation{Trasplant}{Traspl}
\DefineJournalPartialAbbreviation{Traumatolog}{Traumatol}
\DefineJournalWordException{Trial}{Trial}
\DefineJournalWordException{Triathlon}{Triathlon}
\DefineJournalWordException{Tribu}{Tribu}
\DefineJournalAbbreviation{Tribulation}{Tribul}
\DefineJournalPartialAbbreviation{Tricolor}{Tricolor}
\DefineJournalWordException{Trident}{Trident}
\DefineJournalPartialAbbreviation{Trilingu}{Triling}
\DefineJournalAbbreviation{Trisaccharide}{Trisacch}
\DefineJournalWordException{Tritium}{Tritium}
\DefineJournalAbbreviation{Trombone}{Tromb}
\DefineJournalPartialAbbreviation{Trompet}{Trompet}
\DefineJournalPartialAbbreviation{Tropi}{Trop}
\DefineJournalPartialAbbreviation{Troubl}{Troubl}
\DefineJournalPartialAbbreviation{Trypanos}{Trypanos}
\DefineJournalPartialAbbreviation{Tuberkuloz}{Tuberk}
\DefineJournalWordException{Tutor}{Tutor}
\DefineJournalPartialAbbreviation{Ufolog}{Ufol}
\DefineJournalPartialAbbreviation{Ugostit}{Ugost}
\DefineJournalAbbreviation{Ulster}{Ulst}
\DefineJournalWordException{Ultra}{Ultra}
\DefineJournalWordException{Ultrapure}{Ultrapure}
\DefineJournalPartialAbbreviation{Ultrason}{Ultrason}
\DefineJournalAbbreviation{Ultraterrestre}{Ultraterr}
%\DefineJournalPartialWordException{Unifi}{Unifi-}
\DefineJournalAbbreviation{Uniforme}{Unif}
\DefineJournalWordException{Unique}{Unique}
\DefineJournalPartialAbbreviation{Urbanis}{Urban}
\DefineJournalAbbreviation{Urogynaecologia}{Urogynaecol}
\DefineJournalPartialAbbreviation{Urolog}{Urol}
\DefineJournalWordException{Utgift}{Utgift}
\DefineJournalAbbreviation{Vaccination}{Vaccin}
%\DefineJournalPartialWordException{Vagin}{Vagin-}
\DefineJournalAbbreviation{Validation}{Valid}
\DefineJournalWordException{Valuta}{Valuta}
\DefineJournalWordException{Varia}{Varia}
\DefineJournalWordException{Vatican}{Vatican}
\DefineJournalPartialAbbreviation{Velocit}{Veloc}
\DefineJournalPartialAbbreviation{Veneri}{Vener}
\DefineJournalPartialAbbreviation{Venerolog}{Venerol}
%\DefineJournalPartialWordException{Venet}{Venet-}
\DefineJournalWordException{Veranda}{Veranda}
\DefineJournalWordException{Vernis}{Vernis}
\DefineJournalWordException{Version}{Version}
\DefineJournalPartialAbbreviation{Vestig}{Vestig}
\DefineJournalAbbreviation{Videotaping}{Videotap}
\DefineJournalPartialAbbreviation{Vietnam}{Vietnam}
\DefineJournalPartialAbbreviation{Vigilanc}{Vigil}
\DefineJournalWordException{Villa}{Villa}
\DefineJournalWordException{Violence}{Violence}
\DefineJournalWordException{Violet}{Violet}
\DefineJournalPartialAbbreviation{Violin}{Violin}
\DefineJournalPartialAbbreviation{Virolog}{Virol}
\DefineJournalWordException{Virus}{Virus}
\DefineJournalAbbreviation{Visayas}{Vis}
\DefineJournalWordException{Vista}{Vista}
\DefineJournalPartialAbbreviation{Vitamini}{Vitam}
\DefineJournalPartialAbbreviation{Vitaminolog}{Vitaminol}
\DefineJournalWordException{Vitiligo}{Vitiligo}
\DefineJournalWordException{Vogue}{Vogue}
\DefineJournalPartialAbbreviation{Volum}{Vol}
\DefineJournalPartialAbbreviation{Volunt}{Volunt}
\DefineJournalPartialAbbreviation{Vulcanism}{Vulcan}
\DefineJournalWordException{Watersport}{Watersport}
\DefineJournalWordException{Website}{Website}
\DefineJournalAbbreviation{Xenofobia}{Xenofob}
\DefineJournalPartialAbbreviation{Xylophon}{Xyloph}
\DefineJournalWordException{Yacht}{Yacht}
\DefineJournalWordException{Ydyapeetha}{Ydyapeetha}
\DefineJournalPartialAbbreviation{Yiddish}{Yid}
\DefineJournalPartialAbbreviation{Yidish}{Yid}
\DefineJournalWordException{Zagreb}{Zagreb}
\DefineJournalPartialAbbreviation{Zagreb}{Zagreb}
\DefineJournalWordException{Za\"ire}{Za\"ire}
\DefineJournalPartialAbbreviation{Zaklad}{Zakl}
\DefineJournalPartialAbbreviation{Zeland}{Zeland}
\DefineJournalWordException{Zeppelin}{Zeppelin}
\DefineJournalWordException{Zigzag}{Zigzag}
\DefineJournalAbbreviation{Zimbabwe}{Zimb}
\DefineJournalAbbreviation{Zirconium}{Zircon}
\DefineJournalPartialAbbreviation{Zna\v c}{Zna\v c}
\DefineJournalPartialAbbreviation{Zoolog}{Zo\"ol}
\DefineJournalPartialAbbreviation{Zoophysiolog}{Zoophysiol}
\DefineJournalPartialAbbreviation{Zooveterinar}{Zoovet}
\DefineJournalPartialAbbreviation{Zymolog}{Zymol}

==> jabbrv-ltwa-en.ldf.tex <==
%% Copyright 2010-2019 Erich E. Hoover
%% E-mail: erich.e.hoover@gmail.com
%% 
%% =============================================
%% IMPORTANT NOTICE:
%% 
%% This work may be distributed and/or modified under the conditions
%% of the LaTeX Project Public License, either version 1.3c of this
%% license or (at your option) any later version.
%% The latest version of this license is available at
%%   http://www.latex-project.org/lppl.txt
%% =============================================
%% The List of Title Word Abbreviations below is automatically
%% generated from the ISSN LTWA database, publicly accessible from
%% their website:
%%   http://www.issn.org/2-22660-LTWA.php

\DefineJournalWordException{Abacus}{Abacus}
\DefineJournalWordException{Abalone}{Abalone}
\DefineJournalAbbreviation{Abatement}{Abat}
\DefineJournalWordException{Abbasid}{Abbasid}
\DefineJournalWordException{Abbey}{Abbey}
\DefineJournalAbbreviation{Abbreviation}{Abbr}
\DefineJournalAbbreviation{Abdominal}{Abdom}
\DefineJournalAbbreviation{Abeokuta}{Abeok}
\DefineJournalWordException{Abercrombie}{Abercrombie}
\DefineJournalAbbreviation{Aberdeen}{Aberd}
\DefineJournalWordException{Aberystwyth}{Aberystwyth}
\DefineJournalAbbreviation{Abiding}{Abid}
\DefineJournalWordException{Abietta}{Abietta}
\DefineJournalPartialAbbreviation{Abilit}{Abil}
\DefineJournalAbbreviation{Abington}{Abingt}
\DefineJournalWordException{Abixedarian}{Abixedarian}
\DefineJournalPartialAbbreviation{Abnormal}{Abnorm}
\DefineJournalWordException{Abode}{Abode}
\DefineJournalPartialAbbreviation{Aborig}{Aborig}
\DefineJournalPartialAbbreviation{Abort}{Abort}
\DefineJournalAbbreviation{Abrasive}{Abras}
\DefineJournalWordException{Abreast}{Abreast}
\DefineJournalAbbreviation{Abridged}{Abr}
\DefineJournalAbbreviation{Abridgment}{Abr}
\DefineJournalWordException{Abroad}{Abroad}
\DefineJournalAbbreviation{Absenteism}{Absent}
\DefineJournalAbbreviation{Absorption}{Absorpt}
\DefineJournalAbbreviation{Abstinence}{Abstin}
\DefineJournalPartialAbbreviation{Abstract}{Abstr}
\DefineJournalWordException{Abuja}{Abuja}
\DefineJournalPartialAbbreviation{Abundant}{Abund}
\DefineJournalPartialAbbreviation{Abus}{Abus}
\DefineJournalWordException{Acacia}{Acacia}
\DefineJournalPartialAbbreviation{Academ}{Acad}
\DefineJournalWordException{Acamedia}{Acamedia}
\DefineJournalAbbreviation{Acaricide}{Acaric}
\DefineJournalPartialAbbreviation{Acarolog}{Acarol}
\DefineJournalPartialAbbreviation{Accelerat}{Accel}
\DefineJournalPartialAbbreviation{Accept}{Accept}
\DefineJournalWordException{Access}{Access}
\DefineJournalAbbreviation{Accessing}{Access}
\DefineJournalPartialAbbreviation{Accession}{Access}
\DefineJournalWordException{Accessory}{Accessory}
\DefineJournalPartialAbbreviation{Accident}{Accid}
\DefineJournalPartialAbbreviation{Acclimat}{Acclim}
\DefineJournalPartialAbbreviation{Accommodat}{Accommod}
\DefineJournalAbbreviation{Accomodation}{Accomod}
\DefineJournalAbbreviation{Accompany}{Acco}
\DefineJournalPartialAbbreviation{Accord}{Accord}
\DefineJournalWordException{Accordion}{Accordion}
\DefineJournalAbbreviation{Account}{Acc}
\DefineJournalAbbreviation{Accountability}{Account}
\DefineJournalAbbreviation{Accountancy}{Account}
\DefineJournalAbbreviation{Accountant}{Account}
\DefineJournalAbbreviation{Accounting}{Account}
\DefineJournalAbbreviation{Accredited}{Accredit}
\DefineJournalPartialAbbreviation{Accultur}{Accult}
\DefineJournalAbbreviation{Accumulative}{Accumul}
\DefineJournalAbbreviation{Accumulator}{Accumul}
\DefineJournalWordException{Accuracy}{Accuracy}
\DefineJournalWordException{Achaemenid}{Achaemenid}
\DefineJournalPartialAbbreviation{Achievement}{Achiev}
\DefineJournalAbbreviation{Achiever}{Achiev}
\DefineJournalAbbreviation{Achieving}{Achiev}
\DefineJournalWordException{Achimoowin}{Achimoowin}
\DefineJournalPartialAbbreviation{Acidificat}{Acidif}
\DefineJournalPartialAbbreviation{Acousti}{Acoust}
\DefineJournalPartialAbbreviation{Acoustoelectroni}{Acoustoelectron}
\DefineJournalPartialAbbreviation{Acquir}{Acquir}
\DefineJournalPartialAbbreviation{Acquisition}{Acquis}
\DefineJournalWordException{Acreage}{Acreage}
\DefineJournalAbbreviation{Acrobatic}{Acrobat}
\DefineJournalAbbreviation{Acronym}{Acron}
\DefineJournalWordException{Across}{Across}
\DefineJournalAbbreviation{Acting}{Act}
\DefineJournalPartialAbbreviation{Actinotherap}{Actinother}
\DefineJournalWordException{Action}{Action}
\DefineJournalWordException{Actor}{Actor}
\DefineJournalWordException{Actress}{Actress}
\DefineJournalWordException{Actual}{Actual}
\DefineJournalPartialAbbreviation{Actuali}{Actual}
\DefineJournalPartialAbbreviation{Actuar}{Actuar}
\DefineJournalWordException{Actuator}{Actuator}
\DefineJournalAbbreviation{Acupuncture}{Acupunct}
\DefineJournalAbbreviation{Adamantine}{Adamant}
\DefineJournalPartialAbbreviation{Adapt}{Adapt}
\DefineJournalPartialAbbreviation{Adaptogen}{Adaptog}
\DefineJournalAbbreviation{Adbook}{Adb}
\DefineJournalPartialAbbreviation{Addicti}{Addict}
\DefineJournalAbbreviation{Addington}{Addingt}
\DefineJournalPartialAbbreviation{Addition}{Addit}
\DefineJournalPartialAbbreviation{Additive}{Addit}
\DefineJournalWordException{Address}{Address}
\DefineJournalAbbreviation{Adelaide}{Adel}
\DefineJournalWordException{Aden}{Aden}
\DefineJournalWordException{Adequacy}{Adequacy}
\DefineJournalWordException{Adequate}{Adequate}
\DefineJournalWordException{Adipose}{Adipose}
\DefineJournalAbbreviation{Adirondack}{Adirond}
\DefineJournalPartialAbbreviation{Adjoin}{Adjoin}
\DefineJournalAbbreviation{Adjunct}{Adjun}
\DefineJournalPartialAbbreviation{Adjust}{Adjust}
\DefineJournalAbbreviation{Adjuster}{Adjust}
\DefineJournalAbbreviation{Adjutant}{Adjut}
\DefineJournalPartialAbbreviation{Adjuvan}{Adjuv}
\DefineJournalWordException{Adlerian}{Adlerian}
\DefineJournalPartialAbbreviation{Adletter}{Adlett}
\DefineJournalPartialAbbreviation{Administer}{Adm}
\DefineJournalWordException{Admirable}{Admirable}
\DefineJournalAbbreviation{Admiralty}{Admir}
\DefineJournalAbbreviation{Admission}{Admiss}
\DefineJournalAbbreviation{Admixture}{Admix}
\DefineJournalPartialAbbreviation{Adolescen}{Adolesc}
\DefineJournalPartialAbbreviation{Adrenerg}{Adren}
\DefineJournalPartialAbbreviation{Adsorpti}{Adsorpt}
\DefineJournalPartialAbbreviation{Advanc}{Adv}
\DefineJournalAbbreviation{Advantage}{Advant}
\DefineJournalWordException{Advent}{Advent}
\DefineJournalAbbreviation{Adventist}{Advent}
\DefineJournalWordException{Adventure}{Adventure}
\DefineJournalWordException{Adventurer}{Adventurer}
\DefineJournalPartialAbbreviation{Advertis}{Advert}
\DefineJournalWordException{Advice}{Advice}
\DefineJournalPartialAbbreviation{Advis}{Advis}
\DefineJournalWordException{Advocacy}{Advocacy}
\DefineJournalWordException{Advocate}{Advocate}
\DefineJournalWordException{Aegean}{Aegean}
\DefineJournalWordException{Aerated}{Aerated}
\DefineJournalAbbreviation{Aerial}{Aer}
\DefineJournalPartialAbbreviation{Aerobic}{Aerob}
\DefineJournalPartialAbbreviation{Aerobiolog}{Aerobiol}
\DefineJournalPartialAbbreviation{Aeroioniz}{Aeroioniz}
\DefineJournalAbbreviation{Aerojet}{Aeroj}
\DefineJournalAbbreviation{Aeromagnetic}{Aeromagn}
\DefineJournalPartialAbbreviation{Aeromedica}{Aeromed}
\DefineJournalPartialAbbreviation{Aeroplan}{Aeropl}
\DefineJournalAbbreviation{Aerospace}{Aerosp}
\DefineJournalPartialAbbreviation{Aerospatial}{Aerosp}
\DefineJournalPartialAbbreviation{Aerothermochemi}{Aerothermochem}
\DefineJournalPartialAbbreviation{Aerothermodynami}{Aerothermodyn}
\DefineJournalAbbreviation{Aesthetics}{Aesthet}
\DefineJournalPartialAbbreviation{Affair}{Aff}
\DefineJournalPartialAbbreviation{Affect}{Affect}
\DefineJournalPartialAbbreviation{Affili}{Affil}
\DefineJournalAbbreviation{Affiliateship}{Affiliatesh}
\DefineJournalPartialAbbreviation{Affirm}{Affirm}
\DefineJournalAbbreviation{Affordability}{Affordabil}
\DefineJournalAbbreviation{Affordable}{Afford}
\DefineJournalWordException{Afghanaid}{Afghanaid}
\DefineJournalWordException{Afield}{Afield}
\DefineJournalWordException{Aflame}{Aflame}
\DefineJournalWordException{Afloat}{Afloat}
\DefineJournalPartialAbbreviation{Africa}{Afr}
\DefineJournalAbbreviation{Afroasiatic}{Afroasiat}
\DefineJournalAbbreviation{Afterloading}{Afterload}
\DefineJournalAbbreviation{Aftermarket}{Aftermark}
\DefineJournalWordException{Afternoon}{Afternoon}
\DefineJournalWordException{Aftersales}{Aftersales}
\DefineJournalAbbreviation{Aftertreatment}{Aftertreat}
\DefineJournalWordException{Against}{Against}
\DefineJournalWordException{Agassiz}{Agassiz}
\DefineJournalAbbreviation{Agbioindustry}{Agbioind}
\DefineJournalWordException{Agbowo}{Agbowo}
\DefineJournalWordException{Ageing}{Ageing}
\DefineJournalWordException{Agency}{Agency}
\DefineJournalWordException{Agenda}{Agenda}
\DefineJournalWordException{Agent}{Agent}
%\DefineJournalPartialWordException{Ageway}{Ageway-}
\DefineJournalPartialAbbreviation{Agglomerat}{Agglom}
\DefineJournalAbbreviation{Aggregate}{Aggreg}
\DefineJournalAbbreviation{Aggregation}{Aggreg}
\DefineJournalPartialAbbreviation{Aggressi}{Aggress}
\DefineJournalWordException{Aghadoe}{Aghadoe}
\DefineJournalWordException{Agincourt}{Agincourt}
\DefineJournalWordException{Aging}{Aging}
\DefineJournalWordException{Aglow}{Aglow}
\DefineJournalWordException{Agnosia}{Agnosia}
\DefineJournalPartialAbbreviation{Agrari}{Agrar}
\DefineJournalAbbreviation{Agreement}{Agreem}
\DefineJournalPartialAbbreviation{Agribiolog}{Agribiol}
\DefineJournalAbbreviation{Agrichemical}{Agrichem}
\DefineJournalPartialAbbreviation{Agr\'icol}{Agric}
\DefineJournalPartialAbbreviation{Agricult}{Agric}
\DefineJournalPartialAbbreviation{Agrochemi}{Agrochem}
\DefineJournalPartialAbbreviation{Agroecol}{Agroecol}
\DefineJournalAbbreviation{Agroforestry}{Agrofor}
\DefineJournalWordException{Ahead}{Ahead}
\DefineJournalWordException{Aided}{Aided}
\DefineJournalAbbreviation{Ailment}{Ailm}
\DefineJournalWordException{Aiming}{Aiming}
\DefineJournalWordException{Air-cushion}{Air-cushion}
\DefineJournalWordException{Airborne}{Airborne}
\DefineJournalAbbreviation{Airbrush}{Airbr}
\DefineJournalAbbreviation{Aircraft}{Aircr}
\DefineJournalAbbreviation{Airforce}{Airf}
\DefineJournalAbbreviation{Airfreight}{Airfr}
\DefineJournalWordException{Airgun}{Airgun}
\DefineJournalAbbreviation{Airline}{Airl}
\DefineJournalWordException{Airman}{Airman}
\DefineJournalWordException{Airmiss}{Airmiss}
\DefineJournalAbbreviation{Airplane}{Airpl}
\DefineJournalAbbreviation{Airport}{Airpt}
\DefineJournalAbbreviation{Airship}{Airsh}
\DefineJournalAbbreviation{Airspace}{Airsp}
\DefineJournalAbbreviation{Airway}{Airw}
\DefineJournalAbbreviation{Airworthiness}{Airworth}
\DefineJournalWordException{Akure}{Akure}
\DefineJournalPartialAbbreviation{Alabama}{Ala}
\DefineJournalWordException{Alanvale}{Alanvale}
\DefineJournalWordException{Albacore}{Albacore}
\DefineJournalWordException{Albania}{Albania}
\DefineJournalWordException{Albany}{Albany}
\DefineJournalAbbreviation{Alberta}{Alta}
\DefineJournalWordException{Albertain}{Albertain}
\DefineJournalAbbreviation{Albertan}{Alta}
\DefineJournalWordException{Albino}{Albino}
\DefineJournalWordException{Albion}{Albion}
\DefineJournalAbbreviation{Albuquerque}{Albuq}
\DefineJournalWordException{Albury-Wodonga}{Albury-Wodonga}
\DefineJournalPartialAbbreviation{Alchemist}{Alchem}
\DefineJournalWordException{Alchemy}{Alchemy}
\DefineJournalWordException{Alcohol}{Alcohol}
\DefineJournalPartialAbbreviation{Alcoholi}{Alcohol}
\DefineJournalWordException{Alembic}{Alembic}
\DefineJournalWordException{Alep}{Alep}
\DefineJournalWordException{Alert}{Alert}
\DefineJournalWordException{Alexandra}{Alexandra}
\DefineJournalWordException{Algarve}{Algarve}
\DefineJournalWordException{Algeciras}{Algeciras}
\DefineJournalWordException{Algoma}{Algoma}
\DefineJournalAbbreviation{Algonquian}{Algonq}
\DefineJournalAbbreviation{Algonquin}{Algonq}
\DefineJournalWordException{Algorithm}{Algorithm}
\DefineJournalWordException{Alicyclic}{Alicyclic}
\DefineJournalWordException{Alimony}{Alimony}
\DefineJournalWordException{Aliphatic}{Aliphatic}
\DefineJournalWordException{Alipore}{Alipore}
\DefineJournalWordException{Alive}{Alive}
\DefineJournalWordException{Alkaline}{Alkaline}
\DefineJournalPartialAbbreviation{Alkylat}{Alkylat}
\DefineJournalAbbreviation{Allegheny}{Allegh}
\DefineJournalPartialAbbreviation{Allelochemi}{Allelochem}
\DefineJournalPartialAbbreviation{Allelopath}{Allelopath}
\DefineJournalAbbreviation{Allergen}{Allerg}
\DefineJournalPartialAbbreviation{Allergi}{Allerg}
\DefineJournalWordException{Allergy}{Allergy}
\DefineJournalWordException{Alliage}{Alliage}
\DefineJournalWordException{Alliance}{Alliance}
\DefineJournalWordException{Allied}{Allied}
\DefineJournalWordException{Alligator}{Alligator}
\DefineJournalAbbreviation{Allotment}{Allot}
\DefineJournalPartialAbbreviation{Allow}{Allow}
\DefineJournalPartialAbbreviation{Alloy}{Alloy}
\DefineJournalPartialAbbreviation{Allumin}{Allum}
\DefineJournalPartialAbbreviation{Almanac}{Alm}
\DefineJournalWordException{Alopecia}{Alopecia}
\DefineJournalWordException{Alpes}{Alpes}
\DefineJournalPartialAbbreviation{Alphabet}{Alph}
\DefineJournalAbbreviation{Alpine}{Alp}
\DefineJournalWordException{Alsager}{Alsager}
\DefineJournalWordException{Altaic}{Altaic}
\DefineJournalAbbreviation{Alteration}{Alter}
\DefineJournalPartialAbbreviation{Alternat}{Altern}
\DefineJournalAbbreviation{Altitude}{Alt}
\DefineJournalWordException{Alton}{Alton}
\DefineJournalAbbreviation{Aluminium}{Alum}
\DefineJournalAbbreviation{Aluminum}{Alum}
\DefineJournalWordException{Alumneye}{Alumneye}
\DefineJournalWordException{Alvinston}{Alvinston}
\DefineJournalWordException{Always}{Always}
\DefineJournalWordException{Alyeska}{Alyeska}
\DefineJournalAbbreviation{Amalgamate}{Amalgam}
\DefineJournalPartialAbbreviation{Amaranth}{Amaran}
\DefineJournalPartialAbbreviation{Amaz}{Amaz}
\DefineJournalWordException{Amblyopia}{Amblyopia}
\DefineJournalWordException{Ambrosia}{Ambrosia}
\DefineJournalPartialAbbreviation{Ambulanc}{Ambulanc}
\DefineJournalAbbreviation{Ambulatory}{Ambul}
\DefineJournalWordException{Ameliasburgh}{Ameliasburgh}
\DefineJournalPartialAbbreviation{Amend}{Amend}
\DefineJournalWordException{Amenity}{Amenity}
\DefineJournalWordException{Amenorrhoea}{Amenorrhoea}
%\DefineJournalPartialWordException{Amerasia}{Amerasia-}
\DefineJournalPartialAbbreviation{America}{Am}
\DefineJournalWordException{Amethyst}{Amethyst}
\DefineJournalWordException{Amherst}{Amherst}
\DefineJournalWordException{Amine}{Amine}
\DefineJournalAbbreviation{Amityville}{Amityv}
\DefineJournalPartialAbbreviation{Ammonia}{Ammon}
\DefineJournalAbbreviation{Ammunition}{Ammunit}
\DefineJournalWordException{Amnesty}{Amnesty}
\DefineJournalPartialAbbreviation{Amorph}{Amorph}
\DefineJournalPartialAbbreviation{Amount}{Amount}
\DefineJournalAbbreviation{Amplification}{Amplif}
\DefineJournalAbbreviation{Amplifier}{Amplif}
\DefineJournalWordException{Amtmann}{Amtmann}
\DefineJournalAbbreviation{Amusement}{Amus}
\DefineJournalAbbreviation{Amyotrophic}{Amyotroph}
\DefineJournalWordException{Anabantoid}{Anabantoid}
\DefineJournalPartialAbbreviation{Anaboli}{Anab}
\DefineJournalWordException{Anacampseros}{Anacampseros}
\DefineJournalWordException{Anadrome}{Anadrome}
\DefineJournalWordException{Anaemia}{Anaemia}
\DefineJournalAbbreviation{Anaerobic}{Anaerob}
\DefineJournalAbbreviation{Anaesthesia}{Anaesth}
\DefineJournalPartialAbbreviation{Anaesthesiolog}{Anaesthesiol}
\DefineJournalPartialAbbreviation{Anaesthet}{Anaesth}
\DefineJournalAbbreviation{Anals}{An}
\DefineJournalPartialAbbreviation{Analyt}{Anal}
\DefineJournalPartialAbbreviation{Analyz}{Anal}
\DefineJournalAbbreviation{Anambra}{Anam}
\DefineJournalAbbreviation{Anaphylaxie}{Anaphyl}
\DefineJournalWordException{Anarsis}{Anarsis}
\DefineJournalAbbreviation{Anatolian}{Anatol}
\DefineJournalAbbreviation{Anatomy}{Anat}
\DefineJournalWordException{Ancaster}{Ancaster}
\DefineJournalWordException{Ancestor}{Ancestor}
\DefineJournalWordException{Ancestry}{Ancestry}
\DefineJournalWordException{Anchor}{Anchor}
\DefineJournalWordException{Anchorage}{Anchorage}
\DefineJournalAbbreviation{Ancient}{Anc}
\DefineJournalWordException{Ancillary}{Ancillary}
\DefineJournalWordException{Andean}{Andean}
\DefineJournalWordException{Andover}{Andover}
\DefineJournalPartialAbbreviation{Androgen}{Androg}
\DefineJournalAbbreviation{Andrology}{Androl}
\DefineJournalWordException{Anecdota}{Anecdota}
\DefineJournalPartialAbbreviation{Anesth\'es}{Anesth}
\DefineJournalPartialAbbreviation{Anesthesiolog}{Anesthesiol}
\DefineJournalPartialAbbreviation{Anesthet}{Anesth}
\DefineJournalWordException{Angelus}{Angelus}
\DefineJournalPartialAbbreviation{Angiograph}{Angiogr}
\DefineJournalAbbreviation{Angiosurgery}{Angiosurg}
\DefineJournalPartialAbbreviation{Angiotherap}{Angiother}
\DefineJournalWordException{Angler}{Angler}
\DefineJournalAbbreviation{Anglican}{Angl}
\DefineJournalWordException{Angling}{Angling}
\DefineJournalPartialAbbreviation{Animat}{Animat}
\DefineJournalAbbreviation{Ankylosing}{Ankyl}
\DefineJournalWordException{Ann Arbor}{Ann Arbor}
\DefineJournalPartialAbbreviation{Annal}{Ann}
\DefineJournalWordException{Annandale}{Annandale}
\DefineJournalAbbreviation{Annapolis}{Annap}
\DefineJournalPartialAbbreviation{Annivers}{Anniv}
\DefineJournalPartialAbbreviation{Annotat}{Annot}
\DefineJournalPartialAbbreviation{Announc}{Announc}
\DefineJournalWordException{Annoying}{Annoying}
\DefineJournalPartialAbbreviation{Annu}{Annu}
\DefineJournalWordException{Annuity}{Annuity}
\DefineJournalWordException{Anodic}{Anodic}
\DefineJournalAbbreviation{Anointing}{Anoint}
\DefineJournalAbbreviation{Anomaly}{Anom}
\DefineJournalAbbreviation{Anonymous}{Anon}
\DefineJournalWordException{Another}{Another}
\DefineJournalAbbreviation{Answer}{Answ}
\DefineJournalPartialAbbreviation{Antarcti}{Antarct}
\DefineJournalWordException{Antenna}{Antenna}
\DefineJournalWordException{Anthracite}{Anthracite}
\DefineJournalPartialAbbreviation{Anthropogen}{Anthropog}
\DefineJournalPartialAbbreviation{Anthropograph}{Anthropor}
\DefineJournalAbbreviation{Anthroposophy}{Anthropos}
\DefineJournalAbbreviation{Anti-dumping}{Anti-dump}
\DefineJournalAbbreviation{Antiarrhythmic}{Antiarrhythm}
\DefineJournalAbbreviation{Antibacterial}{Antibact}
\DefineJournalPartialAbbreviation{Antibiotherap}{Antibiother}
\DefineJournalAbbreviation{Antibody}{Antib}
\DefineJournalPartialAbbreviation{Anticancer}{Anticancer}
\DefineJournalPartialAbbreviation{Anticarcinogen}{Anticarcinog}
\DefineJournalPartialAbbreviation{Anticip}{Anticip}
\DefineJournalPartialAbbreviation{Antifung}{Antifung}
\DefineJournalWordException{Antigens}{Antigens}
\DefineJournalPartialAbbreviation{Antihypertensi}{Antihypertens}
\DefineJournalPartialAbbreviation{Antiinfecti}{Antiinfect}
\DefineJournalPartialAbbreviation{Antimalaria}{Antimalar}
\DefineJournalPartialAbbreviation{Antimicrobi}{Antimicrob}
\DefineJournalAbbreviation{Antineoplastic}{Antineoplast}
\DefineJournalWordException{Antinomy}{Antinomy}
\DefineJournalPartialAbbreviation{Antinuclear}{Antinucl}
\DefineJournalPartialAbbreviation{Antinutrient}{Antinutr}
\DefineJournalAbbreviation{Antioxidant}{Antioxid}
\DefineJournalWordException{Antiplague}{Antiplague}
%\DefineJournalPartialWordException{Antipoison}{Antipoison-}
\DefineJournalAbbreviation{Antipollution}{Antipollut}
\DefineJournalPartialAbbreviation{Antiqu}{Antiq}
\DefineJournalPartialAbbreviation{Antirecessi}{Antirecess}
\DefineJournalPartialAbbreviation{Antiretrovir}{Antiretrovir}
\DefineJournalPartialAbbreviation{Antirheumati}{Antirheum}
\DefineJournalPartialAbbreviation{Antiseismi}{Antiseism}
\DefineJournalWordException{Antiserum}{Antiserum}
\DefineJournalWordException{Antitrust}{Antitrust}
\DefineJournalPartialAbbreviation{Antituberculos}{Antituberc}
\DefineJournalWordException{Antitumor}{Antitumor}
\DefineJournalAbbreviation{Antiviral}{Antivir}
\DefineJournalWordException{Antwerp}{Antwerp}
\DefineJournalWordException{Anxiety}{Anxiety}
\DefineJournalWordException{Apartheid}{Apartheid}
\DefineJournalAbbreviation{Apartment}{Apartm}
\DefineJournalPartialAbbreviation{Apathogenic}{Apathog}
\DefineJournalPartialAbbreviation{Aphaere}{Aphaer}
\DefineJournalWordException{Aphasia}{Aphasia}
\DefineJournalPartialAbbreviation{Aphere}{Apher}
\DefineJournalPartialAbbreviation{Apicult}{Apic}
\DefineJournalPartialAbbreviation{Aplica}{Apl}
\DefineJournalAbbreviation{Apostolate}{Apostol}
\DefineJournalAbbreviation{Apostolic}{Apostol}
\DefineJournalAbbreviation{Appalachian}{Appalach}
\DefineJournalWordException{Appaloosa}{Appaloosa}
\DefineJournalAbbreviation{Apparel}{Appar}
\DefineJournalWordException{Appeal}{Appeal}
\DefineJournalPartialAbbreviation{Appear}{Appear}
\DefineJournalAbbreviation{Appetiser}{Appet}
\DefineJournalWordException{Applecore}{Applecore}
\DefineJournalAbbreviation{Appliance}{Appl}
\DefineJournalPartialAbbreviation{Applica}{Appl}
\DefineJournalAbbreviation{Applied}{Appl}
\DefineJournalAbbreviation{Applying}{Appl}
\DefineJournalPartialAbbreviation{Appoint}{Appoint}
\DefineJournalAbbreviation{Appointment}{Appointm}
\DefineJournalPartialAbbreviation{Apprais}{Apprais}
\DefineJournalWordException{Appraise}{Appraise}
\DefineJournalAbbreviation{Appreciation}{Apprec}
\DefineJournalPartialAbbreviation{Apprentic}{Apprent}
\DefineJournalAbbreviation{Apprenticeship}{Apprenticesh}
\DefineJournalWordException{Approach}{Approach}
\DefineJournalAbbreviation{Appropriate}{Appropr}
\DefineJournalAbbreviation{Appropriation}{Appropr}
\DefineJournalPartialAbbreviation{Approv}{Approv}
\DefineJournalPartialAbbreviation{Approximat}{Approx}
\DefineJournalPartialAbbreviation{Aprax}{Aprax}
\DefineJournalAbbreviation{Apricot}{Apric}
\DefineJournalPartialAbbreviation{Aquacultur}{Aquac}
\DefineJournalPartialAbbreviation{Aquaricultur}{Aquaric}
\DefineJournalPartialAbbreviation{Aquatech}{Aquatech}
\DefineJournalPartialAbbreviation{Aquati}{Aquat}
\DefineJournalWordException{Arable}{Arable}
\DefineJournalWordException{Arachis}{Arachis}
\DefineJournalWordException{Aramaic}{Aramaic}
\DefineJournalWordException{Aramoana}{Aramoana}
\DefineJournalPartialAbbreviation{Arboricult}{Arboric}
\DefineJournalWordException{Arcadia}{Arcadia}
\DefineJournalWordException{Arcata}{Arcata}
\DefineJournalPartialAbbreviation{Archaeoastronom}{Archaeoastron}
\DefineJournalPartialAbbreviation{Archaeolog}{Archaeol}
\DefineJournalPartialAbbreviation{Archaeometallurg}{Archaeometall}
\DefineJournalPartialAbbreviation{Archaeometr}{Archaeom}
\DefineJournalAbbreviation{Archdeaconry}{Archdeac}
\DefineJournalAbbreviation{Archdiocese}{Archdioc}
\DefineJournalPartialAbbreviation{Archeolog}{Archeol}
\DefineJournalWordException{Archer}{Archer}
\DefineJournalWordException{Archery}{Archery}
\DefineJournalAbbreviation{Archipelago}{Archipel}
\DefineJournalPartialAbbreviation{Architect}{Archit}
\DefineJournalPartialAbbreviation{Architectoni}{Architecton}
\DefineJournalAbbreviation{Arctic}{Arct}
\DefineJournalWordException{Ardfert}{Ardfert}
\DefineJournalWordException{Ardmore}{Ardmore}
\DefineJournalWordException{Arecanut}{Arecanut}
\DefineJournalPartialAbbreviation{Argonaut}{Argon}
\DefineJournalAbbreviation{Arising}{Aris}
\DefineJournalPartialAbbreviation{Aristotel}{Aristot}
\DefineJournalPartialAbbreviation{Arithmeti}{Arith}
\DefineJournalPartialAbbreviation{Arizona}{Ariz}
\DefineJournalAbbreviation{Arkansas}{Ark}
\DefineJournalAbbreviation{Arlington}{Arlingt}
\DefineJournalWordException{Armchair}{Armchair}
\DefineJournalAbbreviation{Armdale}{Armd}
\DefineJournalWordException{Armed}{Armed}
\DefineJournalAbbreviation{Armenia}{Armen}
\DefineJournalAbbreviation{Armenian}{Armen}
\DefineJournalWordException{Armoury}{Armoury}
\DefineJournalAbbreviation{Aromatherapy}{Aromather}
\DefineJournalWordException{Around}{Around}
\DefineJournalPartialAbbreviation{Arrangement}{Arrange}
\DefineJournalPartialAbbreviation{Arrear}{Arrear}
\DefineJournalWordException{Arrest}{Arrest}
\DefineJournalAbbreviation{Arrhythmias}{Arrhythm}
\DefineJournalAbbreviation{Arrival}{Arriv}
\DefineJournalWordException{Arrow}{Arrow}
\DefineJournalAbbreviation{Arrowhead}{Arrowh}
\DefineJournalWordException{Arsenal}{Arsenal}
\DefineJournalWordException{Artcraft}{Artcraft}
\DefineJournalWordException{Artemia}{Artemia}
\DefineJournalWordException{Artery}{Artery}
\DefineJournalPartialAbbreviation{Artheroscleros}{Artheroscler}
\DefineJournalPartialAbbreviation{Arthroplast}{Arthroplast}
\DefineJournalWordException{Arthropod}{Arthropod}
\DefineJournalPartialAbbreviation{Arthroscop}{Arthrosc}
\DefineJournalAbbreviation{Arthroscopy}{Arthrosc}
\DefineJournalAbbreviation{Arthurian}{Arthur}
\DefineJournalPartialAbbreviation{Articul}{Articul}
\DefineJournalWordException{Artifact}{Artifact}
\DefineJournalPartialAbbreviation{Artifici}{Artif}
\DefineJournalAbbreviation{Artillery}{Artill}
\DefineJournalWordException{Artview}{Artview}
\DefineJournalWordException{Aryan}{Aryan}
\DefineJournalWordException{Asbestos}{Asbestos}
\DefineJournalAbbreviation{Asbestosis}{Asbestos}
\DefineJournalWordException{Asbury}{Asbury}
\DefineJournalWordException{Ascot}{Ascot}
\DefineJournalWordException{Ashante}{Ashante}
\DefineJournalWordException{Asheboro}{Asheboro}
\DefineJournalAbbreviation{Ashford}{Ashf}
\DefineJournalAbbreviation{Ashkenazic}{Ashken}
\DefineJournalWordException{Asian}{Asian}
\DefineJournalPartialAbbreviation{Asistenc}{Asist}
\DefineJournalWordException{Asking}{Asking}
\DefineJournalWordException{Asparagus}{Asparagus}
\DefineJournalWordException{Aspergillus}{Aspergillus}
%\DefineJournalPartialWordException{Assault}{Assault-}
\DefineJournalAbbreviation{Assayer}{Assay}
\DefineJournalPartialAbbreviation{Assert}{Assert}
\DefineJournalAbbreviation{Assessed}{Assess}
\DefineJournalAbbreviation{Assessing}{Assess}
\DefineJournalAbbreviation{Assessment}{Assess}
\DefineJournalAbbreviation{Assignment}{Assign}
\DefineJournalPartialAbbreviation{Assimil}{Assim}
\DefineJournalWordException{Assiniboia}{Assiniboia}
\DefineJournalPartialAbbreviation{Associ}{Assoc}
\DefineJournalAbbreviation{Assumption}{Assumpt}
\DefineJournalPartialAbbreviation{Assur}{Assur}
\DefineJournalWordException{Assyrian}{Assyrian}
\DefineJournalPartialAbbreviation{Asteroseismolog}{Asteroseismol}
\DefineJournalAbbreviation{Astonishing}{Astonish}
\DefineJournalPartialAbbreviation{Astrobiolog}{Astrobiol}
\DefineJournalPartialAbbreviation{Astrochemi}{Astrochem}
\DefineJournalPartialAbbreviation{Astrodynam}{Astrodyn}
\DefineJournalPartialAbbreviation{Astrometr}{Astrom}
\DefineJournalAbbreviation{Astroparticle}{Astropart}
\DefineJournalWordException{Astute}{Astute}
\DefineJournalWordException{Asylum}{Asylum}
\DefineJournalAbbreviation{Asymptotic}{Asymptot}
\DefineJournalWordException{Ataxia}{Ataxia}
\DefineJournalWordException{Athabaska}{Athabaska}
\DefineJournalWordException{Atheist}{Atheist}
\DefineJournalAbbreviation{Athenian}{Athen}
\DefineJournalWordException{Athens}{Athens}
\DefineJournalPartialAbbreviation{Atherogen}{Atherog}
\DefineJournalPartialAbbreviation{Atherosclero}{Atheroscler}
\DefineJournalPartialAbbreviation{Atherosclerolog}{Atherosclerol}
\DefineJournalPartialAbbreviation{Athletic}{Athl}
\DefineJournalWordException{Atlanta}{Atlanta}
\DefineJournalPartialAbbreviation{Atlanti}{Atl}
\DefineJournalAbbreviation{Atlantic}{Atl}
\DefineJournalWordException{Atomindex}{Atomindex}
\DefineJournalAbbreviation{Atrial}{Atr}
\DefineJournalAbbreviation{Attainment}{Attain}
\DefineJournalPartialAbbreviation{Attend}{Attend}
\DefineJournalAbbreviation{Attention}{Atten}
\DefineJournalWordException{Attitude}{Attitude}
\DefineJournalPartialAbbreviation{Attorney}{Atty}
\DefineJournalPartialAbbreviation{Attraction}{Attract}
\DefineJournalAbbreviation{Attractive}{Attract}
\DefineJournalAbbreviation{Atypical}{Atyp}
\DefineJournalWordException{Auburn}{Auburn}
\DefineJournalWordException{Auburndale}{Auburndale}
\DefineJournalAbbreviation{Auchenorrhyncha}{Auchen}
\DefineJournalAbbreviation{Auckland}{Auckl}
\DefineJournalPartialAbbreviation{Auction}{Auction}
\DefineJournalAbbreviation{Audaccount}{Audacc}
\DefineJournalWordException{Audience}{Audience}
\DefineJournalAbbreviation{Audio-visual}{Audio-v}
\DefineJournalWordException{Audiotape}{Audiotape}
\DefineJournalAbbreviation{Audiovision}{Audiov}
\DefineJournalAbbreviation{Audiovisual}{Audiov}
\DefineJournalWordException{Augusta}{Augusta}
\DefineJournalWordException{Augustan}{Augustan}
\DefineJournalPartialAbbreviation{Augustinian}{Augustin}
\DefineJournalWordException{Auricular}{Auricular}
\DefineJournalAbbreviation{Auroral}{Auror}
\DefineJournalWordException{Ausoil}{Ausoil}
\DefineJournalWordException{Auspice}{Auspice}
\DefineJournalWordException{Aussie}{Aussie}
\DefineJournalWordException{Austin}{Austin}
\DefineJournalPartialAbbreviation{Australasia}{Australas}
\DefineJournalWordException{Austria}{Austria}
\DefineJournalWordException{Austrian}{Austrian}
\DefineJournalAbbreviation{Authenticity}{Authent}
\DefineJournalWordException{Author}{Author}
\DefineJournalPartialAbbreviation{Authoris}{Auth}
\DefineJournalAbbreviation{Authority}{Auth}
\DefineJournalPartialAbbreviation{Authoriz}{Auth}
\DefineJournalWordException{Autism}{Autism}
\DefineJournalWordException{Autoharp}{Autoharp}
\DefineJournalPartialAbbreviation{Autoimmunit}{Autoimmun}
\DefineJournalAbbreviation{Autoionization}{Autoioniz}
\DefineJournalWordException{Autoline}{Autoline}
\DefineJournalPartialAbbreviation{Automobil}{Automob}
\DefineJournalWordException{Automotion}{Automotion}
\DefineJournalAbbreviation{Automotive}{Automot}
\DefineJournalWordException{Autoparts}{Autoparts}
\DefineJournalAbbreviation{Autoxidation}{Autoxid}
\DefineJournalWordException{Autumn}{Autumn}
\DefineJournalPartialAbbreviation{Auxilia}{Aux}
\DefineJournalAbbreviation{Availability}{Availab}
\DefineJournalWordException{Available}{Available}
\DefineJournalWordException{Avebury}{Avebury}
\DefineJournalAbbreviation{Avenger}{Aveng}
\DefineJournalPartialAbbreviation{Avenue}{Ave}
\DefineJournalAbbreviation{Average}{Aver}
\DefineJournalWordException{Aviary}{Aviary}
\DefineJournalPartialAbbreviation{Aviation}{Aviat}
\DefineJournalAbbreviation{Aviator}{Aviat}
\DefineJournalPartialAbbreviation{Avion}{Avion}
\DefineJournalWordException{Avocado}{Avocado}
\DefineJournalPartialAbbreviation{Avoid}{Avoid}
\DefineJournalWordException{Avonmore}{Avonmore}
\DefineJournalPartialAbbreviation{Awak}{Awak}
\DefineJournalPartialAbbreviation{Award}{Award}
\DefineJournalAbbreviation{Awareness}{Aware}
\DefineJournalWordException{Awning}{Awning}
\DefineJournalWordException{Aylesbury}{Aylesbury}
\DefineJournalWordException{Aylmer}{Aylmer}
\DefineJournalAbbreviation{Ayrshire}{Ayrsh}
\DefineJournalWordException{\=Ayurvedic}{\=Ayurvedic}
\DefineJournalAbbreviation{Babylonian}{Babylon}
\DefineJournalPartialAbbreviation{Babysitt}{Babysitt}
\DefineJournalWordException{Bachelor}{Bachelor}
\DefineJournalAbbreviation{Bacillary}{Bacill}
\DefineJournalPartialAbbreviation{Backcalculat}{Backcalc}
\DefineJournalAbbreviation{Backgammon}{Backgam}
\DefineJournalAbbreviation{Background}{Backgr}
\DefineJournalAbbreviation{Backpacker}{Backpack}
\DefineJournalWordException{Backstage}{Backstage}
\DefineJournalWordException{Backstretch}{Backstretch}
\DefineJournalWordException{Backwoods}{Backwoods}
\DefineJournalAbbreviation{Backwoodsman}{Backwoodsm}
\DefineJournalWordException{Backyard}{Backyard}
\DefineJournalWordException{Bacon}{Bacon}
\DefineJournalPartialAbbreviation{Bacteria}{Bact}
\DefineJournalPartialAbbreviation{Bacterie}{Bact}
\DefineJournalPartialAbbreviation{Bacteriolog}{Bacteriol}
\DefineJournalAbbreviation{Bacterium}{Bact}
\DefineJournalWordException{Badger}{Badger}
\DefineJournalWordException{Badminton}{Badminton}
\DefineJournalWordException{Baghdad}{Baghdad}
\DefineJournalWordException{Bahamas}{Bahamas}
\DefineJournalWordException{Bahrain}{Bahrain}
\DefineJournalWordException{Bailout}{Bailout}
\DefineJournalWordException{Bairnsdale}{Bairnsdale}
\DefineJournalPartialAbbreviation{Baker}{Bak}
\DefineJournalAbbreviation{Baking}{Bak}
\DefineJournalWordException{Balaclava}{Balaclava}
\DefineJournalWordException{Balasore}{Balasore}
\DefineJournalPartialAbbreviation{Balcanic}{Balc}
\DefineJournalPartialAbbreviation{Ballad}{Ballad}
\DefineJournalWordException{Ballarat}{Ballarat}
\DefineJournalWordException{Ballast}{Ballast}
\DefineJournalAbbreviation{Ballerina}{Baller}
\DefineJournalWordException{Ballet}{Ballet}
\DefineJournalWordException{Ballina}{Ballina}
\DefineJournalWordException{Ballincollig}{Ballincollig}
\DefineJournalWordException{Ballintrillick}{Ballintrillick}
\DefineJournalPartialAbbreviation{Ballisti}{Ballist}
\DefineJournalPartialAbbreviation{Balloon}{Balloon}
\DefineJournalWordException{Ballroom}{Ballroom}
\DefineJournalWordException{Ballydonoghue}{Ballydonoghue}
\DefineJournalPartialAbbreviation{Balneotherap}{Balneother}
\DefineJournalAbbreviation{Baltimore}{Baltim}
\DefineJournalWordException{Bamboo}{Bamboo}
\DefineJournalAbbreviation{Bamfield}{Bamf}
\DefineJournalPartialAbbreviation{Banan}{Banan}
\DefineJournalAbbreviation{Banding}{Band}
\DefineJournalWordException{Bandmaster}{Bandmaster}
\DefineJournalAbbreviation{Bandsman}{Bandsm}
\DefineJournalAbbreviation{Bandwagon}{Bandwag}
\DefineJournalWordException{Bangalore}{Bangalore}
\DefineJournalAbbreviation{Bangor}{Bang}
\DefineJournalWordException{Banjul}{Banjul}
\DefineJournalWordException{Bankcard}{Bankcard}
\DefineJournalAbbreviation{Banker}{Bank}
\DefineJournalAbbreviation{Banking}{Bank}
\DefineJournalWordException{Banknote}{Banknote}
\DefineJournalWordException{Bankruptcy}{Bankruptcy}
\DefineJournalAbbreviation{Bankstown}{Bankst}
\DefineJournalWordException{Banner}{Banner}
\DefineJournalWordException{Bannister}{Bannister}
\DefineJournalWordException{Banquet}{Banquet}
\DefineJournalWordException{Bantam}{Bantam}
\DefineJournalWordException{Banyan}{Banyan}
\DefineJournalPartialAbbreviation{Baptist}{Baptist}
\DefineJournalWordException{Baradine}{Baradine}
\DefineJournalPartialAbbreviation{Barbar}{Barbar}
\DefineJournalWordException{Barber}{Barber}
\DefineJournalPartialAbbreviation{Bargain}{Bargain}
\DefineJournalAbbreviation{Bariatric}{Bariatr}
\DefineJournalAbbreviation{Barker}{Bark}
\DefineJournalWordException{Barley}{Barley}
\DefineJournalPartialAbbreviation{Baroreceptor}{Barorecept}
\DefineJournalWordException{Barrackpore}{Barrackpore}
\DefineJournalWordException{Barrens}{Barrens}
\DefineJournalWordException{Barrier}{Barrier}
\DefineJournalAbbreviation{Barrington}{Barringt}
\DefineJournalWordException{Barrister}{Barrister}
\DefineJournalAbbreviation{Barrytown}{Barryt}
\DefineJournalAbbreviation{Barter}{Bart}
\DefineJournalWordException{Barton}{Barton}
\DefineJournalAbbreviation{Baseball}{Baseb}
\DefineJournalWordException{Basebook}{Basebook}
\DefineJournalWordException{Baseline}{Baseline}
\DefineJournalWordException{Basement}{Basement}
\DefineJournalWordException{Basic}{Basic}
\DefineJournalAbbreviation{Basically}{Basic}
\DefineJournalAbbreviation{Basilian}{Basil}
\DefineJournalWordException{Basin}{Basin}
\DefineJournalWordException{Basingstoke}{Basingstoke}
\DefineJournalAbbreviation{Basketball}{Basketb}
\DefineJournalAbbreviation{Basketmaker}{Basketmak}
\DefineJournalAbbreviation{Bassist}{Bass}
\DefineJournalAbbreviation{Bassoonist}{Bassoon}
\DefineJournalWordException{Bastard}{Bastard}
\DefineJournalAbbreviation{Basutoland}{Basutol}
\DefineJournalAbbreviation{Bathing}{Bath}
\DefineJournalAbbreviation{Bathroom}{Bathr}
\DefineJournalWordException{Bathurst}{Bathurst}
\DefineJournalPartialAbbreviation{Bathymetri}{Bathym\`etr}
\DefineJournalWordException{Baton Rouge}{Baton Rouge}
\DefineJournalWordException{Battalion}{Battalion}
\DefineJournalPartialAbbreviation{Batter}{Batter}
\DefineJournalWordException{Battersea}{Battersea}
\DefineJournalWordException{Battery}{Battery}
\DefineJournalWordException{Battle}{Battle}
\DefineJournalPartialAbbreviation{Battlefield}{Battlef}
\DefineJournalAbbreviation{Battleford}{Battlef}
\DefineJournalWordException{Bauchi}{Bauchi}
\DefineJournalWordException{Baulkham Hills}{Baulkham Hills}
\DefineJournalAbbreviation{Bavarian}{Bavar}
\DefineJournalWordException{Bayesian}{Bayesian}
\DefineJournalWordException{Bayline}{Bayline}
\DefineJournalAbbreviation{Baylor}{Bayl}
\DefineJournalWordException{Bayonet}{Bayonet}
\DefineJournalWordException{Bayview}{Bayview}
\DefineJournalWordException{Bazaar}{Bazaar}
\DefineJournalWordException{Beach}{Beach}
\DefineJournalAbbreviation{Beacon}{Beac}
\DefineJournalAbbreviation{Beaconsfield}{Beaconsfld}
\DefineJournalWordException{Beagle}{Beagle}
\DefineJournalAbbreviation{Beamsville}{Beamsv}
\DefineJournalAbbreviation{Bearer}{Bear}
\DefineJournalPartialAbbreviation{Bearing}{Bear}
\DefineJournalWordException{Beaten}{Beaten}
\DefineJournalAbbreviation{Beatitude}{Beatit}
\DefineJournalAbbreviation{Beauceville}{Beaucev}
\DefineJournalWordException{Beaumont}{Beaumont}
\DefineJournalWordException{Beautician}{Beautician}
\DefineJournalWordException{Beautiful}{Beautiful}
\DefineJournalWordException{Beauty}{Beauty}
\DefineJournalWordException{Beaver}{Beaver}
\DefineJournalAbbreviation{Bechuanaland}{Bechuanal}
\DefineJournalAbbreviation{Becoming}{Becom}
\DefineJournalWordException{Bedding}{Bedding}
\DefineJournalWordException{Beddington}{Beddington}
\DefineJournalWordException{Bedford}{Bedford}
\DefineJournalAbbreviation{Bedfordshire}{Beds}
\DefineJournalWordException{Bedroom}{Bedroom}
\DefineJournalWordException{Bedside}{Bedside}
\DefineJournalAbbreviation{Beechcraft}{Beechcr}
\DefineJournalWordException{Beehive}{Beehive}
\DefineJournalPartialAbbreviation{Beekeeper}{Beekeep}
\DefineJournalAbbreviation{Beekeeping}{Beekeep}
\DefineJournalWordException{Before}{Before}
\DefineJournalAbbreviation{Befriending}{Befriend}
\DefineJournalAbbreviation{Beginner}{Begin}
\DefineJournalAbbreviation{Beginning}{Begin}
\DefineJournalPartialAbbreviation{Behavior}{Behav}
\DefineJournalPartialAbbreviation{Behaviour}{Behav}
\DefineJournalWordException{Behind}{Behind}
\DefineJournalAbbreviation{Belarussian}{Belarus}
\DefineJournalWordException{Belconnen}{Belconnen}
\DefineJournalAbbreviation{Belfast}{Belf}
\DefineJournalPartialAbbreviation{Belgi}{Belg}
\DefineJournalWordException{Belief}{Belief}
\DefineJournalWordException{Believe}{Believe}
\DefineJournalWordException{Bellanca}{Bellanca}
\DefineJournalWordException{Bellflower}{Bellflower}
\DefineJournalWordException{Bellow}{Bellow}
\DefineJournalWordException{Belmont}{Belmont}
\DefineJournalPartialAbbreviation{Belong}{Belong}
\DefineJournalWordException{Belting}{Belting}
\DefineJournalWordException{Benchmark}{Benchmark}
\DefineJournalWordException{Bendel}{Bendel}
\DefineJournalPartialAbbreviation{Benefici}{Benef}
\DefineJournalWordException{Benefit}{Benefit}
\DefineJournalWordException{Benevolent}{Benevolent}
\DefineJournalWordException{Bengal}{Bengal}
\DefineJournalWordException{Bengali}{Bengali}
\DefineJournalWordException{Benin}{Benin}
\DefineJournalWordException{Bennie}{Bennie}
\DefineJournalPartialAbbreviation{Bentholog}{Benthol}
\DefineJournalWordException{Bentley}{Bentley}
\DefineJournalWordException{Benue}{Benue}
\DefineJournalWordException{Benzene}{Benzene}
\DefineJournalWordException{Benzole}{Benzole}
\DefineJournalWordException{Bequest}{Bequest}
\DefineJournalAbbreviation{Bereavement}{Bereave}
\DefineJournalAbbreviation{Bergenfield}{Bergenf}
\DefineJournalWordException{Berkeley}{Berkeley}
\DefineJournalWordException{Berkhamstead}{Berkhamstead}
\DefineJournalWordException{Berkhamsted}{Berkhamsted}
\DefineJournalAbbreviation{Berkshire}{Berks}
\DefineJournalPartialAbbreviation{Bermud}{Bermud}
\DefineJournalAbbreviation{Bermudagrass}{Bermudagr}
\DefineJournalWordException{Berne}{Berne}
\DefineJournalWordException{Berry}{Berry}
\DefineJournalWordException{Berwick}{Berwick}
\DefineJournalAbbreviation{Berwickshire}{Berwicks}
\DefineJournalAbbreviation{Bestseller}{Bestsell}
\DefineJournalWordException{Bethesda}{Bethesda}
\DefineJournalWordException{Better}{Better}
%\DefineJournalPartialWordException{Betting}{Betting-}
\DefineJournalWordException{Between}{Between}
\DefineJournalWordException{Beverage}{Beverage}
\DefineJournalWordException{Beverly Hills}{Beverly Hills}
\DefineJournalWordException{Beware}{Beware}
\DefineJournalWordException{Beyond}{Beyond}
\DefineJournalWordException{Bhubaneswar}{Bhubaneswar}
\DefineJournalAbbreviation{Bi-weekly}{Bi-wkly}
\DefineJournalAbbreviation{Biannual}{Biannu}
\DefineJournalAbbreviation{Biblioservice}{Biblioserv}
\DefineJournalPartialAbbreviation{Bibliothec}{Bibl}
\DefineJournalPartialAbbreviation{Bicenten}{Bicenten}
\DefineJournalWordException{Bichon}{Bichon}
\DefineJournalPartialAbbreviation{Bicycl}{Bicycl}
\DefineJournalWordException{Bidlake}{Bidlake}
\DefineJournalAbbreviation{Bienal}{Bien}
\DefineJournalAbbreviation{Biennial}{Bienn}
\DefineJournalPartialAbbreviation{Biennual}{Bienn}
\DefineJournalPartialAbbreviation{Bifidobacteri}{Bifidobact}
\DefineJournalWordException{Biggles}{Biggles}
\DefineJournalWordException{Biker}{Biker}
\DefineJournalAbbreviation{Bilateral}{Bilat\'er}
\DefineJournalAbbreviation{Bilharziasis}{Bilharz}
\DefineJournalWordException{Biliary}{Biliary}
\DefineJournalPartialAbbreviation{Bilingu}{Biling}
\DefineJournalWordException{Billboard}{Billboard}
\DefineJournalAbbreviation{Billennium}{Billen}
\DefineJournalWordException{Billiard}{Billiard}
\DefineJournalWordException{Billing}{Billing}
\DefineJournalAbbreviation{Bimonthly}{Bimon}
\DefineJournalPartialAbbreviation{Binar}{Bin}
\DefineJournalAbbreviation{Binational}{Binatl}
\DefineJournalPartialAbbreviation{Bind}{Bind}
\DefineJournalWordException{Bindery}{Bindery}
\DefineJournalAbbreviation{Binghamton}{Binghamt}
\DefineJournalAbbreviation{Binocular}{Binocul}
\DefineJournalPartialAbbreviation{Bioactive}{Bioact}
\DefineJournalPartialAbbreviation{Bioanaly}{Bioanal}
\DefineJournalAbbreviation{Bioavailability}{Bioavailab}
\DefineJournalPartialAbbreviation{Biobehav}{Biobehav}
\DefineJournalPartialAbbreviation{Biocataly}{Biocatal}
\DefineJournalPartialAbbreviation{Biocenolog}{Biocenol}
\DefineJournalPartialAbbreviation{Biocerami}{Bioceram}
\DefineJournalPartialAbbreviation{Biochem}{Biochem}
\DefineJournalPartialAbbreviation{Bioclimatolog}{Bioclimatol}
\DefineJournalPartialAbbreviation{Biocompatibil}{Biocompat}
\DefineJournalPartialAbbreviation{Biocomput}{Biocomput}
\DefineJournalPartialAbbreviation{Bioconcentrat}{Bioconc}
\DefineJournalWordException{Biocrostiches}{Biocrostiches}
\DefineJournalPartialAbbreviation{Biocybernetic}{Biocybern}
\DefineJournalPartialAbbreviation{Biod\'egrad}{Biodegrad}
\DefineJournalPartialAbbreviation{Biodeteriorat}{Biodeterior}
\DefineJournalAbbreviation{Biodiversity}{Biodivers}
\DefineJournalPartialAbbreviation{Biodynamic}{Biodyn}
\DefineJournalAbbreviation{Bioelectricity}{Bioelectr}
\DefineJournalPartialAbbreviation{Bioelectroanaly}{Bioelectroanal}
\DefineJournalPartialAbbreviation{Bioelectromagn}{Bioelectromagn}
\DefineJournalPartialAbbreviation{Bioelectroni}{Bioelectron}
\DefineJournalPartialAbbreviation{Bioengineer}{Bioeng}
\DefineJournalWordException{Bioessay}{Bioessay}
\DefineJournalAbbreviation{Bioethics}{Bioeth}
\DefineJournalWordException{Biofeedback}{Biofeedback}
\DefineJournalAbbreviation{Biofertilizer}{Biofertil}
\DefineJournalPartialAbbreviation{Biogenerat}{Biogener}
\DefineJournalPartialAbbreviation{Biogenet}{Biogenet}
\DefineJournalPartialAbbreviation{Biogeochemi}{Biogeochem}
\DefineJournalPartialAbbreviation{Biohydrometallurg}{Biohydrometall}
\DefineJournalPartialAbbreviation{Bioindustr}{Bioind}
\DefineJournalAbbreviation{Bioinformatics}{Bioinform}
\DefineJournalWordException{Biointerface}{Biointerface}
\DefineJournalPartialAbbreviation{Bioluminescen}{Biolumin}
\DefineJournalPartialAbbreviation{Biomagneti}{Biomagn}
\DefineJournalAbbreviation{Biomarker}{Biomark}
%\DefineJournalPartialWordException{Biomass}{Biomass-}
\DefineJournalPartialAbbreviation{Biomedic}{Biomed}
\DefineJournalPartialAbbreviation{Biomembran}{Biomembr}
\DefineJournalAbbreviation{Biomimetic}{Biomim}
\DefineJournalPartialAbbreviation{Biomolecul}{Biomol}
\DefineJournalPartialAbbreviation{Bionanotechnolog}{Bionanotechnol}
\DefineJournalPartialAbbreviation{Biopatholog}{Biopathol}
\DefineJournalPartialAbbreviation{Biopesticid}{Biopestic}
\DefineJournalPartialAbbreviation{Biopharmaceut}{Biopharm}
\DefineJournalPartialAbbreviation{Bioprepar}{Bioprep}
\DefineJournalWordException{Bioprocess}{Bioprocess}
\DefineJournalAbbreviation{Bioprocessing}{Bioprocess}
\DefineJournalPartialAbbreviation{Bioproduct}{Bioprod}
\DefineJournalWordException{Biopsy}{Biopsy}
\DefineJournalAbbreviation{Biopsychosocial}{Biopsychosoc}
\DefineJournalPartialAbbreviation{Bioreacti}{Bioreact}
\DefineJournalPartialAbbreviation{Bioreactor}{Bioreact}
\DefineJournalAbbreviation{Biorecognition}{Biorecognit}
\DefineJournalPartialAbbreviation{Bioresourc}{Bioresour}
\DefineJournalAbbreviation{Biorganic}{Biorgan}
\DefineJournalPartialAbbreviation{Biorythm}{Biorythm}
\DefineJournalPartialAbbreviation{Biosafety}{Biosaf}
\DefineJournalPartialAbbreviation{Bioscien}{Biosci}
\DefineJournalAbbreviation{Biosensor}{Biosens}
\DefineJournalAbbreviation{Biosensors}{Biosens}
\DefineJournalPartialAbbreviation{Bioseparation}{Biosep}
\DefineJournalAbbreviation{Biosocial}{Biosoc}
\DefineJournalPartialAbbreviation{Biostatist}{Biostat}
\DefineJournalPartialAbbreviation{Biostereometr}{Biostereom}
\DefineJournalAbbreviation{Biosynthesis}{Biosynth}
\DefineJournalPartialAbbreviation{Biosystem}{Biosyst}
\DefineJournalPartialAbbreviation{Biotest}{Biotest}
\DefineJournalAbbreviation{Biotreatment}{Biotreat}
\DefineJournalWordException{Bipolar}{Bipolar}
\DefineJournalAbbreviation{Birding}{Bird}
\DefineJournalAbbreviation{Birdkeeper}{Birdkeep}
\DefineJournalWordException{Birdlife}{Birdlife}
\DefineJournalWordException{Birkbeck}{Birkbeck}
\DefineJournalAbbreviation{Birmingham}{Birm}
\DefineJournalAbbreviation{Birthday}{Birthd}
\DefineJournalWordException{Birthnote}{Birthnote}
\DefineJournalAbbreviation{Birthplace}{Birthpl}
\DefineJournalAbbreviation{Bisannuel}{Bisannu}
\DefineJournalAbbreviation{Bishop}{Bish}
\DefineJournalAbbreviation{Bishops Stortford}{Bish Stortford}
\DefineJournalAbbreviation{Bistability}{Bistab}
\DefineJournalWordException{Bitter}{Bitter}
\DefineJournalWordException{Bitterness}{Bitterness}
\DefineJournalWordException{Bittersweet}{Bittersweet}
\DefineJournalAbbreviation{Bitumen}{Bitum}
\DefineJournalAbbreviation{Bituminous}{Bitum}
\DefineJournalAbbreviation{Biweekly}{Biwkly}
\DefineJournalWordException{Bizaad}{Bizaad}
\DefineJournalWordException{Blabook}{Blabook}
\DefineJournalWordException{Black}{Black}
\DefineJournalWordException{Blackall}{Blackall}
\DefineJournalWordException{Blackboard}{Blackboard}
\DefineJournalWordException{Blackjack}{Blackjack}
\DefineJournalWordException{Blackpool}{Blackpool}
\DefineJournalWordException{Blackrock}{Blackrock}
\DefineJournalAbbreviation{Blacksburg}{Blacksbg}
\DefineJournalAbbreviation{Blacksmith}{Blacksm}
\DefineJournalWordException{Blackwood Hodge}{Blackwood Hodge}
\DefineJournalWordException{Blank}{Blank}
\DefineJournalWordException{Blazed}{Blazed}
\DefineJournalWordException{Blazer}{Blazer}
\DefineJournalPartialAbbreviation{Bleach}{Bleach}
\DefineJournalAbbreviation{Blenheim}{Blenh}
\DefineJournalAbbreviation{Blessing}{Bless}
\DefineJournalWordException{Bleter}{Bleter}
\DefineJournalPartialAbbreviation{Blind}{Blind}
\DefineJournalWordException{Blizzard}{Blizzard}
\DefineJournalWordException{Bloodborne}{Bloodborne}
\DefineJournalWordException{Bloodhorse}{Bloodhorse}
\DefineJournalWordException{Bloodless}{Bloodless}
\DefineJournalPartialAbbreviation{Bloom}{Bloom}
\DefineJournalAbbreviation{Bloomington}{Bloomingt}
\DefineJournalWordException{Bloomsbury}{Bloomsbury}
\DefineJournalPartialAbbreviation{Blossom}{Bloss}
\DefineJournalWordException{Blueberry}{Blueberry}
\DefineJournalAbbreviation{Bluebook}{Blueb}
\DefineJournalWordException{Bluegrass}{Bluegrass}
\DefineJournalWordException{Bluemap}{Bluemap}
\DefineJournalWordException{Bluemoon}{Bluemoon}
\DefineJournalAbbreviation{Blueprint}{Bluepr}
\DefineJournalWordException{Bluewater}{Bluewater}
\DefineJournalWordException{Board}{Board}
\DefineJournalAbbreviation{Boarder}{Board}
\DefineJournalAbbreviation{Boarding}{Board}
\DefineJournalAbbreviation{Boardroom}{Boardr}
\DefineJournalAbbreviation{Boardsailor}{Boardsail}
\DefineJournalWordException{Boardwalk}{Boardwalk}
\DefineJournalPartialAbbreviation{Boatbuild}{Boatbuild}
\DefineJournalAbbreviation{Boating}{Boat}
\DefineJournalWordException{Bobbin}{Bobbin}
\DefineJournalAbbreviation{Bodybuilder}{Bodybuild}
\DefineJournalAbbreviation{Bodybuilding}{Bodybuild}
\DefineJournalWordException{Bodyshop}{Bodyshop}
\DefineJournalAbbreviation{Bodytraining}{Bodytrain}
\DefineJournalAbbreviation{Bodywork}{Bodyw}
\DefineJournalPartialAbbreviation{Boil}{Boil}
\DefineJournalPartialAbbreviation{Boilerhous}{Boilerh}
\DefineJournalWordException{Bolangir}{Bolangir}
\DefineJournalWordException{Bombay}{Bombay}
\DefineJournalWordException{Bomber}{Bomber}
\DefineJournalPartialAbbreviation{Bond}{Bond}
\DefineJournalWordException{Bonsai}{Bonsai}
\DefineJournalWordException{Book}{Book}
\DefineJournalWordException{Bookbank}{Bookbank}
\DefineJournalPartialAbbreviation{Bookbind}{Bookbind}
\DefineJournalAbbreviation{Bookbuyer}{Bookbuy}
\DefineJournalAbbreviation{Bookdealer}{Bookdeal}
\DefineJournalAbbreviation{Bookfund}{Bookf}
\DefineJournalAbbreviation{Booking}{Book}
\DefineJournalPartialAbbreviation{Bookkeep}{Bookkeep}
\DefineJournalAbbreviation{Bookkeeper}{Bookkeep}
\DefineJournalAbbreviation{Booklet}{Bookl}
\DefineJournalWordException{Booklist}{Booklist}
\DefineJournalWordException{Booklore}{Booklore}
\DefineJournalAbbreviation{Bookmaker}{Bookmak}
\DefineJournalAbbreviation{Bookman}{Bookm}
\DefineJournalPartialAbbreviation{Bookmark}{Bookmark}
\DefineJournalAbbreviation{Bookplate}{Bookpl}
\DefineJournalWordException{Bookroom}{Bookroom}
\DefineJournalPartialAbbreviation{Booksell}{Books}
\DefineJournalWordException{Bookshelf}{Bookshelf}
\DefineJournalWordException{Bookshop}{Bookshop}
\DefineJournalWordException{Bookstalls}{Bookstalls}
\DefineJournalAbbreviation{Bookstore}{Bookst}
\DefineJournalAbbreviation{Bookworm}{Bookw}
\DefineJournalWordException{Boomerang}{Boomerang}
\DefineJournalPartialAbbreviation{Boost}{Boost}
\DefineJournalAbbreviation{Border}{Bord}
\DefineJournalPartialAbbreviation{Borderland}{Borderl}
\DefineJournalWordException{Boreal}{Boreal}
\DefineJournalAbbreviation{Borehole}{Boreh}
\DefineJournalWordException{Borno}{Borno}
\DefineJournalWordException{Borough}{Borough}
\DefineJournalAbbreviation{Borrowing}{Borrow}
\DefineJournalAbbreviation{Borstal}{Borst}
\DefineJournalWordException{Boston}{Boston}
\DefineJournalWordException{Bothnian}{Bothnian}
\DefineJournalAbbreviation{Botswana}{Botsw}
\DefineJournalWordException{Bottle}{Bottle}
\DefineJournalWordException{Bottler}{Bottler}
\DefineJournalWordException{Bottom}{Bottom}
\DefineJournalWordException{Bottomline}{Bottomline}
\DefineJournalWordException{Boulder}{Boulder}
\DefineJournalAbbreviation{Boulevard}{Blvd}
\DefineJournalWordException{Boulter}{Boulter}
\DefineJournalWordException{Bound}{Bound}
\DefineJournalAbbreviation{Boundary}{Bound}
\DefineJournalAbbreviation{Boundry}{Bound}
\DefineJournalWordException{Bounty}{Bounty}
\DefineJournalWordException{Bourdages}{Bourdages}
\DefineJournalAbbreviation{Bournemouth}{Bournem}
\DefineJournalWordException{Bowbender}{Bowbender}
\DefineJournalPartialAbbreviation{Bowhunt}{Bowhunt}
\DefineJournalWordException{Bowler}{Bowler}
\DefineJournalAbbreviation{Bowling}{Bowl}
\DefineJournalWordException{Bowmanville}{Bowmanville}
\DefineJournalWordException{Boxboard}{Boxboard}
\DefineJournalAbbreviation{Boxing}{Box}
\DefineJournalPartialAbbreviation{Boycott}{Boycott}
\DefineJournalWordException{Bozeman}{Bozeman}
\DefineJournalWordException{Bracebridge}{Bracebridge}
\DefineJournalWordException{Brachycera}{Brachycera}
\DefineJournalWordException{Brackishwater}{Brackishwater}
\DefineJournalWordException{Bracknell}{Bracknell}
\DefineJournalWordException{Braddon}{Braddon}
\DefineJournalAbbreviation{Bradford}{Bradf}
\DefineJournalAbbreviation{Bradstreet}{Bradstr}
\DefineJournalAbbreviation{Braiding}{Braid}
\DefineJournalWordException{Braille}{Braille}
\DefineJournalWordException{Brakishwater}{Brakishwater}
\DefineJournalWordException{Branch}{Branch}
\DefineJournalAbbreviation{Branching}{Branch}
\DefineJournalAbbreviation{Branchline}{Branchl}
\DefineJournalWordException{Brandon}{Brandon}
\DefineJournalWordException{Brandy}{Brandy}
\DefineJournalWordException{Brantford}{Brantford}
\DefineJournalWordException{Brattleboro}{Brattleboro}
\DefineJournalWordException{Bravery}{Bravery}
\DefineJournalPartialAbbreviation{Brazil}{Braz}
\DefineJournalWordException{Brazing}{Brazing}
\DefineJournalPartialAbbreviation{Break}{Break}
\DefineJournalWordException{Breakdown}{Breakdown}
\DefineJournalAbbreviation{Breakfast}{Breakf}
\DefineJournalAbbreviation{Breakthrough}{Breakthr}
\DefineJournalWordException{Breaktime}{Breaktime}
\DefineJournalWordException{Breast}{Breast}
\DefineJournalAbbreviation{Breastfeeding}{Breastfeed}
\DefineJournalAbbreviation{Breathing}{Breath}
\DefineJournalAbbreviation{Breechloading}{Breechload}
\DefineJournalAbbreviation{Breeder}{Breed}
\DefineJournalAbbreviation{Breeding}{Breed}
\DefineJournalWordException{Breedplan}{Breedplan}
\DefineJournalWordException{Brentwood}{Brentwood}
\DefineJournalAbbreviation{Brethren}{Brethr}
\DefineJournalWordException{Bretton-Woods}{Bretton-Woods}
\DefineJournalPartialAbbreviation{Brewer}{Brew}
\DefineJournalAbbreviation{Brewing}{Brew}
\DefineJournalWordException{Brickendon}{Brickendon}
\DefineJournalPartialAbbreviation{Bricklay}{Bricklay}
\DefineJournalWordException{Brickwork}{Brickwork}
\DefineJournalWordException{Bridal}{Bridal}
\DefineJournalWordException{Briddle}{Briddle}
\DefineJournalWordException{Bridelways}{Bridelways}
\DefineJournalPartialAbbreviation{Bridg}{Bridg}
\DefineJournalWordException{Bridge}{Bridge}
\DefineJournalAbbreviation{Bridgetown}{Bridget}
\DefineJournalAbbreviation{Bridgewater}{Bridgew}
\DefineJournalAbbreviation{Briefcase}{Briefc}
\DefineJournalAbbreviation{Briefing}{Brief}
\DefineJournalWordException{Briefly}{Briefly}
\DefineJournalWordException{Briercrest}{Briercrest}
\DefineJournalAbbreviation{Brigham}{Brigh}
\DefineJournalPartialAbbreviation{Bright}{Bright}
\DefineJournalWordException{Brighton}{Brighton}
\DefineJournalAbbreviation{Brillant}{Brill}
\DefineJournalPartialAbbreviation{Brillian}{Brill}
\DefineJournalAbbreviation{Briquetting}{Briquet}
\DefineJournalAbbreviation{Brisbane}{Brisb}
\DefineJournalWordException{Bristol}{Bristol}
\DefineJournalAbbreviation{Britain}{Br}
\DefineJournalAbbreviation{British}{Br}
\DefineJournalAbbreviation{British Columbia}{B C}
\DefineJournalWordException{Briton}{Briton}
\DefineJournalWordException{Broadband}{Broadband}
\DefineJournalWordException{Broadcast}{Broadcast}
\DefineJournalPartialAbbreviation{Broadcast}{Broadcast}
\DefineJournalWordException{Broadlands}{Broadlands}
\DefineJournalAbbreviation{Broadsheet}{Broadsh}
\DefineJournalAbbreviation{Broadside}{Broads}
\DefineJournalWordException{Broadway}{Broadway}
\DefineJournalAbbreviation{Brockport}{Brockp}
\DefineJournalAbbreviation{Brockville}{Brockv}
\DefineJournalWordException{Broiler}{Broiler}
\DefineJournalWordException{Broken}{Broken}
\DefineJournalAbbreviation{Broker}{Brok}
\DefineJournalAbbreviation{Brokerage}{Brok}
\DefineJournalAbbreviation{Broking}{Brok}
\DefineJournalPartialAbbreviation{Bromeli}{Bromel}
\DefineJournalWordException{Bromley}{Bromley}
\DefineJournalWordException{Bronchitis}{Bronchitis}
\DefineJournalAbbreviation{Bronchology}{Bronchol}
\DefineJournalAbbreviation{Bronxville}{Bronxv}
\DefineJournalAbbreviation{Brooking}{Brook}
\DefineJournalWordException{Brookline}{Brookline}
\DefineJournalWordException{Brooklyn}{Brooklyn}
\DefineJournalPartialAbbreviation{Brother}{Brother}
\DefineJournalPartialAbbreviation{Brows}{Brows}
\DefineJournalWordException{Brunei}{Brunei}
\DefineJournalWordException{Brunel}{Brunel}
\DefineJournalWordException{Brunette}{Brunette}
\DefineJournalAbbreviation{Brunswick}{Brunsw}
\DefineJournalPartialAbbreviation{Brushmak}{Brushmak}
\DefineJournalAbbreviation{Brussels}{Bruss}
\DefineJournalPartialAbbreviation{Bryoecolog}{Bryoecol}
\DefineJournalPartialAbbreviation{Bryozoolog}{Bryozool}
\DefineJournalAbbreviation{Buccaner}{Buccan}
\DefineJournalAbbreviation{Bucharest}{Buchar}
\DefineJournalWordException{Buckeye}{Buckeye}
\DefineJournalAbbreviation{Buckingham}{Buck}
\DefineJournalAbbreviation{Buckinghamshire}{Bucks}
\DefineJournalWordException{Buckle}{Buckle}
\DefineJournalWordException{Buckley}{Buckley}
\DefineJournalAbbreviation{Buckmaster}{Buckmast}
\DefineJournalWordException{Bucksin}{Bucksin}
\DefineJournalAbbreviation{Buddhist}{Buddh}
\DefineJournalAbbreviation{Budgerigar}{Budger}
\DefineJournalAbbreviation{Budget}{Budg}
\DefineJournalAbbreviation{Budgetary}{Budg}
\DefineJournalAbbreviation{Budgeting}{Budg}
\DefineJournalWordException{Budworm}{Budworm}
\DefineJournalWordException{Buffalo}{Buffalo}
\DefineJournalAbbreviation{Buggy}{Bug}
\DefineJournalPartialAbbreviation{Builder}{Build}
\DefineJournalPartialAbbreviation{Building}{Build}
\DefineJournalPartialAbbreviation{Bulgar}{Bulg}
\DefineJournalWordException{Bulker}{Bulker}
\DefineJournalAbbreviation{Bulking}{Bulk}
\DefineJournalWordException{Bullion}{Bullion}
\DefineJournalPartialAbbreviation{Bump}{Bump}
\DefineJournalWordException{Bunburg}{Bunburg}
\DefineJournalWordException{Bungalow}{Bungalow}
\DefineJournalWordException{Burbage}{Burbage}
\DefineJournalAbbreviation{Burden}{Burd}
\DefineJournalWordException{Burgerland}{Burgerland}
\DefineJournalWordException{Burial}{Burial}
\DefineJournalWordException{Burkina}{Burkina}
\DefineJournalWordException{Burley}{Burley}
\DefineJournalWordException{Burlingame}{Burlingame}
\DefineJournalAbbreviation{Burlington}{Burlingt}
\DefineJournalWordException{Burma}{Burma}
\DefineJournalPartialAbbreviation{Burn}{Burn}
\DefineJournalWordException{Burnaby}{Burnaby}
\DefineJournalWordException{Burnett}{Burnett}
\DefineJournalWordException{Burnside}{Burnside}
\DefineJournalWordException{Burroughs}{Burroughs}
\DefineJournalAbbreviation{Bursary}{Burs}
\DefineJournalWordException{Burwood}{Burwood}
\DefineJournalPartialAbbreviation{Bushwalk}{Bushwalk}
\DefineJournalPartialAbbreviation{Bushwhack}{Bushwhack}
\DefineJournalAbbreviation{Business}{Bus}
\DefineJournalWordException{Businessgram}{Businessgram}
\DefineJournalAbbreviation{Businessman}{Businessm}
\DefineJournalWordException{Bustard}{Bustard}
\DefineJournalWordException{Butadiene}{Butadiene}
\DefineJournalAbbreviation{Butcher}{Butch}
\DefineJournalAbbreviation{Butler}{Butl}
\DefineJournalWordException{Butter}{Butter}
\DefineJournalWordException{Butterfly}{Butterfly}
\DefineJournalWordException{Butterworths}{Butterworths}
\DefineJournalWordException{Button}{Button}
\DefineJournalAbbreviation{Buttoneer}{Button}
\DefineJournalWordException{Butyleness}{Butyleness}
\DefineJournalAbbreviation{Buyable}{Buy}
\DefineJournalAbbreviation{Buyer}{Buy}
\DefineJournalAbbreviation{Buying}{Buy}
\DefineJournalWordException{Buyline}{Buyline}
\DefineJournalWordException{Buyout}{Buyout}
\DefineJournalWordException{Buzzer}{Buzzer}
\DefineJournalWordException{Byelaw}{Byelaw}
\DefineJournalAbbreviation{Byelorussian}{Byeloruss}
\DefineJournalWordException{Bygone}{Bygone}
\DefineJournalPartialAbbreviation{Byproduct}{Byprod}
\DefineJournalWordException{Bystander}{Bystander}
\DefineJournalWordException{Bytown}{Bytown}
\DefineJournalWordException{Byways}{Byways}
\DefineJournalWordException{Cabal}{Cabal}
\DefineJournalWordException{Cabbage}{Cabbage}
\DefineJournalAbbreviation{Cabinetmaking}{Cabinetmak}
%\DefineJournalPartialWordException{Cachex}{Cachex-}
\DefineJournalWordException{Cadmium}{Cadmium}
\DefineJournalWordException{Cairn}{Cairn}
\DefineJournalWordException{Calabar}{Calabar}
\DefineJournalPartialAbbreviation{Calamit}{Calam}
\DefineJournalWordException{Calapooya}{Calapooya}
\DefineJournalPartialAbbreviation{Calcifi}{Calcif}
%\DefineJournalPartialWordException{Calcitonin}{Calcitonin-}
\DefineJournalPartialAbbreviation{Calcul}{Calc}
\DefineJournalWordException{Calcutta}{Calcutta}
\DefineJournalWordException{Calderdale}{Calderdale}
\DefineJournalWordException{Caledon}{Caledon}
\DefineJournalAbbreviation{Caledonian}{Caled}
\DefineJournalPartialAbbreviation{Calendar}{Cal}
\DefineJournalAbbreviation{Calgary}{Calg}
\DefineJournalWordException{Calicut}{Calicut}
\DefineJournalAbbreviation{California}{Calif}
\DefineJournalAbbreviation{Caliologist}{Caliol}
\DefineJournalPartialAbbreviation{Calisthen}{Calisthen}
\DefineJournalAbbreviation{Callbook}{Callb}
\DefineJournalAbbreviation{Called}{Call}
\DefineJournalPartialAbbreviation{Calligraph}{Calligr}
\DefineJournalAbbreviation{Calling}{Call}
\DefineJournalWordException{Calliope}{Calliope}
\DefineJournalAbbreviation{Calorimetry}{Calorim}
\DefineJournalWordException{Calvary}{Calvary}
\DefineJournalAbbreviation{Calvinism}{Calvin}
\DefineJournalPartialAbbreviation{Cambodgi}{Cambodg}
\DefineJournalWordException{Cambodia}{Cambodia}
\DefineJournalWordException{Cambodian}{Cambodian}
\DefineJournalAbbreviation{Cambrian}{Cambr}
\DefineJournalAbbreviation{Cambridge}{Camb}
\DefineJournalAbbreviation{Cambridgeshire}{Cambs}
\DefineJournalAbbreviation{Camcorder}{Camcord}
\DefineJournalWordException{Camden}{Camden}
\DefineJournalWordException{Camellia}{Camellia}
\DefineJournalWordException{Camera}{Camera}
\DefineJournalWordException{Cameroon}{Cameroon}
\DefineJournalWordException{Cammeray}{Cammeray}
\DefineJournalAbbreviation{Camouflage}{Camoufl}
\DefineJournalPartialAbbreviation{Campaign}{Campaign}
\DefineJournalWordException{Campbellford}{Campbellford}
\DefineJournalWordException{Campbelltown}{Campbelltown}
\DefineJournalWordException{Camper}{Camper}
\DefineJournalWordException{Campfire}{Campfire}
\DefineJournalWordException{Campground}{Campground}
\DefineJournalWordException{Camping}{Camping}
\DefineJournalWordException{Campus}{Campus}
\DefineJournalAbbreviation{Canada}{Can}
\DefineJournalPartialAbbreviation{Canadi}{Can}
\DefineJournalWordException{Canal}{Canal}
\DefineJournalPartialAbbreviation{Canalization}{Canaliz}
\DefineJournalWordException{Canary}{Canary}
\DefineJournalWordException{Canberra}{Canberra}
\DefineJournalPartialAbbreviation{Cancel}{Cancel}
\DefineJournalWordException{Cancer}{Cancer}
\DefineJournalWordException{Cancergram}{Cancergram}
\DefineJournalPartialAbbreviation{Cancerolog}{Cancerol}
\DefineJournalPartialAbbreviation{Cancrolog}{Cancrol}
\DefineJournalWordException{Cancrum}{Cancrum}
\DefineJournalWordException{Candidate}{Candidate}
\DefineJournalAbbreviation{Canegrower}{Canegrow}
\DefineJournalWordException{Canine}{Canine}
\DefineJournalAbbreviation{Canmaker}{Canmak}
\DefineJournalAbbreviation{Canmaking}{Canmak}
\DefineJournalAbbreviation{Canned}{Cann}
\DefineJournalAbbreviation{Canner}{Cann}
\DefineJournalAbbreviation{Canning}{Cann}
\DefineJournalWordException{Cannon}{Cannon}
\DefineJournalPartialAbbreviation{Canoe}{Canoe}
\DefineJournalAbbreviation{Canoesport}{Canoesp}
\DefineJournalWordException{Canteen}{Canteen}
\DefineJournalAbbreviation{Canterbury}{Canterb}
\DefineJournalWordException{Canvas}{Canvas}
\DefineJournalAbbreviation{Canvey Island}{Canvey Isl}
\DefineJournalWordException{Canyon}{Canyon}
\DefineJournalPartialAbbreviation{Capab}{Capab}
\DefineJournalWordException{Cape-Breton}{Cape-Breton}
\DefineJournalWordException{Cape-Canaveral}{Cape-Canaveral}
\DefineJournalWordException{Cape-Town}{Cape-Town}
\DefineJournalAbbreviation{Capillary}{Capill}
\DefineJournalAbbreviation{Capital}{Cap}
\DefineJournalWordException{Capricorn}{Capricorn}
\DefineJournalWordException{Capricornia}{Capricornia}
\DefineJournalPartialAbbreviation{Capsul}{Capsul}
\DefineJournalAbbreviation{Captain}{Capt}
\DefineJournalPartialAbbreviation{Captiv}{Captiv}
\DefineJournalWordException{Carabiner}{Carabiner}
\DefineJournalWordException{Carbanion}{Carbanion}
\DefineJournalWordException{Carbide}{Carbide}
\DefineJournalAbbreviation{Carbocation}{Carbocat}
\DefineJournalAbbreviation{Carbocyclic}{Carbocycl}
\DefineJournalAbbreviation{Carbohydrate}{Carbohydr}
\DefineJournalWordException{Carbonate}{Carbonate}
\DefineJournalWordException{Carbonear}{Carbonear}
\DefineJournalAbbreviation{Carboniferous}{Carbonif}
\DefineJournalAbbreviation{Carburant}{Carbur}
\DefineJournalPartialAbbreviation{Carcinogen}{Carcinog}
\DefineJournalWordException{Carcinoma}{Carcinoma}
\DefineJournalWordException{Cardiff}{Cardiff}
\DefineJournalPartialAbbreviation{Cardioangiolog}{Cardioangiol}
\DefineJournalAbbreviation{Cardiobiology}{Cardiobiol}
\DefineJournalAbbreviation{Cardiocirculation}{Cardiocirc}
\DefineJournalAbbreviation{Cardiograph}{Cardiogr}
\DefineJournalPartialAbbreviation{Cardiolog}{Cardiol}
\DefineJournalPartialAbbreviation{Cardioprotecti}{Cardioprot}
\DefineJournalAbbreviation{Cardiopulmonary}{Cardiopulm}
\DefineJournalPartialAbbreviation{Cardiorespirat}{Cardiorespir}
\DefineJournalAbbreviation{Cardiothoracic}{Cardiothorac}
\DefineJournalPartialAbbreviation{Cardiovasc}{Cardiovasc}
\DefineJournalWordException{Career}{Career}
\DefineJournalAbbreviation{Caregiver}{Caregiv}
\DefineJournalWordException{Cargo}{Cargo}
\DefineJournalWordException{Cargoworld}{Cargoworld}
\DefineJournalAbbreviation{Caribbean}{Caribb}
\DefineJournalWordException{Cariboo}{Cariboo}
\DefineJournalWordException{Caries}{Caries}
\DefineJournalWordException{Caring}{Caring}
\DefineJournalPartialAbbreviation{Cariolog}{Cariol}
\DefineJournalAbbreviation{Carleton}{Carlet}
\DefineJournalWordException{Carload}{Carload}
\DefineJournalWordException{Carlton South}{Carlton South}
\DefineJournalWordException{Carmarthen}{Carmarthen}
\DefineJournalAbbreviation{Carmarthenshire}{Carmarthens}
\DefineJournalAbbreviation{Carnation}{Carnat}
\DefineJournalPartialAbbreviation{Carnivor}{Carniv}
\DefineJournalAbbreviation{Carnoisseur}{Carnoiss}
\DefineJournalPartialAbbreviation{Carolina}{Carol}
\DefineJournalWordException{Caronport}{Caronport}
\DefineJournalAbbreviation{Carpenter}{Carpent}
\DefineJournalWordException{Carpet}{Carpet}
\DefineJournalAbbreviation{Carpeting}{Carpet}
\DefineJournalPartialAbbreviation{Carpinter}{Carpint}
\DefineJournalWordException{Carpool}{Carpool}
\DefineJournalWordException{Carriage}{Carriage}
\DefineJournalAbbreviation{Carrier}{Carr}
\DefineJournalWordException{Carrion}{Carrion}
\DefineJournalWordException{Carrionflower}{Carrionflower}
\DefineJournalWordException{Carrot}{Carrot}
\DefineJournalAbbreviation{Carrying}{Carr}
\DefineJournalWordException{Carson-City}{Carson-City}
%\DefineJournalPartialWordException{Cartag}{Cartag-}
\DefineJournalWordException{Carter}{Carter}
\DefineJournalWordException{Carterton}{Carterton}
\DefineJournalPartialAbbreviation{Cartesian}{Cartes}
\DefineJournalAbbreviation{Cartilage}{Cartil}
\DefineJournalPartialAbbreviation{Cartograph}{Cartogr}
\DefineJournalPartialAbbreviation{Cartoon}{Cartoon}
\DefineJournalWordException{Cartoonweek}{Cartoonweek}
\DefineJournalWordException{Cartridge}{Cartridge}
\DefineJournalWordException{Casebook}{Casebook}
\DefineJournalWordException{Casework}{Casework}
\DefineJournalAbbreviation{Cashed}{Cash}
\DefineJournalWordException{Cashew}{Cashew}
\DefineJournalWordException{Cashflow}{Cashflow}
\DefineJournalWordException{Cashmere}{Cashmere}
\DefineJournalAbbreviation{Casinghead}{Casingh}
\DefineJournalWordException{Casket}{Casket}
\DefineJournalAbbreviation{Caspian}{Casp}
\DefineJournalAbbreviation{Castellano}{Castell}
\DefineJournalPartialAbbreviation{Casting}{Cast}
\DefineJournalWordException{Castle}{Castle}
\DefineJournalWordException{Castlegar}{Castlegar}
\DefineJournalWordException{Castletownbere}{Castletownbere}
\DefineJournalWordException{Casual}{Casual}
\DefineJournalWordException{Casualty}{Casualty}
\DefineJournalPartialAbbreviation{Catalys}{Catal}
\DefineJournalPartialAbbreviation{Catalyt}{Catal}
\DefineJournalAbbreviation{Catastrophism}{Catastr}
\DefineJournalAbbreviation{Catching}{Catch}
\DefineJournalWordException{Catchment}{Catchment}
\DefineJournalWordException{Catchword}{Catchword}
\DefineJournalAbbreviation{Catechist}{Catech}
\DefineJournalWordException{Catecholamines}{Catecholamines}
\DefineJournalPartialAbbreviation{Cat\'egor}{Categ}
\DefineJournalPartialAbbreviation{Cater}{Cater}
\DefineJournalAbbreviation{Caterpillar}{Caterp}
\DefineJournalPartialAbbreviation{Cathar}{Cathar}
\DefineJournalAbbreviation{Catharine}{Cath}
\DefineJournalAbbreviation{Cathedral}{Cathedr}
\DefineJournalPartialAbbreviation{Catheter}{Catheter}
\DefineJournalWordException{Cathlab}{Cathlab}
\DefineJournalPartialAbbreviation{Catholi}{Cathol}
\DefineJournalAbbreviation{Catonsville}{Catonsv}
\DefineJournalWordException{Cattle}{Cattle}
\DefineJournalAbbreviation{Cattleman}{Cattlem}
\DefineJournalAbbreviation{Cattlewoman}{Cattlew}
\DefineJournalWordException{Catwalk}{Catwalk}
\DefineJournalAbbreviation{Caucasian}{Cauc}
\DefineJournalAbbreviation{Caucasus}{Cauc}
\DefineJournalAbbreviation{Caufield}{Caufld}
\DefineJournalWordException{Caughnawaga}{Caughnawaga}
\DefineJournalAbbreviation{Cauliflower}{Caulifl}
\DefineJournalWordException{Causapscal}{Causapscal}
\DefineJournalAbbreviation{Causeway}{Causew}
\DefineJournalWordException{Cavalry}{Cavalry}
\DefineJournalWordException{Caveat}{Caveat}
\DefineJournalWordException{Caver}{Caver}
\DefineJournalWordException{Cavern}{Cavern}
\DefineJournalWordException{Caving}{Caving}
\DefineJournalWordException{Cayman}{Cayman}
\DefineJournalWordException{Cayuse}{Cayuse}
\DefineJournalPartialAbbreviation{Cechoslov}{Cechoslov}
\DefineJournalPartialAbbreviation{Cecidiolog}{Cecidiol}
\DefineJournalAbbreviation{Cedarville}{Cedarv}
\DefineJournalAbbreviation{Ceiling}{Ceil}
\DefineJournalWordException{Celanese}{Celanese}
\DefineJournalAbbreviation{Celestial}{Celest}
\DefineJournalWordException{Cellar}{Cellar}
\DefineJournalPartialAbbreviation{Cellula}{Cell}
\DefineJournalAbbreviation{Cellule}{Cell}
\DefineJournalWordException{Celluloid}{Celluloid}
\DefineJournalPartialAbbreviation{Cellulos}{Cellul}
\DefineJournalPartialAbbreviation{Cement}{Cem}
\DefineJournalAbbreviation{Cemetery}{Cemet}
\DefineJournalWordException{Censor}{Censor}
\DefineJournalAbbreviation{Censorship}{Censorsh}
\DefineJournalPartialAbbreviation{Centen}{Centen}
\DefineJournalAbbreviation{Center}{Cent}
\DefineJournalPartialAbbreviation{Centrafric}{Centrafr}
\DefineJournalWordException{Centrepoint}{Centrepoint}
\DefineJournalWordException{Centrestage}{Centrestage}
\DefineJournalAbbreviation{Centrifugal}{Centrif}
\DefineJournalWordException{Century}{Century}
\DefineJournalAbbreviation{Cephalopod}{Cephalop}
\DefineJournalPartialAbbreviation{Cerami}{Ceram}
\DefineJournalAbbreviation{Cerebral}{Cereb}
\DefineJournalPartialAbbreviation{Cerebrovascular}{Cerebrovasc}
\DefineJournalPartialAbbreviation{Ceremon}{Cerem}
\DefineJournalWordException{Cerium}{Cerium}
\DefineJournalPartialAbbreviation{Certain}{Certain}
\DefineJournalPartialAbbreviation{Certificat}{Certif}
\DefineJournalAbbreviation{Certified}{Certif}
\DefineJournalAbbreviation{Cervical}{Cerv}
\DefineJournalPartialAbbreviation{Cervicofacial}{Cervicofac}
\DefineJournalWordException{Cervix}{Cervix}
\DefineJournalAbbreviation{Cessation}{Cessat}
\DefineJournalWordException{Cetacea}{Cetacea}
\DefineJournalAbbreviation{Chairman}{Chairm}
\DefineJournalWordException{Chairside}{Chairside}
\DefineJournalWordException{Chairwoman}{Chairwoman}
\DefineJournalAbbreviation{Challenge}{Chall}
\DefineJournalAbbreviation{Challenger}{Chall}
\DefineJournalAbbreviation{Chamber}{Chamb}
\DefineJournalAbbreviation{Chambersburg}{Chambersbg}
\DefineJournalWordException{Chambly}{Chambly}
\DefineJournalWordException{Chaminage}{Chaminage}
\DefineJournalWordException{Champaign}{Champaign}
\DefineJournalWordException{Championship}{Championship}
\DefineJournalWordException{Champlain}{Champlain}
\DefineJournalAbbreviation{Chanceller}{Chancell}
\DefineJournalAbbreviation{Chancellor}{Chancell}
\DefineJournalWordException{Chancery}{Chancery}
\DefineJournalWordException{Chandigarh}{Chandigarh}
\DefineJournalAbbreviation{Chandler}{Chandl}
\DefineJournalWordException{Channel}{Channel}
\DefineJournalPartialAbbreviation{Chapbook}{Chapb}
\DefineJournalAbbreviation{Chapel Hill}{Chap Hill}
\DefineJournalAbbreviation{Chapeltown}{Chapelt}
\DefineJournalPartialAbbreviation{Chaplain}{Chaplain}
\DefineJournalWordException{Chappaqua}{Chappaqua}
\DefineJournalWordException{Chapter}{Chapter}
\DefineJournalWordException{Character}{Character}
\DefineJournalPartialAbbreviation{Characteristic}{Charact}
\DefineJournalPartialAbbreviation{Characteriz}{Charact}
\DefineJournalWordException{Chariton}{Chariton}
\DefineJournalWordException{Charity}{Charity}
\DefineJournalAbbreviation{Charleston}{Charlest}
\DefineJournalAbbreviation{Charlottesville}{Charlottesv}
\DefineJournalAbbreviation{Charlottetown}{Charlottet}
\DefineJournalWordException{Charlton}{Charlton}
\DefineJournalWordException{Chartac}{Chartac}
\DefineJournalWordException{Charte}{Charte}
\DefineJournalAbbreviation{Charter}{Chart}
\DefineJournalAbbreviation{Chartered}{Chart}
\DefineJournalWordException{Charting}{Charting}
\DefineJournalWordException{Chartist}{Chartist}
\DefineJournalAbbreviation{Chasing}{Chas}
\DefineJournalAbbreviation{Chastity}{Chast}
\DefineJournalAbbreviation{Chattanooga}{Chatt}
\DefineJournalWordException{Chattel}{Chattel}
\DefineJournalWordException{Chatter}{Chatter}
\DefineJournalAbbreviation{Chauncey}{Chaunc}
\DefineJournalAbbreviation{Checklist}{Checkl}
\DefineJournalWordException{Checkout}{Checkout}
\DefineJournalAbbreviation{Checkpoint}{Checkp}
\DefineJournalWordException{Cheese}{Cheese}
\DefineJournalWordException{Chelates}{Chelates}
\DefineJournalAbbreviation{Chelmsford}{Chelmsf}
\DefineJournalWordException{Chelonia}{Chelonia}
\DefineJournalWordException{Chelonian}{Chelonian}
\DefineJournalAbbreviation{Cheltenham}{Chelten}
\DefineJournalPartialAbbreviation{Chemic}{Chem}
\DefineJournalPartialAbbreviation{Chemigraph}{Chemigr}
\DefineJournalPartialAbbreviation{Chemiluminescen}{Chemilumin}
\DefineJournalAbbreviation{Chemisorption}{Chemisorpt}
\DefineJournalPartialAbbreviation{Chemist}{Chem}
\DefineJournalPartialAbbreviation{Chemiz}{Chem}
\DefineJournalPartialAbbreviation{Chemometr}{Chemom}
\DefineJournalAbbreviation{Chemonomic}{Chemon}
\DefineJournalPartialAbbreviation{Chemorecept}{Chemorecept}
\DefineJournalPartialAbbreviation{Chemorheolog}{Chemorheol}
\DefineJournalPartialAbbreviation{Chemosensor}{Chemosens}
\DefineJournalPartialAbbreviation{Chemosystem}{Chemosyst}
\DefineJournalPartialAbbreviation{Chemotaxonom}{Chemotaxon}
\DefineJournalPartialAbbreviation{Chemotherap}{Chemother}
\DefineJournalPartialAbbreviation{Chemurg}{Chemurg}
\DefineJournalWordException{Chequered}{Chequered}
\DefineJournalWordException{Chernobyl}{Chernobyl}
\DefineJournalAbbreviation{Cherokee}{Cherok}
\DefineJournalWordException{Cherryburn}{Cherryburn}
\DefineJournalWordException{Chertsey}{Chertsey}
\DefineJournalWordException{Cherub}{Cherub}
\DefineJournalPartialAbbreviation{Cherubi}{Cherub}
\DefineJournalPartialAbbreviation{Chesapeake}{Chesap}
\DefineJournalAbbreviation{Cheshire}{Ches}
\DefineJournalWordException{Chesley}{Chesley}
\DefineJournalWordException{Chessbase}{Chessbase}
\DefineJournalPartialAbbreviation{Chessplay}{Chessplay}
\DefineJournalAbbreviation{Chesterville}{Chesterv}
\DefineJournalWordException{Chestnut}{Chestnut}
\DefineJournalWordException{Chevrolet}{Chevrolet}
\DefineJournalWordException{Cheyenne}{Cheyenne}
\DefineJournalWordException{Chianina}{Chianina}
\DefineJournalWordException{Chibret}{Chibret}
\DefineJournalAbbreviation{Chicago}{Chic}
\DefineJournalWordException{Chicano}{Chicano}
\DefineJournalWordException{Chichester}{Chichester}
\DefineJournalAbbreviation{Chicken}{Chick}
\DefineJournalWordException{Chickpea}{Chickpea}
\DefineJournalWordException{Chicoutimi}{Chicoutimi}
\DefineJournalWordException{Chieftaincy}{Chieftaincy}
\DefineJournalWordException{Chigwell}{Chigwell}
\DefineJournalWordException{Chilcotin}{Chilcotin}
\DefineJournalPartialAbbreviation{Childbear}{Childbear}
\DefineJournalWordException{Childbirth}{Childbirth}
\DefineJournalWordException{Childcare}{Childcare}
\DefineJournalAbbreviation{Childhood}{Child}
\DefineJournalWordException{Childminding}{Childminding}
\DefineJournalPartialAbbreviation{Childrear}{Childrear}
\DefineJournalPartialAbbreviation{Children}{Child}
\DefineJournalAbbreviation{Chilean}{Chil}
\DefineJournalPartialAbbreviation{Chill}{Chill}
\DefineJournalWordException{Chilton}{Chilton}
\DefineJournalWordException{Chinaweek}{Chinaweek}
\DefineJournalAbbreviation{Chinese}{Chin}
\DefineJournalWordException{Chinook}{Chinook}
\DefineJournalWordException{Chippendale}{Chippendale}
\DefineJournalPartialAbbreviation{Chiropod}{Chirop}
\DefineJournalAbbreviation{Chiropractic}{Chiropr}
\DefineJournalAbbreviation{Chiropractor}{Chiropr}
\DefineJournalAbbreviation{Chiroptera}{Chiropt}
\DefineJournalPartialAbbreviation{Chirurg}{Chir}
\DefineJournalWordException{Chislehurst}{Chislehurst}
\DefineJournalWordException{Chlamydial}{Chlamydial}
\DefineJournalWordException{Chlorophyll}{Chlorophyll}
\DefineJournalPartialAbbreviation{Chocolat}{Choc}
\DefineJournalWordException{Choice}{Choice}
\DefineJournalAbbreviation{Choiceland}{Choicel}
\DefineJournalWordException{Choirmaster}{Choirmaster}
\DefineJournalWordException{Cholinergic}{Cholinergic}
\DefineJournalAbbreviation{Choosing}{Choos}
\DefineJournalPartialAbbreviation{Chopper}{Chop}
\DefineJournalAbbreviation{Chorister}{Chorist}
\DefineJournalWordException{Chorleywood}{Chorleywood}
\DefineJournalWordException{Chorus}{Chorus}
\DefineJournalAbbreviation{Chowder}{Chowd}
\DefineJournalAbbreviation{Christadelphian}{Christadelph}
\DefineJournalAbbreviation{Christchurch}{Christch}
\DefineJournalWordException{Christmas}{Christmas}
\DefineJournalPartialAbbreviation{Christolog}{Christol}
\DefineJournalAbbreviation{Christorium}{Christ}
\DefineJournalPartialAbbreviation{Chromatograph}{Chromatogr}
\DefineJournalWordException{Chromium}{Chromium}
\DefineJournalAbbreviation{Chromosphere}{Chromosph}
\DefineJournalWordException{Chronic}{Chronic}
\DefineJournalAbbreviation{Chronicle}{Chron}
\DefineJournalPartialAbbreviation{Chronobiotechnolog}{Chronobiotechnol}
\DefineJournalPartialAbbreviation{Chronometr}{Chronom}
\DefineJournalPartialAbbreviation{Chronopharmacolog}{Chronopharmacol}
\DefineJournalAbbreviation{Chronostratigraphic}{Chronostratigr}
\DefineJournalPartialAbbreviation{Chronotherap}{Chronother}
\DefineJournalAbbreviation{Chrysalis}{Chrysal}
\DefineJournalPartialAbbreviation{Chrysanth}{Chrysanth}
\DefineJournalWordException{Chunky}{Chunky}
\DefineJournalWordException{Church}{Church}
\DefineJournalAbbreviation{Churchman}{Churchm}
\DefineJournalPartialAbbreviation{Cibernetic}{Cibern}
\DefineJournalWordException{Cinchona}{Cinchona}
\DefineJournalWordException{Cincinnati}{Cincinnati}
\DefineJournalWordException{Cinekid}{Cinekid}
\DefineJournalAbbreviation{Cinema}{Cin\'e}
\DefineJournalPartialAbbreviation{Cinematograph}{Cinematogr}
\DefineJournalPartialAbbreviation{Cineradiograph}{Cineradiogr}
\DefineJournalAbbreviation{Circle}{Circ}
\DefineJournalWordException{Circumpolar}{Circumpolar}
\DefineJournalAbbreviation{Circumstance}{Circumst}
\DefineJournalWordException{Cistercian}{Cistercian}
\DefineJournalWordException{Citadel}{Citadel}
\DefineJournalAbbreviation{Citation}{Cit}
\DefineJournalAbbreviation{Citizen}{Citiz}
\DefineJournalAbbreviation{Citizenship}{Citizsh}
\DefineJournalPartialAbbreviation{Citograph}{Citogr}
\DefineJournalPartialAbbreviation{Citolog}{Citol}
\DefineJournalPartialAbbreviation{Citricult}{Citric}
\DefineJournalPartialAbbreviation{Citrograph}{Citrogr}
\DefineJournalPartialAbbreviation{Citrolog}{Citrol}
\DefineJournalWordException{Citrus}{Citrus}
\DefineJournalWordException{Citus}{Citus}
\DefineJournalWordException{City}{City}
\DefineJournalWordException{Citylife}{Citylife}
\DefineJournalWordException{Cityscope}{Cityscope}
\DefineJournalWordException{Citytalk}{Citytalk}
\DefineJournalPartialAbbreviation{Civic}{Civ}
\DefineJournalAbbreviation{Civil}{Civ}
\DefineJournalAbbreviation{Civilian}{Civ}
\DefineJournalAbbreviation{Civilised}{Civilis}
\DefineJournalAbbreviation{Civilising}{Civilis}
\DefineJournalAbbreviation{Civilization}{Civiliz}
\DefineJournalAbbreviation{Civils}{Civ}
\DefineJournalAbbreviation{Clackmannanshire}{Clackmannans}
\DefineJournalWordException{Claimant}{Claimant}
\DefineJournalWordException{Clandeboye}{Clandeboye}
\DefineJournalWordException{Clareman}{Clareman}
\DefineJournalWordException{Claremont}{Claremont}
\DefineJournalAbbreviation{Clarion}{Clar}
\DefineJournalWordException{Clarkson}{Clarkson}
\DefineJournalAbbreviation{Class}{Cl}
\DefineJournalAbbreviation{Classe}{Cl}
\DefineJournalPartialAbbreviation{Classic}{Class}
\DefineJournalPartialAbbreviation{Classifi}{Classif}
\DefineJournalAbbreviation{Classroom}{Classr}
\DefineJournalWordException{Claycraft}{Claycraft}
\DefineJournalWordException{Clayton}{Clayton}
\DefineJournalAbbreviation{Clayworker}{Claywork}
\DefineJournalAbbreviation{Cleaner}{Clean}
\DefineJournalAbbreviation{Cleaning}{Clean}
\DefineJournalAbbreviation{Cleansing}{Clean}
\DefineJournalWordException{Cleanup}{Cleanup}
\DefineJournalPartialAbbreviation{Clear}{Clear}
\DefineJournalAbbreviation{Clearance}{Clear}
\DefineJournalAbbreviation{Clearinghouse}{Clgh}
\DefineJournalAbbreviation{Cleethorpes}{Cleeth}
\DefineJournalWordException{Clergy}{Clergy}
\DefineJournalAbbreviation{Clerical}{Cleric}
\DefineJournalAbbreviation{Cleveland}{Clevel}
\DefineJournalWordException{Clever}{Clever}
\DefineJournalWordException{Client}{Client}
\DefineJournalWordException{Clifton}{Clifton}
\DefineJournalPartialAbbreviation{Climat}{Clim}
\DefineJournalPartialAbbreviation{Climatolog}{Climatol}
\DefineJournalWordException{Climax}{Climax}
\DefineJournalAbbreviation{Climber}{Climb}
\DefineJournalPartialAbbreviation{Clinic}{Clin}
\DefineJournalAbbreviation{Clinton}{Clint}
\DefineJournalWordException{Clipboard}{Clipboard}
\DefineJournalAbbreviation{Clipper}{Clipp}
\DefineJournalAbbreviation{Clipping}{Clipp}
\DefineJournalPartialAbbreviation{Clockmak}{Clockmak}
\DefineJournalAbbreviation{Clockwise}{Clockw}
\DefineJournalWordException{Clogher}{Clogher}
\DefineJournalWordException{Clonfert}{Clonfert}
\DefineJournalWordException{Cloning}{Cloning}
\DefineJournalWordException{Closehout}{Closehout}
\DefineJournalWordException{Closely}{Closely}
\DefineJournalWordException{Closeout}{Closeout}
\DefineJournalWordException{Closer}{Closer}
\DefineJournalWordException{Closing}{Closing}
\DefineJournalAbbreviation{Closure}{Clos}
\DefineJournalAbbreviation{Clothier}{Cloth}
\DefineJournalAbbreviation{Clothing}{Cloth}
\DefineJournalAbbreviation{Clothworker}{Clothwork}
\DefineJournalAbbreviation{Clotting}{Clott}
\DefineJournalWordException{Clover}{Clover}
\DefineJournalWordException{Cloverdale}{Cloverdale}
\DefineJournalAbbreviation{Clubhouse}{Clubh}
\DefineJournalAbbreviation{Clubland}{Clubl}
\DefineJournalPartialAbbreviation{Cluster}{Clust}
\DefineJournalWordException{Clydesdale}{Clydesdale}
\DefineJournalAbbreviation{Co-operative}{Co-op}
\DefineJournalPartialAbbreviation{Co-ordinat}{Co-ord}
\DefineJournalPartialAbbreviation{Coach}{Coach}
\DefineJournalAbbreviation{Coalfield}{Coalf}
\DefineJournalWordException{Coalhurst}{Coalhurst}
\DefineJournalWordException{Coarge}{Coarge}
\DefineJournalWordException{Coarse}{Coarse}
\DefineJournalWordException{Coast}{Coast}
\DefineJournalAbbreviation{Coastal}{Coast}
\DefineJournalWordException{Coastguard}{Coastguard}
\DefineJournalWordException{Coastwatch}{Coastwatch}
\DefineJournalWordException{Coastwise}{Coastwise}
\DefineJournalAbbreviation{Coated}{Coat}
\DefineJournalAbbreviation{Coating}{Coat}
\DefineJournalWordException{Cobalt}{Cobalt}
\DefineJournalWordException{Cobham}{Cobham}
\DefineJournalPartialAbbreviation{Cocarcinogen}{Cocarcinog}
%\DefineJournalPartialWordException{Cochlea}{Cochlea-}
\DefineJournalWordException{Cochrane}{Cochrane}
\DefineJournalWordException{Cockpit}{Cockpit}
\DefineJournalWordException{Coconut}{Coconut}
\DefineJournalWordException{Coeliac}{Coeliac}
\DefineJournalPartialAbbreviation{Coerc}{Coerc}
\DefineJournalAbbreviation{Coevolution}{Coevol}
\DefineJournalWordException{Coffee}{Coffee}
\DefineJournalWordException{Coffin}{Coffin}
\DefineJournalPartialAbbreviation{Cogenerat}{Cogener}
\DefineJournalAbbreviation{Cognate}{Cogn}
\DefineJournalPartialAbbreviation{Cogniz}{Cogniz}
\DefineJournalWordException{Coherence}{Coherence}
\DefineJournalAbbreviation{Cohesion}{Cohes}
\DefineJournalAbbreviation{Coinage}{Coin}
\DefineJournalAbbreviation{Coinhunter}{Coinhunt}
\DefineJournalAbbreviation{Cokemaking}{Cokemak}
\DefineJournalAbbreviation{Colchester}{Colch}
\DefineJournalPartialAbbreviation{Colect}{Colect}
\DefineJournalPartialAbbreviation{Coleopter}{Coleopt}
\DefineJournalPartialAbbreviation{Coleopterolog}{Coleopterol}
\DefineJournalWordException{Colitis}{Colitis}
\DefineJournalPartialAbbreviation{Collaborat}{Collab}
\DefineJournalWordException{Collagen}{Collagen}
\DefineJournalWordException{Collar}{Collar}
\DefineJournalWordException{Colleague}{Colleague}
\DefineJournalPartialAbbreviation{Collect}{Collect}
\DefineJournalPartialAbbreviation{College}{Coll}
\DefineJournalPartialAbbreviation{Collegi}{Coll}
\DefineJournalAbbreviation{Collider}{Collid}
\DefineJournalWordException{Collie}{Collie}
\DefineJournalWordException{Collingwood}{Collingwood}
\DefineJournalAbbreviation{Collision}{Collis}
\DefineJournalWordException{Colloid}{Colloid}
\DefineJournalWordException{Colombo}{Colombo}
\DefineJournalWordException{Colon}{Colon}
\DefineJournalWordException{Colonel}{Colonel}
\DefineJournalPartialAbbreviation{Coloni}{Colon}
\DefineJournalWordException{Colony}{Colony}
\DefineJournalAbbreviation{Colorado}{Colo}
\DefineJournalAbbreviation{Colorado Springs}{Colo Springs}
\DefineJournalWordException{Colorectal}{Colorectal}
\DefineJournalWordException{Colossus}{Colossus}
\DefineJournalAbbreviation{Colotomy}{Colotm}
\DefineJournalAbbreviation{Colourage}{Colour}
\DefineJournalAbbreviation{Colouring}{Colour}
\DefineJournalPartialAbbreviation{Colourist}{Colour}
\DefineJournalWordException{Colourmaster}{Colourmaster}
\DefineJournalPartialAbbreviation{Colposcop}{Colposc}
\DefineJournalWordException{Columbia}{Columbia}
\DefineJournalAbbreviation{Columbus}{Columb}
\DefineJournalWordException{Column}{Column}
\DefineJournalWordException{Comanche}{Comanche}
\DefineJournalWordException{Combermere}{Combermere}
\DefineJournalPartialAbbreviation{Combin}{Comb}
\DefineJournalPartialAbbreviation{Combusti}{Combust}
\DefineJournalPartialAbbreviation{Comerci}{Comer}
\DefineJournalWordException{Comet}{Comet}
\DefineJournalPartialAbbreviation{Comfort}{Comf}
\DefineJournalWordException{Comics}{Comics}
\DefineJournalWordException{Coming}{Coming}
\DefineJournalPartialAbbreviation{Commemorant}{Commem}
\DefineJournalPartialAbbreviation{Commemorat}{Commem}
\DefineJournalPartialAbbreviation{Commenc}{Commenc}
\DefineJournalWordException{Comment}{Comment}
\DefineJournalPartialAbbreviation{Commentar}{Comment}
\DefineJournalPartialAbbreviation{Commerc}{Commer}
\DefineJournalPartialAbbreviation{Commissar}{Commis}
\DefineJournalPartialAbbreviation{Commission}{Comm}
\DefineJournalAbbreviation{Commitment}{Commit}
\DefineJournalAbbreviation{Committee}{Comm}
\DefineJournalPartialAbbreviation{Commodit}{Commod}
\DefineJournalWordException{Common}{Common}
\DefineJournalAbbreviation{Commoner}{Common}
\DefineJournalWordException{Commonweal}{Commonweal}
\DefineJournalAbbreviation{Commonwealth}{Commonw}
\DefineJournalPartialAbbreviation{Communica}{Commun}
\DefineJournalWordException{Community}{Community}
\DefineJournalPartialAbbreviation{Commut}{Commut}
\DefineJournalWordException{Comoros}{Comoros}
\DefineJournalPartialAbbreviation{Compact}{Compact}
\DefineJournalAbbreviation{Companies}{Co}
\DefineJournalWordException{Companion}{Companion}
\DefineJournalAbbreviation{Company}{Co}
\DefineJournalPartialAbbreviation{Compara}{Comp}
\DefineJournalPartialAbbreviation{Compare}{Comp}
\DefineJournalPartialAbbreviation{Compari}{Comp}
\DefineJournalWordException{Compass}{Compass}
\DefineJournalPartialAbbreviation{Compatibil}{Compat}
\DefineJournalPartialAbbreviation{Compend}{Compend}
\DefineJournalPartialAbbreviation{Compensat}{Compens}
\DefineJournalWordException{Competence}{Competence}
\DefineJournalAbbreviation{Competing}{Compet}
\DefineJournalPartialAbbreviation{Comp\'etit}{Compet}
\DefineJournalPartialAbbreviation{Compil}{Compil}
\DefineJournalPartialAbbreviation{Complain}{Complain}
\DefineJournalWordException{Compleat}{Compleat}
\DefineJournalPartialAbbreviation{Complet}{Complet}
\DefineJournalWordException{Complex}{Complex}
\DefineJournalAbbreviation{Complexity}{Complex}
\DefineJournalWordException{Compliance}{Compliance}
\DefineJournalPartialAbbreviation{Complicat}{Complicat}
\DefineJournalAbbreviation{Compliment}{Complim}
\DefineJournalAbbreviation{Complimentary}{Compliment}
\DefineJournalAbbreviation{Component}{Compon}
\DefineJournalPartialAbbreviation{Compos}{Compos}
\DefineJournalPartialAbbreviation{Compost}{Compost}
\DefineJournalPartialAbbreviation{Compound}{Compd}
\DefineJournalAbbreviation{Comprehensive}{Compr}
\DefineJournalAbbreviation{Compressed}{Compress}
\DefineJournalAbbreviation{Compression}{Compress}
\DefineJournalAbbreviation{Compressor}{Compress}
\DefineJournalPartialAbbreviation{Comptrol}{Comptrol}
\DefineJournalAbbreviation{Compulsive}{Compuls}
\DefineJournalAbbreviation{Compulsory}{Compuls}
\DefineJournalAbbreviation{Compunetics}{Na}
\DefineJournalPartialAbbreviation{Comput}{Comput}
\DefineJournalAbbreviation{Computerland}{Computerl}
\DefineJournalAbbreviation{Computervision}{Computerv}
\DefineJournalWordException{Computerworld}{Computerworld}
\DefineJournalWordException{Computimes}{Computimes}
\DefineJournalPartialAbbreviation{Comunica}{Comun}
\DefineJournalWordException{Concept}{Concept}
\DefineJournalAbbreviation{Conception}{Concept}
\DefineJournalAbbreviation{Conceptual}{Concept}
\DefineJournalWordException{Concern}{Concern}
\DefineJournalAbbreviation{Concerning}{Concern}
\DefineJournalPartialAbbreviation{Concholog}{Conchol}
\DefineJournalPartialAbbreviation{Conchyliolog}{Conchyliol}
\DefineJournalAbbreviation{Conciliation}{Concil}
\DefineJournalAbbreviation{Conciliator}{Concil}
\DefineJournalWordException{Concise}{Concise}
\DefineJournalAbbreviation{Conclusion}{Conclus}
\DefineJournalWordException{Concord}{Concord}
\DefineJournalAbbreviation{Concordance}{Concord}
\DefineJournalWordException{Concordia}{Concordia}
\DefineJournalPartialAbbreviation{Concrete}{Concr}
\DefineJournalPartialAbbreviation{Condens}{Condens}
\DefineJournalPartialAbbreviation{Condition}{Cond}
\DefineJournalAbbreviation{Condominium}{Condom}
\DefineJournalAbbreviation{Conducive}{Conduc}
\DefineJournalPartialAbbreviation{Confection}{Confect}
\DefineJournalPartialAbbreviation{Confedera}{Confed}
\DefineJournalPartialAbbreviation{Conferen}{Conf}
\DefineJournalPartialAbbreviation{Conferr}{Conferr}
\DefineJournalAbbreviation{Confessional}{Confess}
\DefineJournalAbbreviation{Confidence}{Confid}
\DefineJournalAbbreviation{Confidential}{Confid}
\DefineJournalAbbreviation{Confiscation}{Confisc}
\DefineJournalAbbreviation{Conflict}{Confl}
\DefineJournalAbbreviation{Confluence}{Conflu}
\DefineJournalWordException{Confort}{Confort}
\DefineJournalAbbreviation{Confraternity}{Confratern}
\DefineJournalPartialAbbreviation{Confrontation}{Confront}
\DefineJournalAbbreviation{Congenital}{Congenit}
\DefineJournalAbbreviation{Conglomerate}{Conglom}
\DefineJournalPartialAbbreviation{Congregat}{Congregat}
\DefineJournalPartialAbbreviation{Congres}{Congr}
\DefineJournalAbbreviation{Coniferous}{Conifer}
\DefineJournalWordException{Conjoint}{Conjoint}
\DefineJournalPartialAbbreviation{Connecticut}{Conn}
\DefineJournalPartialAbbreviation{Connection}{Connect}
\DefineJournalAbbreviation{Connective}{Connect}
\DefineJournalAbbreviation{Connector}{Connect}
\DefineJournalWordException{Connexe}{Connexe}
\DefineJournalAbbreviation{Connoisseur}{Connoiss}
\DefineJournalWordException{Connolly}{Connolly}
\DefineJournalAbbreviation{Conquering}{Conqu}
\DefineJournalAbbreviation{Conquest}{Conqu}
\DefineJournalWordException{Conscious}{Conscious}
\DefineJournalAbbreviation{Consciousness}{Conscious}
\DefineJournalWordException{Conserve}{Conserve}
\DefineJournalAbbreviation{Consideration}{Consid}
\DefineJournalAbbreviation{Considered}{Consid}
\DefineJournalAbbreviation{Consisting}{Consist}
\DefineJournalWordException{Consolata}{Consolata}
\DefineJournalPartialAbbreviation{Consolidat}{Consol}
\DefineJournalPartialAbbreviation{Consomm}{Consomm}
\DefineJournalPartialAbbreviation{Conspir}{Conspir}
\DefineJournalWordException{Constable}{Constable}
\DefineJournalAbbreviation{Constabulary}{Constabul}
\DefineJournalWordException{Constant}{Constant}
\DefineJournalAbbreviation{Constantinian}{Constantin}
\DefineJournalAbbreviation{Constellation}{Constell}
\DefineJournalPartialAbbreviation{Constitue}{Const}
\DefineJournalPartialAbbreviation{Constitut}{Const}
\DefineJournalPartialAbbreviation{Construct}{Constr}
\DefineJournalAbbreviation{Consular}{Consul}
\DefineJournalPartialAbbreviation{Consult}{Consult}
\DefineJournalAbbreviation{Consumption}{Consum}
\DefineJournalWordException{Contact}{Contact}
\DefineJournalPartialAbbreviation{Contain}{Contain}
\DefineJournalPartialAbbreviation{Contamina}{Contam}
\DefineJournalPartialAbbreviation{Contempor}{Contemp}
\DefineJournalPartialAbbreviation{Contend}{Contend}
\DefineJournalWordException{Content}{Content}
\DefineJournalWordException{Contest}{Contest}
\DefineJournalWordException{Context}{Context}
\DefineJournalAbbreviation{Continence}{Cont}
\DefineJournalPartialAbbreviation{Continent}{Cont}
\DefineJournalAbbreviation{Contingency}{Conting}
\DefineJournalAbbreviation{Contingent}{Conting}
\DefineJournalAbbreviation{Contraception}{Contracept}
\DefineJournalAbbreviation{Contraceptive}{Contracept}
\DefineJournalWordException{Contract}{Contract}
\DefineJournalPartialAbbreviation{Contract}{Contract}
\DefineJournalWordException{Contrail}{Contrail}
\DefineJournalPartialAbbreviation{Contrar}{Contrar}
\DefineJournalWordException{Contrastive}{Contrastive}
\DefineJournalPartialAbbreviation{Control}{Control}
\DefineJournalPartialAbbreviation{Controv}{Controv}
\DefineJournalAbbreviation{Conurbation}{Conurbat}
\DefineJournalAbbreviation{Convalescent}{Conval}
\DefineJournalPartialAbbreviation{Convecti}{Convect}
\DefineJournalAbbreviation{Conventionland}{Conventionl}
\DefineJournalAbbreviation{Conversation}{Conversat}
\DefineJournalWordException{Converse}{Converse}
\DefineJournalAbbreviation{Conversion}{Convers}
\DefineJournalPartialAbbreviation{Convert}{Convert}
\DefineJournalPartialAbbreviation{Conveyanc}{Convey}
\DefineJournalWordException{Conveyor}{Conveyor}
\DefineJournalAbbreviation{Conviction}{Convict}
\DefineJournalAbbreviation{Convocation}{Convoc}
\DefineJournalAbbreviation{Cookbook}{Cookb}
\DefineJournalAbbreviation{Cookery}{Cook}
\DefineJournalAbbreviation{Cooking}{Cook}
\DefineJournalPartialAbbreviation{Cool}{Cool}
\DefineJournalWordException{Coolah}{Coolah}
\DefineJournalWordException{Coonabarabran}{Coonabarabran}
\DefineJournalWordException{Cooper}{Cooper}
\DefineJournalPartialAbbreviation{Coop\'era}{Coop}
\DefineJournalAbbreviation{Copenhagen}{Cph}
\DefineJournalPartialAbbreviation{Copolymer}{Copolym}
\DefineJournalAbbreviation{Copper}{Copp}
\DefineJournalAbbreviation{Coproduction}{Coprod}
\DefineJournalAbbreviation{Coptic}{Copt}
\DefineJournalAbbreviation{Copyright}{Copyr}
\DefineJournalWordException{Coral}{Coral}
\DefineJournalWordException{Coranto}{Coranto}
\DefineJournalAbbreviation{Corinthian}{Corinth}
\DefineJournalAbbreviation{Cormorant}{Cormor}
\DefineJournalAbbreviation{Cornelian}{Cornel}
\DefineJournalWordException{Corner}{Corner}
\DefineJournalWordException{Cornerstone}{Cornerstone}
\DefineJournalWordException{Cornfield}{Cornfield}
\DefineJournalAbbreviation{Cornish}{Corn}
\DefineJournalWordException{Cornstalk}{Cornstalk}
\DefineJournalWordException{Cornucopia}{Cornucopia}
\DefineJournalAbbreviation{Cornwall}{Corn}
\DefineJournalAbbreviation{Coronary}{Coron}
\DefineJournalWordException{Coroner}{Coroner}
\DefineJournalPartialAbbreviation{Corporat}{Corp}
\DefineJournalAbbreviation{Corporeal}{Corpor}
\DefineJournalPartialAbbreviation{Corpuscula}{Corpusc}
\DefineJournalWordException{Corral}{Corral}
\DefineJournalPartialAbbreviation{Correction}{Correct}
\DefineJournalAbbreviation{Corrective}{Correct}
\DefineJournalPartialAbbreviation{Correlat}{Correl}
\DefineJournalPartialAbbreviation{Correspond}{Corresp}
\DefineJournalPartialAbbreviation{Corrosi}{Corros}
\DefineJournalAbbreviation{Corrugated}{Corrugat}
\DefineJournalWordException{Corsair}{Corsair}
\DefineJournalWordException{Cortisone}{Cortisone}
\DefineJournalWordException{Corvallis}{Corvallis}
\DefineJournalPartialAbbreviation{Cosmeti}{Cosmet}
\DefineJournalPartialAbbreviation{Cosmetolog}{Cosmetol}
\DefineJournalPartialAbbreviation{Cosmochemi}{Cosmochem}
\DefineJournalPartialAbbreviation{Cosmochronolog}{Cosmochronol}
\DefineJournalPartialAbbreviation{Cosmolog}{Cosmol}
\DefineJournalAbbreviation{Cosmophobia}{Cosmophob}
\DefineJournalWordException{Costing}{Costing}
\DefineJournalWordException{Costume}{Costume}
\DefineJournalPartialAbbreviation{Cottag}{Cottag}
\DefineJournalWordException{Cottage}{Cottage}
\DefineJournalWordException{Cottlesloe}{Cottlesloe}
\DefineJournalWordException{Cotton}{Cotton}
\DefineJournalPartialAbbreviation{Coulometr}{Coulom}
\DefineJournalAbbreviation{Councelling}{Counc}
\DefineJournalPartialAbbreviation{Council}{Counc}
\DefineJournalPartialAbbreviation{Counsel}{Couns}
\DefineJournalWordException{Count}{Count}
\DefineJournalWordException{Countdown}{Countdown}
\DefineJournalAbbreviation{Counter}{Count}
\DefineJournalWordException{Counterattack}{Counterattack}
\DefineJournalPartialAbbreviation{Countermeasur}{Countermeas}
\DefineJournalWordException{Counterpoint}{Counterpoint}
\DefineJournalAbbreviation{Countertrade}{Countertr}
\DefineJournalAbbreviation{Counties}{Cties}
\DefineJournalAbbreviation{Counting}{Count}
\DefineJournalAbbreviation{Countries}{Ctries}
\DefineJournalAbbreviation{Country}{Ctry}
\DefineJournalAbbreviation{Countryman}{Countrym}
\DefineJournalAbbreviation{Countryside}{Countrys}
\DefineJournalAbbreviation{Countrywide}{Countryw}
\DefineJournalAbbreviation{County}{Cty}
\DefineJournalWordException{Courage}{Courage}
\DefineJournalPartialAbbreviation{Courier}{Cour}
\DefineJournalAbbreviation{Courseware}{Coursew}
\DefineJournalPartialAbbreviation{Court}{Court}
\DefineJournalAbbreviation{Courthouse}{Courth}
\DefineJournalWordException{Covenant}{Covenant}
\DefineJournalPartialAbbreviation{Covenant}{Covenant}
\DefineJournalWordException{Coventry}{Coventry}
\DefineJournalPartialAbbreviation{Cover}{Cover}
\DefineJournalWordException{Cowboy}{Cowboy}
\DefineJournalWordException{Cowdray}{Cowdray}
\DefineJournalWordException{Cowichan}{Cowichan}
\DefineJournalWordException{Coyote}{Coyote}
\DefineJournalAbbreviation{Cracked}{Crack}
\DefineJournalAbbreviation{Cracking}{Crack}
\DefineJournalWordException{Craft}{Craft}
\DefineJournalAbbreviation{Craftsman}{Craftsm}
\DefineJournalPartialAbbreviation{Craftwork}{Craftwork}
\DefineJournalWordException{Crafty}{Crafty}
\DefineJournalWordException{Cranfield}{Cranfield}
\DefineJournalAbbreviation{Craniomandibular}{Craniomandib}
\DefineJournalWordException{Cranwells}{Cranwells}
\DefineJournalWordException{Crappie}{Crappie}
\DefineJournalWordException{Crawford}{Crawford}
\DefineJournalAbbreviation{Creamery}{Cream}
\DefineJournalAbbreviation{Credibility}{Credibil}
\DefineJournalWordException{Creighton}{Creighton}
%\DefineJournalPartialWordException{Cremat}{Cremat-}
\DefineJournalWordException{Cr\'eole}{Cr\'eole}
\DefineJournalWordException{Crescent}{Crescent}
\DefineJournalWordException{Crested}{Crested}
\DefineJournalAbbreviation{Cretaceous}{Cretac}
\DefineJournalPartialAbbreviation{Cretinism}{Cretin}
\DefineJournalWordException{Cribbage}{Cribbage}
\DefineJournalWordException{Cricket}{Cricket}
\DefineJournalAbbreviation{Cricketer}{Cricket}
\DefineJournalAbbreviation{Crimean}{Crime}
\DefineJournalPartialAbbreviation{Criminal}{Crim}
\DefineJournalPartialAbbreviation{Criminolog}{Criminol}
\DefineJournalPartialAbbreviation{Crippl}{Crippl}
\DefineJournalPartialAbbreviation{Criptogami}{Criptogam}
\DefineJournalWordException{Crisis}{Crisis}
\DefineJournalWordException{Criteria}{Criteria}
\DefineJournalWordException{Criterion}{Criterion}
\DefineJournalWordException{Criterium}{Criterium}
\DefineJournalAbbreviation{Critic}{Crit}
\DefineJournalPartialAbbreviation{Critici}{Crit}
\DefineJournalAbbreviation{Croaker}{Croak}
\DefineJournalPartialAbbreviation{Croati}{Croat}
\DefineJournalWordException{Crocodile}{Crocodile}
\DefineJournalAbbreviation{Crofter}{Croft}
\DefineJournalWordException{Crooked}{Crooked}
\DefineJournalWordException{Crooner}{Crooner}
\DefineJournalPartialAbbreviation{Crop}{Crop}
\DefineJournalWordException{Croquet}{Croquet}
\DefineJournalWordException{Cross}{Cross}
\DefineJournalAbbreviation{Crossbreeding}{Crossbreed}
\DefineJournalAbbreviation{Crosscurrent}{Crosscurr}
\DefineJournalWordException{Crossing}{Crossing}
\DefineJournalAbbreviation{Crosslinking}{Crosslink}
\DefineJournalWordException{Crossroad}{Crossroad}
\DefineJournalWordException{Crossword}{Crossword}
\DefineJournalWordException{Crossworld}{Crossworld}
\DefineJournalWordException{Croydon}{Croydon}
\DefineJournalAbbreviation{Crucible}{Crucib}
\DefineJournalAbbreviation{Cruelty}{Cruel}
\DefineJournalWordException{Cruise}{Cruise}
\DefineJournalWordException{Cruiser}{Cruiser}
\DefineJournalAbbreviation{Cruising}{Cruis}
\DefineJournalWordException{Crumlin}{Crumlin}
\DefineJournalAbbreviation{Crusader}{Crusad}
\DefineJournalAbbreviation{Crusading}{Crusad}
\DefineJournalAbbreviation{Crusher}{Crush}
\DefineJournalAbbreviation{Crushing}{Crush}
\DefineJournalPartialAbbreviation{Cryobiolog}{Cryobiol}
\DefineJournalPartialAbbreviation{Cryoengineer}{Cryoeng}
\DefineJournalPartialAbbreviation{Cryogeni}{Cryog}
\DefineJournalPartialAbbreviation{Cryophysic}{Cryophys}
\DefineJournalPartialAbbreviation{Cryopreserv}{Cryopreserv}
\DefineJournalAbbreviation{Cryptanthus}{Cryptanth}
\DefineJournalPartialAbbreviation{Cryptogami}{Cryptogam}
\DefineJournalPartialAbbreviation{Cryptograph}{Cryptogr}
\DefineJournalAbbreviation{Cryptology}{Cryptol}
\DefineJournalAbbreviation{Crystal}{Cryst}
\DefineJournalPartialAbbreviation{Crystalli}{Cryst}
\DefineJournalPartialAbbreviation{Crystallochemi}{Crystallochem}
\DefineJournalPartialAbbreviation{Crystallograph}{Crystallogr}
\DefineJournalAbbreviation{Crystals}{Cryst}
\DefineJournalPartialAbbreviation{Cuba}{Cuba}
\DefineJournalWordException{Cucumber}{Cucumber}
\DefineJournalWordException{Cucurbit}{Cucurbit}
\DefineJournalWordException{Cuddapah}{Cuddapah}
\DefineJournalAbbreviation{Culinary}{Culin}
\DefineJournalPartialAbbreviation{Cultiv}{Cultiv}
\DefineJournalWordException{Cultuel}{Cultuel}
\DefineJournalPartialAbbreviation{Cultur}{Cult}
\DefineJournalAbbreviation{Cumberland}{Cumberl}
\DefineJournalWordException{Cumbria}{Cumbria}
\DefineJournalPartialAbbreviation{Cumulat}{Cumul}
\DefineJournalAbbreviation{Cuneiform}{Cuneif}
\DefineJournalWordException{Curation}{Curation}
\DefineJournalWordException{Curator}{Curator}
\DefineJournalAbbreviation{Curatorial}{Curator}
\DefineJournalWordException{Curing}{Curing}
\DefineJournalPartialAbbreviation{Curiosit}{Curiosit}
\DefineJournalAbbreviation{Curler}{Curl}
\DefineJournalAbbreviation{Curling}{Curl}
\DefineJournalAbbreviation{Curmudgeon}{Curmudg}
\DefineJournalAbbreviation{Currency}{Curr}
\DefineJournalPartialAbbreviation{Current}{Curr}
\DefineJournalAbbreviation{Curricular}{Curric}
\DefineJournalWordException{Curtain}{Curtain}
\DefineJournalWordException{Curtainwall}{Curtainwall}
\DefineJournalWordException{Cushion}{Cushion}
\DefineJournalWordException{Custer}{Custer}
\DefineJournalAbbreviation{Custodial}{Custod}
\DefineJournalWordException{Custodian}{Custodian}
\DefineJournalWordException{Custody}{Custody}
\DefineJournalPartialAbbreviation{Custom}{Cust}
\DefineJournalAbbreviation{Cutaneous}{Cutan}
\DefineJournalWordException{Cutlass}{Cutlass}
\DefineJournalWordException{Cutlery}{Cutlery}
\DefineJournalWordException{Cuttack}{Cuttack}
\DefineJournalAbbreviation{Cutter}{Cut}
\DefineJournalAbbreviation{Cutting}{Cut}
\DefineJournalWordException{Cyanamid}{Cyanamid}
\DefineJournalPartialAbbreviation{Cyberneti}{Cybern}
\DefineJournalAbbreviation{Cybersecurity}{Cybersecur}
\DefineJournalWordException{Cycle}{Cycle}
\DefineJournalAbbreviation{Cyclic}{Cycl}
\DefineJournalAbbreviation{Cycling}{Cycl}
\DefineJournalAbbreviation{Cyclist}{Cycl}
\DefineJournalPartialAbbreviation{Cycloadditi}{Cycloaddit}
\DefineJournalAbbreviation{Cyclodextrin}{Cyclodext}
\DefineJournalAbbreviation{Cyclopaedia}{Cyclop}
\DefineJournalAbbreviation{Cyclorama}{Cyclor}
\DefineJournalAbbreviation{Cyclostyled}{Cyclost}
\DefineJournalAbbreviation{Cyclotron}{Cyclotr}
\DefineJournalPartialAbbreviation{Cylind}{Cylind}
\DefineJournalWordException{Cyprus}{Cyprus}
\DefineJournalAbbreviation{Cystic}{Cyst}
\DefineJournalPartialAbbreviation{Cytobiolog}{Cytobiol}
\DefineJournalPartialAbbreviation{Cytochem}{Cytochem}
\DefineJournalPartialAbbreviation{Cytodiagnos}{Cytodiagn}
\DefineJournalPartialAbbreviation{Cytoembryolog}{Cytoembryol}
\DefineJournalPartialAbbreviation{Cytogenet}{Cytogenet}
%\DefineJournalPartialWordException{Cytokynes}{Cytokynes-}
\DefineJournalPartialAbbreviation{Cytolog}{Cytol}
\DefineJournalPartialAbbreviation{Cytometr}{Cytom}
\DefineJournalPartialAbbreviation{Cytopatholog}{Cytopathol}
\DefineJournalPartialAbbreviation{Cytopharmacolog}{Cytopharmacol}
\DefineJournalPartialAbbreviation{Cytophotometr}{Cytophotom}
\DefineJournalPartialAbbreviation{Cytoprotect}{Cytoprot}
\DefineJournalAbbreviation{Cytoreduction}{Cytoreduct}
\DefineJournalPartialAbbreviation{Cytoskelet}{Cytoskelet}
\DefineJournalAbbreviation{Cytotoxicity}{Cytotox}
\DefineJournalWordException{Cytyscope}{Cytyscope}
\DefineJournalPartialAbbreviation{Czechoslov}{Czechoslov}
\DefineJournalWordException{Daffodil}{Daffodil}
\DefineJournalWordException{Dagger}{Dagger}
\DefineJournalAbbreviation{Daily}{Dly}
\DefineJournalWordException{Dairy}{Dairy}
\DefineJournalAbbreviation{Dairyfarming}{Dairyfarm}
\DefineJournalAbbreviation{Dairying}{Dairy}
\DefineJournalAbbreviation{Dairyland}{Dairyl}
\DefineJournalAbbreviation{Dairyman}{Dairym}
\DefineJournalAbbreviation{Dakota}{Dak}
\DefineJournalAbbreviation{Dalesman}{Dalesm}
\DefineJournalAbbreviation{Dalhousie}{Dalhous}
\DefineJournalWordException{Dalisy}{Dalisy}
\DefineJournalWordException{Dallas}{Dallas}
\DefineJournalWordException{Damage}{Damage}
\DefineJournalAbbreviation{Dancer}{Danc}
\DefineJournalWordException{Dancework}{Dancework}
\DefineJournalAbbreviation{Dancing}{Danc}
\DefineJournalAbbreviation{Danemark}{Dan}
\DefineJournalAbbreviation{Dangerous}{Danger}
\DefineJournalAbbreviation{Danish}{Dan}
\DefineJournalAbbreviation{Dansville}{Dansv}
\DefineJournalAbbreviation{Daoism}{Dao}
\DefineJournalWordException{Daringly}{Daringly}
\DefineJournalAbbreviation{Darkness}{Darkn}
\DefineJournalWordException{Darkroom}{Darkroom}
\DefineJournalWordException{Darling Downs}{Darling Downs}
\DefineJournalWordException{Darlinghurst}{Darlinghurst}
\DefineJournalWordException{Dartmoor}{Dartmoor}
\DefineJournalAbbreviation{Dartmouth}{Dartm}
\DefineJournalWordException{Darwin}{Darwin}
\DefineJournalAbbreviation{Data-upper}{Data-upp}
\DefineJournalWordException{Databank}{Databank}
\DefineJournalWordException{Database}{Database}
\DefineJournalAbbreviation{Databook}{Datab}
\DefineJournalWordException{Datacom}{Datacom}
\DefineJournalWordException{Datacomm}{Datacomm}
\DefineJournalAbbreviation{Datafile}{Dataf}
\DefineJournalAbbreviation{Datamail}{Datam}
\DefineJournalAbbreviation{Datamatic}{Datamat}
\DefineJournalAbbreviation{Datamation}{Datamat}
\DefineJournalAbbreviation{Datapoint}{Datapt}
\DefineJournalWordException{Datapro}{Datapro}
\DefineJournalAbbreviation{Datareview}{Datarev}
\DefineJournalAbbreviation{Datasystem}{Datasyst}
\DefineJournalAbbreviation{Datebook}{Dateb}
\DefineJournalWordException{Dateline}{Dateline}
\DefineJournalWordException{Dating}{Dating}
\DefineJournalWordException{Daughter}{Daughter}
\DefineJournalWordException{Dauphin}{Dauphin}
\DefineJournalWordException{Dawson}{Dawson}
\DefineJournalWordException{Daycare}{Daycare}
\DefineJournalWordException{Daylight}{Daylight}
\DefineJournalWordException{Daylily}{Daylily}
\DefineJournalWordException{Daytime}{Daytime}
\DefineJournalAbbreviation{Dayton}{Dayt}
\DefineJournalAbbreviation{Daytona Beach}{Dayt Beach}
\DefineJournalAbbreviation{Dayworks}{Dayw}
\DefineJournalPartialAbbreviation{Deactiva}{Deactiv}
\DefineJournalWordException{Deadline}{Deadline}
\DefineJournalPartialAbbreviation{Deaf}{Deaf}
\DefineJournalWordException{Deakin}{Deakin}
\DefineJournalPartialAbbreviation{Deal}{Deal}
\DefineJournalWordException{Debate}{Debate}
\DefineJournalAbbreviation{Debenture}{Debent}
\DefineJournalAbbreviation{Debtor}{Debt}
\DefineJournalPartialAbbreviation{D\'ecad}{D\'ecad}
\DefineJournalWordException{Decade}{Decade}
\DefineJournalAbbreviation{Decanter}{Decant}
\DefineJournalWordException{Decay}{Decay}
\DefineJournalAbbreviation{December}{Dec}
\DefineJournalAbbreviation{Decennial}{Decenn}
\DefineJournalAbbreviation{Deception}{Decept}
\DefineJournalAbbreviation{Decertification}{Decertif}
\DefineJournalWordException{Deciduous}{Deciduous}
\DefineJournalAbbreviation{Decimal}{Decim}
\DefineJournalPartialAbbreviation{Decision}{Decis}
\DefineJournalPartialAbbreviation{Declara}{Declar}
\DefineJournalPartialAbbreviation{Declassifi}{Declassif}
\DefineJournalWordException{Decline}{Decline}
\DefineJournalAbbreviation{Declining}{Declin}
\DefineJournalAbbreviation{Decomposition}{Decompos}
\DefineJournalPartialAbbreviation{Decontaminat}{Decontam}
\DefineJournalAbbreviation{Decorating}{Decor}
\DefineJournalAbbreviation{Decoration}{Decor}
\DefineJournalAbbreviation{Decorative}{Decor}
\DefineJournalPartialAbbreviation{Decorator}{Decor}
\DefineJournalWordException{Decormag}{Decormag}
\DefineJournalPartialAbbreviation{Decorporat}{Decorp}
\DefineJournalWordException{Decoy}{Decoy}
\DefineJournalWordException{Decree}{Decree}
\DefineJournalAbbreviation{Dedicated}{Dedic}
\DefineJournalAbbreviation{Deduction}{Deduc}
\DefineJournalPartialAbbreviation{Deep}{Deep}
\DefineJournalAbbreviation{Deerbreeder}{Deerbreed}
\DefineJournalWordException{Default}{Default}
\DefineJournalWordException{Defect}{Defect}
\DefineJournalAbbreviation{Defence}{Def}
\DefineJournalAbbreviation{Defender}{Def}
\DefineJournalAbbreviation{Defense}{D\'ef}
\DefineJournalPartialAbbreviation{Deficienc}{Defic}
\DefineJournalPartialAbbreviation{Defin}{Defin}
\DefineJournalPartialAbbreviation{Defray}{Defray}
\DefineJournalWordException{Defunct}{Defunct}
\DefineJournalPartialAbbreviation{Degenerati}{Degener}
\DefineJournalAbbreviation{Degradation}{Degrad}
\DefineJournalWordException{Degree}{Degree}
\DefineJournalWordException{Dekalb}{Dekalb}
\DefineJournalWordException{Dekstop}{Dekstop}
\DefineJournalPartialAbbreviation{Delaware}{Del}
\DefineJournalWordException{Delhi}{Delhi}
\DefineJournalAbbreviation{Delicious}{Delic}
\DefineJournalWordException{Delight}{Delight}
\DefineJournalPartialAbbreviation{Deliver}{Deliv}
\DefineJournalWordException{Deluxe}{Deluxe}
\DefineJournalWordException{Demand}{Demand}
\DefineJournalPartialAbbreviation{Deminerali}{Deminer}
\DefineJournalPartialAbbreviation{Democra}{Democr}
\DefineJournalWordException{Denbigh}{Denbigh}
\DefineJournalWordException{Dengue}{Dengue}
\DefineJournalPartialAbbreviation{Denmark}{Den}
\DefineJournalAbbreviation{Denominator}{Denominat}
\DefineJournalPartialAbbreviation{Densificat}{Densif}
\DefineJournalPartialAbbreviation{Densitometr}{Densitom}
\DefineJournalWordException{Density}{Density}
\DefineJournalPartialAbbreviation{Denta}{Dent}
\DefineJournalPartialAbbreviation{Dentist}{Dent}
\DefineJournalAbbreviation{Dentofacial}{Dentofac}
\DefineJournalAbbreviation{Denturist}{Dent}
\DefineJournalWordException{Denver}{Denver}
\DefineJournalPartialAbbreviation{Department}{Dep}
\DefineJournalAbbreviation{Departure}{Depart}
\DefineJournalWordException{Dependable}{Dependable}
\DefineJournalAbbreviation{Dependent}{Depend}
\DefineJournalAbbreviation{Depletion}{Deplet}
\DefineJournalAbbreviation{Deployment}{Deploy}
\DefineJournalAbbreviation{Deposit}{Depos}
\DefineJournalAbbreviation{Depositor}{Depos}
\DefineJournalAbbreviation{Depository}{Depos}
\DefineJournalAbbreviation{Depreciation}{Depreciat}
\DefineJournalPartialAbbreviation{D\'epress}{Depress}
\DefineJournalWordException{Deputy}{Deputy}
\DefineJournalAbbreviation{Derbyshire}{Derbys}
\DefineJournalAbbreviation{Deregulation}{Deregul}
\DefineJournalAbbreviation{Derelict}{Derel}
\DefineJournalPartialAbbreviation{Deriva}{Deriv}
\DefineJournalPartialAbbreviation{Derive}{Deriv}
\DefineJournalAbbreviation{Dermatitis}{Dermat}
\DefineJournalPartialAbbreviation{Dermatopatholog}{Dermatopathol}
\DefineJournalPartialAbbreviation{Dermatopharmacolog}{Dermatopharmacol}
\DefineJournalWordException{Dermatose}{Dermatose}
\DefineJournalPartialAbbreviation{Dermatotoxicolog}{Dermatotoxic}
\DefineJournalWordException{Des Moines}{Des Moines}
\DefineJournalPartialAbbreviation{Desalt}{Desalt}
\DefineJournalPartialAbbreviation{Describ}{Descr}
\DefineJournalPartialAbbreviation{Descripti}{Descr}
\DefineJournalAbbreviation{Descriptor}{Descr}
\DefineJournalPartialAbbreviation{Desegreg}{Desegreg}
\DefineJournalWordException{Desert}{Desert}
\DefineJournalPartialAbbreviation{Design}{Des}
\DefineJournalAbbreviation{Designbook}{Designb}
\DefineJournalWordException{Desire}{Desire}
\DefineJournalAbbreviation{Deskbook}{Deskb}
\DefineJournalWordException{Deskmate}{Deskmate}
\DefineJournalAbbreviation{Desktop}{Deskt}
\DefineJournalWordException{Despatch}{Despatch}
\DefineJournalWordException{Destiny}{Destiny}
\DefineJournalPartialAbbreviation{Destructi}{Destr}
\DefineJournalPartialAbbreviation{Destructor}{Destr}
\DefineJournalAbbreviation{Detailed}{Detail}
\DefineJournalPartialAbbreviation{Detect}{Detect}
\DefineJournalAbbreviation{Detention}{Deten}
\DefineJournalPartialAbbreviation{Detergen}{Deterg}
\DefineJournalAbbreviation{Determination}{Determ}
\DefineJournalPartialAbbreviation{Detoxificat}{Detoxif}
\DefineJournalWordException{Detroit}{Detroit}
\DefineJournalPartialAbbreviation{Develop}{Dev}
%\DefineJournalPartialWordException{Devianc}{Devianc-}
\DefineJournalWordException{Deviant}{Deviant}
\DefineJournalAbbreviation{Deviation}{Deviat}
\DefineJournalWordException{Device}{Device}
\DefineJournalWordException{Devonian}{Devonian}
\DefineJournalAbbreviation{Devonshire}{Devon}
\DefineJournalAbbreviation{Devotion}{Devot}
\DefineJournalAbbreviation{Devotional}{Devot}
\DefineJournalWordException{Dhahran}{Dhahran}
\DefineJournalWordException{Dhanbad}{Dhanbad}
\DefineJournalWordException{Dhenkanal}{Dhenkanal}
\DefineJournalWordException{Diabetes}{Diabetes}
\DefineJournalAbbreviation{Diabetic}{Diabet}
\DefineJournalAbbreviation{Diacyclglycerols}{Diacyclglyc}
\DefineJournalPartialAbbreviation{Diaeteti}{Diaet}
\DefineJournalAbbreviation{Diagram}{Diagr}
\DefineJournalWordException{Dialect}{Dialect}
\DefineJournalAbbreviation{Dialectical}{Dialect}
\DefineJournalAbbreviation{Dialectric}{Dialectr}
\DefineJournalWordException{Dialling}{Dialling}
\DefineJournalAbbreviation{Diamond}{Diam}
\DefineJournalAbbreviation{Dianetic}{Dianet}
\DefineJournalWordException{Diarrhea}{Diarrhea}
\DefineJournalWordException{Diarrhoea}{Diarrhoea}
\DefineJournalWordException{Diarrhoeal}{Diarrhoeal}
\DefineJournalWordException{Diary}{Diary}
\DefineJournalAbbreviation{Diathesis}{Diath}
\DefineJournalWordException{Diatomic}{Diatomic}
\DefineJournalWordException{Diatomist}{Diatomist}
\DefineJournalAbbreviation{Dictionary}{Dict}
\DefineJournalPartialAbbreviation{Didacti}{Didact}
\DefineJournalAbbreviation{Didakometry}{Didakom}
\DefineJournalWordException{Didcot}{Didcot}
\DefineJournalPartialAbbreviation{Dielectric}{Dielectr}
\DefineJournalPartialAbbreviation{Dielectrophore}{Dielectrophor}
\DefineJournalWordException{Diesel}{Diesel}
\DefineJournalAbbreviation{Dietary}{Diet}
\DefineJournalAbbreviation{Dietitian}{Dietit}
\DefineJournalPartialAbbreviation{Differen}{Differ}
\DefineJournalAbbreviation{Difficulty}{Diffic}
\DefineJournalAbbreviation{Diffraction}{Diffr}
\DefineJournalPartialAbbreviation{Diffractometer}{Diffractom}
\DefineJournalPartialAbbreviation{Digest}{Dig}
\DefineJournalWordException{Digger}{Digger}
\DefineJournalAbbreviation{Dihydroxyvitamin}{Dihydroxyvitam}
\DefineJournalAbbreviation{Diligence}{Dilig}
\DefineJournalAbbreviation{Dimension}{Dimens}
\DefineJournalWordException{Dinghy}{Dinghy}
\DefineJournalWordException{Dining}{Dining}
\DefineJournalAbbreviation{Dinner}{Dinn}
\DefineJournalPartialAbbreviation{Dinoflagellat}{Dinoflag}
\DefineJournalPartialAbbreviation{Dinosaur}{Dinosaur}
\DefineJournalAbbreviation{Diocesan}{Dioc}
\DefineJournalAbbreviation{Diplomacy}{Dipl}
\DefineJournalWordException{Dipper}{Dipper}
\DefineJournalAbbreviation{Dipterist}{Dipter}
\DefineJournalAbbreviation{Directed}{Dir}
\DefineJournalPartialAbbreviation{Directi}{Dir}
\DefineJournalPartialAbbreviation{Director}{Dir}
\DefineJournalPartialAbbreviation{Disabilit}{Disabil}
\DefineJournalAbbreviation{Disabled}{Disabl}
\DefineJournalAbbreviation{Disaccharide}{Disacch}
\DefineJournalAbbreviation{Disadvantage}{Disadv}
\DefineJournalPartialAbbreviation{Disarm}{Disarm}
\DefineJournalWordException{Disaster}{Disaster}
\DefineJournalPartialAbbreviation{Disbursement}{Disburse}
\DefineJournalPartialAbbreviation{Discern}{Discern}
\DefineJournalAbbreviation{Discharge}{Disch}
\DefineJournalPartialAbbreviation{Discipl}{Discipl}
\DefineJournalAbbreviation{Discipleship}{Disciplesh}
\DefineJournalPartialAbbreviation{Disciplin}{Discip}
\DefineJournalPartialAbbreviation{Disclosure}{Discl}
\DefineJournalAbbreviation{Discography}{Discogr}
\DefineJournalAbbreviation{Discontinued}{Discontin}
\DefineJournalPartialAbbreviation{Discount}{Discount}
\DefineJournalWordException{Discourse}{Discourse}
\DefineJournalPartialAbbreviation{Discover}{Discov}
\DefineJournalPartialAbbreviation{Discret}{Discret}
\DefineJournalPartialAbbreviation{Discussi}{Discuss}
\DefineJournalPartialAbbreviation{Disease}{Dis}
\DefineJournalPartialAbbreviation{Disinfect}{Disinfect}
\DefineJournalAbbreviation{Dismissal}{Dismiss}
\DefineJournalPartialAbbreviation{Disorder}{Disord}
\DefineJournalAbbreviation{Disparition}{Dispar}
\DefineJournalWordException{Dispatch}{Dispatch}
\DefineJournalPartialAbbreviation{Dispens}{Dispens}
\DefineJournalPartialAbbreviation{Dispetcheriz}{Dispetcher}
\DefineJournalPartialAbbreviation{Displac}{Displac}
\DefineJournalAbbreviation{Display}{Disp}
\DefineJournalPartialAbbreviation{Disponib}{Dispon}
\DefineJournalAbbreviation{Disposal}{Dispos}
\DefineJournalPartialAbbreviation{Disposit}{Dispos}
\DefineJournalAbbreviation{Disruption}{Disrupt}
%\DefineJournalPartialWordException{Dissatisf}{Dissatisf-}
\DefineJournalAbbreviation{Dissemination}{Dissem}
\DefineJournalWordException{Dissent}{Dissent}
\DefineJournalAbbreviation{Dissenting}{Dissent}
\DefineJournalPartialAbbreviation{Disserta}{Diss}
\DefineJournalWordException{Distance}{Distance}
\DefineJournalPartialAbbreviation{Distill}{Distill}
\DefineJournalAbbreviation{Distinction}{Distinct}
\DefineJournalPartialAbbreviation{Distinguish}{Disting}
\DefineJournalWordException{Distress}{Distress}
\DefineJournalAbbreviation{District of Columbia}{DC}
\DefineJournalPartialAbbreviation{District}{Dist}
\DefineJournalAbbreviation{Disturbance}{Disturb}
\DefineJournalAbbreviation{Disturbed}{Disturb}
\DefineJournalAbbreviation{Diuretic}{Diuret}
\DefineJournalPartialAbbreviation{Divers}{Divers}
\DefineJournalAbbreviation{Diversification}{Diversif}
\DefineJournalPartialAbbreviation{Divest}{Divest}
\DefineJournalPartialAbbreviation{Divid}{Divid}
\DefineJournalWordException{Divine}{Divine}
\DefineJournalWordException{Diving}{Diving}
\DefineJournalAbbreviation{Divinity}{Divin}
\DefineJournalPartialAbbreviation{Divis}{Div}
\DefineJournalWordException{Divorce}{Divorce}
\DefineJournalWordException{Docket}{Docket}
\DefineJournalAbbreviation{Docklands}{Dockl}
\DefineJournalPartialAbbreviation{Doctor}{Dr}
\DefineJournalWordException{Doing}{Doing}
\DefineJournalWordException{Dolbeau}{Dolbeau}
\DefineJournalAbbreviation{Dollarwise}{Dollarw}
\DefineJournalWordException{Domain}{Domain}
\DefineJournalPartialAbbreviation{Domesti}{Domest}
\DefineJournalPartialAbbreviation{Dominican}{Dominic}
\DefineJournalAbbreviation{Dominion}{Dom}
\DefineJournalWordException{Don-Mills}{Don-Mills}
\DefineJournalWordException{Doncaster}{Doncaster}
\DefineJournalWordException{Donegal}{Donegal}
\DefineJournalWordException{Donkey}{Donkey}
\DefineJournalWordException{Donnybrook}{Donnybrook}
\DefineJournalWordException{Doobally}{Doobally}
\DefineJournalPartialAbbreviation{Doodl}{Doodl}
\DefineJournalAbbreviation{Dorking}{Dork}
\DefineJournalWordException{Dorset}{Dorset}
\DefineJournalWordException{Doubleday}{Doubleday}
\DefineJournalPartialAbbreviation{Doubt}{Doubt}
\DefineJournalWordException{Downeast}{Downeast}
\DefineJournalAbbreviation{Downland}{Downl}
\DefineJournalWordException{Download}{Download}
\DefineJournalPartialAbbreviation{Downscal}{Downscal}
\DefineJournalAbbreviation{Downstream}{Downstr}
\DefineJournalWordException{Downsview}{Downsview}
\DefineJournalAbbreviation{Downtown}{Downt}
\DefineJournalWordException{Downunder}{Downunder}
\DefineJournalWordException{Dowsing}{Dowsing}
\DefineJournalAbbreviation{Dozenal}{Dozen}
\DefineJournalPartialAbbreviation{Draft}{Draft}
\DefineJournalWordException{Dragonfly}{Dragonfly}
\DefineJournalWordException{Dragster}{Dragster}
\DefineJournalAbbreviation{Drainer}{Drain}
\DefineJournalWordException{Draining}{Draining}
\DefineJournalPartialAbbreviation{Dramati}{Dram}
\DefineJournalPartialAbbreviation{Dramaturg}{Dramaturg}
%\DefineJournalPartialWordException{Draper}{Draper-}
\DefineJournalWordException{Draught}{Draught}
\DefineJournalPartialAbbreviation{Draught}{Draught}
\DefineJournalAbbreviation{Draughting}{Draught}
\DefineJournalWordException{Draughtsman}{Draughtsman}
\DefineJournalAbbreviation{Dravidic}{Dravid}
\DefineJournalPartialAbbreviation{Draw}{Draw}
\DefineJournalAbbreviation{Drayton}{Drayt}
\DefineJournalWordException{Dreadful}{Dreadful}
\DefineJournalAbbreviation{Dreamer}{Dream}
\DefineJournalAbbreviation{Dreamweaver}{Dreamweav}
\DefineJournalAbbreviation{Dredger}{Dredg}
\DefineJournalAbbreviation{Dredging}{Dredg}
\DefineJournalWordException{Dress}{Dress}
\DefineJournalAbbreviation{Dressing}{Dress}
\DefineJournalAbbreviation{Drifting}{Drift}
\DefineJournalWordException{Driftwood}{Driftwood}
\DefineJournalAbbreviation{Drilled}{Drill}
\DefineJournalAbbreviation{Drilling}{Drill}
\DefineJournalPartialAbbreviation{Drink}{Drink}
\DefineJournalWordException{Drivel}{Drivel}
\DefineJournalAbbreviation{Driver}{Driv}
\DefineJournalAbbreviation{Driving}{Driv}
\DefineJournalWordException{Drought}{Drought}
\DefineJournalAbbreviation{Drought-stricken}{Drought-strick}
\DefineJournalPartialAbbreviation{Druggist}{Drug}
\DefineJournalAbbreviation{Drugtherapy}{Drugther}
\DefineJournalAbbreviation{Drumheller}{Drumhell}
\DefineJournalWordException{Drummer}{Drummer}
\DefineJournalWordException{Drummond}{Drummond}
\DefineJournalWordException{Drunkenness}{Drunkenness}
\DefineJournalAbbreviation{Drycleaner}{Dryclean}
\DefineJournalAbbreviation{Dryer}{Dry}
\DefineJournalAbbreviation{Drying}{Dry}
\DefineJournalWordException{Dryland}{Dryland}
\DefineJournalWordException{Dublin}{Dublin}
\DefineJournalWordException{Duleek}{Duleek}
\DefineJournalAbbreviation{Dumbarton}{Dumbart}
\DefineJournalAbbreviation{Dumfriesshire}{Dumfries}
\DefineJournalAbbreviation{Dumping}{Dump}
\DefineJournalWordException{Dunboyne}{Dunboyne}
\DefineJournalWordException{Dundee}{Dundee}
\DefineJournalAbbreviation{Dunedin}{Duned}
\DefineJournalWordException{Dungeon}{Dungeon}
\DefineJournalAbbreviation{Durability}{Durab}
\DefineJournalAbbreviation{Duration}{Durat}
\DefineJournalAbbreviation{Durban}{Durb}
\DefineJournalAbbreviation{Durham}{Durh}
\DefineJournalAbbreviation{During}{Dur}
\DefineJournalWordException{Dutchman}{Dutchman}
\DefineJournalPartialAbbreviation{Dversif}{Diversif}
\DefineJournalAbbreviation{Dwelling}{Dwell}
\DefineJournalPartialAbbreviation{Dye}{Dye}
\DefineJournalPartialAbbreviation{Dyestuff}{Dyest}
\DefineJournalWordException{Dyking}{Dyking}
\DefineJournalPartialAbbreviation{Dynamic}{Dyn}
\DefineJournalAbbreviation{Dysentery}{Dysent}
\DefineJournalAbbreviation{Dysfunction}{Dysfunct}
\DefineJournalWordException{Dyslexia}{Dyslexia}
\DefineJournalPartialAbbreviation{Dysmorpholog}{Dysmorphol}
\DefineJournalWordException{Dystrophy}{Dystrophy}
\DefineJournalWordException{Eaglehawk}{Eaglehawk}
\DefineJournalWordException{Early}{Early}
\DefineJournalAbbreviation{Earner}{Earn}
\DefineJournalPartialAbbreviation{Earning}{Earn}
\DefineJournalWordException{Earthcare}{Earthcare}
\DefineJournalWordException{Earthlife}{Earthlife}
\DefineJournalWordException{Earthlinks}{Earthlinks}
\DefineJournalAbbreviation{Earthquake}{Earthq}
\DefineJournalWordException{Earthquest}{Earthquest}
\DefineJournalWordException{Earthwatch}{Earthwatch}
\DefineJournalWordException{Earthwise}{Earthwise}
\DefineJournalWordException{Easement}{Easement}
\DefineJournalWordException{East}{East}
\DefineJournalWordException{East Grinstead}{East Grinstead}
\DefineJournalWordException{East-Lansing}{East-Lansing}
\DefineJournalWordException{Eastbourne}{Eastbourne}
\DefineJournalWordException{Eastcoast}{Eastcoast}
\DefineJournalWordException{Easter}{Easter}
\DefineJournalAbbreviation{Eastern}{East}
\DefineJournalAbbreviation{Eastland}{Eastl}
\DefineJournalWordException{Easton}{Easton}
\DefineJournalWordException{Eastwood}{Eastwood}
\DefineJournalWordException{Easyrider}{Easyrider}
\DefineJournalAbbreviation{Eating}{Eat}
\DefineJournalPartialAbbreviation{Eccl\'esiast}{Eccles}
\DefineJournalWordException{Echinoderm}{Echinoderm}
\DefineJournalPartialAbbreviation{Echocardiograph}{Echocardiogr}
\DefineJournalWordException{Eckersley}{Eckersley}
\DefineJournalAbbreviation{Eclectic}{Eclect}
\DefineJournalAbbreviation{Eclipsing}{Eclips}
\DefineJournalAbbreviation{Ecobiology}{Ecobiol}
\DefineJournalPartialAbbreviation{Ecogeograph}{Ecogeogr}
\DefineJournalPartialAbbreviation{Ecohydrolog}{Ecohydrol}
\DefineJournalPartialAbbreviation{Ecolog}{Ecol}
\DefineJournalPartialAbbreviation{Ecomateria}{Ecomater}
\DefineJournalPartialAbbreviation{Econom}{Econ}
\DefineJournalPartialAbbreviation{Ecophysiolog}{Ecophysiol}
\DefineJournalPartialAbbreviation{Ecosystem}{Ecosyst}
\DefineJournalPartialAbbreviation{Ecotextil}{Ecotext}
\DefineJournalAbbreviation{Ecotoxicology}{Ecotoxicol}
\DefineJournalAbbreviation{Ecoturism}{Ecotur}
\DefineJournalPartialAbbreviation{Ecuator}{Ecuat}
\DefineJournalAbbreviation{Ecumenical}{Ecum}
\DefineJournalWordException{Edgemont}{Edgemont}
\DefineJournalWordException{Edible}{Edible}
\DefineJournalAbbreviation{Edinburgh}{Edinb}
\DefineJournalPartialAbbreviation{Edit}{Ed}
\DefineJournalAbbreviation{Editorial}{\'Editor}
\DefineJournalAbbreviation{Edmonton}{Edmont}
\DefineJournalPartialAbbreviation{Educa}{Educ}
\DefineJournalAbbreviation{Educology}{Educol}
\DefineJournalAbbreviation{Edward}{Edw}
\DefineJournalPartialAbbreviation{Effect}{Eff}
\DefineJournalPartialAbbreviation{Efficien}{Effic}
\DefineJournalAbbreviation{Effluent}{Effl}
\DefineJournalAbbreviation{Eganville}{Eganv}
\DefineJournalAbbreviation{Eglinton}{Eglint}
\DefineJournalAbbreviation{Egregious}{Egreg}
\DefineJournalWordException{Egypt}{Egypt}
\DefineJournalAbbreviation{Egyptian}{Egypt}
\DefineJournalAbbreviation{Egyptology}{Egyptol}
%\DefineJournalPartialWordException{Eighteen}{Eighteen-}
\DefineJournalAbbreviation{Eindhoven}{Eindh}
\DefineJournalAbbreviation{Ejector}{Eject}
\DefineJournalAbbreviation{Elasticity}{Elast}
\DefineJournalPartialAbbreviation{Elastohydrodynami}{Elastohydrodyn}
\DefineJournalAbbreviation{Elbow}{Elb}
\DefineJournalWordException{Elderhostel}{Elderhostel}
\DefineJournalAbbreviation{Elderly}{Elder}
\DefineJournalWordException{Eldorado}{Eldorado}
\DefineJournalAbbreviation{Elected}{Elect}
\DefineJournalAbbreviation{Elective}{Elect}
\DefineJournalWordException{Electone}{Electone}
\DefineJournalAbbreviation{Electoral}{Elect}
\DefineJournalPartialAbbreviation{Electric}{Electr}
\DefineJournalPartialAbbreviation{Electroactiv}{Electroact}
\DefineJournalPartialAbbreviation{Electroanaly}{Electroanal}
\DefineJournalPartialAbbreviation{Electroanesthes}{Electroanesth}
\DefineJournalPartialAbbreviation{Electrocardiograph}{Electrocardiogr}
\DefineJournalAbbreviation{Electrocardiology}{Electrocardiol}
\DefineJournalPartialAbbreviation{Electrochem}{Electrochem}
\DefineJournalPartialAbbreviation{Electrochemotherap}{Electrochemother}
\DefineJournalPartialAbbreviation{Electrochromatograph}{Electrochromatogr}
\DefineJournalAbbreviation{Electrocomponent}{Electrocompon}
\DefineJournalAbbreviation{Electrodeposition}{Electrodepos}
\DefineJournalAbbreviation{Electrodepositor}{Electrodepos}
\DefineJournalAbbreviation{Electrodiagnostic}{Electrodiagn}
\DefineJournalPartialAbbreviation{Electrodynami}{Electrodyn}
\DefineJournalPartialAbbreviation{Electroencephalograph}{Electroencephalogr}
\DefineJournalPartialAbbreviation{Electroenerget}{Electroenerg}
\DefineJournalPartialAbbreviation{Electroexplosive}{Electroexplos}
\DefineJournalPartialAbbreviation{Electrogenetherap}{Electrogenether}
\DefineJournalPartialAbbreviation{Electrokineti}{Electrokinet}
\DefineJournalPartialAbbreviation{Electrolog}{Electrol}
\DefineJournalPartialAbbreviation{Electromagneti}{Electromagn}
\DefineJournalWordException{Electromatix}{Electromatix}
\DefineJournalPartialAbbreviation{Electromedic}{\'Electrom\'ed}
\DefineJournalPartialAbbreviation{Electrometallurg}{Electrometall}
\DefineJournalPartialAbbreviation{Electromigrati}{Electromigr}
\DefineJournalPartialAbbreviation{Electromyograph}{Electromyogr}
\DefineJournalWordException{Electron}{Electron}
\DefineJournalPartialAbbreviation{Electroni}{Electron}
\DefineJournalPartialAbbreviation{Electronmicroscop}{Electronmicrosc}
\DefineJournalPartialAbbreviation{Electroorgani}{Electroorg}
\DefineJournalPartialAbbreviation{Electrophore}{Electrophor}
\DefineJournalPartialAbbreviation{Electrophysiolog}{Electrophysiol}
\DefineJournalPartialAbbreviation{Electroplat}{Electroplat}
\DefineJournalAbbreviation{Electrorefining}{Electrorefin}
\DefineJournalPartialAbbreviation{Electrostatic}{Electrost}
\DefineJournalPartialAbbreviation{Electrotechni}{Electrotech}
\DefineJournalPartialAbbreviation{Electrotechnolog}{Electrotechnol}
\DefineJournalPartialAbbreviation{Electrotherap}{Electrother}
\DefineJournalPartialAbbreviation{Electrothermal}{Electrotherm}
\DefineJournalWordException{Electrotyping}{Electrotyping}
\DefineJournalWordException{Elegance}{Elegance}
\DefineJournalPartialAbbreviation{\`Element}{Elem}
\DefineJournalWordException{Elephant}{Elephant}
\DefineJournalAbbreviation{Eligible}{Elig}
\DefineJournalPartialAbbreviation{Elimin}{\'Elimin}
\DefineJournalPartialAbbreviation{Elizabeth}{Elizab}
\DefineJournalAbbreviation{Elizabethan}{Elizab}
\DefineJournalWordException{Elmadale}{Elmadale}
\DefineJournalAbbreviation{Elmbridge}{Elmb}
\DefineJournalWordException{Elmvale}{Elmvale}
\DefineJournalAbbreviation{Elmwood}{Elmw}
\DefineJournalAbbreviation{Elusive}{Elus}
\DefineJournalPartialAbbreviation{Emancip}{Emancip}
\DefineJournalWordException{Embassy}{Embassy}
\DefineJournalPartialAbbreviation{Embed}{Embed}
\DefineJournalAbbreviation{Emblem}{Embl}
\DefineJournalAbbreviation{Embracing}{Embrac}
\DefineJournalWordException{Embroidery}{Embroidery}
\DefineJournalWordException{Emerald}{Emerald}
\DefineJournalAbbreviation{Emergency}{Emerg}
\DefineJournalAbbreviation{Emerging}{Emerg}
\DefineJournalAbbreviation{Emeryville}{Emeryv}
\DefineJournalPartialAbbreviation{Emirat}{Emir}
\DefineJournalPartialAbbreviation{Emission}{Emiss}
\DefineJournalPartialAbbreviation{Emit}{Emit}
\DefineJournalAbbreviation{Emolument}{Emol}
\DefineJournalWordException{Emory}{Emory}
\DefineJournalPartialAbbreviation{Emotion}{Emot}
\DefineJournalAbbreviation{Empathic}{Empath}
\DefineJournalAbbreviation{Emphasis}{Emphas}
\DefineJournalWordException{Emphysema}{Emphysema}
\DefineJournalAbbreviation{Empire}{Emp}
\DefineJournalAbbreviation{Empirical}{Empir}
\DefineJournalAbbreviation{Employability}{Employab}
\DefineJournalAbbreviation{Employed}{Employ}
\DefineJournalAbbreviation{Employee}{Empl}
\DefineJournalAbbreviation{Employer}{Empl}
\DefineJournalAbbreviation{Employment}{Employ}
\DefineJournalPartialAbbreviation{Empower}{Empower}
\DefineJournalAbbreviation{Empowering}{Empower}
\DefineJournalWordException{Empress}{Empress}
\DefineJournalWordException{Emptor}{Emptor}
\DefineJournalAbbreviation{Enactment}{Enactm}
\DefineJournalAbbreviation{Enamelist}{Enamel}
\DefineJournalAbbreviation{Enamelling}{Enamel}
\DefineJournalPartialAbbreviation{Encamp}{Encamp}
\DefineJournalPartialAbbreviation{Enceph}{Enceph}
\DefineJournalWordException{Enchytraeidae}{Enchytraeidae}
\DefineJournalAbbreviation{Enclosure}{Enclos}
\DefineJournalPartialAbbreviation{Encount}{Encount}
\DefineJournalPartialAbbreviation{Encyclop}{Encycl}
\DefineJournalAbbreviation{Endangered}{Endanger}
\DefineJournalWordException{Endeavor}{Endeavor}
\DefineJournalPartialAbbreviation{Endeavour}{Endeav}
\DefineJournalAbbreviation{Ended}{End}
\DefineJournalAbbreviation{Ending}{End}
\DefineJournalWordException{Endless}{Endless}
\DefineJournalAbbreviation{Endocrine}{Endocr}
\DefineJournalPartialAbbreviation{Endocrinolog}{Endocrinol}
\DefineJournalAbbreviation{Endocrinopathy}{Endocrinopat}
\DefineJournalPartialAbbreviation{Endocytobiolog}{Endocytobiol}
\DefineJournalWordException{Endocytobiosis}{Endocytobiosis}
\DefineJournalPartialAbbreviation{Endodontic}{Endod}
\DefineJournalAbbreviation{Endometriosis}{Endometr}
\DefineJournalPartialAbbreviation{Endoscop}{Endosc}
\DefineJournalWordException{Endotoxin}{Endotoxin}
\DefineJournalAbbreviation{Endowment}{Endow}
\DefineJournalAbbreviation{Energistic}{Energ}
\DefineJournalPartialAbbreviation{Energochemic}{Energochem}
\DefineJournalWordException{Energy}{Energy}
\DefineJournalWordException{Enersave}{Enersave}
\DefineJournalWordException{Enfield}{Enfield}
\DefineJournalWordException{Enfoque}{Enfoque}
\DefineJournalAbbreviation{Enforcement}{Enforc}
\DefineJournalAbbreviation{Enforcer}{Enforc}
\DefineJournalAbbreviation{Enforcing}{Enforc}
\DefineJournalWordException{Engaged}{Engaged}
\DefineJournalAbbreviation{Engagement}{Engagem}
\DefineJournalWordException{Engine}{Engine}
\DefineJournalPartialAbbreviation{Engineer}{Eng}
\DefineJournalAbbreviation{England}{Engl}
\DefineJournalWordException{Englander}{Englander}
\DefineJournalWordException{Englewood}{Englewood}
\DefineJournalAbbreviation{English}{Engl}
\DefineJournalAbbreviation{Engraver}{Engrav}
\DefineJournalAbbreviation{Engraving}{Engrav}
\DefineJournalPartialAbbreviation{Enhance}{Enhanc}
\DefineJournalPartialAbbreviation{Enlarg}{Enlarg}
\DefineJournalAbbreviation{Enlightened}{Enlight}
\DefineJournalAbbreviation{Enlightenment}{Enlight}
\DefineJournalAbbreviation{Enneagram}{Enneagr}
\DefineJournalWordException{Ennugu}{Ennugu}
\DefineJournalPartialAbbreviation{Enquir}{Enq}
\DefineJournalAbbreviation{Enrichment}{Enrich}
\DefineJournalAbbreviation{Enrolled}{Enroll}
\DefineJournalAbbreviation{Enrollment}{Enroll}
\DefineJournalAbbreviation{Enrolment}{Enrol}
\DefineJournalWordException{Ensearch}{Ensearch}
\DefineJournalWordException{Ensign}{Ensign}
\DefineJournalAbbreviation{Enteral}{Enter}
\DefineJournalWordException{Enteric}{Enteric}
\DefineJournalWordException{Enterie}{Enterie}
\DefineJournalAbbreviation{Entering}{Enter}
\DefineJournalPartialAbbreviation{Enterobacteri}{Enterobact}
\DefineJournalAbbreviation{Enterostomal}{Enteros}
\DefineJournalWordException{Enterovirus}{Enterovirus}
\DefineJournalAbbreviation{Enterpreneur}{Enterp}
\DefineJournalPartialAbbreviation{Enterprise}{Enterp}
\DefineJournalPartialAbbreviation{Entertain}{Entertain}
\DefineJournalAbbreviation{Enthusiast}{Enthus}
\DefineJournalWordException{Entitled}{Entitled}
\DefineJournalWordException{Entity}{Entity}
\DefineJournalWordException{Entoma}{Entoma}
\DefineJournalWordException{Entomofaune}{Entomofaune}
\DefineJournalPartialAbbreviation{Entomopathogen}{Entomopathog}
\DefineJournalWordException{Entopath}{Entopath}
\DefineJournalAbbreviation{Entrance}{Entr}
\DefineJournalAbbreviation{Entrophication}{Entroph}
\DefineJournalPartialAbbreviation{Entrust}{Entrust}
\DefineJournalWordException{Entry}{Entry}
\DefineJournalAbbreviation{Enumeration}{Enumer}
\DefineJournalAbbreviation{Enumerative}{Enumer}
\DefineJournalPartialAbbreviation{Enviroanaly}{Enviroanal}
\DefineJournalWordException{Envirofact}{Envirofact}
\DefineJournalPartialAbbreviation{Environment}{Environ}
\DefineJournalAbbreviation{Envision}{Envis}
\DefineJournalAbbreviation{Enwisdomization}{Enwisdomiz}
\DefineJournalPartialAbbreviation{Enzym}{Enzym}
\DefineJournalPartialAbbreviation{Enzymochem}{Enzymochem}
\DefineJournalPartialAbbreviation{Ephemer}{Ephemer}
\DefineJournalWordException{Ephesus}{Ephesus}
\DefineJournalPartialAbbreviation{Epicur}{Epicur}
\DefineJournalWordException{Epilepsy}{Epilepsy}
\DefineJournalPartialAbbreviation{Epileptogen}{Epileptog}
\DefineJournalPartialAbbreviation{Epioptic}{Epiopt}
\DefineJournalAbbreviation{Episcopal}{Episcop}
\DefineJournalWordException{Epistle}{Epistle}
\DefineJournalAbbreviation{Epithelial}{Epithel}
\DefineJournalAbbreviation{Eponymist}{Eponym}
\DefineJournalPartialAbbreviation{Equal}{Equal}
\DefineJournalAbbreviation{Equation}{Equ}
\DefineJournalPartialAbbreviation{Equator}{Equat}
\DefineJournalAbbreviation{Equestrian}{Equest}
\DefineJournalAbbreviation{Equilibrium}{Equilib}
\DefineJournalWordException{Equine}{Equine}
\DefineJournalAbbreviation{Equipment}{Equip}
\DefineJournalWordException{\'Equitable}{\'Equitable}
\DefineJournalWordException{Equity}{Equity}
\DefineJournalPartialAbbreviation{\'Equivalen}{Equiv}
\DefineJournalAbbreviation{Eradication}{Erad}
\DefineJournalAbbreviation{Ergodic}{Ergod}
\DefineJournalAbbreviation{Ergology}{Ergol}
\DefineJournalWordException{Erindale}{Erindale}
\DefineJournalWordException{Eritrean}{Eritrean}
\DefineJournalWordException{Ermington}{Ermington}
\DefineJournalAbbreviation{Erosion}{Eros}
\DefineJournalAbbreviation{Erotic}{Erot}
\DefineJournalPartialAbbreviation{Erudit}{Erud}
\DefineJournalAbbreviation{Eruption}{Erupt}
\DefineJournalAbbreviation{Erythropoiesis}{Erythrop}
\DefineJournalPartialAbbreviation{Escalat}{Escalat}
\DefineJournalWordException{Escape}{Escape}
\DefineJournalAbbreviation{Escarpment}{Escarpm}
\DefineJournalWordException{Eskimo}{Eskimo}
\DefineJournalWordException{Esophagus}{Esophagus}
\DefineJournalAbbreviation{Espionage}{Espion}
\DefineJournalWordException{Espirit}{Espirit}
\DefineJournalWordException{Esquimalt}{Esquimalt}
\DefineJournalWordException{Esquire}{Esquire}
\DefineJournalWordException{Essay}{Essay}
\DefineJournalAbbreviation{Essential}{Essent}
\DefineJournalWordException{Estate}{Estate}
\DefineJournalPartialAbbreviation{Estimat}{Estim}
\DefineJournalAbbreviation{Estuarine}{Estuar}
\DefineJournalWordException{Estuary}{Estuary}
\DefineJournalAbbreviation{Etching}{Etch}
\DefineJournalWordException{Eternal}{Eternal}
\DefineJournalWordException{Eternity}{Eternity}
%\DefineJournalPartialWordException{Ethic}{Ethic-}
\DefineJournalPartialAbbreviation{Ethiopi}{Ethiop}
\DefineJournalPartialAbbreviation{Ethni}{Ethn}
\DefineJournalAbbreviation{Ethnoarchaeology}{Ethnoarchaeol}
\DefineJournalPartialAbbreviation{Ethnoastronom}{Ethnoastron}
\DefineJournalPartialAbbreviation{Ethnobiolog}{Ethnobiol}
\DefineJournalPartialAbbreviation{Ethnobotan}{Ethnobot}
\DefineJournalPartialAbbreviation{Ethnocultur}{Ethnocult}
\DefineJournalAbbreviation{Ethnohistory}{Ethnohist}
\DefineJournalPartialAbbreviation{Ethnopharmacolog}{Ethnopharmacol}
\DefineJournalAbbreviation{Ethologist}{Ethol}
\DefineJournalAbbreviation{Ethology}{Ethol}
\DefineJournalAbbreviation{Ethylene}{Ethyl}
\DefineJournalWordException{Etobicoke}{Etobicoke}
\DefineJournalPartialAbbreviation{Eugenic}{Eugen}
\DefineJournalAbbreviation{Eukaryotic}{Eukaryot}
\DefineJournalAbbreviation{Euraccount}{Euracc}
\DefineJournalAbbreviation{Euroanalysis}{Euroanal}
\DefineJournalAbbreviation{Eurocurrency}{Eurocurr}
\DefineJournalWordException{Eurolaser}{Eurolaser}
\DefineJournalWordException{Euromeat}{Euromeat}
\DefineJournalWordException{Euromoney}{Euromoney}
\DefineJournalWordException{Euromonies}{Euromonies}
\DefineJournalPartialAbbreviation{Europhysic}{Europhys}
\DefineJournalPartialAbbreviation{Europlastic}{Europlast}
\DefineJournalWordException{Europort}{Europort}
\DefineJournalAbbreviation{Euroscope}{Eurosc}
\DefineJournalWordException{Eurostore}{Eurostore}
\DefineJournalAbbreviation{Eurotechnic}{Eurotech}
\DefineJournalWordException{Eurotrends}{Eurotrends}
\DefineJournalAbbreviation{Evacuee}{Evac}
\DefineJournalPartialAbbreviation{\'Evaluat}{Eval}
\DefineJournalAbbreviation{Evanston}{Evanst}
\DefineJournalWordException{Evaporite}{Evaporite}
\DefineJournalWordException{Evening}{Evening}
\DefineJournalWordException{Event}{Event}
\DefineJournalAbbreviation{Eventor}{Event}
\DefineJournalWordException{Everett}{Everett}
\DefineJournalAbbreviation{Evergreen}{Evergr}
\DefineJournalWordException{Everlasting}{Everlasting}
\DefineJournalWordException{Everybody}{Everybody}
\DefineJournalWordException{Everyday}{Everyday}
\DefineJournalWordException{Everyman}{Everyman}
\DefineJournalWordException{Everyone}{Everyone}
\DefineJournalWordException{Everything}{Everything}
\DefineJournalAbbreviation{Evidence}{\'Evid}
\DefineJournalWordException{Evoked}{Evoked}
\DefineJournalPartialAbbreviation{Evolut}{Evol}
\DefineJournalAbbreviation{Evolving}{Evol}
\DefineJournalPartialAbbreviation{Examination}{Exam}
\DefineJournalPartialAbbreviation{Examiner}{Exam}
\DefineJournalAbbreviation{Example}{Ex}
\DefineJournalPartialAbbreviation{Excavat}{Excav}
\DefineJournalPartialAbbreviation{Exceed}{Exceed}
\DefineJournalPartialAbbreviation{Excell}{Excell}
\DefineJournalPartialAbbreviation{Exchange}{Exch}
\DefineJournalWordException{Exchequer}{Exchequer}
\DefineJournalWordException{Excise}{Excise}
\DefineJournalPartialAbbreviation{Excit}{Excit}
\DefineJournalPartialAbbreviation{Exclud}{Exclud}
\DefineJournalWordException{Excursion}{Excursion}
\DefineJournalPartialAbbreviation{Ex\'ecut}{Exec}
\DefineJournalAbbreviation{Exegesis}{Exeg}
\DefineJournalWordException{Exempt}{Exempt}
\DefineJournalAbbreviation{Exemption}{Exempt}
\DefineJournalPartialAbbreviation{Exerc}{Exerc}
\DefineJournalWordException{Exeter}{Exeter}
\DefineJournalWordException{Exhaust}{Exhaust}
\DefineJournalPartialAbbreviation{Exhibit}{Exhib}
\DefineJournalPartialAbbreviation{Exhum}{Exhum}
\DefineJournalPartialAbbreviation{Existential}{Existent}
\DefineJournalPartialAbbreviation{Exobiolog}{Exobiol}
\DefineJournalPartialAbbreviation{Exogen}{Exog}
\DefineJournalWordException{Exogram}{Exogram}
\DefineJournalPartialAbbreviation{Exoti}{Exot}
\DefineJournalPartialAbbreviation{Expand}{Expand}
\DefineJournalAbbreviation{Expected}{Expect}
\DefineJournalPartialAbbreviation{Expedition}{Exped}
\DefineJournalPartialAbbreviation{Expenditure}{Expend}
\DefineJournalPartialAbbreviation{Expens}{Expens}
\DefineJournalPartialAbbreviation{Experien}{Exp}
\DefineJournalPartialAbbreviation{Experiment}{Exp}
\DefineJournalPartialAbbreviation{Explain}{Explain}
\DefineJournalPartialAbbreviation{Explanat}{Explan}
\DefineJournalAbbreviation{Exploding}{Explod}
\DefineJournalPartialAbbreviation{Explor}{Explor}
\DefineJournalPartialAbbreviation{Explosi}{Explos}
\DefineJournalAbbreviation{Exponent}{Expon}
\DefineJournalPartialAbbreviation{Export}{Export}
\DefineJournalPartialAbbreviation{Expos}{Expo}
\DefineJournalWordException{Express}{Express}
\DefineJournalAbbreviation{Expression}{Expr}
\DefineJournalAbbreviation{Expressletter}{Expresslett}
\DefineJournalAbbreviation{Extended}{Ext}
\DefineJournalAbbreviation{Extender}{Ext}
\DefineJournalAbbreviation{Extension}{Ext}
\DefineJournalPartialAbbreviation{Exterminat}{Exterm}
\DefineJournalAbbreviation{External}{Extern}
\DefineJournalAbbreviation{Extra-licentiate}{Extra-licent}
\DefineJournalAbbreviation{Extracellular}{Extracell}
\DefineJournalAbbreviation{Extracorporeal}{Extracorpor}
\DefineJournalPartialAbbreviation{Extract}{Extr}
\DefineJournalPartialAbbreviation{Extramur}{Extramur}
\DefineJournalWordException{Extranea}{Extranea}
\DefineJournalWordException{Extraordinary}{Extraordinary}
\DefineJournalPartialAbbreviation{Extrapulmonar}{Extrapulm}
\DefineJournalPartialAbbreviation{Extraterrestr}{Extraterr}
\DefineJournalPartialAbbreviation{Extr\^em}{Extrem}
\DefineJournalAbbreviation{Extruding}{Extrud}
\DefineJournalPartialAbbreviation{Extrus}{Extrus}
\DefineJournalWordException{Eyecare}{Eyecare}
\DefineJournalPartialAbbreviation{Fabric}{Fabr}
\DefineJournalWordException{Fabulous}{Fabulous}
\DefineJournalPartialAbbreviation{Facilit}{Facil}
\DefineJournalAbbreviation{Facsimile}{Facsim}
\DefineJournalAbbreviation{Fact-book}{Fact-b}
\DefineJournalAbbreviation{Factbook}{Factb}
\DefineJournalWordException{Factfile}{Factfile}
\DefineJournalWordException{Factfinder}{Factfinder}
\DefineJournalWordException{Faction}{Faction}
\DefineJournalWordException{Factor}{Factor}
\DefineJournalWordException{Factoriel}{Factoriel}
\DefineJournalAbbreviation{Factoring}{Factor}
\DefineJournalAbbreviation{Factory}{Fact}
\DefineJournalWordException{Factsheet}{Factsheet}
\DefineJournalWordException{Factual}{Factual}
\DefineJournalPartialAbbreviation{Facult}{Fac}
\DefineJournalPartialAbbreviation{Fail}{Fail}
\DefineJournalAbbreviation{Failing}{Fail}
\DefineJournalAbbreviation{Failure}{Fail}
\DefineJournalWordException{Fairbanks}{Fairbanks}
\DefineJournalWordException{Fairbase}{Fairbase}
\DefineJournalWordException{Fairchild}{Fairchild}
\DefineJournalWordException{Fairfax}{Fairfax}
\DefineJournalAbbreviation{Fairfield}{Fairfld}
\DefineJournalWordException{Fairnes}{Fairnes}
\DefineJournalWordException{Fairplay}{Fairplay}
\DefineJournalAbbreviation{Fairway}{Fairw}
\DefineJournalWordException{Faith}{Faith}
\DefineJournalAbbreviation{Faithfully}{Faithf}
\DefineJournalWordException{Falcon}{Falcon}
\DefineJournalAbbreviation{Falkland}{Falkl}
\DefineJournalWordException{Fallbrook}{Fallbrook}
\DefineJournalWordException{Falls-Church}{Falls-Church}
\DefineJournalWordException{False Creek}{False Creek}
\DefineJournalPartialAbbreviation{Falsification}{Falsif}
\DefineJournalPartialAbbreviation{Famil}{Fam}
\DefineJournalWordException{Famous}{Famous}
\DefineJournalWordException{Fancier}{Fancier}
\DefineJournalWordException{Fancy}{Fancy}
\DefineJournalWordException{Fandhome}{Fandhome}
\DefineJournalWordException{Fantasy}{Fantasy}
\DefineJournalWordException{Fanzine}{Fanzine}
\DefineJournalWordException{Faraday}{Faraday}
\DefineJournalWordException{Farano}{Farano}
\DefineJournalWordException{Farm}{Farm}
\DefineJournalWordException{Farmer}{Farmer}
\DefineJournalAbbreviation{Farmersville}{Farmersv}
\DefineJournalWordException{Farmgate}{Farmgate}
\DefineJournalWordException{Farmhouse}{Farmhouse}
\DefineJournalWordException{Farming}{Farming}
\DefineJournalAbbreviation{Farmingdale}{Farmingd}
\DefineJournalAbbreviation{Farmland}{Farml}
\DefineJournalWordException{Farmstart}{Farmstart}
\DefineJournalAbbreviation{Farmstead}{Farmst}
\DefineJournalWordException{Farmways}{Farmways}
\DefineJournalAbbreviation{Farmwork}{Farmw}
\DefineJournalAbbreviation{Farnborough}{Farnb}
\DefineJournalWordException{Farnham}{Farnham}
\DefineJournalWordException{Faroes}{Faroes}
\DefineJournalWordException{Farriery}{Farriery}
\DefineJournalPartialAbbreviation{Fascicul}{Fasc}
\DefineJournalPartialAbbreviation{Fashion}{Fash}
\DefineJournalWordException{Fast-alert}{Fast-alert}
\DefineJournalPartialAbbreviation{Fasten}{Fasten}
\DefineJournalAbbreviation{Fastmoving}{Fastmov}
\DefineJournalAbbreviation{Fatality}{Fatal}
\DefineJournalPartialAbbreviation{Father}{Father}
\DefineJournalAbbreviation{Fatty}{Fat}
\DefineJournalPartialAbbreviation{Favor}{Favor}
\DefineJournalAbbreviation{Fayetteville}{Fayettev}
\DefineJournalWordException{Fazeley}{Fazeley}
\DefineJournalWordException{Feather}{Feather}
\DefineJournalAbbreviation{Feathered}{Feather}
\DefineJournalPartialAbbreviation{Featur}{Featur}
\DefineJournalWordException{Feature}{Feature}
\DefineJournalAbbreviation{February}{Febr}
\DefineJournalPartialAbbreviation{Federa}{Fed}
\DefineJournalAbbreviation{Feeble}{Feeb}
\DefineJournalPartialAbbreviation{Feed}{Feed}
\DefineJournalWordException{Feedback}{Feedback}
\DefineJournalAbbreviation{Feedingstuff}{Feedingst}
\DefineJournalWordException{Feedlot}{Feedlot}
\DefineJournalWordException{Feedstock}{Feedstock}
\DefineJournalWordException{Feedstuff}{Feedstuff}
\DefineJournalPartialAbbreviation{Feel}{Feel}
\DefineJournalWordException{Feldspar}{Feldspar}
\DefineJournalWordException{Feline}{Feline}
\DefineJournalWordException{Fellmonger}{Fellmonger}
\DefineJournalWordException{Fellow}{Fellow}
\DefineJournalAbbreviation{Fellowship}{Fellowsh}
\DefineJournalWordException{Female}{Female}
\DefineJournalWordException{Fencible}{Fencible}
\DefineJournalAbbreviation{Fencing}{Fenc}
\DefineJournalAbbreviation{Fenland}{Fenl}
\DefineJournalPartialAbbreviation{Fermenta}{Ferment}
\DefineJournalWordException{Ferozepur}{Ferozepur}
%\DefineJournalPartialWordException{Ferrier}{Ferrier-}
\DefineJournalWordException{Ferring}{Ferring}
\DefineJournalAbbreviation{Ferrocement}{Ferrocem}
\DefineJournalPartialAbbreviation{Ferroelectri}{Ferroelectr}
\DefineJournalPartialAbbreviation{Ferromagneti}{Ferromagn}
\DefineJournalAbbreviation{Ferrous}{Ferr}
\DefineJournalAbbreviation{Festival}{Festiv}
\DefineJournalWordException{Festive}{Festive}
\DefineJournalWordException{Fetal}{Fetal}
\DefineJournalWordException{Fever}{Fever}
\DefineJournalWordException{Ffestiniog}{Ffestiniog}
\DefineJournalWordException{Fiber}{Fiber}
\DefineJournalWordException{Fibrinolysis}{Fibrinolysis}
\DefineJournalAbbreviation{Fibrosis}{Fibros}
\DefineJournalWordException{Fibrous}{Fibrous}
\DefineJournalWordException{Fiddler}{Fiddler}
\DefineJournalAbbreviation{Fidelity}{Fidel}
\DefineJournalWordException{Field}{Field}
\DefineJournalWordException{Fieldiana}{Fieldiana}
\DefineJournalAbbreviation{Fieldman}{Fieldm}
\DefineJournalWordException{Fieldnote}{Fieldnote}
\DefineJournalPartialAbbreviation{Fieldsport}{Fieldsp}
\DefineJournalWordException{Fieldwork}{Fieldwork}
%\DefineJournalPartialWordException{Fifteen}{Fifteen-}
\DefineJournalPartialAbbreviation{Fight}{Fight}
\DefineJournalWordException{Filariasis}{Filariasis}
\DefineJournalWordException{Filbert}{Filbert}
\DefineJournalAbbreviation{Filebook}{Fileb}
\DefineJournalPartialAbbreviation{Filial}{Fil}
\DefineJournalWordException{Filing}{Filing}
\DefineJournalPartialAbbreviation{Fill}{Fill}
\DefineJournalAbbreviation{Filmfestival}{Filmfestiv}
\DefineJournalPartialAbbreviation{Filmmak}{Filmmak}
\DefineJournalAbbreviation{Filmstrip}{Filmstr}
\DefineJournalWordException{Filter}{Filter}
\DefineJournalAbbreviation{Filtering}{Filter}
\DefineJournalPartialAbbreviation{Filtrat}{Filtr}
\DefineJournalPartialAbbreviation{Final}{Final}
\DefineJournalWordException{Finder}{Finder}
\DefineJournalPartialAbbreviation{Finding}{Find}
\DefineJournalWordException{Finescale}{Finescale}
\DefineJournalWordException{Finest}{Finest}
\DefineJournalWordException{Finger}{Finger}
\DefineJournalAbbreviation{Fingerprint}{Fingerpr}
\DefineJournalWordException{Fingertip}{Fingertip}
\DefineJournalPartialAbbreviation{Finish}{Finish}
\DefineJournalAbbreviation{Finisher}{Finish}
\DefineJournalAbbreviation{Finishes}{Finish}
\DefineJournalAbbreviation{Finishing}{Finish}
\DefineJournalWordException{Finite}{Finite}
\DefineJournalAbbreviation{Finksburg}{Finksbg}
\DefineJournalPartialAbbreviation{Finland}{Finl}
\DefineJournalPartialAbbreviation{Finni}{Finn}
\DefineJournalPartialAbbreviation{Finnland}{Finnl}
\DefineJournalAbbreviation{Fiordland}{Fiordl}
%\DefineJournalPartialWordException{Firearm}{Firearm-}
\DefineJournalAbbreviation{Firefighter}{Firef}
\DefineJournalAbbreviation{Firefighting}{Firef}
\DefineJournalPartialAbbreviation{Firehous}{Firehous}
\DefineJournalWordException{Fireman}{Fireman}
\DefineJournalAbbreviation{Fireplace}{Firepl}
\DefineJournalWordException{Fireside}{Fireside}
\DefineJournalAbbreviation{Fireworks}{Firew}
\DefineJournalWordException{Fishbyte}{Fishbyte}
\DefineJournalPartialAbbreviation{Fisher}{Fish}
\DefineJournalWordException{Fisherman}{Fisherman}
\DefineJournalAbbreviation{Fishing}{Fish}
\DefineJournalAbbreviation{Fishkeeping}{Fishkeep}
\DefineJournalWordException{Fistula}{Fistula}
\DefineJournalAbbreviation{Fitness}{Fit}
\DefineJournalAbbreviation{Fittingly}{Fitt}
\DefineJournalAbbreviation{Fittings}{Fitt}
\DefineJournalWordException{Fitzroy}{Fitzroy}
\DefineJournalAbbreviation{Fixture}{Fixt}
\DefineJournalWordException{Flagship}{Flagship}
\DefineJournalWordException{Flamborough}{Flamborough}
\DefineJournalAbbreviation{Flaming}{Flam}
\DefineJournalWordException{Flamingo}{Flamingo}
\DefineJournalAbbreviation{Flammability}{Flammabl}
\DefineJournalWordException{Flammesafe}{Flammesafe}
\DefineJournalWordException{Flander}{Flander}
\DefineJournalWordException{Flashpoint}{Flashpoint}
\DefineJournalWordException{Flavor}{Flavor}
\DefineJournalPartialAbbreviation{Flavordynami}{Flavordyn}
\DefineJournalAbbreviation{Flavoring}{Flavor}
\DefineJournalWordException{Flavour}{Flavour}
\DefineJournalAbbreviation{Flavouring}{Flavour}
\DefineJournalAbbreviation{Flemish}{Flem}
\DefineJournalPartialAbbreviation{Fleuropolymer}{Fleuropolym}
\DefineJournalAbbreviation{Flexibility}{Flex}
\DefineJournalWordException{Flight}{Flight}
\DefineJournalWordException{Flintstone}{Flintstone}
\DefineJournalPartialAbbreviation{Flip}{Flip}
\DefineJournalAbbreviation{Floating}{Float}
\DefineJournalWordException{Floor}{Floor}
\DefineJournalAbbreviation{Floorcovering}{Floorcover}
\DefineJournalAbbreviation{Flooring}{Floor}
\DefineJournalAbbreviation{Floorspace}{Floorsp}
\DefineJournalPartialAbbreviation{Floral}{Flor}
\DefineJournalPartialAbbreviation{Floricult}{Floric}
\DefineJournalAbbreviation{Florida}{Fla}
\DefineJournalAbbreviation{Florist}{Flor}
\DefineJournalPartialAbbreviation{Floristic}{Florist}
\DefineJournalAbbreviation{Floristry}{Flor}
\DefineJournalAbbreviation{Flotation}{Flotat}
\DefineJournalWordException{Flotilla}{Flotilla}
\DefineJournalWordException{Flourspar}{Flourspar}
\DefineJournalWordException{Flower}{Flower}
\DefineJournalAbbreviation{Flowering}{Flower}
\DefineJournalAbbreviation{Flowing}{Flow}
\DefineJournalAbbreviation{Fluency}{Fluen}
\DefineJournalWordException{Fluid}{Fluid}
\DefineJournalPartialAbbreviation{Fluiddynami}{Fluiddyn}
\DefineJournalPartialAbbreviation{Fluidic}{Fluid}
\DefineJournalPartialAbbreviation{Fluidiz}{Fluid}
\DefineJournalPartialAbbreviation{Fluorat}{Fluorat}
\DefineJournalPartialAbbreviation{Fluorescen}{Fluoresc}
\DefineJournalAbbreviation{Fluoridation}{Fluorid}
\DefineJournalWordException{Fluoride}{Fluoride}
\DefineJournalPartialAbbreviation{Fluorimetr}{Fluorim}
\DefineJournalAbbreviation{Fluorine}{Fluor}
\DefineJournalWordException{Fluorocarbon}{Fluorocarbon}
\DefineJournalWordException{Flush}{Flush}
\DefineJournalAbbreviation{Flyer}{Fly}
\DefineJournalAbbreviation{Flyfisher}{Flyfish}
\DefineJournalAbbreviation{Flying}{Fly}
\DefineJournalAbbreviation{Flypast}{Flyp}
\DefineJournalPartialAbbreviation{Foam}{Foam}
\DefineJournalWordException{Focus}{Focus}
\DefineJournalPartialAbbreviation{Focus}{Focus}
\DefineJournalAbbreviation{Fodder}{Fodd}
\DefineJournalWordException{Foetal}{Foetal}
\DefineJournalAbbreviation{Folding}{Fold}
\DefineJournalWordException{Foliage}{Foliage}
\DefineJournalWordException{Folkestone}{Folkestone}
\DefineJournalWordException{Folklife}{Folklife}
\DefineJournalWordException{Folksound}{Folksound}
\DefineJournalWordException{Folktale}{Folktale}
\DefineJournalWordException{Folkwang}{Folkwang}
\DefineJournalAbbreviation{Folkweave}{Folkw}
\DefineJournalPartialAbbreviation{Follow}{Follow}
\DefineJournalWordException{Food}{Food}
\DefineJournalWordException{Foodborne}{Foodborne}
\DefineJournalAbbreviation{Foodbroker}{Foodbrok}
\DefineJournalAbbreviation{Foodcrop}{Foodcr}
\DefineJournalWordException{Foodlink}{Foodlink}
\DefineJournalAbbreviation{Foodprocessing}{Foodprocess}
\DefineJournalAbbreviation{Foodservice}{Foodserv}
\DefineJournalPartialAbbreviation{Foodstuff}{Foodst}
\DefineJournalWordException{Foodweek}{Foodweek}
\DefineJournalAbbreviation{Football}{Footb}
\DefineJournalAbbreviation{Footballer}{Footb}
\DefineJournalWordException{Foothills}{Foothills}
\DefineJournalWordException{Footnote}{Footnote}
\DefineJournalWordException{Footpath}{Footpath}
\DefineJournalAbbreviation{Footprint}{Footpr}
\DefineJournalWordException{Footstep}{Footstep}
\DefineJournalWordException{Footwear}{Footwear}
\DefineJournalWordException{Forage}{Forage}
\DefineJournalAbbreviation{Foraminiferal}{Foraminifer}
\DefineJournalAbbreviation{Forbidden}{Forbid}
\DefineJournalWordException{Forcep}{Forcep}
\DefineJournalPartialAbbreviation{Forecast}{Forecast}
\DefineJournalPartialAbbreviation{Foreclos}{Foreclos}
\DefineJournalAbbreviation{Foreclosure}{Foreclos}
\DefineJournalWordException{Forecourt}{Forecourt}
\DefineJournalAbbreviation{Forefront}{Forefr}
\DefineJournalAbbreviation{Forehead}{Foreh}
\DefineJournalWordException{Foreign}{Foreign}
\DefineJournalWordException{Forensic}{Forensic}
\DefineJournalAbbreviation{Forerunner}{Forerunn}
\DefineJournalAbbreviation{Foreshore}{Foresh}
\DefineJournalWordException{Foresight}{Foresight}
\DefineJournalPartialAbbreviation{Forest}{For}
\DefineJournalWordException{Forever}{Forever}
\DefineJournalPartialAbbreviation{Forger}{Forg}
\DefineJournalPartialAbbreviation{Forging}{Forg}
\DefineJournalAbbreviation{Forgotten}{Forgot}
\DefineJournalWordException{Forintek}{Forintek}
\DefineJournalWordException{Formaldehyde}{Formaldehyde}
\DefineJournalPartialAbbreviation{Formaliz}{Formaliz}
\DefineJournalPartialAbbreviation{Formati}{Form}
\DefineJournalAbbreviation{Formed}{Form}
\DefineJournalWordException{Former}{Former}
\DefineJournalAbbreviation{Formerly}{Former}
\DefineJournalAbbreviation{Forming}{Form}
\DefineJournalAbbreviation{Formosan}{Formos}
\DefineJournalWordException{Formula}{Formula}
\DefineJournalPartialAbbreviation{Forshort}{Forshort}
\DefineJournalAbbreviation{Fort Langley}{Ft Langley}
\DefineJournalAbbreviation{Fort Lauderdale}{Ft Lauderdale}
\DefineJournalAbbreviation{Fort McClellan}{Ft McClell}
\DefineJournalAbbreviation{Fort Tryon Park}{Ft Tryon Park}
\DefineJournalAbbreviation{Fort Worth}{Ft Worth}
\DefineJournalWordException{Fort-McMurray}{Fort-McMurray}
\DefineJournalWordException{Fortepiano}{Fortepiano}
\DefineJournalAbbreviation{Forthcoming}{Forthcom}
\DefineJournalAbbreviation{Fortnightly}{Fortn}
\DefineJournalWordException{Fortran}{Fortran}
\DefineJournalWordException{Fortress}{Fortress}
\DefineJournalWordException{Fortune}{Fortune}
\DefineJournalWordException{Forum}{Forum}
\DefineJournalAbbreviation{Forward}{Forw}
\DefineJournalAbbreviation{Forwarder}{Forw}
\DefineJournalWordException{Forwood}{Forwood}
\DefineJournalWordException{Fossicker}{Fossicker}
\DefineJournalPartialAbbreviation{Foster}{Foster}
\DefineJournalPartialAbbreviation{Foundation}{Found}
\DefineJournalAbbreviation{Founder}{Found}
\DefineJournalAbbreviation{Founding}{Found}
\DefineJournalWordException{Foundry}{Foundry}
\DefineJournalAbbreviation{Foundryman}{Foundrym}
\DefineJournalWordException{Fountain}{Fountain}
\DefineJournalWordException{Fourth}{Fourth}
\DefineJournalWordException{Fractal}{Fractal}
\DefineJournalAbbreviation{Fractional}{Fract}
\DefineJournalPartialAbbreviation{Fractur}{Fract}
\DefineJournalPartialAbbreviation{Fragment}{Fragm}
\DefineJournalAbbreviation{Fragrance}{Fragr}
\DefineJournalPartialAbbreviation{Fram}{Fram}
\DefineJournalWordException{Frame-work}{Frame-work}
\DefineJournalAbbreviation{Framework}{Framew}
\DefineJournalPartialAbbreviation{Franchis}{Franch}
\DefineJournalAbbreviation{Franciscan}{Francisc}
\DefineJournalPartialAbbreviation{Francophil}{Francophil}
\DefineJournalAbbreviation{Frangipani}{Frangip}
\DefineJournalAbbreviation{Frankfort}{Frankf}
\DefineJournalAbbreviation{Franklin}{Frankl}
\DefineJournalAbbreviation{Fraser Valley}{Fraser Val}
\DefineJournalAbbreviation{Fraserville}{Fraserv}
\DefineJournalPartialAbbreviation{Fratern}{Fratern}
\DefineJournalAbbreviation{Fredericton}{Frederict}
\DefineJournalPartialAbbreviation{Free}{Free}
\DefineJournalWordException{Freedom}{Freedom}
\DefineJournalAbbreviation{Freehold}{Freeh}
\DefineJournalPartialAbbreviation{Freelanc}{Freel}
\DefineJournalWordException{Freeman}{Freeman}
\DefineJournalWordException{Freemason}{Freemason}
\DefineJournalWordException{Freestate}{Freestate}
\DefineJournalAbbreviation{Freestyle}{Freest}
\DefineJournalWordException{Freesun}{Freesun}
\DefineJournalPartialAbbreviation{Freeth}{Freeth}
\DefineJournalAbbreviation{Freetown}{Freet}
\DefineJournalAbbreviation{Freewheeler}{Freewheel}
\DefineJournalWordException{Freewill}{Freewill}
\DefineJournalWordException{Freewind}{Freewind}
\DefineJournalAbbreviation{Freezer}{Freez}
\DefineJournalAbbreviation{Freezing}{Freez}
\DefineJournalWordException{Freight}{Freight}
\DefineJournalAbbreviation{Freighting}{Freight}
\DefineJournalWordException{Fremantle}{Fremantle}
\DefineJournalAbbreviation{French}{Fr}
\DefineJournalPartialAbbreviation{Frequen}{Freq}
\DefineJournalAbbreviation{Freshman}{Freshm}
\DefineJournalAbbreviation{Freshwater}{Freshw}
\DefineJournalPartialAbbreviation{Friction}{Frict}
\DefineJournalWordException{Friday}{Friday}
\DefineJournalWordException{Friend}{Friend}
\DefineJournalWordException{Friendly}{Friendly}
\DefineJournalAbbreviation{Friendship}{Friendsh}
\DefineJournalAbbreviation{Friesian}{Fries}
\DefineJournalWordException{Frieze}{Frieze}
\DefineJournalPartialAbbreviation{Fright}{Fright}
\DefineJournalPartialAbbreviation{Frigorif}{Frigorif}
\DefineJournalWordException{Fringe}{Fringe}
\DefineJournalWordException{Frisian}{Frisian}
\DefineJournalWordException{Friskies}{Friskies}
\DefineJournalWordException{Frogmore}{Frogmore}
\DefineJournalWordException{Frome}{Frome}
\DefineJournalPartialAbbreviation{Fronti\`er}{Front}
\DefineJournalWordException{Frontline}{Frontline}
\DefineJournalWordException{Frozen}{Frozen}
\DefineJournalAbbreviation{Fruitgrower}{Fruitgrow}
\DefineJournalAbbreviation{Fryer}{Fry}
\DefineJournalAbbreviation{Frying}{Fry}
\DefineJournalAbbreviation{Fullerene}{Fuller}
\DefineJournalAbbreviation{Fullertown}{Fullert}
\DefineJournalWordException{Fulltext}{Fulltext}
\DefineJournalWordException{Fulton}{Fulton}
\DefineJournalPartialAbbreviation{Function}{Funct}
\DefineJournalPartialAbbreviation{Fundament}{Fundam}
\DefineJournalPartialAbbreviation{Fundat}{Fund}
\DefineJournalWordException{Funded}{Funded}
\DefineJournalWordException{Funding}{Funding}
\DefineJournalAbbreviation{Fundraising}{Fundrais}
\DefineJournalPartialAbbreviation{Funera}{Funer}
\DefineJournalWordException{Funfzig}{Funfzig}
\DefineJournalWordException{Fungal}{Fungal}
\DefineJournalAbbreviation{Funhouse}{Funh}
\DefineJournalPartialAbbreviation{Furbear}{Furbear}
\DefineJournalPartialAbbreviation{Furnace}{Furn}
\DefineJournalAbbreviation{Furnisher}{Furnish}
\DefineJournalAbbreviation{Furnishing}{Furnish}
\DefineJournalPartialAbbreviation{Furniture}{Furnit}
\DefineJournalWordException{Furrier}{Furrier}
\DefineJournalWordException{Furrow}{Furrow}
\DefineJournalAbbreviation{Further}{Furth}
\DefineJournalPartialAbbreviation{Futur}{Futur}
\DefineJournalWordException{Future}{Future}
\DefineJournalWordException{Fuzzy}{Fuzzy}
\DefineJournalWordException{Gaborone}{Gaborone}
\DefineJournalWordException{Gadget}{Gadget}
\DefineJournalAbbreviation{Gaelic}{Gael}
\DefineJournalWordException{Gaggle}{Gaggle}
\DefineJournalAbbreviation{Gainesville}{Gainesv}
%\DefineJournalPartialWordException{Galax}{Galax-}
\DefineJournalWordException{Gallaghan}{Gallaghan}
\DefineJournalWordException{Gallery}{Gallery}
\DefineJournalWordException{Galley}{Galley}
\DefineJournalWordException{Galloway}{Galloway}
\DefineJournalPartialAbbreviation{Galvaniz}{Galvaniz}
\DefineJournalAbbreviation{Galveston}{Galvest}
\DefineJournalWordException{Galway}{Galway}
\DefineJournalAbbreviation{Gambling}{Gambl}
\DefineJournalAbbreviation{Gamekeeper}{Gamekeep}
\DefineJournalWordException{Gamer}{Gamer}
\DefineJournalWordException{Gamete}{Gamete}
\DefineJournalPartialAbbreviation{Gametogenes}{Gametog}
\DefineJournalWordException{Gaming}{Gaming}
\DefineJournalWordException{Gander}{Gander}
\DefineJournalWordException{Ganjam}{Ganjam}
\DefineJournalPartialAbbreviation{Garag}{Garag}
\DefineJournalWordException{Garbage}{Garbage}
\DefineJournalPartialAbbreviation{Garden}{Gard}
\DefineJournalWordException{Gardena}{Gardena}
\DefineJournalWordException{Gardenvale}{Gardenvale}
\DefineJournalWordException{Garganta}{Garganta}
\DefineJournalWordException{Garment}{Garment}
\DefineJournalWordException{Garter}{Garter}
\DefineJournalWordException{Gasaet}{Gasaet}
\DefineJournalAbbreviation{Gasdetection}{Gasdetect}
\DefineJournalPartialAbbreviation{Gasdynami}{Gasdyn}
\DefineJournalPartialAbbreviation{Gasfit}{Gasfit}
\DefineJournalAbbreviation{Gasification}{Gasif}
\DefineJournalAbbreviation{Gasohol}{Gasoh}
\DefineJournalAbbreviation{Gasoline}{Gasol}
\DefineJournalWordException{Gaspipe}{Gaspipe}
\DefineJournalWordException{Gastric}{Gastric}
\DefineJournalPartialAbbreviation{Gastroenterohepatol}{Gastroenterohepatol}
\DefineJournalAbbreviation{Gastrointestinal}{Gastrointest}
\DefineJournalPartialAbbreviation{Gastrokineti}{Gastrokinet}
\DefineJournalPartialAbbreviation{Gastron}{Gastron}
\DefineJournalAbbreviation{Gateshead}{Gatesh}
\DefineJournalAbbreviation{Gateway}{Gatew}
%\DefineJournalPartialWordException{Gather}{Gather-}
\DefineJournalAbbreviation{Gathering}{Gather}
\DefineJournalWordException{Gatton}{Gatton}
\DefineJournalWordException{Gatwick}{Gatwick}
\DefineJournalWordException{Gauging}{Gauging}
\DefineJournalWordException{Gauntlet}{Gauntlet}
\DefineJournalWordException{Gazelle}{Gazelle}
\DefineJournalWordException{Gearbox}{Gearbox}
\DefineJournalWordException{Geelong}{Geelong}
\DefineJournalWordException{Gemstones}{Gemstones}
\DefineJournalAbbreviation{Gender}{Gend}
%\DefineJournalPartialWordException{Genepool}{Genepool-}
\DefineJournalPartialAbbreviation{General}{Gen}
\DefineJournalWordException{Generic}{Generic}
\DefineJournalWordException{Geneva}{Geneva}
\DefineJournalAbbreviation{Genital}{Genit}
\DefineJournalAbbreviation{Genito-urinary}{Genito-urin}
\DefineJournalAbbreviation{Genitourinary}{Genitourin}
\DefineJournalWordException{Genius}{Genius}
\DefineJournalWordException{Genome}{Genome}
\DefineJournalPartialAbbreviation{Genomic}{Genom}
\DefineJournalPartialAbbreviation{Genotoxicolog}{Genotoxicol}
\DefineJournalAbbreviation{Gentleman}{Gentlem}
\DefineJournalPartialAbbreviation{Geoastrophysic}{Geoastrophys}
\DefineJournalPartialAbbreviation{Geobiolog}{Geobiol}
\DefineJournalPartialAbbreviation{Geochem}{Geochem}
\DefineJournalAbbreviation{Geochronology}{Geochronol}
\DefineJournalWordException{Geocode}{Geocode}
\DefineJournalPartialAbbreviation{Geocryolog}{Geocryol}
\DefineJournalPartialAbbreviation{Geodaes}{Geod}
\DefineJournalPartialAbbreviation{Geodaet}{Geod}
\DefineJournalPartialAbbreviation{Geodynami}{Geodyn}
\DefineJournalAbbreviation{Geoecological}{Geoecol}
\DefineJournalPartialAbbreviation{Geoelectric}{Geoelectr}
\DefineJournalPartialAbbreviation{Geoengineer}{Geoengin}
\DefineJournalAbbreviation{Geoexploration}{Geoexplor}
\DefineJournalWordException{Geogram}{Geogram}
\DefineJournalPartialAbbreviation{Geograph}{Geogr}
\DefineJournalAbbreviation{Geojournal}{Geoj}
\DefineJournalAbbreviation{Geolinguistics}{Geolinguist}
\DefineJournalAbbreviation{Geomantic}{Geomant}
\DefineJournalAbbreviation{Geomatic}{Geomat}
\DefineJournalAbbreviation{Geomembrane}{Geomembr}
\DefineJournalPartialAbbreviation{Geomicrobiolog}{Geomicrobiol}
\DefineJournalPartialAbbreviation{Geomorpholog}{Geomorphol}
\DefineJournalPartialAbbreviation{Geophys}{Geophys}
\DefineJournalPartialAbbreviation{Geopoliti}{Geopolit}
\DefineJournalPartialAbbreviation{Geopress}{Geopress}
\DefineJournalAbbreviation{Georgetown}{Georget}
\DefineJournalAbbreviation{Georgia}{Ga}
\DefineJournalWordException{Georgian}{Georgian}
\DefineJournalAbbreviation{Geospace}{Geosp}
\DefineJournalAbbreviation{Geospatial}{Geospat}
\DefineJournalAbbreviation{Geosphere}{Geosph}
\DefineJournalPartialAbbreviation{Geostandard}{Geostand}
\DefineJournalPartialAbbreviation{Geosyntheti}{Geosynth}
\DefineJournalPartialAbbreviation{Geotechnolog}{Geotechnol}
\DefineJournalAbbreviation{Geotextiles}{Geotext}
\DefineJournalAbbreviation{Geothermal}{Geotherm}
\DefineJournalWordException{Geraldine}{Geraldine}
\DefineJournalAbbreviation{Geraldton}{Geraldt}
\DefineJournalWordException{Gerbil}{Gerbil}
\DefineJournalPartialAbbreviation{German}{Ger}
\DefineJournalWordException{Germanium}{Germanium}
\DefineJournalAbbreviation{Germany}{Ger}
\DefineJournalWordException{Gertrudis}{Gertrudis}
\DefineJournalPartialAbbreviation{Gesneria}{Gesner}
\DefineJournalAbbreviation{Gestational}{Gestation}
\DefineJournalAbbreviation{Getting}{Get}
\DefineJournalAbbreviation{Gettysburg}{Gettysbg}
\DefineJournalWordException{Ghana}{Ghana}
\DefineJournalAbbreviation{Ghanaian}{Ghana}
\DefineJournalAbbreviation{Ghostbuster}{Ghostbust}
\DefineJournalWordException{Gibraltar}{Gibraltar}
\DefineJournalPartialAbbreviation{Gift}{Gift}
\DefineJournalWordException{Giftware}{Giftware}
\DefineJournalWordException{Gilead}{Gilead}
\DefineJournalWordException{Gilgandra}{Gilgandra}
\DefineJournalWordException{Gillingham}{Gillingham}
\DefineJournalWordException{Ginning}{Ginning}
\DefineJournalAbbreviation{Gippsland}{Gippsl}
\DefineJournalWordException{Giveaway}{Giveaway}
\DefineJournalAbbreviation{Giving}{Giv}
\DefineJournalPartialAbbreviation{Glaciat}{Glaciat}
\DefineJournalPartialAbbreviation{Glaciolog}{Glaciol}
\DefineJournalWordException{Gladiolus}{Gladiolus}
\DefineJournalWordException{Gladstone}{Gladstone}
\DefineJournalAbbreviation{Glamorgan}{Glam}
\DefineJournalWordException{Glamour}{Glamour}
\DefineJournalWordException{Glance}{Glance}
\DefineJournalAbbreviation{Glaning}{Glan}
\DefineJournalAbbreviation{Glasgow}{Glasg}
\DefineJournalWordException{Glasshouse}{Glasshouse}
\DefineJournalWordException{Glassware}{Glassware}
\DefineJournalWordException{Glaucoma}{Glaucoma}
\DefineJournalAbbreviation{Glazer}{Glaz}
\DefineJournalAbbreviation{Glazing}{Glaz}
\DefineJournalAbbreviation{Gleaner}{Glean}
\DefineJournalPartialAbbreviation{Gleaning}{Glean}
\DefineJournalWordException{Glenbow}{Glenbow}
\DefineJournalWordException{Glendale}{Glendale}
\DefineJournalWordException{Glengarry}{Glengarry}
\DefineJournalWordException{Glenhyrst}{Glenhyrst}
\DefineJournalWordException{Glenmarie}{Glenmarie}
\DefineJournalWordException{Glenormiston}{Glenormiston}
\DefineJournalWordException{Glensview}{Glensview}
\DefineJournalWordException{Glenwaverley}{Glenwaverley}
\DefineJournalPartialAbbreviation{Glid}{Glid}
\DefineJournalWordException{Glimpse}{Glimpse}
\DefineJournalWordException{Globe-trotter}{Globe-trotter}
\DefineJournalWordException{Globefish}{Globefish}
\DefineJournalWordException{Globetree}{Globetree}
\DefineJournalPartialAbbreviation{Globul}{Globul}
\DefineJournalWordException{Glorious}{Glorious}
\DefineJournalWordException{Glory}{Glory}
\DefineJournalAbbreviation{Gloryland}{Gloryl}
\DefineJournalAbbreviation{Glossary}{Gloss}
\DefineJournalAbbreviation{Gloucester}{Glos}
\DefineJournalAbbreviation{Gloucestershire}{Glos}
\DefineJournalWordException{Glycerine}{Glycerine}
\DefineJournalPartialAbbreviation{Glycobiolog}{Glycobiol}
\DefineJournalAbbreviation{Glycoconjugate}{Glycoconj}
\DefineJournalPartialAbbreviation{Glycomedic}{Glycomed}
\DefineJournalAbbreviation{Glycomics}{Glycom}
\DefineJournalPartialAbbreviation{Glycoscienc}{Glycosci}
\DefineJournalPartialAbbreviation{Glycotechnolog}{Glycotechnol}
\DefineJournalAbbreviation{Gnozis}{Gnoz}
\DefineJournalAbbreviation{Goatkeeping}{Goatkeep}
\DefineJournalWordException{Godalming}{Godalming}
\DefineJournalWordException{Goldbelt}{Goldbelt}
\DefineJournalAbbreviation{Golden}{Gold}
\DefineJournalAbbreviation{Goldenbook}{Goldenb}
\DefineJournalWordException{Goldfield}{Goldfield}
\DefineJournalWordException{Goldsmith}{Goldsmith}
\DefineJournalPartialAbbreviation{Golf}{Golf}
\DefineJournalAbbreviation{Gongola}{Gong}
\DefineJournalWordException{Gonorrhea}{Gonorrhea}
\DefineJournalWordException{Goodlife}{Goodlife}
\DefineJournalWordException{Goodnews}{Goodnews}
\DefineJournalWordException{Goodwill}{Goodwill}
\DefineJournalWordException{Goodwood}{Goodwood}
\DefineJournalWordException{Goodyear}{Goodyear}
\DefineJournalWordException{Goonellabah}{Goonellabah}
\DefineJournalWordException{Gosford}{Gosford}
\DefineJournalWordException{Gospel}{Gospel}
\DefineJournalPartialAbbreviation{Gospel}{Gospel}
\DefineJournalWordException{Gosport}{Gosport}
\DefineJournalWordException{Gossip}{Gossip}
\DefineJournalWordException{Gothic}{Gothic}
\DefineJournalAbbreviation{Governance}{Gov}
\DefineJournalWordException{Governess}{Governess}
\DefineJournalAbbreviation{Governing}{Gov}
\DefineJournalPartialAbbreviation{Government}{Gov}
\DefineJournalAbbreviation{Governor}{Gov}
\DefineJournalPartialAbbreviation{Graceful}{Gracef}
\DefineJournalWordException{Grading}{Grading}
\DefineJournalAbbreviation{Grahamstown}{Grahamst}
\DefineJournalAbbreviation{Graingrower}{Graingrow}
\DefineJournalWordException{Grajarat}{Grajarat}
\DefineJournalAbbreviation{Grammar}{Gramm}
\DefineJournalAbbreviation{Gramophone}{Gramoph}
\DefineJournalWordException{Grampian}{Grampian}
\DefineJournalAbbreviation{Grand Falls}{Gd Falls}
\DefineJournalAbbreviation{Grand-Forks}{Gd-Forks}
\DefineJournalWordException{Grandma}{Grandma}
\DefineJournalWordException{Grandparent}{Grandparent}
\DefineJournalWordException{Grandstand}{Grandstand}
\DefineJournalWordException{Granite}{Granite}
\DefineJournalWordException{Grant}{Grant}
\DefineJournalWordException{Grantee}{Grantee}
\DefineJournalAbbreviation{Granting}{Grant}
\DefineJournalPartialAbbreviation{Grantmak}{Grantmak}
\DefineJournalWordException{Granton}{Granton}
\DefineJournalAbbreviation{Grantor}{Grant}
\DefineJournalAbbreviation{Grantsmanship}{Grantsmansh}
\DefineJournalAbbreviation{Granular}{Granul}
\DefineJournalAbbreviation{Grapegrower}{Grapegrow}
\DefineJournalWordException{Grapevine}{Grapevine}
\DefineJournalWordException{Graph}{Graph}
\DefineJournalPartialAbbreviation{Graphi}{Graph}
\DefineJournalPartialAbbreviation{Graphoscop}{Graphosc}
\DefineJournalAbbreviation{Graptolite}{Grapt}
\DefineJournalPartialAbbreviation{Grasshopp}{Grasshopp}
\DefineJournalWordException{Grassroot}{Grassroot}
\DefineJournalPartialAbbreviation{Grateful}{Grateful}
\DefineJournalPartialAbbreviation{Gratuit}{Gratuit}
\DefineJournalWordException{Gravel}{Gravel}
\DefineJournalAbbreviation{Gravelbourg}{Gravelbg}
\DefineJournalWordException{Gravement}{Gravement}
\DefineJournalWordException{Gravesend}{Gravesend}
\DefineJournalWordException{Gravestone}{Gravestone}
\DefineJournalAbbreviation{Gravitation}{Gravit}
\DefineJournalWordException{Gravity}{Gravity}
\DefineJournalAbbreviation{Grayling}{Grayl}
\DefineJournalWordException{Grazier}{Grazier}
\DefineJournalWordException{Grazing}{Grazing}
\DefineJournalAbbreviation{Great Britain}{G B}
\DefineJournalAbbreviation{Great Divide}{Gt Divide}
\DefineJournalAbbreviation{Great Lakes}{Gt Lakes}
\DefineJournalAbbreviation{Great Plains}{Gt Plains}
\DefineJournalPartialAbbreviation{Great}{Gt}
\DefineJournalWordException{Greece}{Greece}
\DefineJournalWordException{Greek}{Greek}
\DefineJournalWordException{Green-River}{Green-River}
\DefineJournalWordException{Greendale}{Greendale}
\DefineJournalWordException{Greenhide}{Greenhide}
\DefineJournalWordException{Greenhill}{Greenhill}
\DefineJournalAbbreviation{Greenhouse}{Greenh}
\DefineJournalAbbreviation{Greening}{Green}
\DefineJournalAbbreviation{Greenkeeper}{Greenkeep}
\DefineJournalAbbreviation{Greenkeeping}{Greenkeep}
\DefineJournalAbbreviation{Greenland}{Greenl}
\DefineJournalWordException{Greenpeace}{Greenpeace}
\DefineJournalAbbreviation{Greensboro}{Greensb}
\DefineJournalWordException{Greenspeak}{Greenspeak}
\DefineJournalWordException{Greenview}{Greenview}
\DefineJournalWordException{Greenweek}{Greenweek}
\DefineJournalWordException{Greenwich}{Greenwich}
\DefineJournalWordException{Greenwood}{Greenwood}
\DefineJournalAbbreviation{Greeting}{Greet}
\DefineJournalPartialAbbreviation{Gregori}{Gregor}
\DefineJournalAbbreviation{Grenville}{Grenv}
\DefineJournalWordException{Greyhound}{Greyhound}
\DefineJournalWordException{Gridiron}{Gridiron}
\DefineJournalAbbreviation{Grievance}{Griev}
\DefineJournalAbbreviation{Grinding}{Grind}
\DefineJournalPartialAbbreviation{Grocer}{Groc}
\DefineJournalWordException{Grotto}{Grotto}
\DefineJournalWordException{Ground}{Ground}
\DefineJournalWordException{Groundcare}{Groundcare}
\DefineJournalAbbreviation{Groundfish}{Groundf}
\DefineJournalAbbreviation{Groundnut}{Groundn}
\DefineJournalAbbreviation{Groundwater}{Groundw}
\DefineJournalWordException{Group}{Group}
\DefineJournalAbbreviation{Grouping}{Group}
\DefineJournalAbbreviation{Groupware}{Groupw}
\DefineJournalPartialAbbreviation{Grower}{Grow}
\DefineJournalAbbreviation{Growing}{Grow}
\DefineJournalWordException{Growth}{Growth}
\DefineJournalWordException{Guangdong}{Guangdong}
\DefineJournalPartialAbbreviation{Guarant}{Guarant}
\DefineJournalPartialAbbreviation{Guard}{Guard}
\DefineJournalAbbreviation{Guardsman}{Guardsm}
\DefineJournalWordException{Guelph}{Guelph}
\DefineJournalWordException{Guernsey}{Guernsey}
\DefineJournalAbbreviation{Guesthouse}{Guesth}
\DefineJournalPartialAbbreviation{Guid}{Guid}
\DefineJournalWordException{Guide}{Guide}
\DefineJournalAbbreviation{Guidebook}{Guideb}
\DefineJournalPartialAbbreviation{Guideline}{Guidel}
\DefineJournalAbbreviation{Guildford}{Guildf}
\DefineJournalAbbreviation{Guildhall}{Guildh}
\DefineJournalWordException{Guilty}{Guilty}
\DefineJournalAbbreviation{Guinea}{Guin}
\DefineJournalWordException{Guinness}{Guinness}
\DefineJournalAbbreviation{Gujarati}{Guj}
\DefineJournalAbbreviation{Gunner}{Gun}
\DefineJournalWordException{Gunpowder}{Gunpowder}
\DefineJournalWordException{Gunsmith}{Gunsmith}
\DefineJournalWordException{Guntur}{Guntur}
\DefineJournalWordException{Guyana}{Guyana}
\DefineJournalPartialAbbreviation{Gymnast}{Gymnast}
\DefineJournalPartialAbbreviation{Gynaecolog}{Gynaecol}
\DefineJournalPartialAbbreviation{Gynecolog}{Gynecol}
\DefineJournalWordException{Gypsum}{Gypsum}
\DefineJournalAbbreviation{Hackensack}{Hackens}
\DefineJournalWordException{Hacker}{Hacker}
\DefineJournalPartialAbbreviation{Hadron}{Hadron}
\DefineJournalPartialAbbreviation{Haematolog}{Haematol}
\DefineJournalPartialAbbreviation{Haematop}{Haematop}
\DefineJournalWordException{Haemic}{Haemic}
\DefineJournalAbbreviation{Haemodialysis}{Haemodial}
\DefineJournalPartialAbbreviation{Haemodynam}{Haemodyn}
\DefineJournalPartialAbbreviation{Haemogeneti}{Haemogenet}
\DefineJournalAbbreviation{Haemophilia}{Haemoph}
\DefineJournalPartialAbbreviation{Haemorheolog}{Haemorheol}
\DefineJournalPartialAbbreviation{Haemorrhagic}{Haemorrh}
\DefineJournalAbbreviation{Hahnemannian}{Hahnemann}
\DefineJournalAbbreviation{Hairdresser}{Hairdr}
\DefineJournalWordException{Hairflair}{Hairflair}
\DefineJournalWordException{Halcyon}{Halcyon}
\DefineJournalWordException{Haldimand}{Haldimand}
\DefineJournalWordException{Halfyard}{Halfyard}
\DefineJournalWordException{Halifax}{Halifax}
\DefineJournalAbbreviation{Hallmarks}{Hallm}
\DefineJournalPartialAbbreviation{Hallucinogen}{Hallucinog}
\DefineJournalWordException{Halophilic}{Halophilic}
\DefineJournalWordException{Hambro}{Hambro}
\DefineJournalWordException{Hambrook}{Hambrook}
\DefineJournalAbbreviation{Hamilton}{Hamilt}
\DefineJournalWordException{Hammer}{Hammer}
\DefineJournalWordException{Hammond}{Hammond}
\DefineJournalWordException{Hampden}{Hampden}
\DefineJournalAbbreviation{Hampshire}{Hamps}
\DefineJournalWordException{Hampstead}{Hampstead}
\DefineJournalWordException{Hampton}{Hampton}
\DefineJournalWordException{Handbell}{Handbell}
\DefineJournalAbbreviation{Handbook}{Handb}
\DefineJournalAbbreviation{Handcraft}{Handcr}
\DefineJournalWordException{Handgun}{Handgun}
\DefineJournalWordException{Handicraft}{Handicraft}
\DefineJournalAbbreviation{Handknitting}{Handknitt}
\DefineJournalWordException{Handle}{Handle}
\DefineJournalAbbreviation{Handler}{Handl}
\DefineJournalPartialAbbreviation{Handling}{Handl}
\DefineJournalWordException{Handlist}{Handlist}
\DefineJournalPartialAbbreviation{Handwrit}{Handwrit}
\DefineJournalWordException{Handyman}{Handyman}
\DefineJournalWordException{Hannan}{Hannan}
\DefineJournalWordException{Happen}{Happen}
\DefineJournalAbbreviation{Happening}{Happen}
\DefineJournalWordException{Happiness}{Happiness}
\DefineJournalWordException{Happy}{Happy}
\DefineJournalPartialAbbreviation{Harass}{Harass}
\DefineJournalPartialAbbreviation{Harbor}{Harb}
\DefineJournalWordException{Hardback}{Hardback}
\DefineJournalWordException{Hardboard}{Hardboard}
\DefineJournalWordException{Hardcore}{Hardcore}
\DefineJournalPartialAbbreviation{Hardcover}{Hardcover}
\DefineJournalAbbreviation{Hardware}{Hardw}
\DefineJournalWordException{Hardwood}{Hardwood}
\DefineJournalWordException{Harlan}{Harlan}
\DefineJournalWordException{Harlow}{Harlow}
\DefineJournalWordException{Harmful}{Harmful}
\DefineJournalPartialAbbreviation{Harmon}{Harmon}
\DefineJournalWordException{Harness}{Harness}
\DefineJournalWordException{Harpenden}{Harpenden}
\DefineJournalWordException{Harpsichord}{Harpsichord}
\DefineJournalAbbreviation{Harrisburg}{Harrisbg}
\DefineJournalWordException{Harrogate}{Harrogate}
\DefineJournalWordException{Harrow}{Harrow}
\DefineJournalWordException{Hartford}{Hartford}
\DefineJournalAbbreviation{Hartlepool}{Hartlep}
\DefineJournalAbbreviation{Harvard}{Harv}
\DefineJournalPartialAbbreviation{Harvest}{Harvest}
\DefineJournalWordException{Haryana}{Haryana}
\DefineJournalPartialAbbreviation{Hast}{H\"ast}
\DefineJournalWordException{Hastings}{Hastings}
\DefineJournalAbbreviation{Hatchery}{Hatch}
\DefineJournalAbbreviation{Hatching}{Hatch}
\DefineJournalPartialAbbreviation{Haul}{Haul}
\DefineJournalWordException{Haverhill}{Haverhill}
\DefineJournalWordException{Hawaii}{Hawaii}
\DefineJournalAbbreviation{Hawaiian}{Hawaii}
\DefineJournalWordException{Hawkesbury}{Hawkesbury}
\DefineJournalWordException{Hawkeye}{Hawkeye}
\DefineJournalWordException{Hawthorn}{Hawthorn}
\DefineJournalWordException{Haymarket}{Haymarket}
\DefineJournalWordException{Hayward}{Hayward}
\DefineJournalWordException{Hazard}{Hazard}
\DefineJournalAbbreviation{Hazardous}{Hazard}
\DefineJournalWordException{Headache}{Headache}
\DefineJournalAbbreviation{Headhunter}{Headhunt}
\DefineJournalPartialAbbreviation{Heading}{Head}
\DefineJournalWordException{Headley}{Headley}
\DefineJournalPartialAbbreviation{Headlin}{Headl}
\DefineJournalAbbreviation{Headmasters}{Headmast}
\DefineJournalWordException{Headnote}{Headnote}
\DefineJournalAbbreviation{Headquarters}{Hqrs}
\DefineJournalWordException{Headwater}{Headwater}
\DefineJournalAbbreviation{Headway}{Headw}
\DefineJournalPartialAbbreviation{Heal}{Heal}
\DefineJournalWordException{Healesville}{Healesville}
\DefineJournalWordException{Health}{Health}
\DefineJournalWordException{Healthbeat}{Healthbeat}
\DefineJournalAbbreviation{Healthcare}{Healthc}
\DefineJournalWordException{Healthwise}{Healthwise}
\DefineJournalWordException{Healthy}{Healthy}
\DefineJournalPartialAbbreviation{Hear}{Hear}
\DefineJournalWordException{Heard}{Heard}
\DefineJournalWordException{Heart}{Heart}
\DefineJournalAbbreviation{Heartbeat}{Heartb}
\DefineJournalWordException{Hearth}{Hearth}
\DefineJournalAbbreviation{Heartland}{Heartl}
\DefineJournalWordException{Heartline}{Heartline}
\DefineJournalAbbreviation{Heater}{Heat}
\DefineJournalWordException{Heathcote}{Heathcote}
\DefineJournalWordException{Heathrow}{Heathrow}
\DefineJournalAbbreviation{Heating}{Heat}
\DefineJournalWordException{Heaton}{Heaton}
\DefineJournalPartialAbbreviation{Heaven}{Heaven}
\DefineJournalWordException{Heavy}{Heavy}
\DefineJournalWordException{Heavyside}{Heavyside}
\DefineJournalAbbreviation{Hebrew}{Hebr}
\DefineJournalAbbreviation{Hebridean}{Hebrid}
\DefineJournalAbbreviation{Heedful}{Heedf}
\DefineJournalAbbreviation{Heidelburg}{Heidelbg}
\DefineJournalWordException{Height}{Height}
\DefineJournalPartialAbbreviation{Height}{Height}
\DefineJournalWordException{Helena}{Helena}
\DefineJournalWordException{Helicopter}{Helicopter}
\DefineJournalAbbreviation{Heliport}{Helipt}
\DefineJournalPartialAbbreviation{Helmintholog}{Helminthol}
\DefineJournalPartialAbbreviation{Help}{Help}
\DefineJournalWordException{Helter}{Helter}
\DefineJournalPartialAbbreviation{Hematop}{Hematop}
\DefineJournalAbbreviation{Hemeroteca}{Hemerot}
\DefineJournalPartialAbbreviation{Hemicellulos}{Hemicellul}
\DefineJournalPartialAbbreviation{Hemochromatos}{Hemochromatos}
\DefineJournalAbbreviation{Hemodialysis}{Hemodial}
\DefineJournalPartialAbbreviation{Hemofiltrat}{Hemofiltr}
\DefineJournalPartialAbbreviation{Hemorheolog}{Hemorheol}
\DefineJournalPartialAbbreviation{Hemostaseolog}{Hemostaseol}
\DefineJournalWordException{Hemstitching}{Hemstitching}
\DefineJournalWordException{Henley}{Henley}
\DefineJournalAbbreviation{Hepatitis}{Hepat}
\DefineJournalPartialAbbreviation{Hepatocellular}{Hepatocell}
\DefineJournalAbbreviation{Hepatotoxicity}{Hepatotoxic}
\DefineJournalWordException{Heraclion}{Heraclion}
\DefineJournalAbbreviation{Herald}{Her}
\DefineJournalWordException{Herbaceous}{Herbaceous}
\DefineJournalAbbreviation{Herbage}{Herb}
\DefineJournalAbbreviation{Herbal}{Herb}
\DefineJournalAbbreviation{Herbalism}{Herbal}
\DefineJournalPartialAbbreviation{Herbari}{Herb}
\DefineJournalPartialAbbreviation{Herbicid}{Herbic}
\DefineJournalPartialAbbreviation{Heredi}{Hered}
\DefineJournalWordException{Hereford}{Hereford}
\DefineJournalAbbreviation{Herefordshire}{Hereford}
\DefineJournalAbbreviation{H\'eritage}{Herit}
\DefineJournalAbbreviation{Hermeneutical}{Hermeneut}
\DefineJournalAbbreviation{Hermetic}{Hermet}
\DefineJournalWordException{Hermitage}{Hermitage}
\DefineJournalWordException{Heroldo}{Heroldo}
\DefineJournalAbbreviation{Heronry}{Heron}
\DefineJournalAbbreviation{Herpetofauna}{Herpetof}
\DefineJournalWordException{Herring}{Herring}
\DefineJournalAbbreviation{Hertfordshire}{Herts}
\DefineJournalPartialAbbreviation{Heteroaromatic}{Heteroaromat}
\DefineJournalAbbreviation{Heteroatom}{Heteroat}
\DefineJournalPartialAbbreviation{Heterocyclic}{Heterocycl}
\DefineJournalAbbreviation{Heteronuclear}{Heteronucl}
\DefineJournalPartialAbbreviation{Heterostructur}{Heterostruct}
\DefineJournalWordException{Hiballer}{Hiballer}
\DefineJournalWordException{Hibiscus}{Hibiscus}
\DefineJournalWordException{Hickory}{Hickory}
\DefineJournalWordException{Hideaway}{Hideaway}
\DefineJournalPartialAbbreviation{Hidrotechni}{Hidrotech}
\DefineJournalWordException{Higging}{Higging}
\DefineJournalAbbreviation{Higher}{High}
\DefineJournalAbbreviation{Highest}{High}
\DefineJournalPartialAbbreviation{Highland}{Highl}
\DefineJournalWordException{Highlight}{Highlight}
\DefineJournalWordException{Highscreen}{Highscreen}
\DefineJournalPartialAbbreviation{Highway}{Highw}
\DefineJournalWordException{Highwood}{Highwood}
\DefineJournalAbbreviation{Hiking}{Hik}
\DefineJournalPartialAbbreviation{Hilar}{Hilar}
\DefineJournalAbbreviation{Hillingdon}{Hillingd}
\DefineJournalAbbreviation{Hillsburgh}{Hillsb}
\DefineJournalWordException{Himachal-Pradesh}{Himachal-Pradesh}
\DefineJournalAbbreviation{Himalayan}{Himal}
\DefineJournalWordException{Himashal Pradesh}{Himashal Pradesh}
\DefineJournalWordException{Hindmarsh}{Hindmarsh}
\DefineJournalWordException{Hindsale}{Hindsale}
\DefineJournalAbbreviation{Hinduism}{Hindu}
\DefineJournalWordException{Hiring}{Hiring}
\DefineJournalPartialAbbreviation{Histochem}{Histochem}
\DefineJournalPartialAbbreviation{Histocompatibil}{Histocompat}
\DefineJournalPartialAbbreviation{Histopatholog}{Histopathol}
\DefineJournalPartialAbbreviation{Histor}{Hist}
\DefineJournalPartialAbbreviation{Hitch}{Hitch}
\DefineJournalWordException{Hitchin}{Hitchin}
\DefineJournalWordException{Hobart}{Hobart}
%\DefineJournalPartialWordException{Hobby}{Hobby-}
\DefineJournalWordException{Hobbyist}{Hobbyist}
\DefineJournalWordException{Hocken}{Hocken}
\DefineJournalWordException{Hockey}{Hockey}
\DefineJournalWordException{Hodgepodge}{Hodgepodge}
\DefineJournalAbbreviation{Holder}{Hold}
\DefineJournalAbbreviation{Holding}{Hold}
\DefineJournalWordException{Holiday}{Holiday}
\DefineJournalAbbreviation{Holiness}{Holin}
\DefineJournalAbbreviation{Holistic}{Holist}
\DefineJournalWordException{Hollywood}{Hollywood}
%\DefineJournalPartialWordException{Holocaust}{Holocaust-}
\DefineJournalWordException{Homathko}{Homathko}
\DefineJournalWordException{Homebased}{Homebased}
\DefineJournalWordException{Homebirth}{Homebirth}
\DefineJournalWordException{Homebuilt}{Homebuilt}
\DefineJournalAbbreviation{Homebuying}{Homebuy}
\DefineJournalWordException{Homecare}{Homecare}
\DefineJournalWordException{Homecoming}{Homecoming}
\DefineJournalWordException{Homefinder}{Homefinder}
\DefineJournalWordException{Homegrown}{Homegrown}
\DefineJournalAbbreviation{Homeland}{Homel}
\DefineJournalWordException{Homeless}{Homeless}
\DefineJournalAbbreviation{Homemaker}{Homemak}
\DefineJournalPartialAbbreviation{Homeopath}{Homeopath}
\DefineJournalAbbreviation{Homeostasis}{Homeost}
\DefineJournalAbbreviation{Homeostatic}{Homeost}
\DefineJournalPartialAbbreviation{Homeown}{Homeown}
\DefineJournalWordException{Homepage}{Homepage}
\DefineJournalPartialAbbreviation{Homeschool}{Homesch}
\DefineJournalAbbreviation{Homestead}{Homestd}
\DefineJournalWordException{Hometown}{Hometown}
\DefineJournalAbbreviation{Homeware}{Homew}
\DefineJournalPartialAbbreviation{Homilet}{Homilet}
\DefineJournalWordException{Homily}{Homily}
\DefineJournalPartialAbbreviation{Homoatomi}{Homoat}
\DefineJournalPartialAbbreviation{Homoeopath}{Homoeopath}
\DefineJournalPartialAbbreviation{Homogen}{Homog}
\DefineJournalPartialAbbreviation{Homolog}{Homol}
\DefineJournalPartialAbbreviation{Homosex}{Homosex}
\DefineJournalWordException{Honest}{Honest}
\DefineJournalWordException{Hong Kong}{Hong Kong}
\DefineJournalWordException{Honour}{Honour}
\DefineJournalAbbreviation{Honourable}{Honour}
\DefineJournalAbbreviation{Hooking}{Hook}
\DefineJournalWordException{Hooray}{Hooray}
\DefineJournalWordException{Hoosier}{Hoosier}
\DefineJournalWordException{Hopeful}{Hopeful}
\DefineJournalAbbreviation{Hopeless}{Hopel}
\DefineJournalWordException{Hopkins}{Hopkins}
\DefineJournalWordException{Horary}{Horary}
\DefineJournalPartialAbbreviation{Horizontal}{Horiz}
\DefineJournalPartialAbbreviation{Hormonogenes}{Hormonog}
\DefineJournalPartialAbbreviation{Hormonotherap}{Hormonother}
\DefineJournalWordException{Horror}{Horror}
\DefineJournalWordException{Horse}{Horse}
\DefineJournalWordException{Horseman}{Horseman}
\DefineJournalPartialAbbreviation{Horticult}{Hortic}
\DefineJournalWordException{Hosiery}{Hosiery}
\DefineJournalPartialAbbreviation{Hospit}{Hosp}
\DefineJournalAbbreviation{Hotelkeeper}{Hotelk}
\DefineJournalAbbreviation{Hotelman}{Hotelm}
\DefineJournalWordException{Hotline}{Hotline}
\DefineJournalWordException{Hotspot}{Hotspot}
\DefineJournalWordException{Hounels}{Hounels}
\DefineJournalAbbreviation{Hourly}{Hour}
\DefineJournalAbbreviation{Houseboating}{Houseboat}
\DefineJournalPartialAbbreviation{Housebuild}{Housebuild}
\DefineJournalAbbreviation{Household}{Househ}
\DefineJournalPartialAbbreviation{Housekeep}{Housekeep}
\DefineJournalAbbreviation{Houseware}{Housew}
\DefineJournalWordException{Housewife}{Housewife}
\DefineJournalAbbreviation{Housing}{Hous}
\DefineJournalAbbreviation{Houston}{Houst}
\DefineJournalAbbreviation{Hovercraft}{Hovercr}
\DefineJournalAbbreviation{Hovering}{Hover}
\DefineJournalAbbreviation{Huddersfield}{Hudders}
\DefineJournalWordException{Hudson}{Hudson}
\DefineJournalWordException{Huguenot}{Huguenot}
\DefineJournalAbbreviation{Human}{Hum}
\DefineJournalAbbreviation{Humane}{Hum}
\DefineJournalWordException{Humanism}{Humanism}
\DefineJournalWordException{Humanist}{Humanist}
\DefineJournalPartialAbbreviation{Humanistic}{Humanist}
\DefineJournalPartialAbbreviation{Humanit}{Humanit}
\DefineJournalPartialAbbreviation{Humaniz}{Humaniz}
\DefineJournalWordException{Humber}{Humber}
\DefineJournalAbbreviation{Humberside}{Humbers}
\DefineJournalAbbreviation{Humdinger}{Humding}
\DefineJournalWordException{Hundred}{Hundred}
\DefineJournalPartialAbbreviation{Hungar}{Hung}
\DefineJournalPartialAbbreviation{Hunger}{Hunger}
\DefineJournalWordException{Hungry}{Hungry}
\DefineJournalAbbreviation{Hunter}{Hunt}
\DefineJournalAbbreviation{Hunting}{Hunt}
\DefineJournalWordException{Huntingdon}{Huntingdon}
\DefineJournalAbbreviation{Huntingdonshire}{Huntingdons}
\DefineJournalAbbreviation{Huntington}{Huntingt}
\DefineJournalWordException{Huntsville}{Huntsville}
\DefineJournalWordException{Huron}{Huron}
\DefineJournalAbbreviation{Hurricane}{Hurric}
\DefineJournalAbbreviation{Husbandry}{Husb}
\DefineJournalWordException{Hustler}{Hustler}
\DefineJournalAbbreviation{Hybridization}{Hybrid}
\DefineJournalAbbreviation{Hybridoma}{Hybrid}
\DefineJournalWordException{Hydatidosis}{Hydatidosis}
\DefineJournalPartialAbbreviation{Hydrocephal}{Hydroceph}
\DefineJournalPartialAbbreviation{Hydrochem}{Hydrochem}
\DefineJournalAbbreviation{Hydrocolloids}{Hydrocoll}
\DefineJournalAbbreviation{Hydrocyclodes}{Hydrocycl}
\DefineJournalPartialAbbreviation{Hydroelectri}{Hydroelectr}
\DefineJournalWordException{Hydroenergy}{Hydroenergy}
\DefineJournalWordException{Hydrofoil}{Hydrofoil}
\DefineJournalAbbreviation{Hydrogasification}{Hydrogasif}
\DefineJournalPartialAbbreviation{Hydrog\`en}{Hydrog}
\DefineJournalPartialAbbreviation{Hydrogeochemi}{Hydrogeochem}
\DefineJournalAbbreviation{Hydrolysis}{Hydrolys}
\DefineJournalPartialAbbreviation{Hydromagneti}{Hydromagn}
\DefineJournalAbbreviation{Hydromechanic}{Hydromech}
\DefineJournalPartialAbbreviation{Hydrometallurg}{Hydrometall}
\DefineJournalPartialAbbreviation{Hydrometeorolog}{Hydrometeorol}
\DefineJournalPartialAbbreviation{Hydrometr}{Hydrom}
\DefineJournalPartialAbbreviation{Hydrophysic}{Hydrophys}
\DefineJournalWordException{Hydroponic}{Hydroponic}
\DefineJournalWordException{Hydropower}{Hydropower}
\DefineJournalPartialAbbreviation{Hydroscienc}{Hydrosci}
\DefineJournalAbbreviation{Hydrospace}{Hydrosp}
\DefineJournalPartialAbbreviation{Hydrotechni}{Hydrotech}
\DefineJournalPartialAbbreviation{Hydrotransport}{Hydrotransp}
\DefineJournalPartialAbbreviation{Hygien}{Hyg}
\DefineJournalPartialAbbreviation{Hygroscop}{Hygrosc}
\DefineJournalWordException{Hymnody}{Hymnody}
\DefineJournalPartialAbbreviation{Hyperaliment}{Hyperaliment}
\DefineJournalPartialAbbreviation{Hyperfunction}{Hyperfunct}
\DefineJournalWordException{Hyperion}{Hyperion}
\DefineJournalAbbreviation{Hyperlipidaemia}{Hyperlipid}
\DefineJournalAbbreviation{Hypernuclear}{Hypernucl}
\DefineJournalPartialAbbreviation{Hyperreacti}{Hyperreact}
\DefineJournalPartialAbbreviation{Hypertensi}{Hypertens}
\DefineJournalAbbreviation{Hyperthermia}{Hyperth}
\DefineJournalPartialAbbreviation{Hypnoanal}{Hypnoanal}
\DefineJournalAbbreviation{Hypnosis}{Hypn}
\DefineJournalPartialAbbreviation{Hypnotherap}{Hypnother}
\DefineJournalPartialAbbreviation{Hypnoti}{Hypn}
\DefineJournalPartialAbbreviation{Hypotensi}{Hypotens}
\DefineJournalAbbreviation{Hysterectomy}{Hysterect}
\DefineJournalAbbreviation{Iatrogenic}{Iatrog}
\DefineJournalAbbreviation{Ibadan}{Ib}
\DefineJournalAbbreviation{Iberian}{Iber}
\DefineJournalWordException{Icefield}{Icefield}
\DefineJournalPartialAbbreviation{Iceland}{Icel}
\DefineJournalWordException{Icing}{Icing}
\DefineJournalPartialAbbreviation{Iconograph}{Iconogr}
\DefineJournalAbbreviation{Idaho}{Ida}
\DefineJournalAbbreviation{Idealistic}{Ideal}
\DefineJournalAbbreviation{Identification}{Identif}
%\DefineJournalPartialWordException{Identit}{Identit-}
\DefineJournalPartialAbbreviation{Ideolog}{Ideol}
\DefineJournalAbbreviation{Igalaland}{Igalal}
\DefineJournalWordException{Ileitis}{Ileitis}
\DefineJournalWordException{Illawarra}{Illawarra}
\DefineJournalAbbreviation{Illeteracy}{Illet}
\DefineJournalAbbreviation{Illinois}{Ill}
\DefineJournalAbbreviation{Illness}{Illn}
\DefineJournalPartialAbbreviation{Illuminat}{Illum}
\DefineJournalPartialAbbreviation{Ill\^ustr}{Illus}
\DefineJournalWordException{Ilorin}{Ilorin}
\DefineJournalAbbreviation{Imagery}{Imag}
\DefineJournalWordException{Imaging}{Imaging}
\DefineJournalWordException{Imbecile}{Imbecile}
\DefineJournalAbbreviation{Immigrant}{Immigr}
\DefineJournalAbbreviation{Immigration}{Immigr}
\DefineJournalPartialAbbreviation{Immobiliz}{Immobil}
\DefineJournalWordException{Immune}{Immune}
\DefineJournalAbbreviation{Immunisation}{Immun}
\DefineJournalAbbreviation{Immunity}{Immun}
\DefineJournalAbbreviation{Immunization}{Immun}
\DefineJournalPartialAbbreviation{Immunoalergol}{Immunoalergol}
\DefineJournalPartialAbbreviation{Immunoanaly}{Immunoanal}
\DefineJournalAbbreviation{Immunoassay}{Immunoass}
\DefineJournalPartialAbbreviation{Immunobiolog}{Immunobiol}
\DefineJournalPartialAbbreviation{Immunochemi}{Immunochem}
\DefineJournalAbbreviation{Immunoconjugate}{Immunoconjug}
\DefineJournalAbbreviation{Immunocytochemistry}{Immunocytochem}
\DefineJournalPartialAbbreviation{Immunodeficien}{Immunodefic}
\DefineJournalPartialAbbreviation{Immunodiagnos}{Immunodiagn}
\DefineJournalPartialAbbreviation{Immunofluorescen}{Immunofluoresc}
\DefineJournalAbbreviation{Immunogastroenterology}{Immunogastroenterol}
\DefineJournalPartialAbbreviation{Immunohematol}{Immunohematol}
\DefineJournalPartialAbbreviation{Immunohemotherap}{Immunohemother}
\DefineJournalPartialAbbreviation{Immunohistochemi}{Immunohistochem}
\DefineJournalPartialAbbreviation{Immunolog}{Immunol}
\DefineJournalPartialAbbreviation{Immunomicrobiolog}{Immunomicrobiol}
\DefineJournalPartialAbbreviation{Immunomodif}{Immunomodif}
\DefineJournalPartialAbbreviation{Immunopatholog}{Immunopathol}
\DefineJournalAbbreviation{Immunopeptid}{Immunopept}
\DefineJournalPartialAbbreviation{Immunopharmacolog}{Immunopharmacol}
\DefineJournalPartialAbbreviation{Immunoprophylax}{Immunoprophyl}
\DefineJournalPartialAbbreviation{Immunoregulat}{Immunoregul}
\DefineJournalPartialAbbreviation{Immunorehabilit}{Immunorehabil}
\DefineJournalPartialAbbreviation{Immunoreproducti}{Immunoreprod}
\DefineJournalPartialAbbreviation{Immunostimula}{Immunostimul}
\DefineJournalPartialAbbreviation{Immunosuppress}{Immunosuppr}
\DefineJournalAbbreviation{Immunosurveillance}{Immunosurveill}
\DefineJournalPartialAbbreviation{Immunotherap}{Immunother}
\DefineJournalPartialAbbreviation{Immunotoxicolog}{Immunotoxicol}
\DefineJournalWordException{Impact}{Impact}
\DefineJournalPartialAbbreviation{Impair}{Impair}
\DefineJournalWordException{Impala}{Impala}
\DefineJournalPartialAbbreviation{Implant}{Implant}
\DefineJournalWordException{Implement}{Implement}
\DefineJournalAbbreviation{Implementation}{Implement}
\DefineJournalAbbreviation{Implementing}{Implement}
\DefineJournalPartialAbbreviation{Implication}{Implic}
\DefineJournalWordException{Import}{Import}
\DefineJournalWordException{Important}{Important}
\DefineJournalPartialAbbreviation{Importat}{Import}
\DefineJournalWordException{Importcar}{Importcar}
\DefineJournalAbbreviation{Imported}{Import}
\DefineJournalPartialAbbreviation{Impos}{Impos}
\DefineJournalAbbreviation{Impotence}{Impot}
\DefineJournalPartialAbbreviation{Impound}{Impound}
\DefineJournalAbbreviation{Impression}{Impr}
\DefineJournalAbbreviation{Imprint}{Impr}
\DefineJournalPartialAbbreviation{Improv}{Improv}
\DefineJournalPartialAbbreviation{Impuls}{Impuls}
\DefineJournalWordException{Impulse}{Impulse}
\DefineJournalWordException{In-house}{In-house}
\DefineJournalPartialAbbreviation{Inactiv}{Inact}
\DefineJournalAbbreviation{Inaugural}{Inaug}
\DefineJournalWordException{Inboard}{Inboard}
\DefineJournalWordException{Inbound}{Inbound}
\DefineJournalPartialAbbreviation{Incapacit}{Incapac}
\DefineJournalPartialAbbreviation{Incarcerat}{Incarcer}
\DefineJournalWordException{Incite}{Incite}
\DefineJournalPartialAbbreviation{Inclin}{Inclin}
\DefineJournalPartialAbbreviation{Includ}{Incl}
\DefineJournalAbbreviation{Inclusive}{Incl}
\DefineJournalWordException{Income}{Income}
\DefineJournalPartialAbbreviation{Incompatibil}{Incompat}
\DefineJournalWordException{Increase}{Increase}
\DefineJournalPartialAbbreviation{Incred}{Incred}
\DefineJournalAbbreviation{Incremental}{Increm}
\DefineJournalAbbreviation{Incurred}{Incur}
\DefineJournalAbbreviation{Incursion}{Incurs}
\DefineJournalPartialAbbreviation{Indagation}{Indag}
\DefineJournalAbbreviation{Indebtedness}{Indebt}
\DefineJournalAbbreviation{Indemnification}{Indemnif}
\DefineJournalAbbreviation{Independent}{Indep}
\DefineJournalAbbreviation{Indexation}{Index}
\DefineJournalAbbreviation{Indexed}{Index}
\DefineJournalAbbreviation{Indexer}{Index}
\DefineJournalAbbreviation{Indexing}{Index}
\DefineJournalWordException{Indian}{Indian}
\DefineJournalWordException{Indiana}{Indiana}
\DefineJournalAbbreviation{Indianapolis}{Indianap}
\DefineJournalPartialAbbreviation{Indicat}{Indic}
\DefineJournalAbbreviation{Indictable}{Indict}
\DefineJournalPartialAbbreviation{Indigen}{Indig}
\DefineJournalWordException{Indium}{Indium}
\DefineJournalPartialAbbreviation{Individual}{Individ}
\DefineJournalAbbreviation{Indochemical}{Indochem}
\DefineJournalAbbreviation{Indochina}{Indoch}
\DefineJournalAbbreviation{Indological}{Indol}
\DefineJournalWordException{Indoor}{Indoor}
\DefineJournalWordException{Indooroopilly}{Indooroopilly}
\DefineJournalAbbreviation{Induced}{Induc}
\DefineJournalAbbreviation{Inebriety}{Inebr}
\DefineJournalAbbreviation{Inelastic}{Inelast}
\DefineJournalAbbreviation{Inequality}{Inequal}
\DefineJournalAbbreviation{Inertial}{Inert}
\DefineJournalWordException{Infancy}{Infancy}
\DefineJournalWordException{Infant}{Infant}
\DefineJournalPartialAbbreviation{Infantil}{Infant}
\DefineJournalWordException{Infantry}{Infantry}
\DefineJournalAbbreviation{Infarction}{Infarct}
\DefineJournalPartialAbbreviation{Infecti}{Infect}
\DefineJournalWordException{Inference}{Inference}
\DefineJournalPartialAbbreviation{Inferent}{Inferent}
\DefineJournalPartialAbbreviation{Inferior}{Infer}
\DefineJournalWordException{Inferno}{Inferno}
\DefineJournalPartialAbbreviation{Infertilit}{Infertil}
\DefineJournalAbbreviation{Infestation}{Infest}
\DefineJournalPartialAbbreviation{Infirm}{Infirm}
\DefineJournalAbbreviation{Inflammation}{Inflamm}
\DefineJournalAbbreviation{Inflammatory}{Inflamm}
\DefineJournalAbbreviation{Inflation}{Inflat}
\DefineJournalWordException{Inflight}{Inflight}
\DefineJournalPartialAbbreviation{Influen}{Influ}
\DefineJournalWordException{Influenza}{Influenza}
\DefineJournalWordException{Infocus}{Infocus}
\DefineJournalPartialAbbreviation{Infoletter}{Infolett}
\DefineJournalAbbreviation{Inform}{Inf}
\DefineJournalWordException{Informal}{Informal}
\DefineJournalAbbreviation{Informant}{Inf}
\DefineJournalAbbreviation{Informatic}{Inform}
\DefineJournalPartialAbbreviation{Informativ}{Inf}
\DefineJournalPartialAbbreviation{Informator}{Inf}
\DefineJournalAbbreviation{Informetric}{Informetr}
\DefineJournalAbbreviation{Infoscience}{Infosci}
\DefineJournalAbbreviation{Infotainment}{Infotain}
\DefineJournalPartialAbbreviation{Inframicrobiolog}{Inframicrobiol}
\DefineJournalWordException{Infrared}{Infrared}
\DefineJournalAbbreviation{Ingenuity}{Ingen}
\DefineJournalAbbreviation{Inglewood}{Inglew}
\DefineJournalWordException{Ingram}{Ingram}
\DefineJournalAbbreviation{Ingredient}{Ingred}
\DefineJournalPartialAbbreviation{Inhala}{Inhal}
\DefineJournalWordException{Inhaled}{Inhaled}
\DefineJournalAbbreviation{Inheritance}{Inherit}
\DefineJournalAbbreviation{Inherited}{Inherit}
\DefineJournalWordException{Inhouse}{Inhouse}
\DefineJournalPartialAbbreviation{Inject}{Inject}
\DefineJournalPartialAbbreviation{Injur}{Inj}
\DefineJournalWordException{Inkberrow}{Inkberrow}
\DefineJournalPartialAbbreviation{Inkmak}{Inkmak}
\DefineJournalWordException{Inland}{Inland}
\DefineJournalAbbreviation{Inlander}{Inland}
\DefineJournalPartialAbbreviation{Inlight}{Inlight}
\DefineJournalWordException{Inmate}{Inmate}
\DefineJournalPartialAbbreviation{Inner}{Inn}
\DefineJournalWordException{Inning}{Inning}
\DefineJournalPartialAbbreviation{Innkeep}{Innkeep}
\DefineJournalAbbreviation{Inorganic}{Inorg}
\DefineJournalAbbreviation{Inositides}{Inosit}
\DefineJournalWordException{Inotropes}{Inotropes}
\DefineJournalWordException{Inpatient}{Inpatient}
\DefineJournalAbbreviation{Inquest}{Inq}
\DefineJournalPartialAbbreviation{Inquir}{Inq}
\DefineJournalPartialAbbreviation{Inrichting}{Inricht}
\DefineJournalWordException{Insect}{Insect}
\DefineJournalPartialAbbreviation{Insecticide}{Insectic}
\DefineJournalPartialAbbreviation{Insectofungicid}{Insectofungic}
\DefineJournalAbbreviation{Insemination}{Insemin}
\DefineJournalWordException{Insert}{Insert}
\DefineJournalAbbreviation{Inservice}{Inserv}
\DefineJournalWordException{Inshore}{Inshore}
\DefineJournalPartialAbbreviation{Insid}{Insid}
\DefineJournalWordException{Inside}{Inside}
\DefineJournalWordException{Insight}{Insight}
\DefineJournalAbbreviation{Insignia}{Insign}
\DefineJournalAbbreviation{Insolvency}{Insolv}
\DefineJournalPartialAbbreviation{Inspect}{Insp}
\DefineJournalAbbreviation{Inspirator}{Inspir}
\DefineJournalPartialAbbreviation{Instabilit}{Instab}
\DefineJournalAbbreviation{Instalment}{Instalm}
\DefineJournalWordException{Instant}{Instant}
\DefineJournalPartialAbbreviation{Instantane}{Instant}
\DefineJournalAbbreviation{Institute}{Inst}
\DefineJournalWordException{Instream}{Instream}
\DefineJournalPartialAbbreviation{Instruct}{Instr}
\DefineJournalAbbreviation{Instrument}{Instrum}
\DefineJournalPartialAbbreviation{Instrumental}{Instrum}
\DefineJournalAbbreviation{Instrumentation}{Instrum}
\DefineJournalPartialAbbreviation{Insur}{Insur}
\DefineJournalAbbreviation{Insurgent}{Insurg}
\DefineJournalAbbreviation{Insurrectionary}{Insurrect}
\DefineJournalWordException{Intarsia}{Intarsia}
\DefineJournalAbbreviation{Integrated}{Integr}
\DefineJournalAbbreviation{Integrative}{Integr}
\DefineJournalPartialAbbreviation{Integrator}{Integr}
\DefineJournalAbbreviation{Integrity}{Integr}
\DefineJournalAbbreviation{Intellectual}{Intellect}
\DefineJournalPartialAbbreviation{Intelligenc}{Intell}
\DefineJournalAbbreviation{Intended}{Intend}
\DefineJournalAbbreviation{Intendent}{Intend}
\DefineJournalAbbreviation{Intending}{Intend}
\DefineJournalWordException{Intense}{Intense}
\DefineJournalAbbreviation{Intensification}{Intensif}
\DefineJournalWordException{Intensive}{Intensive}
\DefineJournalAbbreviation{Intention}{Intent}
\DefineJournalAbbreviation{Interacting}{Interact}
\DefineJournalAbbreviation{Interaction}{Interact}
\DefineJournalAbbreviation{Interactive}{Interact}
\DefineJournalPartialAbbreviation{Interafrica}{Interafr}
\DefineJournalAbbreviation{Interagency}{Interag}
\DefineJournalAbbreviation{Interatomic}{Interat}
\DefineJournalWordException{Intercargo}{Intercargo}
\DefineJournalAbbreviation{Intercellular}{Intercell}
\DefineJournalPartialAbbreviation{Intercept}{Intercept}
\DefineJournalPartialAbbreviation{Intercess}{Intercess}
\DefineJournalWordException{Interchange}{Interchange}
\DefineJournalAbbreviation{Interchemical}{Interchem}
\DefineJournalWordException{Interchurch}{Interchurch}
\DefineJournalWordException{Intercity}{Intercity}
\DefineJournalAbbreviation{Intercollegiate}{Intercoll}
\DefineJournalAbbreviation{Intercomparison}{Intercomp}
\DefineJournalWordException{Interconnect}{Interconnect}
\DefineJournalAbbreviation{Interconnection}{Interconnect}
\DefineJournalAbbreviation{Interconversion}{Interconvers}
\DefineJournalPartialAbbreviation{Intercrystall}{Intercryst}
\DefineJournalPartialAbbreviation{Intercultur}{Intercult}
\DefineJournalWordException{Interdata}{Interdata}
\DefineJournalAbbreviation{Interdenominational}{Interdenominatl}
\DefineJournalPartialAbbreviation{Interdepartment}{Interdep}
\DefineJournalPartialAbbreviation{Interdependenc}{Interdepend}
\DefineJournalAbbreviation{Interdiffusion}{Interdiffus}
\DefineJournalPartialAbbreviation{Interdisciplin}{Interdiscip}
\DefineJournalWordException{Interest}{Interest}
\DefineJournalAbbreviation{Interested}{Interest}
\DefineJournalWordException{Interface}{Interface}
\DefineJournalWordException{Interfacial}{Interfacial}
\DefineJournalWordException{Interfaith}{Interfaith}
\DefineJournalPartialAbbreviation{Interfer}{Interf}
\DefineJournalPartialAbbreviation{Interferometr}{Interferom}
\DefineJournalPartialAbbreviation{Intergovernement}{Intergov}
\DefineJournalPartialAbbreviation{Intergovernment}{Intergov}
\DefineJournalWordException{Interights}{Interights}
\DefineJournalAbbreviation{Interlaboratory}{Interlab}
\DefineJournalWordException{Interlake}{Interlake}
\DefineJournalAbbreviation{Interlanguage}{Interlang}
\DefineJournalAbbreviation{Interlending}{Interlend}
\DefineJournalWordException{Interline}{Interline}
\DefineJournalWordException{Interloan}{Interloan}
\DefineJournalPartialAbbreviation{Intermediate}{Intermed}
\DefineJournalPartialAbbreviation{Intermetalli}{Intermet}
\DefineJournalAbbreviation{Intermountain}{Intermt}
\DefineJournalWordException{Intern}{Intern}
\DefineJournalAbbreviation{Internal}{Intern}
\DefineJournalPartialAbbreviation{Internation}{Int}
\DefineJournalWordException{Internet}{Internet}
\DefineJournalAbbreviation{Internship}{Internsh}
\DefineJournalPartialAbbreviation{Interparlement}{Interparlem}
\DefineJournalPartialAbbreviation{Interpenetrat}{Interpenetr}
\DefineJournalAbbreviation{Interpersonal}{Interpers}
\DefineJournalPartialAbbreviation{Interphotorecept}{Interphotorecept}
\DefineJournalAbbreviation{Interplanetary}{Interplanet}
\DefineJournalPartialAbbreviation{Interplastic}{Interplast}
\DefineJournalAbbreviation{Interpolation}{Interpolat}
\DefineJournalPartialAbbreviation{Interprovinc}{Interprov}
\DefineJournalPartialAbbreviation{Interregion}{Interreg}
\DefineJournalPartialAbbreviation{Interrelation}{Interrelat}
\DefineJournalAbbreviation{Interreligious}{Interrelig}
\DefineJournalAbbreviation{Interscience}{Intersci}
\DefineJournalAbbreviation{Interservice}{Interserv}
\DefineJournalAbbreviation{Intersociety}{Intersoc}
\DefineJournalWordException{Interstate}{Interstate}
\DefineJournalPartialAbbreviation{Interstud}{Interstud}
\DefineJournalWordException{Interstudy}{Interstudy}
\DefineJournalAbbreviation{Intersyndical}{Intersynd}
\DefineJournalWordException{Intertrade}{Intertrade}
\DefineJournalWordException{Intertravel}{Intertravel}
\DefineJournalPartialAbbreviation{Interuniversit}{Interuniv}
\DefineJournalWordException{Interwader}{Interwader}
\DefineJournalWordException{Interweave}{Interweave}
\DefineJournalAbbreviation{Intimacy}{Intim}
\DefineJournalPartialAbbreviation{Intimat}{Intim}
\DefineJournalAbbreviation{Intimate}{Intim}
\DefineJournalAbbreviation{Intolerant}{Intoler}
\DefineJournalPartialAbbreviation{Intoxicat}{Intox}
\DefineJournalAbbreviation{Intracellular}{Intracell}
\DefineJournalPartialAbbreviation{Intracontinent}{Intracont}
\DefineJournalPartialAbbreviation{Intramolecul}{Intramol}
\DefineJournalWordException{Intrastate}{Intrastate}
\DefineJournalAbbreviation{Intrauterine}{Intrauter}
\DefineJournalPartialAbbreviation{Intravascul}{Intravasc}
\DefineJournalPartialAbbreviation{Intraven}{Intraven}
\DefineJournalPartialAbbreviation{Introduc}{Introd}
\DefineJournalPartialAbbreviation{Introspec}{Introsp}
\DefineJournalWordException{Intrude}{Intrude}
\DefineJournalWordException{Invasion}{Invasion}
\DefineJournalWordException{Invasive}{Invasive}
\DefineJournalWordException{Invent}{Invent}
\DefineJournalAbbreviation{Inventing}{Invent}
\DefineJournalPartialAbbreviation{Invention}{Invent}
\DefineJournalPartialAbbreviation{Inventor}{Invent}
\DefineJournalWordException{Inventory}{Inventory}
\DefineJournalWordException{Invercargill}{Invercargill}
\DefineJournalWordException{Inverness}{Inverness}
\DefineJournalWordException{Inverse}{Inverse}
\DefineJournalPartialAbbreviation{Invertebrat}{Invertebr}
\DefineJournalAbbreviation{Inverted}{Invert}
\DefineJournalAbbreviation{Inverter}{Invert}
\DefineJournalWordException{Invest}{Invest}
\DefineJournalAbbreviation{Investing}{Invest}
\DefineJournalAbbreviation{Investment}{Invest}
\DefineJournalAbbreviation{Investor}{Invest}
\DefineJournalWordException{Invicta}{Invicta}
\DefineJournalAbbreviation{Invisible}{Invis}
\DefineJournalPartialAbbreviation{Invit}{Invit}
\DefineJournalWordException{Invoice}{Invoice}
\DefineJournalPartialAbbreviation{Involv}{Involv}
\DefineJournalAbbreviation{Involvement}{Involv}
\DefineJournalWordException{Iodine}{Iodine}
\DefineJournalPartialAbbreviation{Ioniz}{Ioniz}
\DefineJournalPartialAbbreviation{Ionospher}{Ionos}
\DefineJournalWordException{Ipswich}{Ipswich}
\DefineJournalWordException{Iraqi}{Iraqi}
\DefineJournalAbbreviation{Ireland}{Irel}
\DefineJournalAbbreviation{Irish}{Ir}
\DefineJournalPartialAbbreviation{Irland}{Irl}
\DefineJournalWordException{Ironic}{Ironic}
\DefineJournalAbbreviation{Ironmaking}{Ironmak}
\DefineJournalAbbreviation{Ironworker}{Ironwork}
\DefineJournalAbbreviation{Iroquoian}{Iroq}
\DefineJournalAbbreviation{Irradiated}{Irradiat}
\DefineJournalAbbreviation{Irradiation}{Irradiat}
\DefineJournalAbbreviation{Irregular}{Irregul}
\DefineJournalWordException{Irving}{Irving}
\DefineJournalWordException{Irvington}{Irvington}
\DefineJournalAbbreviation{Ischaemia}{Ischaem}
\DefineJournalAbbreviation{Ischaemic}{Ischaem}
\DefineJournalWordException{Isles}{Isles}
\DefineJournalWordException{Isleworth}{Isleworth}
\DefineJournalWordException{Islington}{Islington}
\DefineJournalAbbreviation{Isochronous}{Isochron}
\DefineJournalPartialAbbreviation{Isoelectroni}{Isoelectron}
\DefineJournalAbbreviation{Isokinetics}{Isokinet}
\DefineJournalPartialAbbreviation{Isolat}{Isol}
\DefineJournalWordException{Isozyme}{Isozyme}
\DefineJournalWordException{Issue}{Issue}
\DefineJournalWordException{Issued}{Issued}
\DefineJournalAbbreviation{Issuing}{Issu}
\DefineJournalWordException{Italy}{Italy}
%\DefineJournalPartialWordException{Item}{Item-}
\DefineJournalWordException{Ithaca}{Ithaca}
\DefineJournalWordException{Ivory}{Ivory}
\DefineJournalWordException{Jabbering}{Jabbering}
\DefineJournalWordException{Jacket}{Jacket}
\DefineJournalWordException{Jackson}{Jackson}
\DefineJournalAbbreviation{Jacksonville}{Jacksonv}
\DefineJournalWordException{Jaipur}{Jaipur}
\DefineJournalPartialAbbreviation{Jamaica}{Jam}
\DefineJournalWordException{Jammu}{Jammu}
\DefineJournalPartialAbbreviation{Japan}{Jpn}
\DefineJournalPartialAbbreviation{Jazzolog}{Jazzol}
\DefineJournalWordException{Jeddah}{Jeddah}
\DefineJournalWordException{Jefferson-City}{Jefferson-City}
\DefineJournalAbbreviation{Jenkintown}{Jenkint}
\DefineJournalWordException{Jerramungup}{Jerramungup}
\DefineJournalWordException{Jersey}{Jersey}
\DefineJournalAbbreviation{Jerusalem}{Jerus}
\DefineJournalAbbreviation{Jetting}{Jet}
\DefineJournalPartialAbbreviation{Jewel}{Jewel}
\DefineJournalAbbreviation{Jewish}{Jew}
\DefineJournalAbbreviation{Jewry}{Jew}
\DefineJournalWordException{Jindabyne}{Jindabyne}
\DefineJournalWordException{Jingle}{Jingle}
\DefineJournalWordException{Jobber}{Jobber}
\DefineJournalAbbreviation{Jobcentre}{Jobcent}
\DefineJournalAbbreviation{Jobholding}{Jobhold}
\DefineJournalAbbreviation{Jobseeker}{Jobseek}
\DefineJournalWordException{Jockey}{Jockey}
\DefineJournalAbbreviation{Jogger}{Jog}
\DefineJournalAbbreviation{Jogging}{Jog}
\DefineJournalAbbreviation{Johannesburg}{Johannesbg}
\DefineJournalAbbreviation{Johnson}{Johns}
\DefineJournalAbbreviation{Joinery}{Join}
\DefineJournalAbbreviation{Joining}{Join}
\DefineJournalAbbreviation{Joint}{Jt}
\DefineJournalAbbreviation{Jointing}{Jt}
\DefineJournalWordException{Joker}{Joker}
\DefineJournalWordException{Jonapher}{Jonapher}
\DefineJournalWordException{Jordan}{Jordan}
\DefineJournalAbbreviation{Jotting}{Jott}
\DefineJournalAbbreviation{Journal}{J}
\DefineJournalAbbreviation{Journalist}{Journal}
\DefineJournalWordException{Journey}{Journey}
\DefineJournalAbbreviation{Joyful}{Joyf}
\DefineJournalAbbreviation{Jubilee}{Jubil}
\DefineJournalAbbreviation{Judaic}{Jud}
\DefineJournalPartialAbbreviation{Judaism}{Jud}
\DefineJournalAbbreviation{Judging}{Judg}
\DefineJournalAbbreviation{Judgment}{Judgm}
\DefineJournalAbbreviation{Judicature}{Judic}
\DefineJournalPartialAbbreviation{Judicia}{Judic}
\DefineJournalAbbreviation{Jugendrecht}{Jugendr}
\DefineJournalPartialAbbreviation{Juggl}{Juggl}
\DefineJournalPartialAbbreviation{Jump}{Jump}
\DefineJournalWordException{Junction}{Junction}
\DefineJournalWordException{Juneau}{Juneau}
\DefineJournalAbbreviation{Junior}{Jr}
\DefineJournalAbbreviation{Jurassic}{Jurass}
\DefineJournalAbbreviation{Jurimetric}{Jurimetr}
\DefineJournalPartialAbbreviation{Jurisdiction}{Jurisd}
\DefineJournalWordException{Justice}{Justice}
\DefineJournalAbbreviation{Justification}{Justif}
\DefineJournalPartialAbbreviation{Juvenil}{Juv}
\DefineJournalWordException{Kadina}{Kadina}
\DefineJournalAbbreviation{Kaduna}{Kad}
\DefineJournalWordException{Kalahandi}{Kalahandi}
\DefineJournalWordException{Kalamazoo}{Kalamazoo}
\DefineJournalWordException{Kalgoorlie}{Kalgoorlie}
\DefineJournalWordException{Kamloops}{Kamloops}
\DefineJournalWordException{Kampala}{Kampala}
\DefineJournalWordException{Kanaky}{Kanaky}
\DefineJournalWordException{Kananaskis}{Kananaskis}
\DefineJournalWordException{Kanata}{Kanata}
\DefineJournalWordException{Kanawake}{Kanawake}
\DefineJournalWordException{Kangaroo}{Kangaroo}
\DefineJournalAbbreviation{Kansas}{Kans}
\DefineJournalWordException{Karachi}{Karachi}
\DefineJournalWordException{Karnataka}{Karnataka}
\DefineJournalWordException{Karting}{Karting}
\DefineJournalWordException{Kashmir}{Kashmir}
\DefineJournalPartialAbbreviation{Katedr}{Kat\textlefthalfring edr}
\DefineJournalWordException{Kathmandu}{Kathmandu}
\DefineJournalWordException{Kawartha}{Kawartha}
\DefineJournalPartialAbbreviation{Kayak}{Kayak}
\DefineJournalAbbreviation{Kayaker}{Kayak}
\DefineJournalAbbreviation{Kayaking}{Kayak}
\DefineJournalWordException{Keeleyside}{Keeleyside}
\DefineJournalAbbreviation{Keeper}{Keep}
\DefineJournalAbbreviation{Keeping}{Keep}
\DefineJournalWordException{Kelowna}{Kelowna}
\DefineJournalAbbreviation{Kelvington}{Kelvingt}
\DefineJournalAbbreviation{Kemptville}{Kemptv}
\DefineJournalWordException{Kenilworth}{Kenilworth}
\DefineJournalWordException{Kennebecasis}{Kennebecasis}
\DefineJournalWordException{Kensington}{Kensington}
\DefineJournalAbbreviation{Kentucky}{Ky}
\DefineJournalAbbreviation{Kentville}{Kentv}
\DefineJournalWordException{Kenya}{Kenya}
\DefineJournalWordException{Kenyon}{Kenyon}
\DefineJournalWordException{Keonjhar}{Keonjhar}
\DefineJournalWordException{Kerala}{Kerala}
\DefineJournalAbbreviation{Kerato-refractive}{Kerato-refract}
\DefineJournalWordException{Kernel}{Kernel}
\DefineJournalWordException{Kerosine}{Kerosine}
\DefineJournalWordException{Keston}{Keston}
\DefineJournalWordException{Kettle}{Kettle}
\DefineJournalWordException{Key-word}{Key-word}
\DefineJournalWordException{Keyboard}{Keyboard}
\DefineJournalAbbreviation{Keynesian}{Keynes}
\DefineJournalWordException{Keynote}{Keynote}
\DefineJournalWordException{Keypsake}{Keypsake}
\DefineJournalAbbreviation{Keystone}{Keyst}
\DefineJournalWordException{Keyword}{Keyword}
\DefineJournalWordException{Khartoum}{Khartoum}
\DefineJournalAbbreviation{Khedivial}{Khediv}
\DefineJournalWordException{Kiama}{Kiama}
\DefineJournalWordException{Kickoff}{Kickoff}
\DefineJournalWordException{Kiddie}{Kiddie}
\DefineJournalWordException{Kidney}{Kidney}
\DefineJournalWordException{Kidsguide}{Kidsguide}
\DefineJournalWordException{Kildare}{Kildare}
\DefineJournalWordException{Kilkenny}{Kilkenny}
\DefineJournalPartialAbbreviation{Kill}{Kill}
\DefineJournalWordException{Killaloe}{Killaloe}
\DefineJournalWordException{Killifish}{Killifish}
\DefineJournalWordException{Kilmacduagh}{Kilmacduagh}
\DefineJournalWordException{Kilmore}{Kilmore}
\DefineJournalWordException{Kilobaud}{Kilobaud}
\DefineJournalWordException{Kimberley}{Kimberley}
\DefineJournalAbbreviation{Kimberlite}{Kimberl}
\DefineJournalWordException{Kindness}{Kindness}
\DefineJournalWordException{Kindred}{Kindred}
\DefineJournalAbbreviation{Kinematics}{Kinemat}
\DefineJournalPartialAbbreviation{Kinesiol}{Kinesiol}
\DefineJournalAbbreviation{Kinesiology}{Kinesiol}
\DefineJournalAbbreviation{Kingdom}{Kingd}
\DefineJournalWordException{Kings Ripton}{Kings Ripton}
\DefineJournalAbbreviation{Kingsto(w)n}{Kingst}
\DefineJournalAbbreviation{Kingsville}{Kingsv}
\DefineJournalWordException{Kingswood}{Kingswood}
\DefineJournalWordException{Kinross}{Kinross}
\DefineJournalAbbreviation{Kinship}{Kinsh}
\DefineJournalAbbreviation{Kinsman}{Kinsm}
\DefineJournalWordException{Kinvara}{Kinvara}
\DefineJournalWordException{Kipling}{Kipling}
\DefineJournalWordException{Kiplinger}{Kiplinger}
\DefineJournalAbbreviation{Kirchenmusikalisch}{Kirchenmusik}
\DefineJournalAbbreviation{Kirkland}{Kirkl}
\DefineJournalAbbreviation{Kirksville}{Kirksv}
\DefineJournalAbbreviation{Kirkwood}{Kirkw}
\DefineJournalWordException{Kitcar}{Kitcar}
\DefineJournalWordException{Kitchen}{Kitchen}
\DefineJournalWordException{Kitchener}{Kitchener}
\DefineJournalWordException{Kitsch}{Kitsch}
\DefineJournalWordException{Kiwifruit}{Kiwifruit}
\DefineJournalWordException{Klaxon}{Klaxon}
\DefineJournalWordException{Kneehill}{Kneehill}
\DefineJournalPartialAbbreviation{Knitt}{Knitt}
\DefineJournalPartialAbbreviation{Knitwear}{Knitw}
\DefineJournalWordException{Knocknagoshel}{Knocknagoshel}
\DefineJournalAbbreviation{Knowledge}{Knowl}
\DefineJournalAbbreviation{Knowlton}{Knowlt}
\DefineJournalAbbreviation{Knoxville}{Knoxv}
\DefineJournalWordException{Kohima}{Kohima}
\DefineJournalWordException{Kootenay}{Kootenay}
\DefineJournalWordException{Korean}{Korean}
\DefineJournalPartialAbbreviation{Koreanolog}{Koreanol}
\DefineJournalWordException{Kosher}{Kosher}
\DefineJournalAbbreviation{Kronicle}{Kron}
\DefineJournalWordException{Kumquat}{Kumquat}
\DefineJournalWordException{Kunamurra}{Kunamurra}
\DefineJournalAbbreviation{Kurdish}{Kurd}
\DefineJournalWordException{Kuwait}{Kuwait}
\DefineJournalWordException{Kuwaiti}{Kuwaiti}
\DefineJournalWordException{Kwara}{Kwara}
\DefineJournalWordException{Kyungpook}{Kyungpook}
\DefineJournalAbbreviation{Labanotation}{Labanot}
\DefineJournalAbbreviation{Labelled}{Label}
\DefineJournalAbbreviation{Labelling}{Label}
\DefineJournalWordException{Labour}{Labour}
\DefineJournalWordException{Labrador}{Labrador}
\DefineJournalAbbreviation{Lacanian}{Lacan}
\DefineJournalAbbreviation{Lacemaker}{Lacemak}
\DefineJournalWordException{Lackwanna}{Lackwanna}
\DefineJournalAbbreviation{Lacquer}{Lacq}
\DefineJournalPartialAbbreviation{Lact}{Lact}
\DefineJournalAbbreviation{Lactogenic}{Lactog}
\DefineJournalPartialAbbreviation{Lactolog}{Lactol}
\DefineJournalWordException{Ladybug}{Ladybug}
\DefineJournalWordException{Lagos}{Lagos}
\DefineJournalWordException{Lahore}{Lahore}
\DefineJournalWordException{Lakefield}{Lakefield}
\DefineJournalAbbreviation{Lakeland}{Lakel}
\DefineJournalWordException{Lakeshore}{Lakeshore}
\DefineJournalAbbreviation{Laketown}{Laket}
\DefineJournalWordException{Lamaze}{Lamaze}
\DefineJournalAbbreviation{Lambton}{Lambt}
\DefineJournalWordException{Lamont-Doherty}{Lamont-Doherty}
\DefineJournalWordException{Lampeter}{Lampeter}
\DefineJournalWordException{Lampoon}{Lampoon}
\DefineJournalWordException{Lanark}{Lanark}
\DefineJournalAbbreviation{Lancashire}{Lancs}
\DefineJournalAbbreviation{Lancaster}{Lanc}
\DefineJournalWordException{Lancet}{Lancet}
\DefineJournalWordException{Land}{Land}
\DefineJournalAbbreviation{Landesverein}{Landesver}
\DefineJournalWordException{Landfall}{Landfall}
\DefineJournalAbbreviation{Landform}{Landf}
\DefineJournalAbbreviation{Landing}{Land}
\DefineJournalWordException{Landline}{Landline}
\DefineJournalWordException{Landlord}{Landlord}
\DefineJournalWordException{Landmark}{Landmark}
\DefineJournalAbbreviation{Landowning}{Landown}
\DefineJournalPartialAbbreviation{Landrac}{Landrac}
\DefineJournalWordException{Landrace}{Landrace}
\DefineJournalWordException{Landsat}{Landsat}
\DefineJournalAbbreviation{Landscape}{Landsc}
\DefineJournalAbbreviation{Landward}{Landw}
\DefineJournalWordException{Langley}{Langley}
\DefineJournalPartialAbbreviation{Language}{Lang}
\DefineJournalWordException{Lansdowne}{Lansdowne}
\DefineJournalWordException{Lansing}{Lansing}
\DefineJournalWordException{Lanslide}{Lanslide}
\DefineJournalWordException{Lantern}{Lantern}
\DefineJournalAbbreviation{Lanthanide}{Lanthan}
\DefineJournalPartialAbbreviation{Laparoendoscop}{Laparoendosc}
\DefineJournalAbbreviation{Laparoscopic}{Laparosc}
\DefineJournalPartialAbbreviation{Laparoscopy}{Laparosc}
\DefineJournalAbbreviation{Lapidary}{Lapid}
\DefineJournalWordException{Laptop}{Laptop}
\DefineJournalAbbreviation{Laramie}{Laram}
\DefineJournalAbbreviation{Larchmont}{Larchmt}
\DefineJournalAbbreviation{Larger}{Larg}
\DefineJournalAbbreviation{Largest}{Larg}
\DefineJournalWordException{Larkspur}{Larkspur}
\DefineJournalAbbreviation{Larviculture}{Larvic}
\DefineJournalWordException{Las Vegas}{Las Vegas}
\DefineJournalWordException{Lasercorp}{Lasercorp}
\DefineJournalWordException{Laserdisk}{Laserdisk}
\DefineJournalWordException{Lateral}{Lateral}
\DefineJournalWordException{Lateritisation}{Lateritisation}
\DefineJournalWordException{Latest}{Latest}
\DefineJournalAbbreviation{Latin}{Lat}
\DefineJournalWordException{Lattice}{Lattice}
\DefineJournalPartialAbbreviation{Latv}{Latv}
\DefineJournalPartialAbbreviation{Laugh}{Laugh}
\DefineJournalWordException{Launceston}{Launceston}
\DefineJournalWordException{Launch}{Launch}
\DefineJournalPartialAbbreviation{Laund}{Laund}
\DefineJournalWordException{Laurel}{Laurel}
\DefineJournalAbbreviation{Laurentian}{Laurent}
\DefineJournalWordException{Lavender}{Lavender}
\DefineJournalWordException{Lawrence}{Lawrence}
\DefineJournalWordException{Lawsuit}{Lawsuit}
\DefineJournalWordException{Lawyer}{Lawyer}
\DefineJournalAbbreviation{Layered}{Layer}
\DefineJournalAbbreviation{Laying}{Lay}
\DefineJournalWordException{Layman}{Layman}
\DefineJournalWordException{Layout}{Layout}
\DefineJournalAbbreviation{Leader}{Lead}
\DefineJournalAbbreviation{Leadership}{Leadersh}
\DefineJournalAbbreviation{Leading}{Lead}
\DefineJournalPartialAbbreviation{Leaflet}{Leafl}
\DefineJournalAbbreviation{League}{Leag}
\DefineJournalAbbreviation{Leaking}{Leak}
\DefineJournalPartialAbbreviation{Learn}{Learn}
\DefineJournalWordException{Lease}{Lease}
\DefineJournalAbbreviation{Leasehold}{Leaseh}
\DefineJournalAbbreviation{Leasing}{Leas}
\DefineJournalWordException{Leather}{Leather}
\DefineJournalWordException{Leathercraft}{Leathercraft}
\DefineJournalWordException{Leathergood}{Leathergood}
\DefineJournalAbbreviation{Leaver}{Leav}
\DefineJournalWordException{Leaves}{Leaves}
\DefineJournalAbbreviation{Lebanese}{Leban}
\DefineJournalAbbreviation{Lebanon}{Leban}
\DefineJournalWordException{Lectin}{Lectin}
\DefineJournalAbbreviation{Lectionary}{Lection}
\DefineJournalPartialAbbreviation{Lectur}{Lect}
\DefineJournalAbbreviation{Lectureship}{Lecturesh}
\DefineJournalWordException{Ledger}{Ledger}
\DefineJournalAbbreviation{Legacy}{Leg}
\DefineJournalPartialAbbreviation{Legal}{Leg}
\DefineJournalPartialAbbreviation{Legend}{Legend}
\DefineJournalPartialAbbreviation{L\'egion}{Legion}
\DefineJournalAbbreviation{Leicester}{Leic}
\DefineJournalAbbreviation{Leicestershire}{Leics}
\DefineJournalPartialAbbreviation{Leisur}{Leis}
\DefineJournalAbbreviation{Leisurewear}{Leisurew}
\DefineJournalWordException{Leitrim}{Leitrim}
\DefineJournalWordException{Lelemedia}{Lelemedia}
\DefineJournalAbbreviation{Lending}{Lend}
\DefineJournalWordException{Length}{Length}
\DefineJournalWordException{Lenkotriene}{Lenkotriene}
\DefineJournalWordException{Lennox}{Lennox}
\DefineJournalAbbreviation{Lennoxville}{Lennoxv}
\DefineJournalAbbreviation{Leprosy}{Lepr}
\DefineJournalWordException{Leptospirosis}{Leptospirosis}
\DefineJournalWordException{Lesbian}{Lesbian}
\DefineJournalWordException{Lesion}{Lesion}
\DefineJournalAbbreviation{Leslieville}{Lesliev}
\DefineJournalWordException{Lesser}{Lesser}
\DefineJournalWordException{Lesser Slave Lake}{Lesser Slave Lake}
\DefineJournalWordException{Lesson}{Lesson}
\DefineJournalWordException{Letchmore Heath}{Letchmore Heath}
\DefineJournalWordException{Lethbridge}{Lethbridge}
\DefineJournalPartialAbbreviation{Letter}{Lett}
\DefineJournalPartialAbbreviation{Leukaemogenes}{Leukaemog}
\DefineJournalAbbreviation{Leukemogenesis}{Leukemogenes}
\DefineJournalAbbreviation{Leukocyte}{Leukoc}
\DefineJournalPartialAbbreviation{Leukotri}{Leukot}
\DefineJournalWordException{Lev\'el}{Lev\'el}
%\DefineJournalPartialWordException{Leverag}{Leverag-}
\DefineJournalWordException{Levied}{Levied}
\DefineJournalAbbreviation{Lexicography}{Lexicogr}
\DefineJournalAbbreviation{Lexington}{Lexingt}
\DefineJournalAbbreviation{Liability}{Liabil}
\DefineJournalPartialAbbreviation{Liberal}{Lib}
\DefineJournalAbbreviation{Liberator}{Lib}
\DefineJournalWordException{Liberian}{Liberian}
\DefineJournalAbbreviation{Libertarian}{Libert}
\DefineJournalAbbreviation{Liberty}{Lib}
\DefineJournalPartialAbbreviation{Librar}{Libr}
\DefineJournalAbbreviation{Librarianship}{Librariansh}
\DefineJournalPartialAbbreviation{Librettist}{Librett}
\DefineJournalWordException{Libyan}{Libyan}
\DefineJournalWordException{Licence}{Licence}
\DefineJournalAbbreviation{Licenced}{Licenc}
\DefineJournalPartialAbbreviation{Licens}{Licens}
\DefineJournalAbbreviation{Licentiate}{Licent}
\DefineJournalWordException{Lichen}{Lichen}
\DefineJournalAbbreviation{Lichfield}{Lichf}
\DefineJournalWordException{Lidcombe}{Lidcombe}
\DefineJournalAbbreviation{Lieutenant}{Lieuten}
\DefineJournalWordException{Life-boat}{Life-boat}
\DefineJournalWordException{Lifeline}{Lifeline}
\DefineJournalWordException{Lifelong}{Lifelong}
\DefineJournalAbbreviation{Lifesaving}{Lifesav}
\DefineJournalPartialAbbreviation{Lifeskill}{Lifesk}
\DefineJournalAbbreviation{Lifespan}{Lifesp}
\DefineJournalWordException{Lifestream}{Lifestream}
\DefineJournalWordException{Lifestyle}{Lifestyle}
\DefineJournalWordException{Lifetime}{Lifetime}
\DefineJournalAbbreviation{Lifting}{Lift}
\DefineJournalWordException{Ligand}{Ligand}
\DefineJournalWordException{Light}{Light}
\DefineJournalPartialAbbreviation{Light}{Light}
\DefineJournalWordException{Lighthouse}{Lighthouse}
\DefineJournalWordException{Lightware}{Lightware}
\DefineJournalWordException{Lightweight}{Lightweight}
\DefineJournalWordException{Lignite}{Lignite}
\DefineJournalAbbreviation{Lignitic}{Lignit}
\DefineJournalPartialAbbreviation{Lignocellulos}{Lignocellul}
\DefineJournalWordException{Limelight}{Limelight}
\DefineJournalWordException{Limerick}{Limerick}
\DefineJournalAbbreviation{Limestone}{Limest}
\DefineJournalWordException{Limit}{Limit}
\DefineJournalAbbreviation{Limitation}{Limit}
\DefineJournalAbbreviation{Limited}{Ltd}
\DefineJournalAbbreviation{Lincoln}{Linc}
\DefineJournalAbbreviation{Lincolnshire}{Lincs}
\DefineJournalWordException{Linear}{Linear}
\DefineJournalWordException{Lining}{Lining}
\DefineJournalAbbreviation{Linkage}{Link}
\DefineJournalAbbreviation{Linker}{Link}
\DefineJournalAbbreviation{Linking}{Link}
\DefineJournalAbbreviation{Linkletter}{Linklett}
\DefineJournalAbbreviation{Linnean}{Linn}
\DefineJournalWordException{Linoleum}{Linoleum}
\DefineJournalWordException{Linter}{Linter}
\DefineJournalWordException{Lipid}{Lipid}
\DefineJournalAbbreviation{Lipidology}{Lipidol}
\DefineJournalAbbreviation{Lipidomics}{Lipidom}
\DefineJournalAbbreviation{Lipped}{Lipp}
\DefineJournalPartialAbbreviation{Liquef}{Liq}
\DefineJournalPartialAbbreviation{Liquid}{Liq}
\DefineJournalPartialAbbreviation{Liquor}{Liquor}
\DefineJournalWordException{Lismore}{Lismore}
\DefineJournalWordException{Listen}{Listen}
\DefineJournalWordException{Listing}{Listing}
\DefineJournalAbbreviation{Listok}{List}
\DefineJournalAbbreviation{Literacy}{Lit}
\DefineJournalPartialAbbreviation{Literar}{Lit}
\DefineJournalWordException{Lithgow}{Lithgow}
\DefineJournalWordException{Lithic}{Lithic}
\DefineJournalWordException{Lithium}{Lithium}
\DefineJournalAbbreviation{Lithoprinter}{Lithopr}
\DefineJournalPartialAbbreviation{Lithostratigraph}{Lithostratigr}
\DefineJournalAbbreviation{Lithotripsy}{Lithotr}
\DefineJournalAbbreviation{Litigation}{Litig}
\DefineJournalAbbreviation{Litigator}{Litig}
\DefineJournalWordException{Little}{Little}
\DefineJournalWordException{Little-Rock}{Little-Rock}
\DefineJournalWordException{Littlefoot}{Littlefoot}
\DefineJournalPartialAbbreviation{Liturg}{Liturg}
\DefineJournalWordException{Liturgy}{Liturgy}
\DefineJournalWordException{Livable}{Livable}
\DefineJournalAbbreviation{Live-stock}{Live-st}
\DefineJournalAbbreviation{Liverpool}{Liverp}
\DefineJournalAbbreviation{Livestock}{Livest}
\DefineJournalWordException{Living}{Living}
\DefineJournalWordException{Livingstone}{Livingstone}
\DefineJournalWordException{Lloydminster}{Lloydminster}
\DefineJournalAbbreviation{Loading}{Load}
\DefineJournalAbbreviation{Lobbyist}{Lobby}
\DefineJournalWordException{Lobster}{Lobster}
\DefineJournalWordException{Locality}{Locality}
\DefineJournalAbbreviation{Locally}{Local}
\DefineJournalWordException{Locater}{Locater}
\DefineJournalPartialAbbreviation{Location}{Locat}
\DefineJournalWordException{Locator}{Locator}
\DefineJournalWordException{Lock-out}{Lock-out}
\DefineJournalWordException{Lockeport}{Lockeport}
\DefineJournalWordException{Locksmith}{Locksmith}
\DefineJournalPartialAbbreviation{Locksmith}{Locksmith}
\DefineJournalWordException{Locust}{Locust}
\DefineJournalPartialAbbreviation{Lodg}{Lodg}
\DefineJournalAbbreviation{Logbook}{Logb}
\DefineJournalWordException{Logger}{Logger}
\DefineJournalWordException{Logging}{Logging}
\DefineJournalAbbreviation{Logic}{Log}
\DefineJournalAbbreviation{Logical}{Log}
\DefineJournalPartialAbbreviation{Logistic}{Logist}
\DefineJournalPartialAbbreviation{Logopaedi}{Logop}
\DefineJournalPartialAbbreviation{Logotherap}{Logother}
\DefineJournalWordException{Lollipop}{Lollipop}
\DefineJournalWordException{Lollypop}{Lollypop}
\DefineJournalAbbreviation{London}{Lond}
\DefineJournalWordException{Londonderry}{Londonderry}
\DefineJournalWordException{Long-Beach}{Long-Beach}
\DefineJournalWordException{Long-term}{Long-term}
\DefineJournalAbbreviation{Longest}{Long}
\DefineJournalAbbreviation{Longevity}{Longev}
\DefineJournalWordException{Longford}{Longford}
\DefineJournalWordException{Longhorn}{Longhorn}
\DefineJournalAbbreviation{Longitudinal}{Longitud}
\DefineJournalWordException{Longriffles}{Longriffles}
\DefineJournalAbbreviation{Looking}{Look}
\DefineJournalWordException{Lookout}{Lookout}
\DefineJournalWordException{Looseleaf}{Looseleaf}
\DefineJournalWordException{Lorhian}{Lorhian}
\DefineJournalWordException{Los alamos}{Los alamos}
\DefineJournalAbbreviation{Los Angeles}{Los Angel}
\DefineJournalWordException{Lothian}{Lothian}
\DefineJournalWordException{Lottery}{Lottery}
\DefineJournalAbbreviation{Loughborough}{Loughb}
\DefineJournalAbbreviation{Louisiana}{La}
\DefineJournalWordException{Lovell}{Lovell}
\DefineJournalWordException{Loving}{Loving}
\DefineJournalPartialAbbreviation{Lower}{Low}
\DefineJournalAbbreviation{Lowground}{Lowgr}
\DefineJournalPartialAbbreviation{Lowland}{Lowl}
\DefineJournalPartialAbbreviation{Loyal}{Loyal}
\DefineJournalWordException{Lubbock}{Lubbock}
\DefineJournalPartialAbbreviation{Lubricant}{Lubr}
\DefineJournalPartialAbbreviation{Lubricat}{Lubr}
\DefineJournalWordException{Lucas Heights}{Lucas Heights}
\DefineJournalWordException{Lucknow}{Lucknow}
\DefineJournalWordException{Ludlow}{Ludlow}
\DefineJournalAbbreviation{Luggage}{Lugg}
\DefineJournalWordException{Lullwater}{Lullwater}
\DefineJournalWordException{Lumber}{Lumber}
\DefineJournalAbbreviation{Lumberman}{Lumberm}
\DefineJournalAbbreviation{Lumberyard}{Lumbery}
\DefineJournalWordException{Lumine}{Lumine}
\DefineJournalPartialAbbreviation{Luminescen}{Lumin}
\DefineJournalAbbreviation{Luminous}{Lumin}
\DefineJournalWordException{Lunacy}{Lunacy}
\DefineJournalWordException{Lunatic}{Lunatic}
\DefineJournalWordException{Lupins}{Lupins}
\DefineJournalWordException{Lusaka}{Lusaka}
\DefineJournalAbbreviation{Lusatian}{Lus}
\DefineJournalWordException{Lutheran}{Lutheran}
\DefineJournalAbbreviation{Lutheraner}{Luther}
\DefineJournalPartialAbbreviation{Luxur}{Lux}
%\DefineJournalPartialWordException{Lwow}{Lwow-}
\DefineJournalWordException{Lymphokine}{Lymphokine}
\DefineJournalWordException{Lymphoma}{Lymphoma}
\DefineJournalWordException{Lynden}{Lynden}
\DefineJournalAbbreviation{Lynnwood}{Lynnw}
\DefineJournalAbbreviation{Lyric}{Lyr}
\DefineJournalWordException{Macadamia}{Macadamia}
\DefineJournalWordException{Macaroni}{Macaroni}
\DefineJournalWordException{Macclesfield}{Macclesfield}
\DefineJournalWordException{Machias}{Machias}
\DefineJournalPartialAbbreviation{Machin}{Mach}
\DefineJournalWordException{Macintosh}{Macintosh}
\DefineJournalWordException{Mackay}{Mackay}
\DefineJournalWordException{Mackenzie}{Mackenzie}
\DefineJournalWordException{Macrobenthic}{Macrobenthic}
\DefineJournalAbbreviation{Macrocyclic}{Macrocycl}
\DefineJournalPartialAbbreviation{Macroeconom}{Macroecon}
\DefineJournalPartialAbbreviation{Macromolecul}{Macromol}
\DefineJournalPartialAbbreviation{Macronutrient}{Macronutr}
\DefineJournalWordException{Macrophyte}{Macrophyte}
\DefineJournalPartialAbbreviation{Macroprudent}{Macroprudent}
\DefineJournalPartialAbbreviation{Macroscop}{Macrosc}
\DefineJournalWordException{Madison}{Madison}
\DefineJournalWordException{Madness}{Madness}
\DefineJournalWordException{Madonna}{Madonna}
\DefineJournalWordException{Madras}{Madras}
\DefineJournalPartialAbbreviation{Magazin}{Mag}
\DefineJournalWordException{Maghreb}{Maghreb}
\DefineJournalWordException{Magic}{Magic}
\DefineJournalAbbreviation{Magical}{Magic}
\DefineJournalWordException{Magill}{Magill}
\DefineJournalPartialAbbreviation{Magnetoelectroni}{Magnetoelectron}
\DefineJournalPartialAbbreviation{Magnetorheolog}{Magnetorheol}
\DefineJournalPartialAbbreviation{Magnetospher}{Magnetos}
\DefineJournalPartialAbbreviation{Magnify}{Magnify}
\DefineJournalWordException{Maharashtra}{Maharashtra}
\DefineJournalAbbreviation{Mahogany}{Mahog}
\DefineJournalWordException{Maidstone}{Maidstone}
\DefineJournalAbbreviation{Maiduguri}{Maid}
\DefineJournalPartialAbbreviation{Mail}{Mail}
\DefineJournalAbbreviation{Mailbox}{Mailb}
\DefineJournalWordException{Mailcoach}{Mailcoach}
\DefineJournalWordException{Mainframe}{Mainframe}
\DefineJournalAbbreviation{Mainland}{Mainl}
\DefineJournalWordException{Mainline}{Mainline}
\DefineJournalWordException{Mainly}{Mainly}
\DefineJournalWordException{Mainstream}{Mainstream}
\DefineJournalPartialAbbreviation{Maintain}{Maint}
\DefineJournalAbbreviation{Maintainability}{Maintainab}
\DefineJournalWordException{Majesty}{Majesty}
\DefineJournalWordException{Major}{Major}
\DefineJournalPartialAbbreviation{Majorit}{Major}
\DefineJournalAbbreviation{Maker}{Mak}
\DefineJournalAbbreviation{Making}{Mak}
\DefineJournalPartialAbbreviation{Malacolog}{Malacol}
\DefineJournalAbbreviation{Maladjusted}{Maladjust}
\DefineJournalWordException{Malahat}{Malahat}
\DefineJournalAbbreviation{Malaria}{Malar}
\DefineJournalWordException{Malawian}{Malawian}
\DefineJournalWordException{Malaya}{Malaya}
\DefineJournalAbbreviation{Malayan}{Malay}
\DefineJournalPartialAbbreviation{Malaysia}{Malays}
\DefineJournalAbbreviation{Malesian}{Males}
\DefineJournalAbbreviation{Malformation}{Malform}
\DefineJournalAbbreviation{Malfunction}{Malfunct}
\DefineJournalWordException{Malibu}{Malibu}
\DefineJournalPartialAbbreviation{Malignan}{Malig}
\DefineJournalWordException{Mallow}{Mallow}
\DefineJournalAbbreviation{Malpractice}{Malpract}
\DefineJournalAbbreviation{Maltese}{Malt}
\DefineJournalAbbreviation{Malting}{Malt}
\DefineJournalAbbreviation{Mamillaria}{Mamill}
\DefineJournalPartialAbbreviation{Mammalog}{Mammal}
\DefineJournalAbbreviation{Mammals}{Mamm}
\DefineJournalWordException{Mammary}{Mammary}
\DefineJournalAbbreviation{Mammography}{Mammogr}
\DefineJournalWordException{Mammoth}{Mammoth}
\DefineJournalWordException{Man-hour}{Man-hour}
\DefineJournalAbbreviation{Manchester}{Manch}
\DefineJournalWordException{Manchurian}{Manchurian}
\DefineJournalWordException{Mandala}{Mandala}
\DefineJournalWordException{Mandate}{Mandate}
\DefineJournalAbbreviation{Mandatory}{Mandat}
\DefineJournalPartialAbbreviation{Mandolin}{Mandol}
\DefineJournalWordException{Manganese}{Manganese}
\DefineJournalPartialAbbreviation{Mangl}{Mangl}
\DefineJournalWordException{Mangrove}{Mangrove}
\DefineJournalWordException{Manhattan}{Manhattan}
\DefineJournalWordException{Manhour}{Manhour}
\DefineJournalWordException{Manicaouagan}{Manicaouagan}
\DefineJournalAbbreviation{Manichean}{Manich}
\DefineJournalAbbreviation{Manifesto}{Manif}
\DefineJournalWordException{Manifold}{Manifold}
\DefineJournalWordException{Manila}{Manila}
\DefineJournalAbbreviation{Manilana}{Manil}
\DefineJournalPartialAbbreviation{Manipul}{Manip}
\DefineJournalAbbreviation{Manitoba}{Manit}
\DefineJournalWordException{Manjimup}{Manjimup}
\DefineJournalAbbreviation{Mankind}{Mank}
\DefineJournalWordException{Manly}{Manly}
\DefineJournalWordException{Manmade}{Manmade}
\DefineJournalWordException{Manorama}{Manorama}
\DefineJournalAbbreviation{Manorial}{Manor}
\DefineJournalAbbreviation{Manpower}{Manpow}
\DefineJournalAbbreviation{Manual}{Man}
\DefineJournalPartialAbbreviation{Manufactor}{Manuf}
\DefineJournalPartialAbbreviation{Manufactur}{Manuf}
\DefineJournalWordException{Manure}{Manure}
\DefineJournalAbbreviation{Manuscript}{Manuscr}
\DefineJournalWordException{Maple-Ridge}{Maple-Ridge}
\DefineJournalAbbreviation{Mapping}{Mapp}
\DefineJournalWordException{Maranoa}{Maranoa}
\DefineJournalWordException{Marathwada}{Marathwada}
\DefineJournalWordException{Marble}{Marble}
\DefineJournalWordException{Margarine}{Margarine}
\DefineJournalWordException{Margin}{Margin}
\DefineJournalWordException{Mariannhill}{Mariannhill}
\DefineJournalPartialAbbreviation{Maricult}{Maric}
\DefineJournalPartialAbbreviation{Marin}{Mar}
\DefineJournalPartialAbbreviation{Marital}{Marital}
\DefineJournalPartialAbbreviation{Maritime}{Marit}
\DefineJournalWordException{Marker}{Marker}
\DefineJournalPartialAbbreviation{Market}{Mark}
\DefineJournalAbbreviation{Marketbook}{Marketb}
\DefineJournalWordException{Marketguide}{Marketguide}
\DefineJournalAbbreviation{Marketletter}{Marketlett}
\DefineJournalAbbreviation{Marketman}{Marketm}
\DefineJournalWordException{Marketnews}{Marketnews}
\DefineJournalAbbreviation{Marketplace}{Marketpl}
\DefineJournalWordException{Markham}{Markham}
\DefineJournalWordException{Marking}{Marking}
\DefineJournalWordException{Marksman}{Marksman}
\DefineJournalAbbreviation{Marlborough}{Marlbgh}
\DefineJournalWordException{Maroochy}{Maroochy}
\DefineJournalWordException{Marousi}{Marousi}
\DefineJournalWordException{Marpole}{Marpole}
\DefineJournalWordException{Marquee}{Marquee}
\DefineJournalWordException{Marquetry}{Marquetry}
\DefineJournalWordException{Marriage}{Marriage}
\DefineJournalAbbreviation{Marrickville}{Marrickv}
\DefineJournalWordException{Marrow}{Marrow}
\DefineJournalWordException{Marryalyan}{Marryalyan}
\DefineJournalWordException{Marshal}{Marshal}
\DefineJournalAbbreviation{Marshalltown}{Marshallt}
\DefineJournalWordException{Mar\J@C tial}{Mar\J@C tial}
\DefineJournalAbbreviation{Maryborough}{Marybgh}
\DefineJournalAbbreviation{Maryland}{Md}
\DefineJournalWordException{Masonic}{Masonic}
\DefineJournalAbbreviation{Masonry}{Mason}
\DefineJournalAbbreviation{Massachusetts}{Mass}
\DefineJournalWordException{Master}{Master}
\DefineJournalAbbreviation{Masterclass}{Mastercl}
\DefineJournalWordException{Masterfile}{Masterfile}
\DefineJournalWordException{Masterpiece}{Masterpiece}
\DefineJournalWordException{Mastersport}{Mastersport}
\DefineJournalAbbreviation{Matchbox}{Matchb}
\DefineJournalWordException{Matched}{Matched}
\DefineJournalAbbreviation{Materials}{Mater}
\DefineJournalAbbreviation{Materiel}{Mater}
\DefineJournalWordException{Materion}{Materion}
\DefineJournalPartialAbbreviation{Mathemat}{Math}
\DefineJournalWordException{Matheson}{Matheson}
\DefineJournalAbbreviation{Mathware}{Mathw}
\DefineJournalWordException{Matrix}{Matrix}
\DefineJournalWordException{Matter}{Matter}
\DefineJournalPartialAbbreviation{Matur}{Matur}
\DefineJournalAbbreviation{Mauritius}{Maurit}
\DefineJournalAbbreviation{Mausoleum}{Mausol}
\DefineJournalAbbreviation{Maxillo-facial}{Maxillo-fac}
\DefineJournalPartialAbbreviation{Maxillofacial}{Maxillofac}
\DefineJournalWordException{Maydan}{Maydan}
\DefineJournalWordException{Mayerthorpe}{Mayerthorpe}
\DefineJournalWordException{Mayflower}{Mayflower}
\DefineJournalWordException{Maynooth}{Maynooth}
\DefineJournalWordException{Mayurbhanj}{Mayurbhanj}
\DefineJournalWordException{Mbabane}{Mbabane}
\DefineJournalWordException{McKinney}{McKinney}
\DefineJournalWordException{Meadow}{Meadow}
\DefineJournalPartialAbbreviation{Meander}{Meand}
\DefineJournalAbbreviation{Meaning}{Mean}
\DefineJournalWordException{Measles}{Measles}
\DefineJournalPartialAbbreviation{Measur}{Meas}
\DefineJournalWordException{Measuretest}{Measuretest}
\DefineJournalPartialAbbreviation{Mechani}{Mech}
\DefineJournalPartialAbbreviation{Mechanobiolog}{Mechanobiol}
\DefineJournalPartialAbbreviation{Mechaoptoelectron}{Mechaoptoelectron}
\DefineJournalAbbreviation{Mechatronic}{Mechatron}
\DefineJournalPartialAbbreviation{Medecin}{Med}
\DefineJournalWordException{Medford}{Medford}
\DefineJournalWordException{Mediafacts}{Mediafacts}
\DefineJournalWordException{Mediafile}{Mediafile}
\DefineJournalWordException{Medialink}{Medialink}
\DefineJournalPartialAbbreviation{Mediat}{Mediat}
\DefineJournalWordException{Medicaid}{Medicaid}
\DefineJournalAbbreviation{M\'edical}{Med}
\DefineJournalWordException{Medicare}{Medicare}
\DefineJournalPartialAbbreviation{Medicat}{Medicat}
\DefineJournalPartialAbbreviation{M\'edi\'ev}{Mediev}
\DefineJournalAbbreviation{Mediotechnica}{Mediotech}
\DefineJournalPartialAbbreviation{Mediterrane}{Mediterr}
\DefineJournalWordException{Medlar}{Medlar}
\DefineJournalPartialAbbreviation{Medlin}{Medlin}
\DefineJournalPartialAbbreviation{Meeting}{Meet}
\DefineJournalWordException{Megabox}{Megabox}
\DefineJournalWordException{Meghalaya}{Meghalaya}
\DefineJournalWordException{Mekong}{Mekong}
\DefineJournalWordException{M\'elange}{M\'elange}
\DefineJournalWordException{Melanoma}{Melanoma}
\DefineJournalPartialAbbreviation{Melding}{Meld}
\DefineJournalPartialAbbreviation{Meliorati}{Melior}
\DefineJournalWordException{Melrose}{Melrose}
\DefineJournalAbbreviation{Member}{Memb}
\DefineJournalAbbreviation{Membership}{Membsh}
\DefineJournalPartialAbbreviation{Membran}{Membr}
\DefineJournalPartialAbbreviation{Memento}{Mem}
\DefineJournalAbbreviation{Memetics}{Memet}
\DefineJournalAbbreviation{Memoir}{Mem}
\DefineJournalPartialAbbreviation{Memorab}{Memorab}
\DefineJournalPartialAbbreviation{Memorand}{Memo}
\DefineJournalAbbreviation{Memorial}{Meml}
\DefineJournalPartialAbbreviation{Memory}{Mem}
\DefineJournalWordException{Memphis}{Memphis}
\DefineJournalWordException{Meningitis}{Meningitis}
\DefineJournalPartialAbbreviation{Mennonit}{Mennon}
\DefineJournalWordException{Menopause}{Menopause}
\DefineJournalPartialAbbreviation{Mensual}{Mens}
\DefineJournalAbbreviation{Menswear}{Mensw}
\DefineJournalPartialAbbreviation{Mental}{Ment}
\DefineJournalWordException{Mentor}{Mentor}
\DefineJournalAbbreviation{Mentoring}{Mentor}
\DefineJournalPartialAbbreviation{Mercantil}{Merc}
\DefineJournalWordException{Mercer}{Mercer}
\DefineJournalPartialAbbreviation{Merchandis}{Merch}
\DefineJournalPartialAbbreviation{Merchant}{Merch}
\DefineJournalWordException{Mercury}{Mercury}
\DefineJournalWordException{Mergers}{Mergers}
\DefineJournalWordException{Meridian}{Meridian}
\DefineJournalAbbreviation{Merseyside}{Merseys}
\DefineJournalWordException{Meshed}{Meshed}
\DefineJournalAbbreviation{Mesoamerica}{Mesoam}
\DefineJournalPartialAbbreviation{Mesomechani}{Mesomech}
\DefineJournalAbbreviation{Mesopotamia}{Mesop}
\DefineJournalPartialAbbreviation{Mesospher}{Mesos}
\DefineJournalAbbreviation{Mesozoic}{Mesoz}
\DefineJournalWordException{Message}{Message}
\DefineJournalWordException{Messagestick}{Messagestick}
\DefineJournalAbbreviation{Messemagazine}{Messemag}
\DefineJournalWordException{Messenger}{Messenger}
\DefineJournalAbbreviation{Metabole}{Metab}
\DefineJournalPartialAbbreviation{Metalloceram}{Metalloceram}
\DefineJournalPartialAbbreviation{Metallograph}{Metallogr}
\DefineJournalAbbreviation{Metallorganic}{Metallorg}
\DefineJournalAbbreviation{Metalworker}{Metalwork}
\DefineJournalAbbreviation{Metalworking}{Metalwork}
\DefineJournalPartialAbbreviation{Metamorph}{Metamorph}
\DefineJournalPartialAbbreviation{Metaphor}{Metaphor}
\DefineJournalPartialAbbreviation{Metaphysi}{Metaphys}
%\DefineJournalPartialWordException{M\'etastas}{M\'etastas-}
\DefineJournalAbbreviation{Meteorite}{Meteor}
\DefineJournalPartialAbbreviation{Meteoritic}{Meteorit}
\DefineJournalWordException{Meter}{Meter}
\DefineJournalAbbreviation{Methadone}{Methad}
\DefineJournalWordException{Methanol}{Methanol}
\DefineJournalWordException{Method}{Method}
\DefineJournalWordException{Methodist}{Methodist}
\DefineJournalPartialAbbreviation{Methodolog}{Methodol}
\DefineJournalWordException{Methotrexate}{Methotrexate}
\DefineJournalAbbreviation{Metric}{Metr}
\DefineJournalPartialAbbreviation{Metroeconom}{Metroecon}
\DefineJournalWordException{Miami}{Miami}
\DefineJournalWordException{Michiana}{Michiana}
\DefineJournalAbbreviation{Michigan}{Mich}
\DefineJournalPartialAbbreviation{Microanalys}{Microanal}
\DefineJournalPartialAbbreviation{Microanalyt}{Microanal}
\DefineJournalPartialAbbreviation{Microanatom}{Microanat}
\DefineJournalPartialAbbreviation{Microautoradiograph}{Microautoradiogr}
\DefineJournalWordException{Microbe}{Microbe}
\DefineJournalAbbreviation{Microbial}{Microb}
\DefineJournalPartialAbbreviation{Microbiolog}{Microbiol}
\DefineJournalPartialAbbreviation{Microcalorimetr}{Microcalorim}
\DefineJournalPartialAbbreviation{Microcardiograph}{Microcardiogr}
\DefineJournalPartialAbbreviation{Microchem}{Microchem}
\DefineJournalWordException{Microchip}{Microchip}
\DefineJournalPartialAbbreviation{Microcirculat}{Microcirc}
\DefineJournalPartialAbbreviation{Microclimat}{Microclim}
\DefineJournalPartialAbbreviation{Microcomponent}{Microcompon}
\DefineJournalPartialAbbreviation{Microcomput}{Microcomput}
\DefineJournalPartialAbbreviation{Microcrystal}{Microcryst}
\DefineJournalPartialAbbreviation{Microdensitometr}{Microdensitom}
\DefineJournalPartialAbbreviation{Microdosimetr}{Microdosim}
\DefineJournalAbbreviation{Microeconomic}{Microecon}
\DefineJournalPartialAbbreviation{Microelectroni}{Microelectron}
\DefineJournalAbbreviation{Microencapsulation}{Microencapsul}
\DefineJournalPartialAbbreviation{Microenvironment}{Microenviron}
\DefineJournalPartialAbbreviation{Microfabricat}{Microfabr}
\DefineJournalWordException{Microfauna}{Microfauna}
\DefineJournalWordException{Microfile}{Microfile}
\DefineJournalWordException{Microfilm}{Microfilm}
\DefineJournalPartialAbbreviation{Microfluid}{Microfluid}
\DefineJournalWordException{Microform}{Microform}
\DefineJournalWordException{Microgram}{Microgram}
\DefineJournalPartialAbbreviation{Micrograph}{Microgr}
\DefineJournalWordException{Microgravity}{Microgravity}
\DefineJournalPartialAbbreviation{Microheterogen}{Microheterog}
\DefineJournalPartialAbbreviation{Microinstrument}{Microinstrum}
\DefineJournalAbbreviation{Microinvertebrate}{Microinvertebr}
\DefineJournalPartialAbbreviation{Microlithograph}{Microlithogr}
\DefineJournalWordException{Microlog}{Microlog}
\DefineJournalAbbreviation{Micromachining}{Micromach}
\DefineJournalAbbreviation{Microminiaturization}{Microminiat}
\DefineJournalPartialAbbreviation{Micromorpholog}{Micromorphol}
\DefineJournalWordException{Micron}{Micron}
\DefineJournalPartialAbbreviation{Micronesia}{Micrones}
\DefineJournalPartialAbbreviation{Microneurosurg}{Microneurosurg}
\DefineJournalPartialAbbreviation{Micronutrient}{Micronutr}
\DefineJournalPartialAbbreviation{Microorganism}{Microorg}
\DefineJournalPartialAbbreviation{Micropaleontolog}{Micropaleontol}
\DefineJournalPartialAbbreviation{Microphotometr}{Microphotom}
\DefineJournalPartialAbbreviation{Microphysic}{Microphys}
\DefineJournalWordException{Microporous}{Microporous}
\DefineJournalWordException{Microprobe}{Microprobe}
\DefineJournalPartialAbbreviation{Microprocess}{Microprocess}
\DefineJournalAbbreviation{Microprofessional}{Microprof}
\DefineJournalAbbreviation{Microprogramm}{Microprogr}
\DefineJournalAbbreviation{Micropropagation}{Micropropag}
\DefineJournalPartialAbbreviation{Micropropuls}{Micropropuls}
\DefineJournalPartialAbbreviation{Micropublish}{Micropubl}
\DefineJournalPartialAbbreviation{Microradiograph}{Microradiogr}
\DefineJournalPartialAbbreviation{Microreaction}{Microreact}
\DefineJournalPartialAbbreviation{Microscop}{Microsc}
\DefineJournalPartialAbbreviation{Microsensor}{Microsens}
\DefineJournalAbbreviation{Microsocial}{Microsoc}
\DefineJournalWordException{Microsoft}{Microsoft}
\DefineJournalPartialAbbreviation{Microspectroscop}{Microspectrosc}
\DefineJournalPartialAbbreviation{Microstructur}{Microstruct}
\DefineJournalPartialAbbreviation{Microsurg}{Microsurg}
\DefineJournalPartialAbbreviation{Microsymposi}{Microsymp}
\DefineJournalAbbreviation{Microsystem}{Microsyst}
\DefineJournalWordException{Microtable}{Microtable}
\DefineJournalPartialAbbreviation{Microtechni}{Microtech}
\DefineJournalWordException{Microtext}{Microtext}
\DefineJournalPartialAbbreviation{Microvascul}{Microvasc}
\DefineJournalWordException{Microware}{Microware}
\DefineJournalAbbreviation{Microwavable}{Microwav}
\DefineJournalAbbreviation{Microwave}{Microw}
\DefineJournalWordException{Microworld}{Microworld}
\DefineJournalAbbreviation{Microzonation}{Microzonat}
\DefineJournalAbbreviation{MidAtlantic}{MidAtl}
\DefineJournalAbbreviation{Midcentral}{Midcent}
\DefineJournalPartialAbbreviation{Midcontinent}{Midcont}
\DefineJournalWordException{Middle}{Middle}
\DefineJournalWordException{Middle Age}{Middle Age}
\DefineJournalWordException{Middle East}{Middle East}
\DefineJournalAbbreviation{Middlesbrough}{Middlesb}
\DefineJournalAbbreviation{Middlesex}{Middx}
\DefineJournalAbbreviation{Middleton}{Middlet}
\DefineJournalAbbreviation{Middletown}{Middlet}
\DefineJournalAbbreviation{Middleware}{Middlew}
\DefineJournalWordException{Mideast}{Mideast}
\DefineJournalPartialAbbreviation{Mideast}{Mideast}
\DefineJournalAbbreviation{Midget}{Midg}
\DefineJournalAbbreviation{Midland}{Midl}
\DefineJournalWordException{Midlife}{Midlife}
\DefineJournalWordException{Midlothian}{Midlothian}
\DefineJournalWordException{Midnight}{Midnight}
\DefineJournalPartialAbbreviation{Midnorth}{Midnorth}
\DefineJournalWordException{Midrange}{Midrange}
\DefineJournalWordException{Midsouth}{Midsouth}
\DefineJournalWordException{Midtown}{Midtown}
\DefineJournalWordException{Midweek}{Midweek}
\DefineJournalWordException{Midwest}{Midwest}
\DefineJournalAbbreviation{Midwestern}{Midwest}
\DefineJournalWordException{Midwife}{Midwife}
\DefineJournalWordException{Midwifery}{Midwifery}
\DefineJournalWordException{Midyear}{Midyear}
\DefineJournalAbbreviation{Mightier}{Might}
\DefineJournalWordException{Mighty}{Mighty}
\DefineJournalWordException{Migraine}{Migraine}
\DefineJournalAbbreviation{Migrant}{Migr}
\DefineJournalPartialAbbreviation{Migration}{Migr}
\DefineJournalAbbreviation{Migratory}{Migr}
\DefineJournalWordException{Mildmay}{Mildmay}
\DefineJournalWordException{Mileage}{Mileage}
\DefineJournalWordException{Milepost}{Milepost}
\DefineJournalAbbreviation{Milestone}{Milest}
\DefineJournalAbbreviation{Militant}{Milit}
\DefineJournalPartialAbbreviation{Militar}{Mil}
\DefineJournalAbbreviation{Milking}{Milk}
\DefineJournalWordException{Millbrook}{Millbrook}
\DefineJournalPartialAbbreviation{Millenni}{Millenn}
\DefineJournalAbbreviation{Miller}{Mill}
\DefineJournalWordException{Millet}{Millet}
\DefineJournalAbbreviation{Millimeter}{Millim}
\DefineJournalWordException{Million}{Million}
\DefineJournalAbbreviation{Millionaire}{Million}
\DefineJournalAbbreviation{Milltown}{Millt}
\DefineJournalWordException{Millwork}{Millwork}
\DefineJournalWordException{Milton}{Milton}
\DefineJournalWordException{Milwaukee}{Milwaukee}
\DefineJournalAbbreviation{Minced}{Minc}
\DefineJournalWordException{Minded}{Minded}
\DefineJournalWordException{Minder}{Minder}
\DefineJournalWordException{Minding}{Minding}
\DefineJournalWordException{Mineola}{Mineola}
\DefineJournalAbbreviation{Miner}{Min}
\DefineJournalPartialAbbreviation{Minerolog}{Minerol}
\DefineJournalAbbreviation{Mineworker}{Minework}
\DefineJournalWordException{Mini-guide}{Mini-guide}
\DefineJournalAbbreviation{Miniaturist}{Miniat}
\DefineJournalPartialAbbreviation{Minicomputer}{Minicomput}
\DefineJournalPartialAbbreviation{Miniconferen}{Miniconf}
\DefineJournalWordException{Minilab}{Minilab}
\DefineJournalAbbreviation{Minimally}{Minim}
\DefineJournalAbbreviation{Minimum}{Minim}
\DefineJournalAbbreviation{Mining}{Min}
\DefineJournalWordException{Miniprint}{Miniprint}
\DefineJournalPartialAbbreviation{Minister}{Minist}
\DefineJournalPartialAbbreviation{Minisympos}{Minisymp}
\DefineJournalWordException{Minna}{Minna}
\DefineJournalAbbreviation{Minneapolis}{Minneap}
\DefineJournalAbbreviation{Minnesota}{Minn}
\DefineJournalWordException{Minor}{Minor}
\DefineJournalWordException{Minster}{Minster}
\DefineJournalWordException{Minute}{Minute}
\DefineJournalWordException{Minutes}{Minutes}
\DefineJournalWordException{Mirror}{Mirror}
\DefineJournalAbbreviation{Miscarriage}{Miscarr}
\DefineJournalPartialAbbreviation{Miscellan}{Misc}
\DefineJournalWordException{Misconduct}{Misconduct}
\DefineJournalAbbreviation{Misdemeanant}{Misdemean}
\DefineJournalWordException{Missile}{Missile}
\DefineJournalWordException{Missing}{Missing}
\DefineJournalAbbreviation{Missiological}{Missiol}
\DefineJournalWordException{Missiskoui}{Missiskoui}
\DefineJournalWordException{Missisquoi}{Missisquoi}
\DefineJournalWordException{Mississauga}{Mississauga}
\DefineJournalAbbreviation{Mississippi}{Miss}
\DefineJournalWordException{Missoula}{Missoula}
\DefineJournalPartialAbbreviation{Missouri}{Mo}
\DefineJournalWordException{Mistassini}{Mistassini}
\DefineJournalWordException{Mister}{Mister}
\DefineJournalWordException{Mistletoe}{Mistletoe}
\DefineJournalWordException{Mistress}{Mistress}
\DefineJournalWordException{Misuse}{Misuse}
\DefineJournalAbbreviation{Mitchellville}{Mitchellv}
\DefineJournalWordException{Mithraic}{Mithraic}
\DefineJournalAbbreviation{Mitigation}{Mitig}
\DefineJournalWordException{Mitten}{Mitten}
\DefineJournalPartialAbbreviation{Mix}{Mix}
\DefineJournalPartialAbbreviation{Mnemonic}{Mnemon}
\DefineJournalAbbreviation{Mobile}{Mob}
\DefineJournalAbbreviation{Mobility}{Mobil}
\DefineJournalWordException{Moccasin}{Moccasin}
\DefineJournalPartialAbbreviation{Model}{Model}
\DefineJournalAbbreviation{Modelisation}{Model}
\DefineJournalPartialAbbreviation{Modell}{Model}
\DefineJournalWordException{Modelworld}{Modelworld}
\DefineJournalPartialAbbreviation{Modern}{Mod}
\DefineJournalPartialAbbreviation{Modul}{Modul}
\DefineJournalWordException{Mojave}{Mojave}
\DefineJournalWordException{Moksha}{Moksha}
\DefineJournalWordException{Molasse}{Molasse}
\DefineJournalPartialAbbreviation{Moldav}{Mold}
\DefineJournalWordException{Molding}{Molding}
\DefineJournalPartialAbbreviation{Molecul}{Mol}
\DefineJournalAbbreviation{Molinology}{Molinol}
\DefineJournalWordException{Mollusc}{Mollusc}
\DefineJournalAbbreviation{Molluscicide}{Molluscic}
\DefineJournalWordException{Mollusk}{Mollusk}
\DefineJournalAbbreviation{Molybdenium}{Molybd}
\DefineJournalWordException{Molysulfide}{Molysulfide}
\DefineJournalWordException{Mombasa}{Mombasa}
\DefineJournalWordException{Monaghan}{Monaghan}
\DefineJournalAbbreviation{Monagricultural}{Monagric}
\DefineJournalWordException{Monchanin}{Monchanin}
\DefineJournalAbbreviation{Moncton}{Monct}
\DefineJournalWordException{Monday}{Monday}
\DefineJournalPartialAbbreviation{Mondial}{Mond}
\DefineJournalWordException{Money}{Money}
\DefineJournalAbbreviation{Money-lender}{Money-lend}
\DefineJournalPartialAbbreviation{Moneymak}{Moneymak}
%\DefineJournalPartialWordException{Moneywis}{Moneywis-}
\DefineJournalWordException{Monger}{Monger}
\DefineJournalPartialAbbreviation{Mongolia}{Mong}
\DefineJournalPartialAbbreviation{Monitor}{Monit}
\DefineJournalWordException{Monkey}{Monkey}
\DefineJournalAbbreviation{Monkeyshine}{Monkeysh}
\DefineJournalWordException{Monmouth}{Monmouth}
\DefineJournalAbbreviation{Monmouthshire}{Monmouths}
\DefineJournalAbbreviation{Monoclonal}{Monoclon}
\DefineJournalPartialAbbreviation{Monoenergetic}{Monoenerg}
\DefineJournalPartialAbbreviation{Monograph}{Monogr}
\DefineJournalPartialAbbreviation{Monomolecul}{Monomol}
\DefineJournalAbbreviation{Mononuclear}{Mononucl}
\DefineJournalAbbreviation{Monosaccharide}{Monosacch}
\DefineJournalWordException{Monotype}{Monotype}
\DefineJournalWordException{Montachusett}{Montachusett}
\DefineJournalWordException{Montague}{Montague}
\DefineJournalAbbreviation{Montana}{Mont}
\DefineJournalWordException{Montclair}{Montclair}
\DefineJournalWordException{Montebello}{Montebello}
\DefineJournalWordException{Monterey}{Monterey}
\DefineJournalWordException{Montgomery}{Montgomery}
\DefineJournalPartialAbbreviation{Month}{Mon}
\DefineJournalAbbreviation{Montpelier}{Montpel}
\DefineJournalAbbreviation{Montreal}{Montr}
\DefineJournalPartialAbbreviation{Montserrat}{Montserrat}
\DefineJournalPartialAbbreviation{Monument}{Monum}
%\DefineJournalPartialWordException{Moonlight}{Moonlight-}
\DefineJournalAbbreviation{Moorland}{Moorl}
\DefineJournalAbbreviation{Morality}{Moral}
\DefineJournalAbbreviation{Moratorium}{Morat}
\DefineJournalAbbreviation{Morgantown}{Morgant}
\DefineJournalWordException{Mormon}{Mormon}
\DefineJournalWordException{Morning}{Morning}
\DefineJournalWordException{Mornington}{Mornington}
\DefineJournalPartialAbbreviation{Morocc}{Moroc}
\DefineJournalPartialAbbreviation{Morphogen}{Morphog}
\DefineJournalPartialAbbreviation{Morpholog}{Morphol}
\DefineJournalAbbreviation{Morrinsville}{Morrinsv}
\DefineJournalAbbreviation{Mortality}{Mortal}
\DefineJournalWordException{Mortar}{Mortar}
\DefineJournalAbbreviation{Mortgage}{Mortg}
\DefineJournalPartialAbbreviation{Mortu}{Mortu}
\DefineJournalWordException{Mosaic}{Mosaic}
\DefineJournalAbbreviation{Moscow}{Mosc}
\DefineJournalWordException{Moslim}{Moslim}
\DefineJournalWordException{Motel}{Motel}
\DefineJournalWordException{Mother}{Mother}
\DefineJournalAbbreviation{Motherhood}{Mother}
\DefineJournalAbbreviation{Motility}{Motil}
\DefineJournalWordException{Motion}{Motion}
\DefineJournalPartialAbbreviation{Motocross}{Motocr}
\DefineJournalPartialAbbreviation{Motor}{Mot}
\DefineJournalPartialAbbreviation{Motorboat}{Motorboat}
\DefineJournalWordException{Motorcycle}{Motorcycle}
\DefineJournalAbbreviation{Motorcyclist}{Motorcycl}
\DefineJournalAbbreviation{Motorhome}{Motorh}
\DefineJournalPartialAbbreviation{Motormak}{Motormak}
\DefineJournalWordException{Motorsport}{Motorsport}
\DefineJournalAbbreviation{Motorway}{Motorw}
\DefineJournalPartialAbbreviation{Motric}{Mot}
\DefineJournalPartialAbbreviation{Mould}{Mould}
\DefineJournalAbbreviation{Mount}{Mt}
\DefineJournalPartialAbbreviation{Mountain}{Mt}
\DefineJournalWordException{Mounted}{Mounted}
\DefineJournalWordException{Mountview}{Mountview}
\DefineJournalWordException{Mouth}{Mouth}
\DefineJournalWordException{Mouthpiece}{Mouthpiece}
\DefineJournalWordException{Moveable}{Moveable}
\DefineJournalAbbreviation{Movement}{Mov}
\DefineJournalAbbreviation{Mover}{Mov}
\DefineJournalWordException{Movie}{Movie}
\DefineJournalAbbreviation{Moving}{Mov}
\DefineJournalAbbreviation{Mozambican}{Mozamb}
\DefineJournalAbbreviation{Mucopolysaccharide}{Mucopolysacch}
\DefineJournalWordException{Mucoprotein}{Mucoprotein}
\DefineJournalWordException{Mudgee}{Mudgee}
\DefineJournalPartialAbbreviation{Muffl}{Muff}
\DefineJournalAbbreviation{Multicellular}{Multicell}
\DefineJournalPartialAbbreviation{Multicenter}{Multicent}
\DefineJournalPartialAbbreviation{Multichemi}{Multichem}
\DefineJournalAbbreviation{Multicritical}{Multicrit}
\DefineJournalPartialAbbreviation{Multidenta}{Multident}
\DefineJournalPartialAbbreviation{Multidisciplin}{Multidiscip}
\DefineJournalPartialAbbreviation{Multielement}{Multielem}
\DefineJournalPartialAbbreviation{Multifunction}{Multifunct}
\DefineJournalPartialAbbreviation{Multihandicap}{Multihandicap}
\DefineJournalPartialAbbreviation{Multihormon}{Multihorm}
\DefineJournalAbbreviation{Multilaboratory}{Multilab}
\DefineJournalAbbreviation{Multilateral}{Multilater}
\DefineJournalWordException{Multilinear}{Multilinear}
\DefineJournalAbbreviation{Multilingual}{Multiling}
\DefineJournalAbbreviation{Multilingualism}{Multiling}
\DefineJournalPartialAbbreviation{Multimetalli}{Multimet}
\DefineJournalPartialAbbreviation{Multinational}{Multinatl}
\DefineJournalPartialAbbreviation{Multinuclear}{Multinucl}
\DefineJournalAbbreviation{Multiphase}{Multiph}
\DefineJournalAbbreviation{Multiprofessional}{Multiprof}
\DefineJournalAbbreviation{Multipurpose}{Multipurp}
\DefineJournalWordException{Multiracial}{Multiracial}
\DefineJournalAbbreviation{Multisensor}{Multisens}
\DefineJournalWordException{Multisport}{Multisport}
\DefineJournalWordException{Multistate}{Multistate}
\DefineJournalAbbreviation{Multitarget}{Multitarg}
\DefineJournalAbbreviation{Multitasking}{Multitask}
\DefineJournalWordException{Multiuser}{Multiuser}
\DefineJournalAbbreviation{Multivariate}{Multivar}
\DefineJournalWordException{Muncy}{Muncy}
\DefineJournalWordException{Mundane}{Mundane}
\DefineJournalWordException{Munich}{Munich}
\DefineJournalPartialAbbreviation{Municip}{Munic}
\DefineJournalWordException{Muppet}{Muppet}
\DefineJournalWordException{Muramyl}{Muramyl}
\DefineJournalPartialAbbreviation{Murder}{Murd}
\DefineJournalWordException{Murdoch}{Murdoch}
\DefineJournalWordException{Muscle}{Muscle}
\DefineJournalWordException{Muscular}{Muscular}
\DefineJournalAbbreviation{Musculoskeletal}{Musculoskelet}
\DefineJournalAbbreviation{Museum}{Mus}
\DefineJournalWordException{Mushroom}{Mushroom}
\DefineJournalPartialAbbreviation{Music}{Music}
\DefineJournalWordException{Muskeg}{Muskeg}
\DefineJournalWordException{Muslim}{Muslim}
\DefineJournalWordException{Mustang}{Mustang}
\DefineJournalWordException{Mustard}{Mustard}
\DefineJournalAbbreviation{Mustelid}{Mustel}
\DefineJournalWordException{Mutagen}{Mutagen}
\DefineJournalPartialAbbreviation{Mutagen}{Mutagen}
\DefineJournalPartialAbbreviation{Mutation}{Mutat}
\DefineJournalWordException{Mutual}{Mutual}
\DefineJournalPartialAbbreviation{Mutuali}{Mutual}
\DefineJournalWordException{Muzaffarpur}{Muzaffarpur}
\DefineJournalWordException{Myasthenia}{Myasthenia}
\DefineJournalAbbreviation{Mycenaean}{Mycen}
\DefineJournalAbbreviation{Mycobacteria}{Mycobact}
\DefineJournalAbbreviation{Mycobacterial}{Mycobact}
\DefineJournalPartialAbbreviation{Mycolog}{Mycol}
\DefineJournalPartialAbbreviation{Mycopatholog}{Mycopathol}
\DefineJournalAbbreviation{Mycoplasmal}{Mycoplasm}
\DefineJournalPartialAbbreviation{Mycoplasmolog}{Mycoplasmol}
\DefineJournalWordException{Mycorrhizasts}{Mycorrhizasts}
\DefineJournalWordException{Mycose}{Mycose}
\DefineJournalWordException{Mycotoxin}{Mycotoxin}
\DefineJournalWordException{Myeloma}{Myeloma}
\DefineJournalAbbreviation{Myocardial}{Myocard}
\DefineJournalPartialAbbreviation{Myocardiolog}{Myocardiol}
\DefineJournalAbbreviation{Myochemistry}{Myochem}
\DefineJournalWordException{Myopathy}{Myopathy}
\DefineJournalWordException{Myopia}{Myopia}
\DefineJournalAbbreviation{Myriapod}{Myriap}
\DefineJournalWordException{Mysore}{Mysore}
\DefineJournalWordException{Mystery}{Mystery}
\DefineJournalWordException{Mystica}{Mystica}
\DefineJournalWordException{Mystical}{Mystical}
\DefineJournalWordException{Mystral}{Mystral}
\DefineJournalPartialAbbreviation{Myxobacteria}{Myxobact}
\DefineJournalWordException{Nairobi}{Nairobi}
\DefineJournalAbbreviation{Nameplate}{Namepl}
\DefineJournalPartialAbbreviation{Namibi}{Namib}
\DefineJournalPartialAbbreviation{Nanoelectroni}{Nanoelectron}
\DefineJournalPartialAbbreviation{Nanoengineer}{Nanoeng}
\DefineJournalPartialAbbreviation{Nanomater}{Nanomater}
\DefineJournalAbbreviation{Nanomedicine}{Nanomed}
\DefineJournalAbbreviation{Nanopharmaceutics}{Nanopharm}
\DefineJournalPartialAbbreviation{Nanoscienc}{Nanosci}
\DefineJournalPartialAbbreviation{Nanosystem}{Nanosyst}
\DefineJournalAbbreviation{Nanotechnology}{Nanotechnol}
\DefineJournalPartialAbbreviation{Nanotub}{Nanotub}
\DefineJournalWordException{Naphtha}{Naphtha}
\DefineJournalWordException{Napier}{Napier}
\DefineJournalWordException{Narborough}{Narborough}
\DefineJournalAbbreviation{Narcotic}{Narc}
\DefineJournalWordException{Narrabeen}{Narrabeen}
\DefineJournalPartialAbbreviation{Narrat}{Narrat}
\DefineJournalWordException{Narrow}{Narrow}
\DefineJournalWordException{Nashoba}{Nashoba}
\DefineJournalWordException{Nashua}{Nashua}
\DefineJournalAbbreviation{Nashville}{Nashv}
\DefineJournalAbbreviation{Nasopharyngeal }{Nasopharyng}
\DefineJournalAbbreviation{Natality}{Natal}
\DefineJournalPartialAbbreviation{Na\J@C tional}{Natl}
\DefineJournalAbbreviation{Nationality}{Natly}
\DefineJournalWordException{Nationwide}{Nationwide}
\DefineJournalPartialAbbreviation{Nativ}{Nativ}
\DefineJournalAbbreviation{Natriuretic}{Natriuret}
\DefineJournalWordException{Natter}{Natter}
\DefineJournalPartialAbbreviation{Natural}{Nat}
\DefineJournalAbbreviation{Nature}{Nat}
\DefineJournalPartialAbbreviation{Naturegraph}{Naturegr}
\DefineJournalPartialAbbreviation{Natureopath}{Natureopath}
\DefineJournalAbbreviation{Naturist}{Natur}
\DefineJournalPartialAbbreviation{Nauti}{Naut}
\DefineJournalWordException{Navajo}{Navajo}
\DefineJournalAbbreviation{Naval}{Nav}
\DefineJournalPartialAbbreviation{Near-East}{Near-East}
\DefineJournalWordException{Nearshore}{Nearshore}
\DefineJournalWordException{Nebenverdienst}{Nebenverdienst}
\DefineJournalAbbreviation{Nebraska}{Neb}
\DefineJournalPartialAbbreviation{Nebul}{Nebul}
\DefineJournalAbbreviation{Necessarily}{Necessar}
\DefineJournalWordException{Nedlands}{Nedlands}
\DefineJournalWordException{Needle}{Needle}
\DefineJournalWordException{Needlework}{Needlework}
\DefineJournalAbbreviation{Negative}{Negat}
\DefineJournalAbbreviation{Neglect}{Negl}
\DefineJournalPartialAbbreviation{Neglig}{Neglig}
\DefineJournalPartialAbbreviation{Negocia}{Negoc}
\DefineJournalPartialAbbreviation{Negoti}{Negot}
\DefineJournalPartialAbbreviation{Neighbour}{Neighb}
\DefineJournalAbbreviation{Nematicide}{Nematic}
\DefineJournalWordException{Nematode}{Nematode}
\DefineJournalWordException{N\'eonatal}{N\'eonatal}
\DefineJournalPartialAbbreviation{Neonatolog}{Neonatol}
\DefineJournalWordException{Neoplasm}{Neoplasm}
\DefineJournalAbbreviation{Neoplastic}{Neoplast}
\DefineJournalWordException{Neoprene}{Neoprene}
\DefineJournalAbbreviation{Nepalese}{Nepal}
\DefineJournalWordException{Nepean}{Nepean}
\DefineJournalPartialAbbreviation{Nepholog}{Nephol}
\DefineJournalPartialAbbreviation{Nephrolog}{Nephrol}
\DefineJournalPartialAbbreviation{Nephropatholog}{Nephropathol}
\DefineJournalAbbreviation{Nephropathy}{Nephrop}
\DefineJournalPartialAbbreviation{Nephrotoxicit}{Nephrotox}
\DefineJournalPartialAbbreviation{Nephrourolog}{Nephrourol}
\DefineJournalAbbreviation{Nervous}{Nerv}
\DefineJournalWordException{Netball}{Netball}
\DefineJournalAbbreviation{Netherlands}{Neth}
\DefineJournalWordException{Netware}{Netware}
\DefineJournalAbbreviation{Network}{Netw}
\DefineJournalAbbreviation{Networking}{Netw}
\DefineJournalWordException{Neural}{Neural}
\DefineJournalPartialAbbreviation{Neuroactiv}{Neuroact}
\DefineJournalPartialAbbreviation{Neuroanaesthes}{Neuroanaesth}
\DefineJournalPartialAbbreviation{Neurobehavior}{Neurobehav}
\DefineJournalPartialAbbreviation{Neurochem}{Neurochem}
\DefineJournalPartialAbbreviation{Neurochirurg}{Neurochir}
\DefineJournalPartialAbbreviation{Neurocytochemi}{Neurocytochem}
\DefineJournalPartialAbbreviation{Neurocytolog}{Neurocytol}
\DefineJournalPartialAbbreviation{Neurodegenerati}{Neurodegener}
\DefineJournalPartialAbbreviation{Neurodevelop}{Neurodev}
\DefineJournalPartialAbbreviation{Neuroendocrinolog}{Neuroendocrinol}
\DefineJournalAbbreviation{Neuroengineering}{Neuroeng}
\DefineJournalPartialAbbreviation{Neuroetholog}{Neuroethol}
\DefineJournalPartialAbbreviation{Neurogastroenterolog}{Neurogastroenterol}
\DefineJournalAbbreviation{Neurogenetic}{Neurogenet}
\DefineJournalAbbreviation{Neuroglia}{Neurogl}
\DefineJournalAbbreviation{Neuroimmunoendocrinology}{Neuroimmunoendocrinol}
\DefineJournalPartialAbbreviation{Neuroimmunolog}{Neuroimmunol}
\DefineJournalWordException{Neuroma}{Neuroma}
\DefineJournalPartialAbbreviation{Neuromorpholog}{Neuromorphol}
\DefineJournalAbbreviation{Neuromuscular}{Neuromuscul}
\DefineJournalAbbreviation{Neuromusculoskeletal}{Neuromusculoskel}
\DefineJournalWordException{Neuron}{Neuron}
\DefineJournalWordException{Neurone}{Neurone}
\DefineJournalAbbreviation{Neuronuclear}{Neuronucl}
\DefineJournalPartialAbbreviation{Neuroophthalmolog}{Neuroophthalmol}
\DefineJournalAbbreviation{Neuropeptide}{Neuropept}
\DefineJournalPartialAbbreviation{Neuropharmacolog}{Neuropharmacol}
\DefineJournalPartialAbbreviation{Neuroplastic}{Neuroplast}
\DefineJournalWordException{Neuropsychiatry}{Neuropsychiatry}
\DefineJournalPartialAbbreviation{Neuropsychopharmacolog}{Neuropsychopharmacol}
\DefineJournalPartialAbbreviation{Neuropsychotherap}{Neuropsychother}
\DefineJournalAbbreviation{Neuropterology}{Neuropterol}
\DefineJournalPartialAbbreviation{Neuroradiolog}{Neuroradiol}
\DefineJournalPartialAbbreviation{Neuroreceptor}{Neurorecept}
\DefineJournalPartialAbbreviation{Neuroregulat}{Neuroregul}
\DefineJournalAbbreviation{Neurorehabilitation}{Neurorehabilit}
\DefineJournalPartialAbbreviation{Neuroscien}{Neurosci}
\DefineJournalAbbreviation{Neurosurgery}{Neurosurg}
\DefineJournalPartialAbbreviation{Neurosurgic}{Neurosurg}
\DefineJournalPartialAbbreviation{Neuroteratolog}{Neuroteratol}
\DefineJournalPartialAbbreviation{Neurotherap}{Neurother}
\DefineJournalPartialAbbreviation{Neurotolog}{Neurotol}
\DefineJournalAbbreviation{Neurotoxicity}{Neurotox}
\DefineJournalAbbreviation{Neurotransmitter}{Neurotransm}
\DefineJournalWordException{Neurotrauma}{Neurotrauma}
\DefineJournalPartialAbbreviation{Neurotraumatolog}{Neurotraumatol}
\DefineJournalAbbreviation{Neurotropic}{Neurotrop}
\DefineJournalAbbreviation{Neurourology}{Neurourol}
\DefineJournalAbbreviation{Neurovisceral}{Neurovisc}
\DefineJournalWordException{Neutron}{Neutron}
\DefineJournalWordException{Neuwsclip}{Neuwsclip}
\DefineJournalAbbreviation{Nevada}{Nev}
\DefineJournalAbbreviation{New Brunswick}{N B}
\DefineJournalAbbreviation{New England}{N Engl}
\DefineJournalAbbreviation{New Guinea}{N Guin}
\DefineJournalAbbreviation{New Hampshire}{N H}
\DefineJournalAbbreviation{New Haven}{N Hav}
\DefineJournalAbbreviation{New Hebrides}{N Hebr}
\DefineJournalAbbreviation{New Jersey}{N J}
\DefineJournalAbbreviation{New Mexico}{N M}
\DefineJournalAbbreviation{New South Wales}{N S W}
\DefineJournalAbbreviation{New York}{N Y}
\DefineJournalAbbreviation{New Zealand}{N Z}
\DefineJournalWordException{New-Carlisle}{New-Carlisle}
\DefineJournalWordException{New-Delhi}{New-Delhi}
\DefineJournalWordException{New-Orleans}{New-Orleans}
\DefineJournalAbbreviation{New-Zelandesa}{N-Z}
\DefineJournalWordException{Newark}{Newark}
\DefineJournalWordException{Newberry}{Newberry}
\DefineJournalAbbreviation{Newcastle}{Newctle}
\DefineJournalPartialAbbreviation{Newcom}{Newcom}
\DefineJournalAbbreviation{Newfoundland}{Nfld}
\DefineJournalAbbreviation{Newly}{New}
\DefineJournalAbbreviation{Newmarket}{Newmark}
\DefineJournalWordException{Newport}{Newport}
\DefineJournalWordException{Newport-on-Tay}{Newport-on-Tay}
\DefineJournalAbbreviation{News-sheet}{News-sh}
\DefineJournalAbbreviation{Newsagent}{Newsag}
\DefineJournalWordException{Newsberth}{Newsberth}
\DefineJournalAbbreviation{Newsbrief}{Newsbr}
\DefineJournalWordException{Newscall}{Newscall}
\DefineJournalAbbreviation{Newsclipping}{Newsclipp}
\DefineJournalWordException{Newsdata}{Newsdata}
\DefineJournalWordException{Newsday}{Newsday}
\DefineJournalAbbreviation{Newservice}{Newserv}
\DefineJournalWordException{Newsfacts}{Newsfacts}
\DefineJournalAbbreviation{Newsfile}{Newsf}
\DefineJournalWordException{Newsflash}{Newsflash}
\DefineJournalAbbreviation{Newsheet}{Newsh}
\DefineJournalAbbreviation{Newsjournal}{Newsj}
\DefineJournalAbbreviation{Newsletter}{Newsl}
\DefineJournalWordException{Newsline}{Newsline}
\DefineJournalPartialAbbreviation{Newsmag}{Newsmag}
\DefineJournalPartialAbbreviation{Newsmak}{Newsmak}
\DefineJournalWordException{Newsnote}{Newsnote}
\DefineJournalWordException{Newsoft}{Newsoft}
\DefineJournalAbbreviation{Newspaper}{Newsp}
\DefineJournalWordException{Newspatch}{Newspatch}
\DefineJournalAbbreviation{Newsprint}{Newspr}
\DefineJournalWordException{Newsreel}{Newsreel}
\DefineJournalAbbreviation{Newsreport}{Newsrep}
\DefineJournalAbbreviation{Newsreview}{Newsrev}
\DefineJournalAbbreviation{Newssheet}{Newssh}
\DefineJournalWordException{Newstorch}{Newstorch}
\DefineJournalAbbreviation{Newstrend}{Newstr}
\DefineJournalWordException{Newswatch}{Newswatch}
\DefineJournalWordException{Newsweek}{Newsweek}
\DefineJournalWordException{Newsworld}{Newsworld}
\DefineJournalWordException{Newton}{Newton}
\DefineJournalAbbreviation{Newtonian}{Newton}
\DefineJournalAbbreviation{Niagara Falls}{Niagara F}
\DefineJournalWordException{Nickname}{Nickname}
\DefineJournalAbbreviation{Nicosia}{Nicos}
\DefineJournalPartialAbbreviation{Nigeria}{Niger}
\DefineJournalWordException{Nightclub}{Nightclub}
\DefineJournalWordException{Nightingale}{Nightingale}
\DefineJournalWordException{Nightlife}{Nightlife}
\DefineJournalWordException{Nightmare}{Nightmare}
\DefineJournalPartialAbbreviation{Nineteen}{Ninet}
\DefineJournalWordException{Nineties}{Nineties}
\DefineJournalWordException{Nintendo}{Nintendo}
\DefineJournalPartialAbbreviation{Nitrocellulos}{Nitrocellul}
\DefineJournalWordException{Nitrogen}{Nitrogen}
\DefineJournalWordException{Nittany}{Nittany}
\DefineJournalWordException{Noarlunga}{Noarlunga}
\DefineJournalWordException{Nobody}{Nobody}
\DefineJournalWordException{Noetic}{Noetic}
%\DefineJournalPartialWordException{Nomad}{Nomad-}
\DefineJournalPartialAbbreviation{Nomenclat}{Nomencl}
\DefineJournalAbbreviation{Nominee}{Nomin}
\DefineJournalAbbreviation{Non-governement}{Non-gov}
\DefineJournalAbbreviation{Non-league}{Non-leag}
\DefineJournalWordException{Non-linear}{Non-linear}
\DefineJournalAbbreviation{Non-official}{Non-off}
\DefineJournalAbbreviation{Non-perishable}{Non-perish}
\DefineJournalAbbreviation{Non-proliferation}{Non-prolif}
\DefineJournalAbbreviation{Non-residential}{Non-resid}
\DefineJournalWordException{Non-wood}{Non-wood}
\DefineJournalAbbreviation{Nonbacterial}{Nonbact}
\DefineJournalPartialAbbreviation{Nonconservat}{Nonconserv}
\DefineJournalAbbreviation{Nonconventional}{Nonconv}
\DefineJournalAbbreviation{Noncrystal}{Noncryst}
\DefineJournalPartialAbbreviation{Noncultur}{Noncult}
\DefineJournalWordException{Nondegree}{Nondegree}
\DefineJournalPartialAbbreviation{Nondestruct}{Nondestruct}
\DefineJournalAbbreviation{Nondramatic}{Nondram}
\DefineJournalPartialAbbreviation{Nonfermentali}{Nonferment}
\DefineJournalAbbreviation{Nonfiction}{Nonfict}
\DefineJournalWordException{Nonfood}{Nonfood}
\DefineJournalAbbreviation{Nonformal}{Nonform}
\DefineJournalAbbreviation{Nonhuman}{Nonhum}
\DefineJournalWordException{Noninvasive}{Noninvasive}
\DefineJournalAbbreviation{Nonionic}{Nonion}
\DefineJournalPartialAbbreviation{Nonisotopi}{Nonisot}
\DefineJournalWordException{Nonlinear}{Nonlinear}
\DefineJournalPartialAbbreviation{Nonlithograph}{Nonlithogr}
\DefineJournalWordException{Nonliving}{Nonliving}
\DefineJournalAbbreviation{Nonmetallic}{Nonmet}
\DefineJournalWordException{Nonprofit}{Nonprofit}
\DefineJournalPartialAbbreviation{Nonpsychiatri}{Nonpsychiatr}
\DefineJournalWordException{Nonpublic}{Nonpublic}
\DefineJournalAbbreviation{Nonresonant}{Nonreson}
\DefineJournalPartialAbbreviation{Nonrespirat}{Nonrespir}
\DefineJournalWordException{Nonrubber}{Nonrubber}
\DefineJournalWordException{Nonsense}{Nonsense}
\DefineJournalPartialAbbreviation{Nonsmok}{Nonsmok}
\DefineJournalPartialAbbreviation{Nonstoichiometr}{Nonstoichiom}
\DefineJournalPartialAbbreviation{Nontradition}{Nontradit}
\DefineJournalWordException{Nonverbal}{Nonverbal}
\DefineJournalWordException{Nonwoven}{Nonwoven}
\DefineJournalWordException{Norcross}{Norcross}
\DefineJournalWordException{Norfolk}{Norfolk}
\DefineJournalWordException{Norman}{Norman}
\DefineJournalAbbreviation{Norseman}{Norsem}
\DefineJournalWordException{North}{North}
\DefineJournalAbbreviation{North America}{N Am}
\DefineJournalAbbreviation{North Atlantic}{N Atl}
\DefineJournalAbbreviation{North Brunswick}{N Brunsw}
\DefineJournalAbbreviation{North Carolina}{N C}
\DefineJournalAbbreviation{North Dakota}{N D}
\DefineJournalAbbreviation{North Melbourne}{N Melb}
\DefineJournalAbbreviation{North Queensland}{N Qld}
\DefineJournalWordException{North York}{North York}
\DefineJournalAbbreviation{North-Holland}{N-Holl}
\DefineJournalAbbreviation{Northampton}{Northamp}
\DefineJournalAbbreviation{Northamptonshire}{Northants}
\DefineJournalWordException{Northborogh}{Northborogh}
\DefineJournalWordException{Northbridge}{Northbridge}
\DefineJournalWordException{Northcliff}{Northcliff}
\DefineJournalPartialAbbreviation{Northeast}{Northeast}
\DefineJournalAbbreviation{Northern}{North}
\DefineJournalWordException{Northian}{Northian}
\DefineJournalAbbreviation{Northland}{Northl}
\DefineJournalWordException{Northside}{Northside}
\DefineJournalWordException{Northsouth}{Northsouth}
\DefineJournalAbbreviation{Northumberland}{Northumberl}
\DefineJournalAbbreviation{Northumbria}{Northumbr}
\DefineJournalWordException{Northwest}{Northwest}
\DefineJournalAbbreviation{Northwest Territories}{N W T}
\DefineJournalAbbreviation{Northwestern}{Northwest}
\DefineJournalAbbreviation{Norton}{Nort}
\DefineJournalAbbreviation{Norway}{Nor}
\DefineJournalAbbreviation{Norwegian}{Nor}
\DefineJournalWordException{Norwich}{Norwich}
\DefineJournalWordException{Norwood}{Norwood}
\DefineJournalAbbreviation{Nosocomial}{Nosocom}
\DefineJournalWordException{Notable}{Notable}
\DefineJournalPartialAbbreviation{Notaria}{Notar}
\DefineJournalWordException{Notary}{Notary}
\DefineJournalWordException{Note}{Note}
\DefineJournalAbbreviation{Notebook}{Noteb}
\DefineJournalWordException{Noter-up}{Noter-up}
\DefineJournalWordException{Noteworthy}{Noteworthy}
\DefineJournalWordException{Noticeboard}{Noticeboard}
\DefineJournalAbbreviation{Notifiable}{Notif}
\DefineJournalPartialAbbreviation{Notifica}{Notif}
\DefineJournalAbbreviation{Notified}{Notif}
\DefineJournalWordException{Notion}{Notion}
\DefineJournalAbbreviation{Nottingham}{Nottm}
\DefineJournalAbbreviation{Nottinghamshire}{Notts}
\DefineJournalPartialAbbreviation{Novel}{Nov}
\DefineJournalWordException{Nowhere}{Nowhere}
\DefineJournalWordException{Noxious}{Noxious}
\DefineJournalAbbreviation{Nterpolation}{Interpolat}
\DefineJournalPartialAbbreviation{Nuclear}{Nucl}
\DefineJournalAbbreviation{Nuclei}{Nucl}
\DefineJournalWordException{Nucleic}{Nucleic}
\DefineJournalPartialAbbreviation{Nucleonic}{Nucleon}
\DefineJournalWordException{Nucleoside}{Nucleoside}
\DefineJournalWordException{Nucleotide}{Nucleotide}
\DefineJournalAbbreviation{Nucleus}{Nucl}
\DefineJournalWordException{Nugget}{Nugget}
\DefineJournalAbbreviation{Nuisance}{Nuis}
\DefineJournalWordException{Number}{Number}
\DefineJournalPartialAbbreviation{Numeri}{Numer}
\DefineJournalAbbreviation{Numisletter}{Numislett}
\DefineJournalWordException{Nuneaton}{Nuneaton}
\DefineJournalWordException{Nurse}{Nurse}
\DefineJournalAbbreviation{Nursery}{Nurs}
\DefineJournalAbbreviation{Nurseryman}{Nurserym}
\DefineJournalAbbreviation{Nursing}{Nurs}
\DefineJournalPartialAbbreviation{Nurtur}{Nurtur}
\DefineJournalAbbreviation{Nutgrower}{Nutgrow}
\DefineJournalAbbreviation{Nutmegger}{Nutmegg}
\DefineJournalWordException{Nutshell}{Nutshell}
\DefineJournalWordException{Nyankpala}{Nyankpala}
\DefineJournalAbbreviation{Nyasaland}{Nyasal}
\DefineJournalAbbreviation{Oakland}{Oakl}
\DefineJournalAbbreviation{Oakville}{Oakv}
\DefineJournalWordException{Obedience}{Obedience}
\DefineJournalAbbreviation{Obesity}{Obes}
\DefineJournalWordException{Obiter}{Obiter}
\DefineJournalPartialAbbreviation{Obituar}{Obit}
\DefineJournalWordException{Object}{Object}
\DefineJournalAbbreviation{Obligation}{Oblig}
\DefineJournalWordException{Obsidian}{Obsidian}
\DefineJournalAbbreviation{Obstructive}{Obstr}
\DefineJournalPartialAbbreviation{Occasion}{Occas}
\DefineJournalAbbreviation{Occupancy}{Occup}
\DefineJournalPartialAbbreviation{Occupation}{Occup}
\DefineJournalAbbreviation{Occupied}{Occup}
\DefineJournalPartialAbbreviation{Occur}{Occur}
\DefineJournalAbbreviation{Oceania}{Ocean}
\DefineJournalAbbreviation{Oceanic}{Ocean}
\DefineJournalPartialAbbreviation{Oceanograph}{Oceanogr}
\DefineJournalPartialAbbreviation{Oceanolog}{Oceanol}
\DefineJournalWordException{Ocooh}{Ocooh}
\DefineJournalAbbreviation{Octagon}{Octag}
\DefineJournalAbbreviation{October}{Oct}
\DefineJournalWordException{Octopus}{Octopus}
\DefineJournalPartialAbbreviation{Oculist}{Ocul}
\DefineJournalPartialAbbreviation{Oculomotor}{Oculomot}
\DefineJournalWordException{Ododuma}{Ododuma}
\DefineJournalPartialAbbreviation{\oe colog}{\oe col}
\DefineJournalPartialAbbreviation{\oe conom}{\oe con}
\DefineJournalWordException{Offaly}{Offaly}
\DefineJournalWordException{Offence}{Offence}
\DefineJournalWordException{Offender}{Offender}
\DefineJournalWordException{Offense}{Offense}
\DefineJournalPartialAbbreviation{Offer}{Offer}
\DefineJournalAbbreviation{Offprint}{Offpr}
\DefineJournalWordException{Offroad}{Offroad}
\DefineJournalWordException{Offset}{Offset}
\DefineJournalAbbreviation{Offshoot}{Offsh}
\DefineJournalWordException{Offshore}{Offshore}
\DefineJournalAbbreviation{Ogdensburg}{Ogdensbg}
\DefineJournalWordException{Oilcake}{Oilcake}
\DefineJournalWordException{Oilfield}{Oilfield}
\DefineJournalWordException{Oilgram}{Oilgram}
\DefineJournalWordException{Oilman}{Oilman}
\DefineJournalWordException{Oilseed}{Oilseed}
\DefineJournalWordException{Oilspill}{Oilspill}
\DefineJournalWordException{Oilway}{Oilway}
\DefineJournalAbbreviation{Oilwell}{Oilw}
\DefineJournalWordException{Ointment}{Ointment}
\DefineJournalWordException{Ojibway}{Ojibway}
\DefineJournalWordException{Okanagan}{Okanagan}
\DefineJournalAbbreviation{Oklahoma}{Okla}
\DefineJournalAbbreviation{Oldsmobile}{Olds}
\DefineJournalPartialAbbreviation{Oldtim}{Oldtim}
\DefineJournalPartialAbbreviation{Olfactometr}{Olfactom}
\DefineJournalAbbreviation{Oligogenetic}{Oligogenet}
\DefineJournalAbbreviation{Oligosaccharide}{Oligosacch}
\DefineJournalPartialAbbreviation{Olymp}{Olymp}
\DefineJournalWordException{Ombudsman}{Ombudsman}
\DefineJournalAbbreviation{Oncobiomarkers}{Oncobiomark}
\DefineJournalAbbreviation{Oncofetal}{Oncofet}
\DefineJournalPartialAbbreviation{Oncogenes}{Oncog}
\DefineJournalPartialAbbreviation{Oncogeni}{Oncog}
\DefineJournalPartialAbbreviation{Oncolog}{Oncol}
\DefineJournalWordException{Ongoing}{Ongoing}
\DefineJournalWordException{Online}{Online}
\DefineJournalPartialAbbreviation{Onomasiolog}{Onomasiol}
\DefineJournalWordException{Onondaga}{Onondaga}
\DefineJournalWordException{Onoway}{Onoway}
\DefineJournalWordException{Onshore}{Onshore}
\DefineJournalWordException{Onsite}{Onsite}
\DefineJournalAbbreviation{Ontario}{Ont}
\DefineJournalWordException{Onward}{Onward}
\DefineJournalWordException{Opencast}{Opencast}
\DefineJournalWordException{Opener}{Opener}
\DefineJournalAbbreviation{Opening}{Open}
\DefineJournalWordException{Opera}{Opera}
\DefineJournalPartialAbbreviation{Operant}{Operant}
\DefineJournalWordException{Ophtalmic}{Ophtalmic}
\DefineJournalWordException{Ophthalmic}{Ophthalmic}
\DefineJournalPartialAbbreviation{Ophthalmolog}{Ophthalmol}
\DefineJournalPartialAbbreviation{Opinion}{Opin}
\DefineJournalPartialAbbreviation{Opportunit}{Oppor}
\DefineJournalAbbreviation{Opposition}{Oppos}
\DefineJournalPartialAbbreviation{Optic}{Opt}
\DefineJournalPartialAbbreviation{Optimal}{Optim}
\DefineJournalAbbreviation{Optimistic}{Optimist}
\DefineJournalPartialAbbreviation{Optimiz}{Optim}
\DefineJournalWordException{Option}{Option}
\DefineJournalAbbreviation{Optoacoustic}{Optoacoust}
\DefineJournalPartialAbbreviation{Optoelectron}{Optoelectron}
\DefineJournalPartialAbbreviation{Optomechani}{Optomech}
\DefineJournalAbbreviation{Optronics}{Optron}
\DefineJournalWordException{Opvertone}{Opvertone}
\DefineJournalWordException{Oracle}{Oracle}
\DefineJournalWordException{Oradell}{Oradell}
\DefineJournalWordException{Oratinese}{Oratinese}
\DefineJournalWordException{Oration}{Oration}
\DefineJournalPartialAbbreviation{Orchard}{Orchard}
\DefineJournalPartialAbbreviation{Orchestr}{Orch}
%\DefineJournalPartialWordException{Order}{Order-}
\DefineJournalPartialAbbreviation{Ordinanc}{Ord}
\DefineJournalWordException{Ordinary}{Ordinary}
\DefineJournalPartialAbbreviation{Ordinolog}{Ordinol}
\DefineJournalWordException{Ordnance}{Ordnance}
\DefineJournalAbbreviation{Oregon}{Or}
\DefineJournalWordException{Orford}{Orford}
\DefineJournalPartialAbbreviation{Organbuild}{Organbuild}
\DefineJournalAbbreviation{Organic}{Org}
\DefineJournalPartialAbbreviation{Organism}{Org}
\DefineJournalWordException{Organist}{Organist}
\DefineJournalPartialAbbreviation{Organize}{Organ}
\DefineJournalAbbreviation{Organizing}{Organ}
\DefineJournalAbbreviation{Organochlorine}{Organochlor}
\DefineJournalAbbreviation{Organofluorine}{Organofluor}
\DefineJournalPartialAbbreviation{Organogen}{Organog}
\DefineJournalAbbreviation{Organometallic}{Organomet}
\DefineJournalAbbreviation{Organosulfer}{Organosulf}
\DefineJournalAbbreviation{Orgonomy}{Orgon}
\DefineJournalPartialAbbreviation{Oriental}{Orient}
\DefineJournalAbbreviation{Orientation}{Orientat}
\DefineJournalWordException{Oriented}{Oriented}
\DefineJournalWordException{Orienteer}{Orienteer}
\DefineJournalAbbreviation{Orienteering}{Orienteer}
\DefineJournalAbbreviation{Orientique}{Orient}
\DefineJournalPartialAbbreviation{Origin}{Orig}
\DefineJournalWordException{Orillia}{Orillia}
\DefineJournalWordException{Oriole}{Oriole}
\DefineJournalWordException{Orissa}{Orissa}
\DefineJournalWordException{Orkney}{Orkney}
\DefineJournalWordException{Ormond}{Ormond}
\DefineJournalAbbreviation{Ornamental}{Ornam}
\DefineJournalPartialAbbreviation{Ornitholog}{Ornithol}
\DefineJournalAbbreviation{Orofacial}{Orofac}
\DefineJournalWordException{Orona}{Orona}
\DefineJournalWordException{Orphanage}{Orphanage}
\DefineJournalWordException{Orpheus}{Orpheus}
\DefineJournalPartialAbbreviation{Orthodont}{Orthod}
\DefineJournalPartialAbbreviation{Orthomolecular}{Orthomol}
\DefineJournalAbbreviation{Orthontic}{Orthont}
\DefineJournalPartialAbbreviation{Orthopaedagogi}{Orthopaedagog}
\DefineJournalPartialAbbreviation{Orthopaedi}{Orthop}
\DefineJournalPartialAbbreviation{Orthoped}{Orthop}
\DefineJournalPartialAbbreviation{Orthopsychiatri}{Orthopsychiatr}
\DefineJournalPartialAbbreviation{Orthoptic}{Orthopt}
\DefineJournalAbbreviation{Orthotics}{Orthot}
\DefineJournalWordException{Osgoode}{Osgoode}
\DefineJournalPartialAbbreviation{Osmoregul}{Osmoregul}
\DefineJournalWordException{Osprey}{Osprey}
\DefineJournalAbbreviation{Ossetian}{Osset}
\DefineJournalPartialAbbreviation{Ostdeutsch}{Ostdtsch}
\DefineJournalPartialAbbreviation{Osteoarchaeol}{Osteoarchaeol}
\DefineJournalAbbreviation{Osteoarthritis}{Osteoarthr}
\DefineJournalAbbreviation{Osteogenesis}{Osteogenes}
\DefineJournalPartialAbbreviation{Osteolog}{Osteol}
\DefineJournalWordException{Osteopath}{Osteopath}
\DefineJournalPartialAbbreviation{Osteopathic}{Osteopath}
\DefineJournalAbbreviation{Osteoporosis}{Osteoporos}
\DefineJournalWordException{Osteotomy}{Osteotomy}
\DefineJournalWordException{Ostomy}{Ostomy}
\DefineJournalWordException{Ostracod}{Ostracod}
\DefineJournalWordException{Osumenyi}{Osumenyi}
\DefineJournalWordException{Oswego}{Oswego}
\DefineJournalWordException{Other}{Other}
\DefineJournalAbbreviation{Ottawa}{Ott}
\DefineJournalWordException{Otterburne}{Otterburne}
%\DefineJournalPartialWordException{Ottom}{Ottom-}
\DefineJournalWordException{Ourself}{Ourself}
\DefineJournalWordException{Outaouais}{Outaouais}
\DefineJournalWordException{Outback}{Outback}
\DefineJournalPartialAbbreviation{Outboard}{Outboard}
\DefineJournalWordException{Outbound}{Outbound}
\DefineJournalWordException{Outbreak}{Outbreak}
\DefineJournalWordException{Outcome}{Outcome}
\DefineJournalWordException{Outcry}{Outcry}
\DefineJournalWordException{Outdoor}{Outdoor}
\DefineJournalWordException{Outdoorsman}{Outdoorsman}
\DefineJournalPartialAbbreviation{Outfit}{Outfit}
\DefineJournalWordException{Outing}{Outing}
\DefineJournalWordException{Outlaw}{Outlaw}
\DefineJournalWordException{Outlay}{Outlay}
\DefineJournalWordException{Outlet}{Outlet}
\DefineJournalAbbreviation{Outline}{Outl}
\DefineJournalWordException{Outlook}{Outlook}
\DefineJournalWordException{Outpatient}{Outpatient}
\DefineJournalWordException{Outport}{Outport}
\DefineJournalWordException{Outpost}{Outpost}
\DefineJournalWordException{Output}{Output}
\DefineJournalWordException{Outreach}{Outreach}
\DefineJournalWordException{Outremont}{Outremont}
\DefineJournalPartialAbbreviation{Outside}{Outs}
\DefineJournalAbbreviation{Outstanding}{Outst}
\DefineJournalAbbreviation{Outward}{Outw}
\DefineJournalWordException{Overall}{Overall}
\DefineJournalWordException{Overcheck}{Overcheck}
\DefineJournalWordException{Overcome}{Overcome}
\DefineJournalAbbreviation{Overcrowding}{Overcrowd}
\DefineJournalWordException{Overdrive}{Overdrive}
%\DefineJournalPartialWordException{Overfish}{Overfish-}
\DefineJournalWordException{Overhaul}{Overhaul}
\DefineJournalWordException{Overhead}{Overhead}
\DefineJournalWordException{Overige}{Overige}
\DefineJournalAbbreviation{Overland}{Overl}
\DefineJournalAbbreviation{Overland Park}{Overl Park}
\DefineJournalWordException{Overseas}{Overseas}
\DefineJournalPartialAbbreviation{Oversight}{Overs}
\DefineJournalWordException{Overstress}{Overstress}
\DefineJournalWordException{Overtone}{Overtone}
\DefineJournalAbbreviation{Overture}{Overt}
\DefineJournalAbbreviation{Overview}{Overv}
\DefineJournalAbbreviation{Overvoltage}{Overvolt}
\DefineJournalAbbreviation{Ovulation}{Ovul}
\DefineJournalWordException{Owen-Sound}{Owen-Sound}
\DefineJournalWordException{Owerri}{Owerri}
\DefineJournalAbbreviation{Owned}{Own}
\DefineJournalAbbreviation{Owner}{Own}
\DefineJournalAbbreviation{Ownership}{Ownersh}
\DefineJournalWordException{Oxbridge}{Oxbridge}
\DefineJournalAbbreviation{Oxford}{Oxf}
\DefineJournalAbbreviation{Oxfordshire}{Oxfs}
\DefineJournalPartialAbbreviation{Oxidant}{Oxid}
\DefineJournalAbbreviation{Oxidation}{Oxid}
\DefineJournalAbbreviation{Oxidising}{Oxid}
\DefineJournalAbbreviation{Oxidizing}{Oxid}
\DefineJournalAbbreviation{Oxidoreduction}{Oxidoreduct}
\DefineJournalAbbreviation{Oxoniensia}{Oxon}
\DefineJournalWordException{Oxted}{Oxted}
\DefineJournalPartialAbbreviation{Oxygen}{Oxyg}
\DefineJournalWordException{Oyster}{Oyster}
\DefineJournalAbbreviation{Pacemaker}{Pacemak}
\DefineJournalAbbreviation{Pacific}{Pac}
\DefineJournalWordException{Pacing}{Pacing}
\DefineJournalPartialAbbreviation{Packag}{Packag}
\DefineJournalWordException{Package}{Package}
\DefineJournalAbbreviation{Packer}{Pack}
\DefineJournalPartialAbbreviation{Packet}{Pack}
\DefineJournalAbbreviation{Packing}{Pack}
\DefineJournalAbbreviation{Packinghouse}{Packingh}
\DefineJournalWordException{Paddle}{Paddle}
\DefineJournalPartialAbbreviation{Paedagogi}{Paedagog}
\DefineJournalPartialAbbreviation{Paediatri}{Paediatr}
\DefineJournalPartialAbbreviation{Paedopsychiatri}{Paedopsychiatr}
\DefineJournalWordException{Pagan}{Pagan}
\DefineJournalWordException{Pageant}{Pageant}
\DefineJournalPartialAbbreviation{Paint}{Paint}
\DefineJournalAbbreviation{Paintball}{Paintb}
\DefineJournalPartialAbbreviation{Pakistan}{Pak}
\DefineJournalWordException{Palace}{Palace}
\DefineJournalAbbreviation{Palaearctic}{Palaearct}
\DefineJournalPartialAbbreviation{Palaenthropolog}{Palaenthropol}
\DefineJournalPartialAbbreviation{Palaeobotan}{Palaeobot}
\DefineJournalPartialAbbreviation{Palaeoclimat}{Palaeoclim}
\DefineJournalPartialAbbreviation{Palaeoclimatolog}{Palaeoclimatol}
\DefineJournalPartialAbbreviation{Palaeoecolog}{Palaeoecol}
\DefineJournalPartialAbbreviation{Palaeogeograph}{Palaeogeogr}
\DefineJournalAbbreviation{Palaeoichthyological}{Palaeoichthyol}
\DefineJournalPartialAbbreviation{Palaeontograph}{Palaeontogr}
\DefineJournalPartialAbbreviation{Palaeontolog}{Palaeontol}
\DefineJournalAbbreviation{Palaeozoic}{Palaeoz}
\DefineJournalWordException{Palate}{Palate}
\DefineJournalAbbreviation{Palearctic}{Palearct}
\DefineJournalPartialAbbreviation{Paleobotani}{Paleobot}
\DefineJournalAbbreviation{Paleocarpology}{Paleocarpol}
\DefineJournalPartialAbbreviation{Paleoceanograph}{Paleoceanogr}
\DefineJournalPartialAbbreviation{Paleoenvironment}{Paleoenviron}
\DefineJournalPartialAbbreviation{Pal\'eo\'ethnolog}{Paleoethnol}
\DefineJournalWordException{Paleogene}{Paleogene}
\DefineJournalPartialAbbreviation{Paleogeograf}{Paleogeogr}
\DefineJournalPartialAbbreviation{Paleolimnolog}{Paleolimnol}
\DefineJournalAbbreviation{Paleopathology}{Paleopathol}
\DefineJournalPartialAbbreviation{Paleosurfac}{Paleosurf}
\DefineJournalAbbreviation{Paleovisitology}{Paleovisitol}
\DefineJournalAbbreviation{Paleozoic}{Paleoz}
\DefineJournalWordException{Palisade}{Palisade}
\DefineJournalWordException{Pallet}{Pallet}
\DefineJournalAbbreviation{Palliative}{Palliat}
\DefineJournalWordException{Palmer}{Palmer}
\DefineJournalAbbreviation{Palmerston}{Palmerst}
\DefineJournalAbbreviation{Palmerston North}{Palmerst N}
\DefineJournalAbbreviation{Palmetto}{Palm}
\DefineJournalWordException{Palmistry}{Palmistry}
\DefineJournalWordException{Palmoil}{Palmoil}
\DefineJournalWordException{Palynomorph}{Palynomorph}
\DefineJournalWordException{Pamleco}{Pamleco}
\DefineJournalPartialAbbreviation{Pamphlet}{Pam}
\DefineJournalAbbreviation{Pan-European}{Pan-Eur}
\DefineJournalWordException{Panamax}{Panamax}
\DefineJournalPartialAbbreviation{Panamerican}{Panam}
\DefineJournalWordException{Pancake}{Pancake}
\DefineJournalAbbreviation{Pancreatic}{Pancreat}
\DefineJournalAbbreviation{Pancreatitis}{Pancreat}
\DefineJournalPartialAbbreviation{Pancreatolog}{Pancreatol}
\DefineJournalWordException{Pandora}{Pandora}
\DefineJournalAbbreviation{Paneuropean}{Paneur}
\DefineJournalPartialAbbreviation{Panhand}{Panhand}
\DefineJournalAbbreviation{Panjabi}{Panj}
\DefineJournalAbbreviation{Panoptic}{Panopt}
\DefineJournalAbbreviation{Panoramic}{Panor}
\DefineJournalPartialAbbreviation{Paper}{Pap}
\DefineJournalAbbreviation{Paperback}{Paperb}
\DefineJournalWordException{Paperboard}{Paperboard}
\DefineJournalWordException{Paperbound}{Paperbound}
\DefineJournalPartialAbbreviation{Papermachin}{Papermach}
\DefineJournalPartialAbbreviation{Papermak}{Papermak}
\DefineJournalWordException{Paperprintpack}{Paperprintpack}
\DefineJournalWordException{Papillomavirus}{Papillomavirus}
\DefineJournalWordException{Papua}{Papua}
\DefineJournalAbbreviation{Papua New Guinea}{P N G}
\DefineJournalAbbreviation{Paquetville}{Paquetv}
\DefineJournalWordException{Parable}{Parable}
\DefineJournalWordException{Paraclete}{Paraclete}
\DefineJournalPartialAbbreviation{Paraclinic}{Paraclin}
\DefineJournalWordException{Parade}{Parade}
\DefineJournalWordException{Parader}{Parader}
\DefineJournalWordException{Paradise}{Paradise}
\DefineJournalWordException{Paragon}{Paragon}
\DefineJournalWordException{Paralegal}{Paralegal}
\DefineJournalWordException{Parallel}{Parallel}
\DefineJournalAbbreviation{Parall\'elogramme}{Parallelogr}
\DefineJournalWordException{Parameter}{Parameter}
\DefineJournalAbbreviation{Paraphernalia}{Paraphern}
\DefineJournalAbbreviation{Paraplegic}{Parapleg}
\DefineJournalAbbreviation{Parapublic}{Parapub}
\DefineJournalPartialAbbreviation{Parasita}{Parasit}
\DefineJournalWordException{Parasite}{Parasite}
\DefineJournalPartialAbbreviation{Parasiti}{Parasit}
\DefineJournalAbbreviation{Parasitoid}{Parasit}
\DefineJournalPartialAbbreviation{Parasitolog}{Parasitol}
\DefineJournalWordException{Paratec}{Paratec}
\DefineJournalAbbreviation{Parathyroid}{Parathyr}
\DefineJournalWordException{Parent}{Parent}
\DefineJournalAbbreviation{Parental}{Parent}
\DefineJournalAbbreviation{Parenteral}{Parenter}
\DefineJournalAbbreviation{Parenthood}{Parent}
\DefineJournalAbbreviation{Parenting}{Parent}
\DefineJournalWordException{Parish}{Parish}
\DefineJournalAbbreviation{Parishioner}{Parish}
\DefineJournalWordException{Park}{Park}
\DefineJournalPartialAbbreviation{Park}{Park}
\DefineJournalWordException{Park-Ridge}{Park-Ridge}
\DefineJournalWordException{Parksville}{Parksville}
\DefineJournalWordException{Parkville}{Parkville}
\DefineJournalAbbreviation{Parkway}{Parkw}
\DefineJournalPartialAbbreviation{Parlement}{Parlem}
\DefineJournalPartialAbbreviation{Parliament}{Parliam}
\DefineJournalAbbreviation{Parnassus}{Parnass}
\DefineJournalPartialAbbreviation{Parol}{Parol}
\DefineJournalWordException{Parramatta}{Parramatta}
\DefineJournalWordException{Parrot}{Parrot}
\DefineJournalWordException{Part}{Part}
\DefineJournalAbbreviation{Partaxis}{Partax}
\DefineJournalPartialAbbreviation{Partial}{Partial}
\DefineJournalPartialAbbreviation{Particle}{Part}
\DefineJournalWordException{Particleboard}{Particleboard}
\DefineJournalPartialAbbreviation{Particul}{Part}
\DefineJournalAbbreviation{Partisan}{Partis}
\DefineJournalAbbreviation{Partner}{Partn}
\DefineJournalAbbreviation{Partnership}{Partnersh}
\DefineJournalWordException{Pasadena}{Pasadena}
\DefineJournalAbbreviation{Passarella}{Passar}
\DefineJournalAbbreviation{Passed}{Pass}
\DefineJournalAbbreviation{Passenger}{Passeng}
\DefineJournalAbbreviation{Passerella}{Passer}
\DefineJournalPartialAbbreviation{Passiv}{Passiv}
\DefineJournalAbbreviation{Passport}{Passpt}
\DefineJournalWordException{Password}{Password}
\DefineJournalWordException{Pastime}{Pastime}
\DefineJournalPartialAbbreviation{Pastor}{Pastor}
\DefineJournalAbbreviation{Pastoral}{Pastor}
\DefineJournalPartialAbbreviation{Pastrycook}{Pastrycook}
\DefineJournalWordException{Pasture}{Pasture}
\DefineJournalAbbreviation{Patchwork}{Patchw}
\DefineJournalAbbreviation{Patent}{Pat}
\DefineJournalPartialAbbreviation{Patente}{Pat}
\DefineJournalPartialAbbreviation{Pathfind}{Pathfind}
\DefineJournalPartialAbbreviation{Pathochemi}{Pathochem}
\DefineJournalPartialAbbreviation{Pathophysiolog}{Pathophysiol}
\DefineJournalAbbreviation{Pathway}{Pathw}
\DefineJournalWordException{Patient}{Patient}
%\DefineJournalPartialWordException{Patriarch}{Patriarch-}
\DefineJournalPartialAbbreviation{Patriot}{Patriot}
\DefineJournalWordException{Patrol}{Patrol}
\DefineJournalWordException{Pattern}{Pattern}
\DefineJournalWordException{Pavement}{Pavement}
\DefineJournalWordException{Pavilion}{Pavilion}
\DefineJournalAbbreviation{Pawtucket}{Pawtuck}
\DefineJournalPartialAbbreviation{Payant}{Pay}
\DefineJournalWordException{Payback}{Payback}
\DefineJournalWordException{Paying}{Paying}
\DefineJournalAbbreviation{Payment}{Paym}
\DefineJournalPartialAbbreviation{Payroll}{Payr}
\DefineJournalWordException{Peace}{Peace}
\DefineJournalAbbreviation{Peaceful}{Peac}
\DefineJournalWordException{Peacefund}{Peacefund}
\DefineJournalAbbreviation{Peacemaker}{Peacemak}
\DefineJournalWordException{Peanut}{Peanut}
\DefineJournalWordException{Pearl}{Pearl}
\DefineJournalPartialAbbreviation{Peasant}{Peasant}
\DefineJournalAbbreviation{Peatland}{Peatl}
\DefineJournalWordException{Pedal}{Pedal}
\DefineJournalAbbreviation{Pedestrian}{Pedestr}
\DefineJournalWordException{Pedigree}{Pedigree}
\DefineJournalPartialAbbreviation{Pedodon}{Pedod}
\DefineJournalAbbreviation{Pedorthics}{Pedorth}
\DefineJournalAbbreviation{Peeling}{Peel}
\DefineJournalPartialAbbreviation{Peen}{Peen}
\DefineJournalWordException{Pegasus}{Pegasus}
\DefineJournalWordException{Pelagic}{Pelagic}
\DefineJournalAbbreviation{Pelargonium}{Pelarg}
\DefineJournalWordException{P\'elican}{P\'elican}
\DefineJournalWordException{Pelvic}{Pelvic}
\DefineJournalAbbreviation{Pembroke}{Pemb}
\DefineJournalAbbreviation{Pembrokeshire}{Pembs}
\DefineJournalPartialAbbreviation{Penal}{Penal}
\DefineJournalWordException{Penang}{Penang}
\DefineJournalWordException{Pencil}{Pencil}
\DefineJournalWordException{Pending}{Pending}
\DefineJournalPartialAbbreviation{Peneolog}{Peneol}
\DefineJournalWordException{Penetanguishene}{Penetanguishene}
\DefineJournalWordException{Penguin}{Penguin}
\DefineJournalWordException{Penicillin}{Penicillin}
\DefineJournalWordException{Penjing}{Penjing}
\DefineJournalAbbreviation{Pennsylvania}{Pa}
\DefineJournalWordException{Pennyball}{Pennyball}
\DefineJournalPartialAbbreviation{Penolog}{Penol}
\DefineJournalWordException{Penryn}{Penryn}
%\DefineJournalPartialWordException{Pension}{Pension-}
\DefineJournalAbbreviation{Pensioner}{Pension}
\DefineJournalWordException{Pentacle}{Pentacle}
\DefineJournalWordException{Pentagram}{Pentagram}
\DefineJournalAbbreviation{Pentane}{Pent}
\DefineJournalWordException{Pentathlon}{Pentathlon}
\DefineJournalWordException{Pentecost}{Pentecost}
\DefineJournalWordException{Pentecostal}{Pentecostal}
\DefineJournalWordException{Penthouse}{Penthouse}
\DefineJournalWordException{Penticost}{Penticost}
\DefineJournalAbbreviation{Penultimate}{Penult}
\DefineJournalWordException{People}{People}
\DefineJournalWordException{Peoria}{Peoria}
\DefineJournalWordException{Pepper}{Pepper}
\DefineJournalPartialAbbreviation{Pepsinogen}{Pepsinog}
\DefineJournalWordException{Peptalk}{Peptalk}
\DefineJournalWordException{Peptic}{Peptic}
\DefineJournalWordException{Percent}{Percent}
\DefineJournalAbbreviation{Percentage}{Percent}
\DefineJournalAbbreviation{Perception}{Percept}
\DefineJournalAbbreviation{Perceptual}{Percept}
\DefineJournalAbbreviation{Perennial}{Perenn}
\DefineJournalWordException{Perfect}{Perfect}
\DefineJournalPartialAbbreviation{Perfection}{Perfect}
\DefineJournalPartialAbbreviation{Perfluorochem}{Perfluorochem}
\DefineJournalAbbreviation{Performability}{Perform}
\DefineJournalAbbreviation{Performance}{Perform}
\DefineJournalAbbreviation{Performer}{Perform}
\DefineJournalAbbreviation{Performing}{Perform}
\DefineJournalAbbreviation{Pericardial}{Pericard}
\DefineJournalAbbreviation{Periglacial}{Periglac}
\DefineJournalAbbreviation{Perinatal}{P\'erinat}
\DefineJournalWordException{Period}{Period}
\DefineJournalWordException{Periodoncia}{Periodoncia}
\DefineJournalWordException{Periodontal}{Periodontal}
\DefineJournalWordException{Periodontic}{Periodontic}
\DefineJournalWordException{Perional}{Perional}
\DefineJournalPartialAbbreviation{Perioperat}{Perioper}
\DefineJournalPartialAbbreviation{Peripher}{Peripher}
\DefineJournalPartialAbbreviation{Periscop}{Perisc}
\DefineJournalAbbreviation{Perishable}{Perish}
\DefineJournalAbbreviation{Peritoneal}{Perit}
\DefineJournalAbbreviation{Permafrost}{Permafr}
\DefineJournalPartialAbbreviation{Permanent}{Perm}
\DefineJournalAbbreviation{Permeation}{Permeat}
\DefineJournalWordException{Permian}{Permian}
\DefineJournalWordException{Permit}{Permit}
\DefineJournalPartialAbbreviation{Permut}{Permut}
\DefineJournalWordException{Perpetual}{Perpetual}
\DefineJournalPartialAbbreviation{Perquisit}{Perquis}
\DefineJournalWordException{Persian}{Persian}
\DefineJournalAbbreviation{Personalist}{Pers}
\DefineJournalPartialAbbreviation{Persuasi}{Persuas}
\DefineJournalPartialAbbreviation{Pertain}{Pertain}
\DefineJournalAbbreviation{Pertinent}{Pertin}
\DefineJournalAbbreviation{Peruvian}{Peruv}
\DefineJournalWordException{Petaluma}{Petaluma}
\DefineJournalWordException{Petawawa}{Petawawa}
\DefineJournalAbbreviation{Peterborough}{Peterb}
\DefineJournalAbbreviation{Peterhead}{Peterh}
\DefineJournalWordException{Peterloo}{Peterloo}
\DefineJournalAbbreviation{Petersfield}{Petersf}
\DefineJournalWordException{Petition}{Petition}
\DefineJournalAbbreviation{Petitioner}{Petition}
\DefineJournalPartialAbbreviation{Petroanaly}{Petroanal}
\DefineJournalPartialAbbreviation{Petrochem}{Petrochem}
\DefineJournalAbbreviation{Petroglyph}{Petrogl}
\DefineJournalPartialAbbreviation{Petrograph}{Petrogr}
\DefineJournalAbbreviation{Petrophysical}{Petrophys}
\DefineJournalPartialAbbreviation{Phaenolog}{Phaenol}
\DefineJournalWordException{Phallet}{Phallet}
\DefineJournalAbbreviation{Phanerozoic}{Phaneroz}
\DefineJournalWordException{Phantasmagoria}{Phantasmagoria}
\DefineJournalPartialAbbreviation{Pharmaceut}{Pharm}
\DefineJournalPartialAbbreviation{Pharmaci}{Pharm}
\DefineJournalAbbreviation{Pharmaco}{Pharm}
\DefineJournalPartialAbbreviation{Pharmacochemi}{Pharmacochem}
\DefineJournalPartialAbbreviation{Pharmacocineti}{Pharmacocinet}
\DefineJournalPartialAbbreviation{Pharmacoepidemiol}{Pharmacoepidemiol}
\DefineJournalPartialAbbreviation{Pharmacognos}{Pharmacogn}
\DefineJournalPartialAbbreviation{Pharmacokineti}{Pharmacokinet}
\DefineJournalPartialAbbreviation{Pharmacolog}{Pharmacol}
\DefineJournalPartialAbbreviation{Pharmacomed}{Pharmacomed}
\DefineJournalAbbreviation{Pharmacometric}{Pharmacomet}
\DefineJournalPartialAbbreviation{Pharmacopsychiatri}{Pharmacopsychiatr}
\DefineJournalAbbreviation{Pharmacopuncture}{Pharmacopunct}
\DefineJournalPartialAbbreviation{Pharmacotherap}{Pharmacother}
\DefineJournalAbbreviation{Pharmacovigilance}{Pharmacovigil}
\DefineJournalAbbreviation{Pharmacy}{Pharm}
\DefineJournalWordException{Pharos}{Pharos}
\DefineJournalAbbreviation{Pheasant}{Pheas}
\DefineJournalPartialAbbreviation{Phenolog}{Phenol}
\DefineJournalAbbreviation{Phenomena}{Phenom}
\DefineJournalAbbreviation{Phenomenon}{Phenom}
\DefineJournalAbbreviation{Philadelphia}{Phila}
\DefineJournalAbbreviation{Philamlife}{Philaml}
\DefineJournalPartialAbbreviation{Philatel}{Philat}
\DefineJournalPartialAbbreviation{Philippin}{Philipp}
\DefineJournalPartialAbbreviation{Philolog}{Philol}
\DefineJournalPartialAbbreviation{Philonic}{Philon}
\DefineJournalWordException{Philwomenian}{Philwomenian}
\DefineJournalWordException{Phoenix}{Phoenix}
\DefineJournalAbbreviation{Phonecard}{Phonec}
\DefineJournalWordException{Phonotape}{Phonotape}
\DefineJournalWordException{Phosphatase}{Phosphatase}
\DefineJournalAbbreviation{Phosphoprotein}{Phosphoprot}
\DefineJournalWordException{Phosphorites}{Phosphorites}
\DefineJournalWordException{Phosphorus}{Phosphorus}
\DefineJournalWordException{Phosphorylation}{Phosphorylation}
\DefineJournalAbbreviation{Photo-engraver}{Photo-engrav}
\DefineJournalAbbreviation{Photoacoustic}{Photoacoust}
\DefineJournalPartialAbbreviation{Photobiochemistr}{Photobiochem}
\DefineJournalPartialAbbreviation{Photobiophysi}{Photobiophys}
\DefineJournalPartialAbbreviation{Photocatalys}{Photocatal}
\DefineJournalPartialAbbreviation{Photochem}{Photochem}
\DefineJournalAbbreviation{Photocoagulation}{Photocoagul}
\DefineJournalPartialAbbreviation{Photoconduct}{Photocond}
\DefineJournalPartialAbbreviation{Photoconversion}{Photoconvers}
\DefineJournalPartialAbbreviation{Photodermatolog}{Photodermatol}
\DefineJournalPartialAbbreviation{Photodynami}{Photodyn}
\DefineJournalPartialAbbreviation{Photoeffect}{Photoeff}
\DefineJournalAbbreviation{Photoelastic}{Photoelast}
\DefineJournalAbbreviation{Photoelectric}{Photoelectr}
\DefineJournalPartialAbbreviation{Photoelectrochemi}{Photoelectrochem}
\DefineJournalPartialAbbreviation{Photoelectroni}{Photoelectron}
\DefineJournalPartialAbbreviation{Photoemission}{Photoemiss}
\DefineJournalPartialAbbreviation{Photofabricat}{Photofabr}
\DefineJournalPartialAbbreviation{Photofunction}{Photofunct}
\DefineJournalPartialAbbreviation{Photogenerati}{Photogener}
\DefineJournalWordException{Photoguide}{Photoguide}
\DefineJournalAbbreviation{Photohistorian}{Photohist}
\DefineJournalPartialAbbreviation{Photoimmunolog}{Photoimmunol}
\DefineJournalPartialAbbreviation{Photoionis}{Photoionis}
\DefineJournalPartialAbbreviation{Photomechani}{Photomech}
\DefineJournalAbbreviation{Photomedicine}{Photomed}
\DefineJournalPartialAbbreviation{Photomicrograph}{Photomicrogr}
%\DefineJournalPartialWordException{Photon}{Photon-}
\DefineJournalWordException{Photonews}{Photonews}
\DefineJournalPartialAbbreviation{Photoperiodi}{Photoperiod}
\DefineJournalWordException{Photoplay}{Photoplay}
\DefineJournalAbbreviation{Photopolymer}{Photopolym}
\DefineJournalPartialAbbreviation{Photosensiti}{Photosensit}
\DefineJournalPartialAbbreviation{Photosynth}{Photosynth}
\DefineJournalPartialAbbreviation{Photosystem}{Photosyst}
\DefineJournalAbbreviation{Phototheque}{Phototh}
\DefineJournalPartialAbbreviation{Phototransformation}{Phototransform}
\DefineJournalWordException{Photovideo}{Photovideo}
\DefineJournalAbbreviation{Photovoltaic}{Photovolt}
\DefineJournalWordException{Photoworld}{Photoworld}
\DefineJournalPartialAbbreviation{Phraseolog}{Phraseol}
\DefineJournalPartialAbbreviation{Phrenolog}{Phrenol}
\DefineJournalWordException{Phulbani}{Phulbani}
\DefineJournalPartialAbbreviation{Phycolog}{Phycol}
\DefineJournalPartialAbbreviation{Physica}{Phys}
\DefineJournalWordException{Physician}{Physician}
\DefineJournalPartialAbbreviation{Physicist}{Phys}
\DefineJournalAbbreviation{Physico}{Phys}
\DefineJournalPartialAbbreviation{Physicochem}{Physicochem}
\DefineJournalPartialAbbreviation{Physicomathemat}{Physicomath}
\DefineJournalPartialAbbreviation{Physicotechni}{Physicotech}
\DefineJournalAbbreviation{Physics}{Phys}
\DefineJournalAbbreviation{Phytodepuration}{Phytodepur}
\DefineJournalPartialAbbreviation{Phytoecolog}{Phytoecol}
\DefineJournalAbbreviation{Phytohormone}{Phytohorm}
\DefineJournalPartialAbbreviation{Phytohygien}{Phytohyg}
\DefineJournalAbbreviation{Phytolitharien}{Phytolith}
\DefineJournalPartialAbbreviation{Phytopharmac}{Phytopharm}
\DefineJournalWordException{Phytophthora}{Phytophthora}
\DefineJournalPartialAbbreviation{Phytophysiolog}{Phytophysiol}
\DefineJournalPartialAbbreviation{Pick}{Pick}
\DefineJournalWordException{Pickup}{Pickup}
\DefineJournalWordException{Pickwick}{Pickwick}
\DefineJournalAbbreviation{Pictorial}{Pict}
\DefineJournalPartialAbbreviation{Picture}{Pict}
\DefineJournalWordException{Pidgin}{Pidgin}
\DefineJournalWordException{Piedmont}{Piedmont}
\DefineJournalWordException{Pielaw}{Pielaw}
\DefineJournalWordException{Pigeonpea}{Pigeonpea}
\DefineJournalAbbreviation{Pikeville}{Pikev}
\DefineJournalAbbreviation{Pilgrim}{Pilgr}
\DefineJournalPartialAbbreviation{Pilgrimag}{Pilgr}
\DefineJournalWordException{Pillar}{Pillar}
\DefineJournalWordException{Pillow}{Pillow}
\DefineJournalAbbreviation{Pillowcase}{Pillowc}
\DefineJournalWordException{Pilot}{Pilot}
\DefineJournalWordException{Pineal}{Pineal}
\DefineJournalWordException{Pinery}{Pinery}
\DefineJournalWordException{Pinnacle}{Pinnacle}
\DefineJournalWordException{Pinpointer}{Pinpointer}
\DefineJournalWordException{Pioneer}{Pioneer}
\DefineJournalAbbreviation{Pioneering}{Pioneer}
\DefineJournalWordException{Pipeband}{Pipeband}
\DefineJournalWordException{Pipeline}{Pipeline}
\DefineJournalPartialAbbreviation{Pipeweld}{Pipeweld}
\DefineJournalAbbreviation{Piping}{Pip}
\DefineJournalAbbreviation{Piroplasmosis}{Piroplasm}
\DefineJournalPartialAbbreviation{Piscicult}{Piscic}
\DefineJournalWordException{Pitfield}{Pitfield}
\DefineJournalWordException{Pitlochry}{Pitlochry}
\DefineJournalAbbreviation{Pittsburg}{Pittsbg}
\DefineJournalWordException{Pittsburgh}{Pittsburgh}
\DefineJournalAbbreviation{Pittsfield}{Pittsfld}
\DefineJournalAbbreviation{Pituitary}{Pituit}
\DefineJournalWordException{Place}{Place}
\DefineJournalAbbreviation{Placental}{Placent}
\DefineJournalAbbreviation{Plainsman}{Plainsm}
\DefineJournalWordException{Plainsong}{Plainsong}
\DefineJournalWordException{Planahome}{Planahome}
\DefineJournalWordException{Plane}{Plane}
\DefineJournalAbbreviation{Planetarium}{Planet}
\DefineJournalAbbreviation{Planetary}{Planet}
\DefineJournalPartialAbbreviation{Planetolog}{Planetol}
\DefineJournalWordException{Planing}{Planing}
\DefineJournalWordException{Plankton}{Plankton}
\DefineJournalWordException{Planktonic}{Planktonic}
\DefineJournalAbbreviation{Planned}{Plan}
\DefineJournalAbbreviation{Planner}{Plan}
\DefineJournalAbbreviation{Planning}{Plan}
\DefineJournalWordException{Plant}{Plant}
\DefineJournalPartialAbbreviation{Plantation}{Plant}
\DefineJournalAbbreviation{Planted}{Plant}
\DefineJournalAbbreviation{Plantgrowing}{Plantgrow}
\DefineJournalAbbreviation{Planting}{Plant}
\DefineJournalPartialAbbreviation{Plantmak}{Plantmak}
\DefineJournalWordException{Plaque}{Plaque}
\DefineJournalWordException{Plasmapheresis}{Plasmapheresis}
\DefineJournalAbbreviation{Plasmonics}{Plasmon}
\DefineJournalPartialAbbreviation{Plaster}{Plaster}
\DefineJournalWordException{Platelet}{Platelet}
\DefineJournalPartialAbbreviation{Platemak}{Platemak}
\DefineJournalAbbreviation{Platform}{Platf}
\DefineJournalAbbreviation{Plating}{Plat}
\DefineJournalAbbreviation{Plattsburgh}{Plattsbg}
\DefineJournalAbbreviation{Plattsville}{Plattsv}
\DefineJournalPartialAbbreviation{Play}{Play}
\DefineJournalAbbreviation{Playbook}{Playb}
\DefineJournalWordException{Playboy}{Playboy}
\DefineJournalAbbreviation{Playcentre}{Playcent}
\DefineJournalWordException{Playcraft}{Playcraft}
\DefineJournalWordException{Playgirl}{Playgirl}
\DefineJournalWordException{Playgolf}{Playgolf}
\DefineJournalAbbreviation{Playing}{Play}
\DefineJournalAbbreviation{Playleader}{Playlead}
\DefineJournalPartialAbbreviation{Playmarket}{Playmark}
\DefineJournalWordException{Playmate}{Playmate}
\DefineJournalAbbreviation{Playstation}{Playstn}
\DefineJournalWordException{Plaything}{Plaything}
\DefineJournalWordException{Playwright}{Playwright}
\DefineJournalAbbreviation{Pleading}{Plead}
\DefineJournalAbbreviation{Pleasant}{Pleas}
\DefineJournalAbbreviation{Pleasure}{Pleas}
\DefineJournalAbbreviation{Pleating}{Pleat}
\DefineJournalWordException{Plenary}{Plenary}
\DefineJournalWordException{Plenty}{Plenty}
\DefineJournalAbbreviation{Ploughman}{Ploughm}
\DefineJournalAbbreviation{Plougshare}{Plougsh}
\DefineJournalPartialAbbreviation{Plumb}{Plumb}
\DefineJournalWordException{Plunket}{Plunket}
\DefineJournalPartialAbbreviation{Pluridisciplin}{Pluridiscip}
\DefineJournalWordException{Plutonium}{Plutonium}
\DefineJournalWordException{Plymouth}{Plymouth}
\DefineJournalWordException{Plywood}{Plywood}
\DefineJournalAbbreviation{Pneumoconiosis}{Pneumocon}
\DefineJournalAbbreviation{Pneumotransport}{Pneumotransp}
\DefineJournalWordException{Pocket}{Pocket}
\DefineJournalAbbreviation{Pocket-book}{Pocket-b}
\DefineJournalWordException{Pocketax}{Pocketax}
\DefineJournalAbbreviation{Pocketbook}{Pocketb}
\DefineJournalWordException{Podiatry}{Podiatry}
\DefineJournalAbbreviation{Poietics}{Poiet}
\DefineJournalWordException{Point Pelee}{Point Pelee}
\DefineJournalAbbreviation{Point Pleasant}{Point Pleas}
\DefineJournalWordException{Pointing}{Pointing}
\DefineJournalAbbreviation{Poland}{Pol}
\DefineJournalPartialAbbreviation{Polarimetr}{Polarim}
\DefineJournalPartialAbbreviation{Polarizat}{Polariz}
\DefineJournalAbbreviation{Polemical}{Polem}
\DefineJournalWordException{Policeman}{Policeman}
\DefineJournalWordException{Policewoman}{Policewoman}
\DefineJournalAbbreviation{Policing}{Polic}
\DefineJournalWordException{Policy}{Policy}
\DefineJournalAbbreviation{Policyholder}{Policyhold}
\DefineJournalPartialAbbreviation{Poliomyelit}{Polio}
\DefineJournalAbbreviation{Polish}{Pol}
%\DefineJournalPartialWordException{Polite}{Polite-}
\DefineJournalAbbreviation{Polled}{Poll}
\DefineJournalWordException{Pollen}{Pollen}
\DefineJournalAbbreviation{Pollination}{Pollinat}
\DefineJournalAbbreviation{Polling}{Poll}
\DefineJournalPartialAbbreviation{Pollutant}{Pollut}
\DefineJournalAbbreviation{Pollution}{Pollut}
\DefineJournalPartialAbbreviation{Polyacryl}{Polyacryl}
\DefineJournalPartialAbbreviation{Polyatomic}{Polyat}
\DefineJournalAbbreviation{Polychaete}{Polych}
\DefineJournalPartialAbbreviation{Polyclini}{Polyclin}
\DefineJournalPartialAbbreviation{Polycrystalli}{Polycryst}
\DefineJournalPartialAbbreviation{Polycultur}{Polycult}
\DefineJournalAbbreviation{Polycyclic}{Polycycl}
\DefineJournalAbbreviation{Polyester}{Polyest}
\DefineJournalAbbreviation{Polyethylene}{Polyethyl}
\DefineJournalPartialAbbreviation{Polygraph}{Polygr}
\DefineJournalAbbreviation{Polyimide}{Polyim}
\DefineJournalPartialAbbreviation{Polymer}{Polym}
\DefineJournalPartialAbbreviation{Polymicrobial}{Polymicrob}
\DefineJournalAbbreviation{Polymorphism}{Polymorph}
\DefineJournalPartialAbbreviation{Polymorphonuclear}{Polymorphonucl}
\DefineJournalPartialAbbreviation{Polynesi}{Polyn}
\DefineJournalPartialAbbreviation{Polypeptid}{Polypept}
\DefineJournalAbbreviation{Polypropylene}{Polypropyl}
\DefineJournalAbbreviation{Polystyrene}{Polystyr}
\DefineJournalPartialAbbreviation{Polytechni}{Polytech}
\DefineJournalAbbreviation{Polythematical}{Polythemat}
\DefineJournalWordException{Polyurethane}{Polyurethane}
\DefineJournalPartialAbbreviation{Pomolog}{Pomol}
\DefineJournalWordException{Pomona}{Pomona}
\DefineJournalAbbreviation{Pondkeeper}{Pondkeep}
\DefineJournalAbbreviation{Pontypool}{Pontyp}
\DefineJournalAbbreviation{Pooled}{Pool}
\DefineJournalWordException{Poona}{Poona}
\DefineJournalWordException{Poorest}{Poorest}
\DefineJournalAbbreviation{Population}{Popul}
\DefineJournalWordException{Porcelain}{Porcelain}
\DefineJournalAbbreviation{Porcupine}{Porcup}
\DefineJournalWordException{Porirua}{Porirua}
\DefineJournalPartialAbbreviation{Porosimetr}{Porosim}
\DefineJournalWordException{Porous}{Porous}
\DefineJournalAbbreviation{Porphyrin}{Porphyr}
\DefineJournalWordException{Port Colborne}{Port Colborne}
\DefineJournalAbbreviation{Port Elizabeth}{Port Elizab}
\DefineJournalAbbreviation{Port Harcourt}{P H}
\DefineJournalAbbreviation{Port Hueneme}{Port Huen}
\DefineJournalAbbreviation{Port of Spain}{Port Spain}
\DefineJournalWordException{Portable}{Portable}
\DefineJournalWordException{Portadown}{Portadown}
\DefineJournalWordException{Porter}{Porter}
\DefineJournalWordException{Portland}{Portland}
\DefineJournalWordException{Portline}{Portline}
\DefineJournalAbbreviation{Porto Rico}{P R}
%\DefineJournalPartialWordException{Portrait}{Portrait-}
\DefineJournalAbbreviation{Portsmouth}{Portsm}
\DefineJournalWordException{Position}{Position}
\DefineJournalAbbreviation{Positioning}{Position}
\DefineJournalAbbreviation{Positive}{Posit}
\DefineJournalPartialAbbreviation{Possess}{Possess}
%\DefineJournalPartialWordException{Possib}{Possib-}
\DefineJournalAbbreviation{Postage}{Post}
\DefineJournalAbbreviation{Postal}{Post}
\DefineJournalAbbreviation{Postcard}{Postc}
\DefineJournalWordException{Postcensal}{Postcensal}
\DefineJournalWordException{Postcode}{Postcode}
\DefineJournalPartialAbbreviation{Postconferen}{Postconf}
\DefineJournalPartialAbbreviation{Postdoctor}{Postdr}
\DefineJournalWordException{Poster}{Poster}
\DefineJournalAbbreviation{Postgraduate}{Postgrad}
\DefineJournalWordException{Postharvest}{Postharvest}
\DefineJournalWordException{Postillion}{Postillion}
\DefineJournalAbbreviation{Posting}{Post}
\DefineJournalWordException{Postman}{Postman}
\DefineJournalWordException{Postmark}{Postmark}
\DefineJournalAbbreviation{Postmaster}{Postmast}
\DefineJournalAbbreviation{Postmodern}{Postmod}
\DefineJournalAbbreviation{Postmyocardial}{Postmyocard}
\DefineJournalPartialAbbreviation{Postoperativ}{Postoper}
\DefineJournalWordException{Postorder}{Postorder}
\DefineJournalAbbreviation{Postscript}{Ps}
\DefineJournalPartialAbbreviation{Postsecond}{Postsecond}
\DefineJournalWordException{Posture}{Posture}
\DefineJournalWordException{Potash}{Potash}
\DefineJournalAbbreviation{Potashville}{Potashv}
\DefineJournalWordException{Potato}{Potato}
\DefineJournalWordException{Potential}{Potential}
\DefineJournalAbbreviation{Potentially}{Potential}
\DefineJournalAbbreviation{Potomac}{Potom}
\DefineJournalWordException{Potter}{Potter}
\DefineJournalWordException{Pottery}{Pottery}
\DefineJournalAbbreviation{Poultry}{Poult}
\DefineJournalAbbreviation{Poultryman}{Poultrym}
\DefineJournalAbbreviation{Pounding}{Pound}
\DefineJournalWordException{Poverty}{Poverty}
\DefineJournalWordException{Powder}{Powder}
\DefineJournalWordException{Power}{Power}
\DefineJournalAbbreviation{Powerboat}{Powerb}
\DefineJournalAbbreviation{Powerboating}{Powerb}
\DefineJournalPartialAbbreviation{Powerlift}{Powerlift}
\DefineJournalAbbreviation{Powerplant}{Powerpl}
\DefineJournalPartialAbbreviation{Practi}{Pract}
\DefineJournalPartialAbbreviation{Praeparat}{Praep}
\DefineJournalPartialAbbreviation{Praesident}{Praes}
\DefineJournalAbbreviation{Pragmatics}{Pragmat}
\DefineJournalAbbreviation{Prairie Valleys}{Prairie Val}
\DefineJournalWordException{Praise}{Praise}
\DefineJournalPartialAbbreviation{Pranc}{Pranc}
\DefineJournalWordException{Prawn}{Prawn}
\DefineJournalPartialAbbreviation{Pray}{Pray}
\DefineJournalAbbreviation{Preaching}{Preach}
\DefineJournalPartialAbbreviation{Prebiolog}{Prebiol}
\DefineJournalPartialAbbreviation{Precast}{Precast}
\DefineJournalAbbreviation{Precaution}{Precaut}
\DefineJournalPartialAbbreviation{Preced}{Pr\'ec\'ed}
\DefineJournalAbbreviation{Preceptor}{Precept}
\DefineJournalWordException{Precious}{Precious}
\DefineJournalAbbreviation{Precipitation}{Precip}
\DefineJournalAbbreviation{Precision}{Precis}
\DefineJournalPartialAbbreviation{Preclinic}{Preclin}
\DefineJournalPartialAbbreviation{Preconcentrat}{Preconc}
\DefineJournalAbbreviation{Preconditioned}{Precond}
\DefineJournalAbbreviation{Predator}{Predat}
\DefineJournalPartialAbbreviation{Predecess}{Predecess}
\DefineJournalAbbreviation{Predental}{Predent}
\DefineJournalPartialAbbreviation{Predict}{Predict}
\DefineJournalAbbreviation{Predominately}{Predom}
\DefineJournalPartialAbbreviation{Prefectur}{Prefect}
\DefineJournalPartialAbbreviation{Pr\'ef\'er}{Prefer}
\DefineJournalAbbreviation{Pregeriatric}{Pregeriatr}
\DefineJournalWordException{Pregnancy}{Pregnancy}
\DefineJournalPartialAbbreviation{Prehistori}{Prehist}
\DefineJournalPartialAbbreviation{Preleukemi}{Preleuk}
\DefineJournalPartialAbbreviation{Prelimin}{Prelim}
\DefineJournalPartialAbbreviation{Premalign}{Premalig}
\DefineJournalAbbreviation{Prematurity}{Prematur}
\DefineJournalWordException{Premise}{Premise}
\DefineJournalPartialAbbreviation{Prenatal}{Prenat}
\DefineJournalPartialAbbreviation{Prepar}{Prep}
\DefineJournalPartialAbbreviation{Preprint}{Prepr}
\DefineJournalPartialAbbreviation{Prerefund}{Prerefund}
\DefineJournalAbbreviation{Presbyterian}{Presbyt}
\DefineJournalPartialAbbreviation{Preschool}{Presch}
\DefineJournalPartialAbbreviation{Prescrib}{Prescr}
\DefineJournalPartialAbbreviation{Prescription}{Prescr}
\DefineJournalWordException{Pr\'esence}{Pr\'esence}
\DefineJournalPartialAbbreviation{Present}{Present}
\DefineJournalPartialAbbreviation{Preserv}{Preserv}
\DefineJournalPartialAbbreviation{Presiden}{Pres}
\DefineJournalAbbreviation{Presiding}{Pres}
\DefineJournalWordException{Press}{Press}
\DefineJournalPartialAbbreviation{Press}{Press}
\DefineJournalWordException{Pressclip}{Pressclip}
\DefineJournalAbbreviation{Pressure}{Press}
\DefineJournalAbbreviation{Pressurize}{Press}
\DefineJournalPartialAbbreviation{Prestress}{Prestress}
\DefineJournalPartialAbbreviation{Presystem}{Presyst}
\DefineJournalPartialAbbreviation{Pretreatment}{Pretreat}
\DefineJournalAbbreviation{Pretrial}{Pretr}
\DefineJournalPartialAbbreviation{Prevail}{Prevail}
\DefineJournalAbbreviation{Prevalence}{Preval}
\DefineJournalPartialAbbreviation{Prevent}{Prev}
\DefineJournalWordException{Preview}{Preview}
\DefineJournalPartialAbbreviation{Previs}{Previs}
\DefineJournalWordException{Price}{Price}
\DefineJournalAbbreviation{Pricebook}{Priceb}
\DefineJournalWordException{Pricing}{Pricing}
\DefineJournalWordException{Priesthood}{Priesthood}
\DefineJournalAbbreviation{Priestley}{Priest}
\DefineJournalAbbreviation{Primary}{Prim}
\DefineJournalWordException{Primate}{Primate}
\DefineJournalWordException{Primer}{Primer}
\DefineJournalAbbreviation{Primitive}{Primit}
\DefineJournalWordException{Prince}{Prince}
\DefineJournalAbbreviation{Prince Edward Island}{P E I}
\DefineJournalWordException{Prince-George}{Prince-George}
\DefineJournalAbbreviation{Princes Risborough}{Princes Risb}
\DefineJournalAbbreviation{Princeton}{Princet}
\DefineJournalPartialAbbreviation{Principal}{Princ}
\DefineJournalPartialAbbreviation{Principle}{Princ}
\DefineJournalAbbreviation{Printed}{Print}
\DefineJournalAbbreviation{Printer}{Print}
\DefineJournalAbbreviation{Printing}{Print}
\DefineJournalPartialAbbreviation{Printmak}{Printmak}
\DefineJournalWordException{Printout}{Printout}
\DefineJournalAbbreviation{Priority}{Prior}
\DefineJournalWordException{Priory}{Priory}
\DefineJournalPartialAbbreviation{Prison}{Prison}
\DefineJournalAbbreviation{Privacy}{Priv}
\DefineJournalPartialAbbreviation{Prize}{Prize}
\DefineJournalWordException{Pro-views}{Pro-views}
\DefineJournalPartialAbbreviation{Probabilit}{Probab}
\DefineJournalAbbreviation{Probablistic}{Probab}
\DefineJournalWordException{Probate}{Probate}
\DefineJournalAbbreviation{Probation}{Probat}
\DefineJournalAbbreviation{Procedural}{Proced}
\DefineJournalPartialAbbreviation{Procedure}{Proced}
\DefineJournalAbbreviation{Proceedings}{Proc}
\DefineJournalPartialAbbreviation{Process}{Process}
\DefineJournalAbbreviation{Proclamation}{Proclam}
\DefineJournalPartialAbbreviation{Proctolog}{Proctol}
\DefineJournalAbbreviation{Procurement}{Procure}
\DefineJournalPartialAbbreviation{Produc}{Prod}
\DefineJournalAbbreviation{Productronic}{Productron}
\DefineJournalPartialAbbreviation{Profession}{Prof}
\DefineJournalAbbreviation{Proficiency}{Profic}
\DefineJournalPartialAbbreviation{Profilact}{Profil}
\DefineJournalWordException{Profile}{Profile}
\DefineJournalWordException{Profit}{Profit}
\DefineJournalAbbreviation{Profiting}{Profit}
\DefineJournalAbbreviation{Progenitor}{Progenit}
\DefineJournalAbbreviation{Programmable}{Program}
\DefineJournalWordException{Programme}{Programme}
\DefineJournalAbbreviation{Programmed}{Program}
\DefineJournalAbbreviation{Programmer}{Program}
\DefineJournalAbbreviation{Programming}{Program}
\DefineJournalAbbreviation{Progress}{Prog}
\DefineJournalPartialAbbreviation{Project}{Proj}
\DefineJournalAbbreviation{Proletarian}{Prolet}
\DefineJournalAbbreviation{Proliferation}{Prolif}
\DefineJournalPartialAbbreviation{Prolong}{Prolong}
\DefineJournalAbbreviation{Prominent}{Promin}
\DefineJournalAbbreviation{Promising}{Promis}
\DefineJournalWordException{Promissory}{Promissory}
\DefineJournalPartialAbbreviation{Promot}{Promot}
\DefineJournalPartialAbbreviation{Pronounc}{Pronounc}
\DefineJournalAbbreviation{Proofreader}{Proofread}
\DefineJournalPartialAbbreviation{Propagand}{Propag}
\DefineJournalAbbreviation{Propagation}{Propag}
\DefineJournalWordException{Propellant}{Propellant}
\DefineJournalWordException{Propeny}{Propeny}
\DefineJournalPartialAbbreviation{Propert}{Prop}
\DefineJournalWordException{Prophecy}{Prophecy}
\DefineJournalPartialAbbreviation{Prophet}{Prophet}
\DefineJournalPartialAbbreviation{Prophylact}{Prophyl}
\DefineJournalPartialAbbreviation{Propos}{Propos}
\DefineJournalPartialAbbreviation{Propriet}{Propr}
\DefineJournalAbbreviation{Propulsion}{Propuls}
\DefineJournalAbbreviation{Propylene}{Propyl}
\DefineJournalWordException{Prorodeo}{Prorodeo}
\DefineJournalPartialAbbreviation{Prosecut}{Prosec}
\DefineJournalWordException{Prosound}{Prosound}
\DefineJournalPartialAbbreviation{Prospect}{Prospect}
\DefineJournalWordException{Prospectus}{Prospectus}
\DefineJournalWordException{Prosper}{Prosper}
\DefineJournalPartialAbbreviation{Prosperit}{Prosper}
\DefineJournalWordException{Prostaglandin}{Prostaglandin}
\DefineJournalAbbreviation{Prosthesis}{Prosthes}
\DefineJournalAbbreviation{Prosthetic}{Prosthet}
\DefineJournalPartialAbbreviation{Prosthodont}{Prosthodont}
\DefineJournalWordException{Protea}{Protea}
\DefineJournalWordException{Protease}{Protease}
\DefineJournalPartialAbbreviation{Protect}{Prot}
\DefineJournalWordException{Protein}{Protein}
\DefineJournalAbbreviation{Proteomics}{Proteom}
\DefineJournalWordException{Protest}{Protest}
\DefineJournalAbbreviation{Prothesis}{Prothes}
\DefineJournalWordException{Protides}{Protides}
\DefineJournalWordException{Protirelin}{Protirelin}
\DefineJournalPartialAbbreviation{Protobiolog}{Protobiol}
\DefineJournalPartialAbbreviation{Protocol}{Protoc}
\DefineJournalAbbreviation{Prototyping}{Prototyp}
\DefineJournalAbbreviation{Protuning}{Protun}
\DefineJournalPartialAbbreviation{Provinc}{Prov}
\DefineJournalAbbreviation{Provision}{Provis}
\DefineJournalWordException{Provisional}{Provisional}
\DefineJournalAbbreviation{Provoking}{Provok}
\DefineJournalAbbreviation{Prudential}{Prudent}
\DefineJournalWordException{Prudhoe}{Prudhoe}
\DefineJournalAbbreviation{Pseudepigrapha}{Pseudepigr}
\DefineJournalWordException{Psionic}{Psionic}
\DefineJournalWordException{Psychedelic}{Psychedelic}
\DefineJournalWordException{Psychiatry}{Psychiatry}
\DefineJournalPartialAbbreviation{Psychic}{Psych}
\DefineJournalAbbreviation{Psychoactive}{Psychoact}
\DefineJournalPartialAbbreviation{Psychoanal}{Psychoanal}
\DefineJournalPartialAbbreviation{Psychochemi}{Psychochem}
\DefineJournalWordException{Psychodrama}{Psychodrama}
\DefineJournalPartialAbbreviation{Psychodynami}{Psychodyn}
\DefineJournalPartialAbbreviation{Psychoeduca}{Psychoeduc}
\DefineJournalAbbreviation{Psychoendocrine}{Psychoendocr}
\DefineJournalPartialAbbreviation{Psychoendocrinolog}{Psychoendocrinol}
\DefineJournalAbbreviation{Psychogeriatric}{Psychogeriatr}
\DefineJournalPartialAbbreviation{Psychohistor}{Psychohist}
\DefineJournalPartialAbbreviation{Psycholinguistic}{Psycholinguist}
\DefineJournalPartialAbbreviation{Psychoneuroendocrine}{Psychoneuroendocr}
\DefineJournalAbbreviation{Psychopathic}{Psychopath}
\DefineJournalPartialAbbreviation{Psychopatholog}{Psychopathol}
\DefineJournalPartialAbbreviation{Psychopharmacolog}{Psychopharmacol}
\DefineJournalPartialAbbreviation{Psychopharmaka}{Psychopharm}
\DefineJournalPartialAbbreviation{Psychophysic}{Psychophys}
\DefineJournalAbbreviation{Psychophysiology}{Psychophysiol}
\DefineJournalAbbreviation{Psychosis}{Psychos}
\DefineJournalPartialAbbreviation{Psychosocial}{Psychosoc}
\DefineJournalPartialAbbreviation{Psychosyndrom}{Psychosyndr}
\DefineJournalAbbreviation{Psychosynthesis}{Psychosynth}
\DefineJournalPartialAbbreviation{Pteridolog}{Pteridol}
\DefineJournalWordException{Public}{Public}
\DefineJournalPartialAbbreviation{Publicat}{Publ}
\DefineJournalAbbreviation{Publicity}{Public}
\DefineJournalWordException{Publicly}{Publicly}
\DefineJournalWordException{Publics}{Publics}
\DefineJournalPartialAbbreviation{Publish}{Publ}
\DefineJournalPartialAbbreviation{Puericultur}{Pueric}
\DefineJournalPartialAbbreviation{Pulmonar}{Pulm}
\DefineJournalAbbreviation{Pulmonology}{Pulmonol}
\DefineJournalWordException{Pulpit}{Pulpit}
\DefineJournalWordException{Pulpwood}{Pulpwood}
\DefineJournalWordException{Pulse}{Pulse}
\DefineJournalAbbreviation{Pumping}{Pump}
\DefineJournalWordException{Punch}{Punch}
\DefineJournalAbbreviation{Punctuality}{Punctual}
\DefineJournalWordException{Punisher}{Punisher}
\DefineJournalAbbreviation{Punishment}{Punishm}
%\DefineJournalPartialWordException{Punjab}{Punjab-}
\DefineJournalWordException{Punter}{Punter}
\DefineJournalWordException{Punting}{Punting}
\DefineJournalWordException{Pupil}{Pupil}
\DefineJournalAbbreviation{Puppeteer}{Puppet}
\DefineJournalPartialAbbreviation{Purchas}{Purch}
\DefineJournalWordException{Purdue}{Purdue}
\DefineJournalAbbreviation{Purification}{Purif}
\DefineJournalWordException{Puritan}{Puritan}
\DefineJournalWordException{Purity}{Purity}
\DefineJournalWordException{Purple}{Purple}
\DefineJournalPartialAbbreviation{Purpose}{Purp}
\DefineJournalAbbreviation{Pursuant}{Purs}
\DefineJournalPartialAbbreviation{Pursuit}{Purs}
\DefineJournalAbbreviation{Purview}{Purv}
\DefineJournalAbbreviation{Pushcart}{Pushc}
\DefineJournalAbbreviation{Pushing}{Push}
\DefineJournalAbbreviation{Putting}{Putt}
\DefineJournalWordException{Puzzle}{Puzzle}
\DefineJournalWordException{Puzzletime}{Puzzletime}
\DefineJournalWordException{Pyramid}{Pyramid}
\DefineJournalWordException{Pyrolysis}{Pyrolysis}
\DefineJournalPartialAbbreviation{Pyrotechni}{Pyrotech}
\DefineJournalAbbreviation{Quadrangle}{Quadrang}
\DefineJournalAbbreviation{Quadrant}{Quadr}
\DefineJournalAbbreviation{Quadrennial}{Quadrenn}
\DefineJournalAbbreviation{Quadriennial}{Quadrienn}
\DefineJournalWordException{Quaker}{Quaker}
\DefineJournalWordException{Quaking}{Quaking}
\DefineJournalAbbreviation{Qualifying}{Qualif}
\DefineJournalPartialAbbreviation{Qualit}{Qual}
\DefineJournalWordException{Quantas}{Quantas}
\DefineJournalWordException{Quantum}{Quantum}
\DefineJournalPartialAbbreviation{Quarantine}{Quar}
\DefineJournalPartialAbbreviation{Quarr}{Quarr}
\DefineJournalWordException{Quarry}{Quarry}
\DefineJournalAbbreviation{Quarrying}{Quarr}
\DefineJournalAbbreviation{Quarter}{Quart}
\DefineJournalAbbreviation{Quarterly}{Q}
\DefineJournalWordException{Quartermaster}{Quartermaster}
\DefineJournalWordException{Quartet}{Quartet}
\DefineJournalWordException{Quartz}{Quartz}
\DefineJournalAbbreviation{Quasi-market}{Quasi-mark}
\DefineJournalPartialAbbreviation{Quasiparticle}{Quasipart}
\DefineJournalPartialAbbreviation{Quaternar}{Quat}
\DefineJournalAbbreviation{Queen-Charlotte-Islands}{Queen-Charlotte-Isl}
\DefineJournalAbbreviation{Queensland}{Qld}
\DefineJournalWordException{Queensway}{Queensway}
\DefineJournalWordException{Query}{Query}
\DefineJournalPartialAbbreviation{Question}{Quest}
\DefineJournalWordException{Quick}{Quick}
\DefineJournalWordException{Quickface}{Quickface}
\DefineJournalWordException{Quiddity}{Quiddity}
\DefineJournalPartialAbbreviation{Quilt}{Quilt}
\DefineJournalAbbreviation{Quiltwork}{Quiltw}
\DefineJournalWordException{Quinolone}{Quinolone}
\DefineJournalAbbreviation{Quinquennial}{Quinquenn}
\DefineJournalWordException{Quintessence}{Quintessence}
\DefineJournalWordException{Quintessential}{Quintessential}
\DefineJournalAbbreviation{Quotation}{Quota}
\DefineJournalPartialAbbreviation{Rabbit}{Rabbit}
\DefineJournalWordException{Racecar}{Racecar}
\DefineJournalAbbreviation{Racehorse}{Raceh}
\DefineJournalWordException{Racial}{Racial}
\DefineJournalWordException{Racing}{Racing}
\DefineJournalWordException{Racism}{Racism}
\DefineJournalWordException{Racket}{Racket}
\DefineJournalAbbreviation{Racking}{Rack}
\DefineJournalAbbreviation{Racquetball}{Racquetb}
\DefineJournalWordException{Radar}{Radar}
\DefineJournalAbbreviation{Radcliffe}{Radcl}
\DefineJournalWordException{Raddle}{Raddle}
\DefineJournalWordException{Radiance}{Radiance}
\DefineJournalAbbreviation{Radiating}{Radiat}
\DefineJournalAbbreviation{Radiation}{Radiat}
\DefineJournalAbbreviation{Radiative}{Radiat}
\DefineJournalWordException{Radiator}{Radiator}
\DefineJournalAbbreviation{Radical}{Radic}
\DefineJournalPartialAbbreviation{Radioactiv}{Radioact}
\DefineJournalWordException{Radioassay}{Radioassay}
\DefineJournalAbbreviation{Radiocarbon}{Radiocarb}
\DefineJournalPartialAbbreviation{Radiochem}{Radiochem}
\DefineJournalAbbreviation{Radiodiagnostic}{Radiodiagn}
\DefineJournalPartialAbbreviation{Radioecolog}{Radioecol}
\DefineJournalPartialAbbreviation{Radioelectric}{Radioelectr}
\DefineJournalPartialAbbreviation{Radioelectroni}{Radioelectron}
\DefineJournalPartialAbbreviation{Radiofrequenc}{Radiofreq}
\DefineJournalPartialAbbreviation{Radioimmunotherap}{Radioimmunother}
\DefineJournalAbbreviation{Radiometer}{Radiom}
\DefineJournalAbbreviation{Radionavigation}{Radionavig}
\DefineJournalWordException{Radionic}{Radionic}
\DefineJournalAbbreviation{Radionuclide}{Radionucl}
\DefineJournalPartialAbbreviation{Radiopharmac}{Radiopharm}
\DefineJournalPartialAbbreviation{Radiopharmacolog}{Radiopharmacol}
\DefineJournalPartialAbbreviation{Radiophysic}{Radiophys}
\DefineJournalPartialAbbreviation{Radioprotect}{Radioprot}
\DefineJournalAbbreviation{Radioscientist}{Radiosci}
\DefineJournalPartialAbbreviation{Radioscop}{Radiosc}
\DefineJournalAbbreviation{Radiosensitizer}{Radiosensit}
\DefineJournalWordException{Radiosonde}{Radiosonde}
\DefineJournalAbbreviation{Radiosterilization}{Radiosteril}
\DefineJournalWordException{Radium}{Radium}
\DefineJournalAbbreviation{Radnorshire}{Radnors}
\DefineJournalWordException{Radwaste}{Radwaste}
\DefineJournalWordException{Raffle}{Raffle}
\DefineJournalAbbreviation{Rafting}{Raft}
\DefineJournalWordException{Ragtrader}{Ragtrader}
\DefineJournalAbbreviation{Raider}{Raid}
\DefineJournalAbbreviation{Railpass}{Railp}
\DefineJournalPartialAbbreviation{Railroad}{Railr}
\DefineJournalPartialAbbreviation{Railway}{Railw}
\DefineJournalWordException{Railwayman}{Railwayman}
\DefineJournalWordException{Rainbow}{Rainbow}
\DefineJournalWordException{Rainfall}{Rainfall}
\DefineJournalAbbreviation{Rainforest}{Rainfor}
\DefineJournalAbbreviation{Raised}{Rais}
\DefineJournalAbbreviation{Raiser}{Rais}
\DefineJournalAbbreviation{Raising}{Rais}
\DefineJournalWordException{Rajasthan}{Rajasthan}
\DefineJournalWordException{Rally}{Rally}
\DefineJournalAbbreviation{Rallying}{Rally}
\DefineJournalPartialAbbreviation{Rambl}{Rambl}
\DefineJournalWordException{Ramsgate}{Ramsgate}
\DefineJournalWordException{Rancher}{Rancher}
\DefineJournalWordException{Random}{Random}
\DefineJournalWordException{Randwick}{Randwick}
\DefineJournalAbbreviation{Rangeland}{Rangel}
\DefineJournalWordException{Rangeman}{Rangeman}
\DefineJournalWordException{Ranger}{Ranger}
\DefineJournalWordException{Rangoon}{Rangoon}
\DefineJournalPartialAbbreviation{Rank}{Rank}
\DefineJournalWordException{Rapeseed}{Rapeseed}
\DefineJournalWordException{Raptor}{Raptor}
\DefineJournalAbbreviation{Raquetball}{Raquetb}
\DefineJournalWordException{Rarefied}{Rarefied}
\DefineJournalWordException{Rascal}{Rascal}
\DefineJournalWordException{Rathgarogue}{Rathgarogue}
\DefineJournalWordException{Rathmichael}{Rathmichael}
\DefineJournalAbbreviation{Rating}{Rat}
\DefineJournalWordException{Ratio}{Ratio}
\DefineJournalPartialAbbreviation{Rational}{Ration}
\DefineJournalWordException{Rawhide}{Rawhide}
\DefineJournalPartialAbbreviation{Reach}{Reach}
\DefineJournalAbbreviation{Reacting}{React}
\DefineJournalPartialAbbreviation{Reaction}{React}
\DefineJournalPartialAbbreviation{Reactiv}{React}
\DefineJournalPartialAbbreviation{Reactor}{React}
\DefineJournalWordException{Readable}{Readable}
\DefineJournalAbbreviation{Reader}{Read}
\DefineJournalAbbreviation{Readership}{Readersh}
\DefineJournalAbbreviation{Reading}{Read}
\DefineJournalAbbreviation{Reagent}{Reag}
\DefineJournalWordException{Real (actual)}{Real (actual)}
\DefineJournalWordException{Realism}{Realism}
\DefineJournalWordException{Realistic}{Realistic}
\DefineJournalAbbreviation{Reality}{Real}
\DefineJournalWordException{Really}{Really}
\DefineJournalPartialAbbreviation{Realt}{Realt}
\DefineJournalWordException{Realtor}{Realtor}
\DefineJournalAbbreviation{Reanimation}{Reanim}
\DefineJournalAbbreviation{Reared}{Rear}
\DefineJournalPartialAbbreviation{Rearrange}{Rearrange}
\DefineJournalPartialAbbreviation{Reason}{Reason}
\DefineJournalPartialAbbreviation{Reassembl}{Reassembl}
\DefineJournalPartialAbbreviation{Reassessment}{Reassess}
\DefineJournalWordException{Recall}{Recall}
\DefineJournalPartialAbbreviation{Receipt}{Receipt}
\DefineJournalPartialAbbreviation{Receiv}{Receiv}
\DefineJournalPartialAbbreviation{Recension}{Recens}
\DefineJournalWordException{Recent}{Recent}
\DefineJournalAbbreviation{Recently}{Recent}
\DefineJournalPartialAbbreviation{Recept}{Recept}
\DefineJournalPartialAbbreviation{Recepterolog}{Recepterol}
\DefineJournalPartialAbbreviation{Recertificat}{Recertif}
\DefineJournalAbbreviation{Recession}{Recess}
\DefineJournalPartialAbbreviation{R\'ecidiv}{Recidiv}
\DefineJournalWordException{Recipe}{Recipe}
\DefineJournalPartialAbbreviation{R\'ecipien}{Recip}
\DefineJournalAbbreviation{Reciprocal}{Recipr}
\DefineJournalPartialAbbreviation{Recirculat}{Recirc}
\DefineJournalAbbreviation{Reckonner}{Reckon}
\DefineJournalAbbreviation{Reclamation}{Reclam}
\DefineJournalPartialAbbreviation{Reclassifi}{Reclassif}
\DefineJournalAbbreviation{Recognition}{Recognit}
\DefineJournalAbbreviation{Recognize}{Recogn}
\DefineJournalPartialAbbreviation{Recollect}{Recollect}
\DefineJournalPartialAbbreviation{Recombin}{Recomb}
\DefineJournalPartialAbbreviation{Recommend}{Recomm}
\DefineJournalAbbreviation{Reconciliation}{Reconcil}
\DefineJournalPartialAbbreviation{Reconnection}{Reconnect}
\DefineJournalPartialAbbreviation{Reconstitut}{Reconst}
\DefineJournalPartialAbbreviation{Reconstruct}{Reconstr}
\DefineJournalPartialAbbreviation{Record}{Rec}
\DefineJournalPartialAbbreviation{Recover}{Recover}
\DefineJournalWordException{Recovery}{Recovery}
\DefineJournalPartialAbbreviation{Recreation}{Recreat}
\DefineJournalPartialAbbreviation{Recruit}{Recruit}
\DefineJournalPartialAbbreviation{Recrystalliz}{Recryst}
\DefineJournalWordException{Rectal}{Rectal}
\DefineJournalWordException{Rectifier}{Rectifier}
\DefineJournalPartialAbbreviation{Recultivat}{Recultiv}
\DefineJournalAbbreviation{Recurrent}{Recurr}
\DefineJournalAbbreviation{Recurring}{Recurr}
\DefineJournalWordException{Recusant}{Recusant}
\DefineJournalPartialAbbreviation{Recycl}{Recycl}
\DefineJournalWordException{Red-Cross}{Red-Cross}
\DefineJournalAbbreviation{Redbook}{Redb}
\DefineJournalPartialAbbreviation{Redeem}{Redeem}
\DefineJournalAbbreviation{Redemption}{Redempt}
\DefineJournalAbbreviation{Redemptorist}{Redempt}
\DefineJournalAbbreviation{Redeployment}{Redeploy}
\DefineJournalPartialAbbreviation{Redevelop}{Redev}
\DefineJournalWordException{Redhead}{Redhead}
\DefineJournalWordException{Redhill}{Redhill}
\DefineJournalPartialAbbreviation{Redistribut}{Redistrib}
\DefineJournalAbbreviation{Reduced}{Reduc}
\DefineJournalAbbreviation{Reduction}{Reduct}
\DefineJournalWordException{Redundancy}{Redundancy}
\DefineJournalWordException{Redwater}{Redwater}
\DefineJournalAbbreviation{Redwood}{Redw}
\DefineJournalAbbreviation{Reefer}{Reef}
\DefineJournalPartialAbbreviation{Reevaluat}{Reeval}
\DefineJournalWordException{Referee}{Referee}
\DefineJournalAbbreviation{Referral}{Ref}
\DefineJournalAbbreviation{Refined}{Refin}
\DefineJournalAbbreviation{Refiner}{Refin}
\DefineJournalAbbreviation{Refinery}{Refin}
\DefineJournalAbbreviation{Refining}{Refin}
\DefineJournalAbbreviation{Reflection}{Reflect}
\DefineJournalAbbreviation{Reforestation}{Refor}
\DefineJournalAbbreviation{Reformation}{Reform}
\DefineJournalAbbreviation{Reformatory}{Reform}
\DefineJournalAbbreviation{Reformed}{Reform}
\DefineJournalAbbreviation{Reformer}{Reform}
\DefineJournalPartialAbbreviation{Reformulat}{Reformul}
\DefineJournalPartialAbbreviation{Refract}{Refract}
\DefineJournalAbbreviation{Refresher}{Refresh}
\DefineJournalAbbreviation{Refreshment}{Refresh}
\DefineJournalPartialAbbreviation{Refrig}{Refrig}
\DefineJournalPartialAbbreviation{Refug}{Refug}
\DefineJournalPartialAbbreviation{Refund}{Refund}
\DefineJournalAbbreviation{Refurbishment}{Refurb}
\DefineJournalWordException{Regal}{Regal}
\DefineJournalWordException{Regency}{Regency}
\DefineJournalPartialAbbreviation{Regener}{Regen}
\DefineJournalWordException{Regent}{Regent}
\DefineJournalWordException{Regina}{Regina}
\DefineJournalAbbreviation{Registrarship}{Registrarsh}
\DefineJournalAbbreviation{Regression}{Regres}
\DefineJournalPartialAbbreviation{Regular}{Regul}
\DefineJournalPartialAbbreviation{Regulat}{Regul}
\DefineJournalWordException{Reigate}{Reigate}
\DefineJournalAbbreviation{Reimbursement}{Reimburse}
\DefineJournalPartialAbbreviation{Reimpr}{Reimpr}
\DefineJournalPartialAbbreviation{Reinforc}{Reinf}
\DefineJournalAbbreviation{Reinsman}{Reinsm}
\DefineJournalPartialAbbreviation{Reinsur}{Reinsur}
\DefineJournalAbbreviation{Related}{Relat}
\DefineJournalAbbreviation{Relating}{Relat}
\DefineJournalAbbreviation{Relation}{Relat}
\DefineJournalAbbreviation{Relationship}{Relatsh}
\DefineJournalPartialAbbreviation{Relative}{Relat}
\DefineJournalPartialAbbreviation{Relativit}{Relativ}
\DefineJournalPartialAbbreviation{Relator}{Relat}
\DefineJournalAbbreviation{Relaxation}{Relax}
\DefineJournalWordException{Relay}{Relay}
\DefineJournalWordException{Release}{Release}
\DefineJournalAbbreviation{Releasing}{Releas}
\DefineJournalPartialAbbreviation{Reliab}{Reliab}
\DefineJournalWordException{Reliance}{Reliance}
\DefineJournalWordException{Relic}{Relic}
\DefineJournalWordException{Relief}{Relief}
\DefineJournalPartialAbbreviation{Relocat}{Relocat}
\DefineJournalPartialAbbreviation{Remain}{Remain}
%\DefineJournalPartialWordException{Remat}{Remat-}
\DefineJournalPartialAbbreviation{Remede}{Rem}
\DefineJournalWordException{Remedial}{Remedial}
\DefineJournalPartialAbbreviation{Remediat}{Remediat}
\DefineJournalAbbreviation{Remedy}{Rem}
\DefineJournalPartialAbbreviation{Rememb}{Rememb}
\DefineJournalAbbreviation{Reminder}{Remind}
\DefineJournalPartialAbbreviation{Reminerali}{Reminer}
\DefineJournalAbbreviation{Reminiscence}{Reminisc}
\DefineJournalPartialAbbreviation{Remit}{Remit}
\DefineJournalAbbreviation{Remnant}{Remn}
\DefineJournalPartialAbbreviation{Remodel}{Remodel}
\DefineJournalPartialAbbreviation{Remote}{Remote}
\DefineJournalAbbreviation{Removal}{Remov}
\DefineJournalAbbreviation{Remuneration}{Remun}
\DefineJournalAbbreviation{Renal}{Ren}
\DefineJournalAbbreviation{Renascence}{Renasc}
\DefineJournalPartialAbbreviation{Render}{Render}
\DefineJournalAbbreviation{Ren\'egotiation}{Ren\'egotiat}
\DefineJournalAbbreviation{Renewable}{Renew}
\DefineJournalAbbreviation{Renewal}{Renew}
\DefineJournalWordException{Renfrew}{Renfrew}
\DefineJournalPartialAbbreviation{Renormal}{Renorm}
\DefineJournalAbbreviation{Rental}{Rent}
\DefineJournalWordException{Repair}{Repair}
\DefineJournalAbbreviation{Repairer}{Repair}
\DefineJournalAbbreviation{Repairing}{Repair}
\DefineJournalAbbreviation{Reparation}{Repar}
\DefineJournalAbbreviation{Repatriation}{Repatr}
\DefineJournalAbbreviation{Repayment}{Repaym}
\DefineJournalAbbreviation{Repellent}{Repel}
\DefineJournalPartialAbbreviation{Repertori}{Repert}
\DefineJournalAbbreviation{Repetition}{Repetit}
\DefineJournalAbbreviation{Replacing}{Replac}
\DefineJournalWordException{Replay}{Replay}
\DefineJournalWordException{Replica}{Replica}
\DefineJournalAbbreviation{Report}{Rep}
\DefineJournalAbbreviation{Reported}{Rep}
\DefineJournalAbbreviation{Reporter}{Report}
\DefineJournalAbbreviation{Reporting}{Report}
\DefineJournalPartialAbbreviation{Repositor}{Repos}
\DefineJournalPartialAbbreviation{Represent}{Represent}
\DefineJournalAbbreviation{Repression}{Repress}
\DefineJournalPartialAbbreviation{Reprint}{Repr}
\DefineJournalAbbreviation{Reprocessing}{Reprocess}
\DefineJournalPartialAbbreviation{Reprograph}{Reprogr}
\DefineJournalWordException{Reptile}{Reptile}
\DefineJournalAbbreviation{Republic}{Repub}
\DefineJournalAbbreviation{Republication}{Republ}
\DefineJournalAbbreviation{Reputation}{Reput}
\DefineJournalAbbreviation{Request}{Req}
\DefineJournalPartialAbbreviation{Requirement}{Requir}
\DefineJournalWordException{Rescue}{Rescue}
\DefineJournalPartialAbbreviation{Research}{Res}
\DefineJournalPartialAbbreviation{Resell}{Resell}
\DefineJournalWordException{Reserve}{Reserve}
\DefineJournalWordException{Reservist}{Reservist}
\DefineJournalPartialAbbreviation{Reservist}{Reservist}
\DefineJournalAbbreviation{Reservoir}{Reserv}
\DefineJournalAbbreviation{Resettlement}{Resettl}
\DefineJournalAbbreviation{Residency}{Resid}
\DefineJournalPartialAbbreviation{Resident}{Resid}
\DefineJournalWordException{Residue}{Residue}
\DefineJournalAbbreviation{Resilience}{Resil}
\DefineJournalWordException{Resin}{Resin}
\DefineJournalPartialAbbreviation{Resist}{Resist}
\DefineJournalPartialAbbreviation{Resolution}{Resolut}
\DefineJournalPartialAbbreviation{Resolv}{Resolv}
\DefineJournalPartialAbbreviation{Reson}{Reson}
\DefineJournalAbbreviation{Resophonic}{Resophon}
\DefineJournalWordException{Resort}{Resort}
\DefineJournalPartialAbbreviation{Resource}{Resour}
\DefineJournalAbbreviation{Respecting}{Respect}
\DefineJournalPartialAbbreviation{Respirat}{Respir}
\DefineJournalAbbreviation{Respirology}{Respirol}
\DefineJournalWordException{Respite}{Respite}
\DefineJournalAbbreviation{Respondent}{Respond}
\DefineJournalWordException{Response}{Response}
\DefineJournalPartialAbbreviation{Responsibilit}{Responsib}
\DefineJournalWordException{Restatement}{Restatement}
\DefineJournalAbbreviation{Restitution}{Restit}
\DefineJournalAbbreviation{Reston}{Rest}
\DefineJournalAbbreviation{Restoration}{Restor}
\DefineJournalAbbreviation{Restorationist}{Restor}
\DefineJournalAbbreviation{Restorative}{Restor}
\DefineJournalAbbreviation{Restorer}{Restor}
\DefineJournalWordException{Restraint}{Restraint}
\DefineJournalPartialAbbreviation{Restricti}{Restrict}
\DefineJournalAbbreviation{Restructuring}{Restruct}
\DefineJournalWordException{Restyling}{Restyling}
\DefineJournalWordException{Result}{Result}
\DefineJournalPartialAbbreviation{Resultat}{Result}
\DefineJournalWordException{Resulting}{Resulting}
\DefineJournalWordException{Resume}{Resume}
\DefineJournalAbbreviation{Resurrection}{Resurrect}
\DefineJournalPartialAbbreviation{Resuscitat}{Resusc}
\DefineJournalPartialAbbreviation{Retail}{Retail}
\DefineJournalAbbreviation{Retained}{Retain}
\DefineJournalAbbreviation{Retention}{Retent}
\DefineJournalPartialAbbreviation{Rethink}{Rethink}
\DefineJournalPartialAbbreviation{Reticulat}{Reticul}
\DefineJournalAbbreviation{Reticuloendothelial}{Reticuloendothel}
\DefineJournalPartialAbbreviation{Retin}{Retin}
\DefineJournalWordException{Retire}{Retire}
\DefineJournalAbbreviation{Retirement}{Retire}
\DefineJournalPartialAbbreviation{Retort}{Retort}
\DefineJournalAbbreviation{Retraining}{Retrain}
\DefineJournalWordException{Retrear}{Retrear}
\DefineJournalAbbreviation{Retrieval}{Retr}
\DefineJournalAbbreviation{Retriever}{Retriev}
\DefineJournalPartialAbbreviation{Retrofitt}{Retrofit}
\DefineJournalPartialAbbreviation{Retrospect}{Retrosp}
\DefineJournalWordException{Return}{Return}
\DefineJournalAbbreviation{Returned}{Return}
\DefineJournalAbbreviation{Returner}{Return}
\DefineJournalAbbreviation{Returning}{Return}
\DefineJournalAbbreviation{Reunion}{Reun}
\DefineJournalPartialAbbreviation{Reutili}{Reutil}
\DefineJournalWordException{Revange}{Revange}
\DefineJournalPartialAbbreviation{Reveal}{Reveal}
\DefineJournalAbbreviation{Revealer}{Reveal}
\DefineJournalPartialAbbreviation{Revegeta}{Reveg}
\DefineJournalPartialAbbreviation{Revel}{Revel}
\DefineJournalWordException{Revenge}{Revenge}
\DefineJournalPartialAbbreviation{Revere}{Revere}
\DefineJournalWordException{Reverse}{Reverse}
\DefineJournalAbbreviation{Reversible}{Revers}
\DefineJournalPartialAbbreviation{Review}{Rev}
\DefineJournalAbbreviation{Revised}{Revis}
\DefineJournalPartialAbbreviation{Revision}{Revis}
\DefineJournalAbbreviation{Revisited}{Revisit}
\DefineJournalPartialAbbreviation{Revitaliz}{Revital}
\DefineJournalWordException{Revival}{Revival}
\DefineJournalAbbreviation{Revivalist}{Revival}
\DefineJournalAbbreviation{Revolting}{Revolt}
\DefineJournalAbbreviation{Revolucija}{Revoluc}
\DefineJournalAbbreviation{Revolution}{Revolut}
\DefineJournalAbbreviation{Revolutionary}{Revolut}
\DefineJournalAbbreviation{Revolving}{Revolv}
\DefineJournalPartialAbbreviation{Reward}{Reward}
\DefineJournalWordException{Rexdale}{Rexdale}
\DefineJournalAbbreviation{Reykjavik}{Reyk}
\DefineJournalPartialAbbreviation{Rheodynamic}{Rheodyn}
\DefineJournalPartialAbbreviation{Rhetoric}{Rhetor}
\DefineJournalWordException{Rhinoceros}{Rhinoceros}
\DefineJournalAbbreviation{Rhode Island}{R I}
\DefineJournalAbbreviation{Rhodesia}{Rhod}
\DefineJournalPartialAbbreviation{Rhodesia}{Rhod}
\DefineJournalPartialAbbreviation{Rhythm}{Rhythm}
\DefineJournalAbbreviation{Rhytmic}{Rhytm}
\DefineJournalAbbreviation{Ribbon}{Ribb}
\DefineJournalAbbreviation{Ribosomes}{Ribos}
\DefineJournalWordException{Ricardian}{Ricardian}
\DefineJournalWordException{Ricemill}{Ricemill}
\DefineJournalWordException{Richardson}{Richardson}
\DefineJournalWordException{Richmond}{Richmond}
\DefineJournalAbbreviation{Rickettsial}{Ricketts}
\DefineJournalWordException{Rickmansworth}{Rickmansworth}
\DefineJournalWordException{Rider}{Rider}
\DefineJournalWordException{Ridgeback}{Ridgeback}
\DefineJournalWordException{Ridgeway}{Ridgeway}
\DefineJournalWordException{Ridgewood}{Ridgewood}
\DefineJournalAbbreviation{Riding}{Rid}
\DefineJournalAbbreviation{Rifleman}{Riflem}
\DefineJournalWordException{Right}{Right}
\DefineJournalWordException{Rimouski}{Rimouski}
\DefineJournalWordException{Rimshot}{Rimshot}
\DefineJournalWordException{Ringette}{Ringette}
\DefineJournalWordException{Ringwood}{Ringwood}
\DefineJournalWordException{Riposte}{Riposte}
\DefineJournalWordException{Ripping}{Ripping}
\DefineJournalWordException{Ripples}{Ripples}
\DefineJournalWordException{Riquena}{Riquena}
\DefineJournalWordException{Rising}{Rising}
\DefineJournalPartialAbbreviation{Ritual}{Ritual}
\DefineJournalWordException{River}{River}
\DefineJournalWordException{Riverbend}{Riverbend}
\DefineJournalAbbreviation{Riverdale}{Riverd}
\DefineJournalWordException{Riverina}{Riverina}
\DefineJournalWordException{Riverside}{Riverside}
\DefineJournalPartialAbbreviation{Riversympos}{Riversymp}
\DefineJournalAbbreviation{Riverview}{Riverv}
\DefineJournalWordException{Riviera}{Riviera}
\DefineJournalAbbreviation{Roadbuilder}{Roadbuild}
\DefineJournalAbbreviation{Roading}{Road}
\DefineJournalAbbreviation{Roadmaking}{Roadmak}
\DefineJournalWordException{Roadmap}{Roadmap}
\DefineJournalWordException{Roadracing}{Roadracing}
\DefineJournalAbbreviation{Roadrunner}{Roadrun}
\DefineJournalWordException{Roadscene}{Roadscene}
\DefineJournalWordException{Roadside}{Roadside}
\DefineJournalAbbreviation{Roaming}{Roam}
\DefineJournalWordException{Roaring}{Roaring}
\DefineJournalWordException{Robson}{Robson}
\DefineJournalAbbreviation{Robustness}{Robust}
\DefineJournalWordException{Rochdale}{Rochdale}
\DefineJournalWordException{Rochester}{Rochester}
\DefineJournalAbbreviation{Rochesterian}{Rochester}
\DefineJournalWordException{Rockburst}{Rockburst}
\DefineJournalPartialAbbreviation{Rocket}{Rocket}
\DefineJournalWordException{Rockhampton}{Rockhampton}
\DefineJournalWordException{Rockhound}{Rockhound}
\DefineJournalAbbreviation{Rockies}{Rock}
\DefineJournalPartialAbbreviation{Rockolog}{Rockol}
\DefineJournalWordException{Rocksport}{Rocksport}
\DefineJournalAbbreviation{Rockville}{Rockv}
\DefineJournalWordException{Rockwood}{Rockwood}
\DefineJournalAbbreviation{Rodenticide}{Rodentic}
\DefineJournalPartialAbbreviation{Roentgenolog}{Roentgenol}
\DefineJournalAbbreviation{Rogationist}{Ragation}
\DefineJournalWordException{Rogue}{Rogue}
\DefineJournalWordException{Roidsnews}{Roidsnews}
\DefineJournalPartialAbbreviation{Roll}{Roll}
\DefineJournalWordException{Rollcall}{Rollcall}
\DefineJournalAbbreviation{Roller}{Roll}
%\DefineJournalPartialWordException{Romanic}{Romanic-}
\DefineJournalPartialAbbreviation{Romanti}{Romant}
\DefineJournalAbbreviation{Romford}{Romf}
\DefineJournalAbbreviation{Roofing}{Roof}
\DefineJournalWordException{Rootrainer}{Rootrainer}
\DefineJournalWordException{Roscommon}{Roscommon}
\DefineJournalWordException{Rosement}{Rosement}
\DefineJournalWordException{Rosewater}{Rosewater}
\DefineJournalWordException{Rosicrucian}{Rosicrucian}
\DefineJournalWordException{Roster}{Roster}
\DefineJournalWordException{Rothamsted}{Rothamsted}
\DefineJournalAbbreviation{Rothberg}{Rothb}
\DefineJournalAbbreviation{Rotorcraft}{Rotorcr}
\DefineJournalWordException{Rotorua}{Rotorua}
\DefineJournalAbbreviation{Roughness}{Rough}
\DefineJournalWordException{Roughride}{Roughride}
\DefineJournalPartialAbbreviation{Rouman}{Roum}
\DefineJournalWordException{Roundabout}{Roundabout}
\DefineJournalWordException{Roundtable}{Roundtable}
\DefineJournalWordException{Roundup}{Roundup}
\DefineJournalWordException{Routing}{Routing}
\DefineJournalWordException{Rubber}{Rubber}
\DefineJournalWordException{Rubella}{Rubella}
\DefineJournalAbbreviation{Rucksack}{Rucks}
\DefineJournalWordException{Rudder}{Rudder}
\DefineJournalWordException{Rudyard}{Rudyard}
\DefineJournalWordException{Rugby}{Rugby}
\DefineJournalWordException{Ruislip}{Ruislip}
\DefineJournalWordException{Ruling}{Ruling}
\DefineJournalPartialAbbreviation{Rumania}{Rum}
\DefineJournalAbbreviation{Rummaging}{Rummag}
\DefineJournalWordException{Runaway}{Runaway}
\DefineJournalPartialAbbreviation{Runn}{Run}
\DefineJournalWordException{Rushden}{Rushden}
\DefineJournalAbbreviation{Rushing}{Rush}
\DefineJournalWordException{Russell}{Russell}
\DefineJournalPartialAbbreviation{Russi}{Russ}
\DefineJournalAbbreviation{Rutland}{Rutl}
\DefineJournalWordException{Rwanda}{Rwanda}
\DefineJournalPartialAbbreviation{Rythm}{Rythm}
\DefineJournalPartialAbbreviation{Sabbath}{Sabbath}
\DefineJournalAbbreviation{Saccharification}{Saccharif}
\DefineJournalAbbreviation{Sackville}{Sackv}
\DefineJournalAbbreviation{Sacrament}{Sacram}
\DefineJournalWordException{Sacred}{Sacred}
\DefineJournalWordException{Saddle}{Saddle}
\DefineJournalWordException{Saddlery}{Saddlery}
\DefineJournalWordException{Sadness}{Sadness}
\DefineJournalWordException{Safeguard}{Safeguard}
\DefineJournalAbbreviation{Safely}{Saf}
\DefineJournalWordException{Safer}{Safer}
\DefineJournalAbbreviation{Safety}{Saf}
\DefineJournalWordException{Safflower}{Safflower}
\DefineJournalWordException{Sagamie}{Sagamie}
\DefineJournalAbbreviation{Saharan}{Sahar}
\DefineJournalWordException{Sailboard}{Sailboard}
\DefineJournalPartialAbbreviation{Sailboat}{Sailboat}
\DefineJournalAbbreviation{Sailing}{Sail}
\DefineJournalAbbreviation{Sailor}{Sail}
\DefineJournalWordException{Salaberry}{Salaberry}
\DefineJournalWordException{Salaberry-de-Valleyfield}{Salaberry-de-Valleyfield}
\DefineJournalWordException{Salary}{Salary}
\DefineJournalAbbreviation{Salesman}{Salesm}
\DefineJournalWordException{Salesmanship}{Salesmanship}
\DefineJournalWordException{Sali}{Sali}
\DefineJournalWordException{Saline}{Saline}
\DefineJournalPartialAbbreviation{Salinit}{Salin}
\DefineJournalAbbreviation{Salisbury}{Salisb}
\DefineJournalWordException{Salmon}{Salmon}
\DefineJournalAbbreviation{Salmonid}{Salmon}
\DefineJournalWordException{Salt-Lake-City}{Salt-Lake-City}
\DefineJournalWordException{Saltwater}{Saltwater}
\DefineJournalWordException{Salvage}{Salvage}
\DefineJournalWordException{Salvation}{Salvation}
\DefineJournalAbbreviation{Samaritan}{Samarit}
\DefineJournalWordException{Sambalpur}{Sambalpur}
\DefineJournalWordException{Samlevnad}{Samlevnad}
\DefineJournalWordException{Samoyed}{Samoyed}
\DefineJournalWordException{Sample}{Sample}
\DefineJournalAbbreviation{Sampler}{Sampl}
\DefineJournalAbbreviation{Sampling}{Sampl}
\DefineJournalWordException{San-Antonio}{San-Antonio}
\DefineJournalAbbreviation{San-Bernardino}{San-Bernard}
\DefineJournalAbbreviation{San-Diego}{S-Diego}
\DefineJournalPartialAbbreviation{Sanator}{Sanat}
\DefineJournalWordException{Sanci\'on}{Sanci\'on}
\DefineJournalWordException{Sanctuary}{Sanctuary}
\DefineJournalWordException{Sandbank}{Sandbank}
\DefineJournalWordException{Sandesh}{Sandesh}
\DefineJournalWordException{Sandpiper}{Sandpiper}
\DefineJournalAbbreviation{Sandwich}{Sandw}
\DefineJournalPartialAbbreviation{Sanguin}{Sang}
\DefineJournalPartialAbbreviation{Sanitari}{Sanit}
\DefineJournalAbbreviation{Sanitary}{Sanit}
\DefineJournalWordException{Sanskrit}{Sanskrit}
\DefineJournalAbbreviation{Santa Monica}{St Monica}
\DefineJournalAbbreviation{Santa-Barbara}{St-Barbara}
\DefineJournalWordException{Santal Parganas}{Santal Parganas}
\DefineJournalWordException{Sapphire}{Sapphire}
\DefineJournalWordException{Saratoga}{Saratoga}
\DefineJournalWordException{Saratoga-Springs}{Saratoga-Springs}
\DefineJournalWordException{Sarawak}{Sarawak}
\DefineJournalWordException{Sarcoma}{Sarcoma}
\DefineJournalWordException{Sarcopenia}{Sarcopenia}
\DefineJournalAbbreviation{Sardinia}{Sard}
\DefineJournalWordException{Sarnia}{Sarnia}
\DefineJournalAbbreviation{Saskatchewan}{Sask}
\DefineJournalAbbreviation{Saskatoon}{Saskat}
\DefineJournalWordException{Sassafras}{Sassafras}
\DefineJournalPartialAbbreviation{Satellite}{Satell}
\DefineJournalWordException{Sathya}{Sathya}
\DefineJournalPartialAbbreviation{Satir}{Satir}
\DefineJournalPartialAbbreviation{Saturat}{Satur}
\DefineJournalWordException{Saturday}{Saturday}
\DefineJournalWordException{Satyric}{Satyric}
\DefineJournalWordException{Saucer}{Saucer}
\DefineJournalAbbreviation{Saudi Arabia}{Saudi Arab}
\DefineJournalWordException{Saugeen}{Saugeen}
\DefineJournalWordException{Savage}{Savage}
\DefineJournalWordException{Savanna}{Savanna}
\DefineJournalWordException{Savannah}{Savannah}
\DefineJournalWordException{Savers}{Savers}
\DefineJournalAbbreviation{Saving}{Sav}
\DefineJournalWordException{Sawbridgeworth}{Sawbridgeworth}
\DefineJournalWordException{Sawmill}{Sawmill}
\DefineJournalWordException{Saxophone}{Saxophone}
\DefineJournalWordException{Scale}{Scale}
\DefineJournalWordException{Scallop}{Scallop}
\DefineJournalWordException{Scalpel}{Scalpel}
\DefineJournalPartialAbbreviation{Scandal}{Scandal}
\DefineJournalPartialAbbreviation{Scandinavi}{Scand}
\DefineJournalWordException{Scanner}{Scanner}
\DefineJournalWordException{Scanning}{Scanning}
\DefineJournalWordException{Scarboro}{Scarboro}
\DefineJournalAbbreviation{Scarborough}{Scarb}
\DefineJournalPartialAbbreviation{Scatter}{Scatt}
\DefineJournalPartialAbbreviation{Scaveng}{Scav}
\DefineJournalAbbreviation{Scenic}{Scen}
\DefineJournalAbbreviation{Sceptic}{Scept}
\DefineJournalPartialAbbreviation{Schausammlung}{Schausamml}
\DefineJournalPartialAbbreviation{Schedul}{Sched}
\DefineJournalWordException{Scheme}{Scheme}
\DefineJournalAbbreviation{Scholarly}{Sch}
\DefineJournalAbbreviation{Scholarship}{Scholarsh}
\DefineJournalPartialAbbreviation{Scholasti}{Scholast}
\DefineJournalPartialAbbreviation{School}{Sch}
\DefineJournalAbbreviation{Schooner}{Schoon}
\DefineJournalPartialAbbreviation{Scienc}{Sci}
\DefineJournalPartialAbbreviation{Scient}{Sci}
\DefineJournalAbbreviation{Scientology}{Scientol}
\DefineJournalAbbreviation{Scientometric}{Scientometr}
\DefineJournalPartialAbbreviation{Scintigraph}{Scintigr}
\DefineJournalWordException{Scleroderma}{Scleroderma}
\DefineJournalAbbreviation{Sclerosis}{Scler}
\DefineJournalAbbreviation{Scooter}{Scoot}
\DefineJournalAbbreviation{Scoreboard}{Scorebrd}
\DefineJournalAbbreviation{Scorebook}{Scoreb}
\DefineJournalAbbreviation{Scorecard}{Scorec}
\DefineJournalAbbreviation{Scotland}{Scotl}
\DefineJournalAbbreviation{Scotsman}{Scotsm}
\DefineJournalAbbreviation{Scottish}{Scott}
\DefineJournalWordException{Scottsdale}{Scottsdale}
\DefineJournalPartialAbbreviation{Scout}{Scout}
\DefineJournalWordException{Scranton}{Scranton}
\DefineJournalAbbreviation{Scrapbook}{Scrapb}
\DefineJournalAbbreviation{Scrapping}{Scrapp}
\DefineJournalWordException{Scratch}{Scratch}
\DefineJournalWordException{Scream}{Scream}
\DefineJournalWordException{Screen}{Screen}
\DefineJournalAbbreviation{Screening}{Screen}
\DefineJournalPartialAbbreviation{Screenprint}{Screenpr}
\DefineJournalAbbreviation{Scribbler}{Scribbl}
\DefineJournalAbbreviation{Scribe}{Scr}
\DefineJournalAbbreviation{Scriber}{Scr}
\DefineJournalAbbreviation{Script}{Scr}
\DefineJournalAbbreviation{Scripture}{Scr}
\DefineJournalWordException{Scroll}{Scroll}
\DefineJournalWordException{Scrutin}{Scrutin}
\DefineJournalAbbreviation{Scrutiny}{Scrut}
\DefineJournalPartialAbbreviation{Scuffl}{Scuff}
\DefineJournalPartialAbbreviation{Sculpt}{Sculpt}
\DefineJournalPartialAbbreviation{Scurril}{Scurr}
\DefineJournalWordException{Scurvy}{Scurvy}
\DefineJournalAbbreviation{Seabird}{Seab}
\DefineJournalAbbreviation{Seaboard}{Seabd}
\DefineJournalWordException{Seaborne}{Seaborne}
\DefineJournalWordException{Seabrook}{Seabrook}
\DefineJournalWordException{Seaduck}{Seaduck}
\DefineJournalPartialAbbreviation{Seafar}{Seafar}
\DefineJournalAbbreviation{Seafood}{Seaf}
\DefineJournalWordException{Sealant}{Sealant}
\DefineJournalAbbreviation{Sealer}{Seal}
\DefineJournalAbbreviation{Sealing}{Seal}
\DefineJournalAbbreviation{Seaman}{Seam}
\DefineJournalAbbreviation{Seamanship}{Seamansh}
\DefineJournalAbbreviation{Seaport}{Seapt}
\DefineJournalAbbreviation{Seapower}{Seapow}
\DefineJournalWordException{Search}{Search}
\DefineJournalAbbreviation{Searcher}{Search}
\DefineJournalAbbreviation{Searching}{Search}
\DefineJournalAbbreviation{Searchlight}{Searchl}
\DefineJournalWordException{Seashell}{Seashell}
\DefineJournalPartialAbbreviation{Season}{Seas}
\DefineJournalAbbreviation{Seating}{Seat}
\DefineJournalAbbreviation{Seatrade}{Seatr}
\DefineJournalWordException{Seattle}{Seattle}
\DefineJournalWordException{Seawater}{Seawater}
\DefineJournalAbbreviation{Seaway}{Seaw}
\DefineJournalWordException{Seaweed}{Seaweed}
\DefineJournalPartialAbbreviation{Second}{Second}
\DefineJournalWordException{Secondhand}{Secondhand}
\DefineJournalPartialAbbreviation{Secretar}{Secr}
\DefineJournalAbbreviation{Secretion}{Secret}
\DefineJournalAbbreviation{Secretory}{Secret}
\DefineJournalPartialAbbreviation{Secti}{Sect}
\DefineJournalPartialAbbreviation{Sector}{Sect}
\DefineJournalPartialAbbreviation{Secul}{Secul}
\DefineJournalWordException{Secunderabad}{Secunderabad}
\DefineJournalPartialAbbreviation{Secur}{Secur}
\DefineJournalAbbreviation{Sedation}{Sedat}
\DefineJournalAbbreviation{Sedimentary}{Sediment}
\DefineJournalAbbreviation{Sedimentation}{Sediment}
\DefineJournalAbbreviation{Seedling}{Seedl}
\DefineJournalWordException{Seedsman}{Seedsman}
\DefineJournalPartialAbbreviation{Seek}{Seek}
\DefineJournalPartialAbbreviation{S\'egr\'eg}{Segreg}
\DefineJournalAbbreviation{Seismograph}{Seismogr}
\DefineJournalPartialAbbreviation{Seismolog}{Seismol}
\DefineJournalWordException{Seizure}{Seizure}
\DefineJournalPartialAbbreviation{Select}{Sel}
\DefineJournalPartialAbbreviation{Selforganiz}{Selforgan}
\DefineJournalAbbreviation{Selling}{Sell}
\DefineJournalWordException{Sellpower}{Sellpower}
\DefineJournalAbbreviation{Semantics}{Semant}
\DefineJournalPartialAbbreviation{Semeiotic}{Semeiot}
\DefineJournalPartialAbbreviation{Semestr}{Semest}
\DefineJournalAbbreviation{Semi-custom}{Semi-cust}
\DefineJournalAbbreviation{Semiannual}{Semiannu}
\DefineJournalPartialAbbreviation{Semiconduct}{Semicond}
\DefineJournalPartialAbbreviation{Semimagneti}{Semimagn}
\DefineJournalAbbreviation{Semimetal}{Semimet}
\DefineJournalPartialAbbreviation{Semiochemical}{Semiochem}
\DefineJournalPartialAbbreviation{Semisynthe}{Semisynth}
\DefineJournalPartialAbbreviation{Semit}{Semit}
\DefineJournalWordException{Sempervivum}{Sempervivum}
\DefineJournalWordException{Senate}{Senate}
\DefineJournalAbbreviation{Senior}{Sr}
\DefineJournalAbbreviation{Seniority}{Sr}
\DefineJournalWordException{Sense}{Sense}
\DefineJournalAbbreviation{Sensing}{Sens}
\DefineJournalAbbreviation{Sensitivity}{Sensit}
\DefineJournalAbbreviation{Sensor}{Sens}
\DefineJournalAbbreviation{Sensory}{Sens}
\DefineJournalWordException{Sentence}{Sentence}
\DefineJournalWordException{Sentencing}{Sentencing}
\DefineJournalWordException{Sentry}{Sentry}
\DefineJournalAbbreviation{Separate}{Sep}
\DefineJournalPartialAbbreviation{Separation}{Sep}
\DefineJournalAbbreviation{Separator}{Sep}
\DefineJournalPartialAbbreviation{Sephardi}{Sephar}
\DefineJournalWordException{Sephradi}{Sephradi}
\DefineJournalWordException{Sepsis}{Sepsis}
\DefineJournalPartialAbbreviation{Septemb}{Sept}
\DefineJournalWordException{Septuagint}{Septuagint}
\DefineJournalPartialAbbreviation{Seraphi}{Seraph}
\DefineJournalPartialAbbreviation{Seria}{Ser}
\DefineJournalPartialAbbreviation{Sericicult}{Sericic}
\DefineJournalAbbreviation{Sericulture}{Seric}
\DefineJournalAbbreviation{Series}{Ser}
\DefineJournalWordException{Serious}{Serious}
\DefineJournalWordException{Sermon}{Sermon}
\DefineJournalPartialAbbreviation{Serodiagnos}{Serodiagn}
\DefineJournalPartialAbbreviation{Seronegati}{Seronegat}
\DefineJournalAbbreviation{Server}{Serv}
\DefineJournalPartialAbbreviation{Servic}{Serv}
\DefineJournalAbbreviation{Serving}{Serv}
\DefineJournalAbbreviation{Sesquicentennial}{Sesquicenten}
\DefineJournalPartialAbbreviation{Sessi}{Sess}
\DefineJournalWordException{Setback}{Setback}
\DefineJournalWordException{Setter}{Setter}
\DefineJournalWordException{Setting}{Setting}
\DefineJournalAbbreviation{Settlement}{Settl}
\DefineJournalAbbreviation{Settler}{Settl}
%\DefineJournalPartialWordException{Seven}{Seven-}
\DefineJournalWordException{Several}{Several}
\DefineJournalAbbreviation{Severance}{Sever}
\DefineJournalAbbreviation{Sewage}{Sew}
\DefineJournalWordException{Sewells}{Sewells}
\DefineJournalWordException{Sewer}{Sewer}
\DefineJournalWordException{Sewerage}{Sewerage}
\DefineJournalWordException{Sewing}{Sewing}
\DefineJournalPartialAbbreviation{Sexual}{Sex}
\DefineJournalWordException{Seymour}{Seymour}
\DefineJournalPartialAbbreviation{Shadow}{Shad}
\DefineJournalAbbreviation{Shaker}{Shak}
\DefineJournalPartialAbbreviation{Shakespear}{Shakespear}
\DefineJournalWordException{Shaman}{Shaman}
\DefineJournalWordException{Shannon}{Shannon}
\DefineJournalPartialAbbreviation{Shaper}{Shap}
\DefineJournalAbbreviation{Shaping}{Shap}
\DefineJournalWordException{Share}{Share}
\DefineJournalAbbreviation{Shared}{Shar}
\DefineJournalWordException{Shareguide}{Shareguide}
\DefineJournalPartialAbbreviation{Sharehold}{Sharehold}
\DefineJournalAbbreviation{Sharemarket}{Sharemark}
\DefineJournalAbbreviation{Shareownership}{Shareownersh}
\DefineJournalWordException{Shareware}{Shareware}
\DefineJournalAbbreviation{Sharing}{Shar}
\DefineJournalAbbreviation{Sharpshoot}{Sharpsh}
\DefineJournalWordException{Shaver}{Shaver}
\DefineJournalWordException{Shawinigan}{Shawinigan}
\DefineJournalPartialAbbreviation{Shear}{Shear}
\DefineJournalAbbreviation{Sheepfarming}{Sheepfarm}
\DefineJournalAbbreviation{Sheepman}{Sheepm}
\DefineJournalWordException{Sheet}{Sheet}
\DefineJournalAbbreviation{Sheetmetal}{Sheetmet}
\DefineJournalAbbreviation{Sheffield}{Sheff}
\DefineJournalWordException{Shefford}{Shefford}
\DefineJournalWordException{Shelburne}{Shelburne}
\DefineJournalWordException{Shellac}{Shellac}
\DefineJournalPartialAbbreviation{Shellfish}{Shellfish}
\DefineJournalPartialAbbreviation{Shellfisher}{Shellfish}
\DefineJournalAbbreviation{Shellharbour}{Shellharb}
\DefineJournalPartialAbbreviation{Shelter}{Shelter}
%\DefineJournalPartialWordException{Shepherd}{Shepherd-}
\DefineJournalWordException{Sherbrooke}{Sherbrooke}
\DefineJournalWordException{Sheriff}{Sheriff}
\DefineJournalWordException{Sherkin}{Sherkin}
\DefineJournalAbbreviation{Sherlockian}{Sherlock}
\DefineJournalWordException{Sherwood-Park}{Sherwood-Park}
\DefineJournalAbbreviation{Shetland}{Shetl}
\DefineJournalWordException{Shield}{Shield}
\DefineJournalPartialAbbreviation{Shield}{Shield}
\DefineJournalAbbreviation{Shiftwork}{Shiftw}
\DefineJournalWordException{Shillelagh}{Shillelagh}
\DefineJournalWordException{Shilling}{Shilling}
\DefineJournalWordException{Shingle}{Shingle}
\DefineJournalWordException{Shinty}{Shinty}
\DefineJournalWordException{Shipborne}{Shipborne}
\DefineJournalAbbreviation{Shipbroker}{Shipbrok}
\DefineJournalPartialAbbreviation{Shipbuilder}{Shipbuild}
\DefineJournalAbbreviation{Shipbuilding}{Shipbuild}
\DefineJournalAbbreviation{Shipment}{Shipm}
\DefineJournalAbbreviation{Shipowner}{Shipown}
\DefineJournalAbbreviation{Shipowning}{Shipown}
\DefineJournalPartialAbbreviation{Shipp}{Shipp}
\DefineJournalWordException{Shipperke}{Shipperke}
\DefineJournalAbbreviation{Shiprepair}{Shiprep}
%\DefineJournalPartialWordException{Shipwreck}{Shipwreck-}
\DefineJournalWordException{Shipwright}{Shipwright}
\DefineJournalWordException{Shipyard}{Shipyard}
\DefineJournalWordException{Shire}{Shire}
\DefineJournalWordException{Shirley}{Shirley}
\DefineJournalWordException{Shivaji}{Shivaji}
\DefineJournalPartialAbbreviation{Shock}{Shock}
\DefineJournalWordException{Shoeing}{Shoeing}
\DefineJournalAbbreviation{Shoemaking}{Shoemak}
\DefineJournalPartialAbbreviation{Shoot}{Shoot}
\DefineJournalAbbreviation{Shopfitter}{Shopfit}
\DefineJournalAbbreviation{Shopfitting}{Shopfit}
\DefineJournalAbbreviation{Shopkeeper}{Shopkeep}
\DefineJournalWordException{Shoppe}{Shoppe}
\DefineJournalAbbreviation{Shopper}{Shopp}
\DefineJournalAbbreviation{Shopping}{Shopp}
\DefineJournalWordException{Shorebird}{Shorebird}
\DefineJournalAbbreviation{Shoreline}{Shorel}
\DefineJournalWordException{Short-term}{Short-term}
\DefineJournalAbbreviation{Shortage}{Short}
\DefineJournalWordException{Shortcut}{Shortcut}
\DefineJournalAbbreviation{Shorthand}{Shorth}
\DefineJournalWordException{Shorthorn}{Shorthorn}
\DefineJournalAbbreviation{Shortland}{Shortl}
\DefineJournalWordException{Shortwave}{Shortwave}
\DefineJournalWordException{Shotgun}{Shotgun}
\DefineJournalWordException{Shoulder}{Shoulder}
\DefineJournalAbbreviation{Showcase}{Showc}
\DefineJournalAbbreviation{Shower}{Show}
\DefineJournalAbbreviation{Showing}{Show}
\DefineJournalPartialAbbreviation{Showjump}{Showjump}
\DefineJournalWordException{Showplace}{Showplace}
\DefineJournalWordException{Showring}{Showring}
\DefineJournalAbbreviation{Showroom}{Showr}
\DefineJournalWordException{Showtime}{Showtime}
\DefineJournalPartialAbbreviation{Shredd}{Shredd}
\DefineJournalAbbreviation{Shreveport}{Shrevep}
\DefineJournalWordException{Shrewsbury}{Shrewsbury}
\DefineJournalWordException{Shrievalty}{Shrievalty}
\DefineJournalWordException{Shrimp}{Shrimp}
\DefineJournalAbbreviation{Shropshire}{Shropsh}
\DefineJournalWordException{Shroud}{Shroud}
\DefineJournalAbbreviation{Shutter}{Shutt}
\DefineJournalWordException{Shuttle}{Shuttle}
\DefineJournalPartialAbbreviation{Siberia}{Sib}
\DefineJournalPartialAbbreviation{Sick}{Sick}
\DefineJournalWordException{Sidcup}{Sidcup}
\DefineJournalWordException{Sidewalk}{Sidewalk}
\DefineJournalAbbreviation{Sideware}{Sidew}
\DefineJournalPartialAbbreviation{Sift}{Sift}
\DefineJournalAbbreviation{Sighted}{Sight}
\DefineJournalAbbreviation{Sightseeing}{Sightsee}
\DefineJournalAbbreviation{Sigillography}{Sigillogr}
\DefineJournalWordException{Signal}{Signal}
\DefineJournalAbbreviation{Signaling}{Signal}
\DefineJournalAbbreviation{Signalling}{Signal}
\DefineJournalAbbreviation{Signalman}{Signalm}
\DefineJournalAbbreviation{Significant}{Signif}
\DefineJournalWordException{Signpost}{Signpost}
\DefineJournalPartialAbbreviation{Silicat}{Silic}
\DefineJournalWordException{Silicon}{Silicon}
\DefineJournalWordException{Silicone}{Silicone}
\DefineJournalWordException{Silicose}{Silicose}
\DefineJournalWordException{Silkworm}{Silkworm}
\DefineJournalAbbreviation{Siloxane}{Silox}
\DefineJournalWordException{Silver}{Silver}
\DefineJournalAbbreviation{Silversmithing}{Silversmith}
\DefineJournalAbbreviation{Silverware}{Silverw}
\DefineJournalPartialAbbreviation{Silvicult}{Silvic}
\DefineJournalWordException{Simba}{Simba}
\DefineJournalWordException{Simframjare}{Simframjare}
\DefineJournalWordException{Similkameen}{Similkameen}
\DefineJournalWordException{Simmental}{Simmental}
\DefineJournalPartialAbbreviation{Simplif}{Simpl}
\DefineJournalWordException{Simula}{Simula}
\DefineJournalAbbreviation{Simulation}{Simul}
\DefineJournalWordException{Simuliid}{Simuliid}
\DefineJournalPartialAbbreviation{Sindicat}{Sind}
\DefineJournalAbbreviation{Singapore}{Singap}
\DefineJournalAbbreviation{Singing}{Sing}
\DefineJournalWordException{Single}{Single}
\DefineJournalPartialAbbreviation{Sinister}{Sinister}
\DefineJournalPartialAbbreviation{Sink}{Sink}
\DefineJournalAbbreviation{Sintering}{Sinter}
\DefineJournalWordException{Sister}{Sister}
\DefineJournalAbbreviation{Situation}{Situat}
\DefineJournalPartialAbbreviation{Sixteen}{Sixt}
\DefineJournalPartialAbbreviation{Sizzl}{Sizz}
\DefineJournalPartialAbbreviation{Skateboard}{Skateboard}
\DefineJournalPartialAbbreviation{Skater}{Skat}
\DefineJournalAbbreviation{Skating}{Skat}
\DefineJournalAbbreviation{Skeletogenesis}{Skeletogenes}
\DefineJournalAbbreviation{Skeleton}{Skelet}
\DefineJournalWordException{Sketch}{Sketch}
\DefineJournalPartialAbbreviation{Ski}{Ski}
\DefineJournalWordException{Skilled}{Skilled}
\DefineJournalWordException{Skillplus}{Skillplus}
\DefineJournalPartialAbbreviation{Skindiv}{Skindiv}
\DefineJournalAbbreviation{Skinner}{Skin}
\DefineJournalPartialAbbreviation{Skipp}{Skipp}
\DefineJournalWordException{Skokholm}{Skokholm}
\DefineJournalWordException{Skomer}{Skomer}
\DefineJournalPartialAbbreviation{Skydiv}{Skydiv}
\DefineJournalAbbreviation{Skyguide}{Skyg}
\DefineJournalWordException{Skylab}{Skylab}
\DefineJournalWordException{Skylark}{Skylark}
\DefineJournalWordException{Skyline}{Skyline}
\DefineJournalWordException{Skytrain}{Skytrain}
\DefineJournalAbbreviation{Skyway}{Skyw}
\DefineJournalAbbreviation{Slaughter}{Slaught}
\DefineJournalAbbreviation{Slaughterhouse}{Slaughterh}
\DefineJournalAbbreviation{Slaughtering}{Slaught}
\DefineJournalWordException{Slavery}{Slavery}
\DefineJournalAbbreviation{Slavic}{Slav}
\DefineJournalAbbreviation{Slavistics}{Slav}
\DefineJournalWordException{Slayer}{Slayer}
\DefineJournalAbbreviation{Sleeping}{Sleep}
\DefineJournalWordException{Sliced}{Sliced}
\DefineJournalWordException{Slideset}{Slideset}
\DefineJournalAbbreviation{Slimbridge}{Slimbr}
\DefineJournalPartialAbbreviation{Slimm}{Slim}
\DefineJournalWordException{Sludge}{Sludge}
\DefineJournalWordException{Smallarm}{Smallarm}
\DefineJournalAbbreviation{Smallholder}{Smallhold}
\DefineJournalAbbreviation{Smallholding}{Smallhold}
\DefineJournalAbbreviation{Smelting}{Smelt}
\DefineJournalAbbreviation{Smithsonian}{Smithson}
\DefineJournalAbbreviation{Smithtown}{Smitht}
\DefineJournalAbbreviation{Smogformation}{Smogform}
\DefineJournalWordException{Smokeless}{Smokeless}
\DefineJournalAbbreviation{Smoking}{Smok}
\DefineJournalWordException{Smooth}{Smooth}
\DefineJournalWordException{Snapshot}{Snapshot}
\DefineJournalPartialAbbreviation{Sniff}{Sniff}
\DefineJournalWordException{Snippet}{Snippet}
\DefineJournalAbbreviation{Snooker}{Snook}
\DefineJournalWordException{Snorkel}{Snorkel}
\DefineJournalPartialAbbreviation{Snowboard}{Snowboard}
\DefineJournalAbbreviation{Snowdonia}{Snowd}
\DefineJournalPartialAbbreviation{Snowmobil}{Snowmob}
\DefineJournalWordException{Snowsh\oe ing}{Snowsh\oe ing}
\DefineJournalWordException{Snowy}{Snowy}
\DefineJournalAbbreviation{Soaring}{Soar}
\DefineJournalWordException{Soccer}{Soccer}
\DefineJournalAbbreviation{Social}{Soc}
\DefineJournalPartialAbbreviation{Socialis}{Social}
\DefineJournalPartialAbbreviation{Societ}{Soc}
\DefineJournalAbbreviation{Sociobiology}{Sociobiol}
\DefineJournalPartialAbbreviation{Sociocriti}{Sociocrit}
\DefineJournalPartialAbbreviation{Socioeconom}{Socioecon}
\DefineJournalPartialAbbreviation{Sociolog}{Sociol}
\DefineJournalPartialAbbreviation{Sociometr}{Sociom}
\DefineJournalWordException{Socket}{Socket}
\DefineJournalAbbreviation{Socratic}{Socrat}
\DefineJournalWordException{Softback}{Softback}
\DefineJournalPartialAbbreviation{Softball}{Softb}
\DefineJournalPartialAbbreviation{Softcover}{Softcover}
\DefineJournalWordException{Softkey}{Softkey}
\DefineJournalAbbreviation{Software}{Softw}
\DefineJournalAbbreviation{Soilless}{Soil}
\DefineJournalWordException{Sokoto}{Sokoto}
\DefineJournalAbbreviation{Solar}{Sol}
\DefineJournalPartialAbbreviation{Solder}{Solder}
\DefineJournalWordException{Soldier}{Soldier}
\DefineJournalPartialAbbreviation{Solicitor}{Solicit}
\DefineJournalWordException{Solid}{Solid}
\DefineJournalWordException{Solid-state}{Solid-state}
\DefineJournalPartialAbbreviation{Solidific}{Solidif}
\DefineJournalWordException{Solihull}{Solihull}
\DefineJournalPartialAbbreviation{Sollicit}{Sollicit}
\DefineJournalWordException{Solomon}{Solomon}
\DefineJournalAbbreviation{Solstice}{Solst}
\DefineJournalAbbreviation{Solution}{Solut}
\DefineJournalAbbreviation{Solvency}{Solv}
\DefineJournalWordException{Solvent}{Solvent}
\DefineJournalWordException{Solving}{Solving}
\DefineJournalWordException{Solway}{Solway}
\DefineJournalWordException{Somali}{Somali}
\DefineJournalPartialAbbreviation{Somati}{Somat}
\DefineJournalPartialAbbreviation{Somatosensor}{Somatosens}
\DefineJournalAbbreviation{Somatostatin}{Somatostat}
\DefineJournalWordException{Someone}{Someone}
\DefineJournalWordException{Somerset}{Somerset}
\DefineJournalAbbreviation{Somerville}{Somerv}
\DefineJournalWordException{Something}{Something}
\DefineJournalAbbreviation{Songbook}{Songb}
\DefineJournalWordException{Sonic}{Sonic}
\DefineJournalPartialAbbreviation{Sonogra}{Sonogr}
\DefineJournalWordException{Sooner}{Sooner}
\DefineJournalWordException{Sophomore}{Sophomore}
\DefineJournalWordException{Sorbent}{Sorbent}
\DefineJournalWordException{Sorcerer}{Sorcerer}
\DefineJournalWordException{Sorcery}{Sorcery}
\DefineJournalWordException{Sorghum}{Sorghum}
\DefineJournalWordException{Sorrow}{Sorrow}
\DefineJournalWordException{Souldust}{Souldust}
\DefineJournalPartialAbbreviation{Sounding}{Sound}
\DefineJournalWordException{Soundline}{Soundline}
\DefineJournalWordException{Soundtrack}{Soundtrack}
\DefineJournalAbbreviation{Sourcebook}{Sourceb}
\DefineJournalAbbreviation{Sourcing}{Sourc}
\DefineJournalWordException{South}{South}
\DefineJournalPartialAbbreviation{South Africa}{S Afr}
\DefineJournalAbbreviation{South America}{S Am}
\DefineJournalWordException{South Asia}{South Asia}
\DefineJournalAbbreviation{South Australia}{S Aust}
\DefineJournalAbbreviation{South Canterbury}{S Canterb}
\DefineJournalAbbreviation{South Carolina}{S C}
\DefineJournalAbbreviation{South Dakota}{S D}
\DefineJournalWordException{South Hobart}{South Hobart}
\DefineJournalAbbreviation{South Melbourne}{S Melb}
\DefineJournalAbbreviation{South Pacific}{S Pac}
\DefineJournalAbbreviation{South Perth}{S Perth}
\DefineJournalWordException{South-Bend}{South-Bend}
\DefineJournalWordException{Southall}{Southall}
\DefineJournalAbbreviation{Southampton}{Southampt}
\DefineJournalWordException{Southbank}{Southbank}
\DefineJournalWordException{Southeast}{Southeast}
\DefineJournalAbbreviation{Southeastern}{Southeast}
\DefineJournalWordException{Southend-on-Sea}{Southend-on-Sea}
\DefineJournalAbbreviation{Southern}{South}
\DefineJournalAbbreviation{Southfield}{Southf}
\DefineJournalAbbreviation{Southland}{Southl}
\DefineJournalWordException{Southpaw}{Southpaw}
\DefineJournalWordException{Southside}{Southside}
\DefineJournalWordException{Southwest}{Southwest}
\DefineJournalAbbreviation{Southwestern}{Southwest}
\DefineJournalWordException{Souvenir}{Souvenir}
\DefineJournalAbbreviation{Sovereign}{Sover}
\DefineJournalWordException{Soybean}{Soybean}
\DefineJournalWordException{Space}{Space}
\DefineJournalAbbreviation{Spacecraft}{Spacecr}
\DefineJournalAbbreviation{Spaceflight}{Spacefl}
\DefineJournalWordException{Spacelab}{Spacelab}
\DefineJournalWordException{Spaceman}{Spaceman}
\DefineJournalWordException{Spain}{Spain}
\DefineJournalAbbreviation{Spanish}{Span}
\DefineJournalWordException{Sparetime}{Sparetime}
\DefineJournalWordException{Sparrow}{Sparrow}
\DefineJournalWordException{Spartacist}{Spartacist}
\DefineJournalWordException{Spastic}{Spastic}
\DefineJournalPartialAbbreviation{Speak}{Speak}
\DefineJournalAbbreviation{Speciation}{Speciat}
\DefineJournalWordException{Species}{Species}
\DefineJournalAbbreviation{Specific}{Specif}
\DefineJournalPartialAbbreviation{Specification}{Specif}
\DefineJournalAbbreviation{Specificity}{Specif}
\DefineJournalPartialAbbreviation{Specifier}{Specif}
\DefineJournalAbbreviation{Specifying}{Specif}
\DefineJournalAbbreviation{Specimen}{Specim}
\DefineJournalAbbreviation{Spectacular}{Spect}
\DefineJournalAbbreviation{Spectral}{Spectr}
\DefineJournalPartialAbbreviation{Spectrochem}{Spectrochem}
\DefineJournalPartialAbbreviation{Spectrofluorimetr}{Spectrofluorim}
\DefineJournalPartialAbbreviation{Spectrograph}{Spectrogr}
\DefineJournalPartialAbbreviation{Spectrometr}{Spectrom}
\DefineJournalPartialAbbreviation{Spectronom}{Spectron}
\DefineJournalPartialAbbreviation{Spectropolarimetr}{Spectropolarim}
\DefineJournalPartialAbbreviation{Spectroscop}{Spectrosc}
\DefineJournalAbbreviation{Spectrum}{Spectr}
\DefineJournalAbbreviation{Speculative}{Specul}
\DefineJournalAbbreviation{Speculator}{Specul}
\DefineJournalWordException{Speech}{Speech}
\DefineJournalWordException{Speedline}{Speedline}
\DefineJournalWordException{Speedpost}{Speedpost}
\DefineJournalAbbreviation{Speedway}{Speedw}
\DefineJournalWordException{Speedy}{Speedy}
\DefineJournalPartialAbbreviation{Spelaeolog}{Spelaeol}
\DefineJournalWordException{Spelean}{Spelean}
\DefineJournalAbbreviation{Spelling}{Spell}
\DefineJournalPartialAbbreviation{Spend}{Spend}
\DefineJournalPartialAbbreviation{Spheniscid}{Sphenis}
\DefineJournalWordException{Sphere}{Sphere}
\DefineJournalWordException{Sphingolipodose}{Sphingolipodose}
\DefineJournalWordException{Spider}{Spider}
\DefineJournalWordException{Spinal}{Spinal}
\DefineJournalPartialAbbreviation{Spindl}{Spindl}
\DefineJournalWordException{Spine}{Spine}
\DefineJournalPartialAbbreviation{Spinn}{Spinn}
\DefineJournalPartialAbbreviation{Spintroni}{Spintron}
\DefineJournalWordException{Spiral}{Spiral}
\DefineJournalWordException{Spirit}{Spirit}
\DefineJournalAbbreviation{Spirituality}{Spiritual}
\DefineJournalWordException{Splash}{Splash}
\DefineJournalAbbreviation{Spoken}{Spok}
\DefineJournalAbbreviation{Spokesman}{Spokesm}
\DefineJournalAbbreviation{Spokesperson}{Spokesp}
\DefineJournalWordException{Spongiform}{Spongiform}
\DefineJournalPartialAbbreviation{Sponsor}{Spons}
\DefineJournalAbbreviation{Sponsorship}{Spons}
\DefineJournalPartialAbbreviation{Sportfish}{Sportfish}
\DefineJournalWordException{Sportlight}{Sportlight}
\DefineJournalAbbreviation{Sportmagazine}{Sportmag}
\DefineJournalWordException{Sportsfan}{Sportsfan}
\DefineJournalWordException{Sportshop}{Sportshop}
\DefineJournalAbbreviation{Sportsland}{Sportsl}
\DefineJournalWordException{Sportslife}{Sportslife}
\DefineJournalWordException{Sportsman}{Sportsman}
\DefineJournalAbbreviation{Sportsmedicine}{Sportsmed}
\DefineJournalWordException{Sportspage}{Sportspage}
\DefineJournalAbbreviation{Sportswear}{Sportsw}
\DefineJournalWordException{Sportsweek}{Sportsweek}
\DefineJournalAbbreviation{Sportswoman}{Sportswom}
\DefineJournalWordException{Spotlight}{Spotlight}
\DefineJournalWordException{Spotter}{Spotter}
\DefineJournalWordException{Spousal}{Spousal}
\DefineJournalWordException{Spouse}{Spouse}
\DefineJournalAbbreviation{Spraying}{Spray}
\DefineJournalWordException{Spread}{Spread}
\DefineJournalWordException{Spring}{Spring}
\DefineJournalWordException{Springboard}{Springboard}
\DefineJournalWordException{Springbok}{Springbok}
\DefineJournalAbbreviation{Springfield}{Springf}
\DefineJournalPartialAbbreviation{Sprinkl}{Sprink}
\DefineJournalWordException{Sprintcar}{Sprintcar}
\DefineJournalWordException{Sprout}{Sprout}
\DefineJournalWordException{Squash}{Squash}
\DefineJournalAbbreviation{Squashplayer}{Squashplay}
\DefineJournalWordException{Squire}{Squire}
\DefineJournalWordException{Squirrel}{Squirrel}
\DefineJournalAbbreviation{Stability}{Stab}
\DefineJournalPartialAbbreviation{Stabiliz}{Stab}
\DefineJournalAbbreviation{Stadium}{Stad}
\DefineJournalPartialAbbreviation{Staff}{Staff}
\DefineJournalAbbreviation{Staffordshire}{Staffs}
\DefineJournalWordException{Stage}{Stage}
\DefineJournalWordException{Stagecoach}{Stagecoach}
\DefineJournalWordException{Staging}{Staging}
\DefineJournalPartialAbbreviation{Stain}{Stain}
\DefineJournalAbbreviation{Stainless}{Stainl}
\DefineJournalAbbreviation{Stakeholder}{Stakehold}
\DefineJournalPartialAbbreviation{Stalk}{Stalk}
\DefineJournalWordException{Stallion}{Stallion}
\DefineJournalWordException{Stamford}{Stamford}
\DefineJournalWordException{Stamina}{Stamina}
\DefineJournalWordException{Stamp}{Stamp}
\DefineJournalWordException{Stampede}{Stampede}
\DefineJournalAbbreviation{Stamping}{Stamp}
\DefineJournalPartialAbbreviation{Standard}{Stand}
\DefineJournalWordException{Standing}{Standing}
\DefineJournalAbbreviation{Stanford}{Stanf}
\DefineJournalWordException{Stanstead}{Stanstead}
\DefineJournalWordException{Staple}{Staple}
\DefineJournalAbbreviation{Starbright}{Starbr}
\DefineJournalWordException{Starburst}{Starburst}
\DefineJournalWordException{Starchroom}{Starchroom}
\DefineJournalWordException{Stardust}{Stardust}
\DefineJournalAbbreviation{Staring}{Star}
\DefineJournalWordException{Start}{Start}
\DefineJournalAbbreviation{Starter}{Start}
\DefineJournalAbbreviation{Starting}{Start}
\DefineJournalWordException{Startup}{Startup}
\DefineJournalAbbreviation{Starving}{Starv}
\DefineJournalWordException{State}{State}
\DefineJournalWordException{Stately}{Stately}
\DefineJournalWordException{Statement}{Statement}
\DefineJournalAbbreviation{Staten Island}{Staten Isl}
\DefineJournalWordException{Stateside}{Stateside}
\DefineJournalWordException{Statesman}{Statesman}
\DefineJournalAbbreviation{Statewide}{Statew}
\DefineJournalWordException{Static}{Static}
\DefineJournalAbbreviation{Station}{Stn}
\DefineJournalPartialAbbreviation{Station}{Station}
\DefineJournalWordException{Status}{Status}
\DefineJournalPartialAbbreviation{Stay}{Stay}
\DefineJournalAbbreviation{Steamboat}{Steamb}
\DefineJournalAbbreviation{Steamer}{Steam}
\DefineJournalAbbreviation{Steamship}{Steamsh}
\DefineJournalWordException{Steel}{Steel}
\DefineJournalWordException{Steelhead}{Steelhead}
\DefineJournalPartialAbbreviation{Steelmak}{Steelmak}
\DefineJournalAbbreviation{Steelworker}{Steelwork}
\DefineJournalAbbreviation{Steering}{Steer}
\DefineJournalWordException{Stellar}{Stellar}
\DefineJournalWordException{St\'er\'eo}{St\'er\'eo}
\DefineJournalPartialAbbreviation{Stereochem}{Stereochem}
\DefineJournalPartialAbbreviation{Stereodynami}{Stereodyn}
\DefineJournalAbbreviation{Stereoencephalotomy}{Stereoenceph}
\DefineJournalAbbreviation{Stereograph}{Stereogr}
\DefineJournalPartialAbbreviation{Stereoscopi}{Stereosc}
\DefineJournalAbbreviation{Stereotactic}{Stereotact}
\DefineJournalWordException{Stereotyping}{Stereotyping}
\DefineJournalWordException{Sterile}{Sterile}
\DefineJournalAbbreviation{Sterility}{Steril}
\DefineJournalAbbreviation{Sterilization}{Steriliz}
\DefineJournalAbbreviation{Sterling}{Sterl}
\DefineJournalWordException{Steroid}{Steroid}
\DefineJournalPartialAbbreviation{Steroidhormon}{Steroidhorm}
\DefineJournalAbbreviation{Stethoscope}{Stethosc}
\DefineJournalPartialAbbreviation{Stevedor}{Stevedor}
\DefineJournalWordException{Stevens Point}{Stevens Point}
\DefineJournalPartialAbbreviation{Steward}{Steward}
\DefineJournalPartialAbbreviation{Stickstoff}{Stickst}
\DefineJournalAbbreviation{Stiletto}{Stilet}
\DefineJournalAbbreviation{Stillbirth}{Stillb}
\DefineJournalWordException{Stillwater}{Stillwater}
\DefineJournalPartialAbbreviation{Stimulant}{Stimul}
\DefineJournalPartialAbbreviation{Stimulat}{Stimul}
\DefineJournalWordException{Stirling}{Stirling}
\DefineJournalWordException{Stitch}{Stitch}
\DefineJournalPartialAbbreviation{Stitch}{Stitch}
\DefineJournalAbbreviation{Stittsville}{Stittsv}
\DefineJournalAbbreviation{Stochastic}{Stoch}
\DefineJournalPartialAbbreviation{Stock}{Stock}
\DefineJournalAbbreviation{Stockbroker}{Stockbrok}
\DefineJournalWordException{Stockfeed}{Stockfeed}
\DefineJournalPartialAbbreviation{Stockhold}{Stockhold}
\DefineJournalAbbreviation{Stocklist}{Stockl}
\DefineJournalAbbreviation{Stockman}{Stockm}
\DefineJournalAbbreviation{Stockmarket}{Stockmark}
\DefineJournalWordException{Stockport}{Stockport}
\DefineJournalAbbreviation{Stockton}{Stockt}
\DefineJournalPartialAbbreviation{Stoichiometr}{Stoichiom}
\DefineJournalAbbreviation{Stokholding}{Stokhold}
\DefineJournalWordException{Stolen}{Stolen}
\DefineJournalWordException{Stomal}{Stomal}
\DefineJournalWordException{Stone}{Stone}
\DefineJournalWordException{Stoneham}{Stoneham}
\DefineJournalWordException{Stoneville}{Stoneville}
\DefineJournalAbbreviation{Stoneware}{Stonew}
\DefineJournalWordException{Stoney Creek}{Stoney Creek}
\DefineJournalAbbreviation{Stoppage}{Stopp}
\DefineJournalWordException{Storage}{Storage}
\DefineJournalWordException{Stored}{Stored}
\DefineJournalWordException{Storefront}{Storefront}
\DefineJournalWordException{Storing}{Storing}
\DefineJournalWordException{Stormy}{Stormy}
\DefineJournalWordException{Story}{Story}
\DefineJournalAbbreviation{Storybook}{Storyb}
\DefineJournalPartialAbbreviation{Storytell}{Storytell}
\DefineJournalAbbreviation{Stouffville}{Stouffv}
\DefineJournalAbbreviation{Stourbridge}{Stourbr}
\DefineJournalWordException{Stove}{Stove}
\DefineJournalWordException{Stowage}{Stowage}
\DefineJournalWordException{Strabismus}{Strabismus}
\DefineJournalWordException{Straight}{Straight}
\DefineJournalWordException{Str\u ain}{Str\u ain}
\DefineJournalWordException{Straits}{Straits}
\DefineJournalWordException{Strange}{Strange}
\DefineJournalWordException{Strategy}{Strategy}
\DefineJournalAbbreviation{Stratford}{Stratf}
\DefineJournalWordException{Strathclyde}{Strathclyde}
\DefineJournalWordException{Strathcona}{Strathcona}
\DefineJournalPartialAbbreviation{Stratif}{Stratif}
\DefineJournalPartialAbbreviation{Stratigraph}{Stratigr}
\DefineJournalPartialAbbreviation{Stratospher}{Stratos}
\DefineJournalAbbreviation{Strawberry}{Strawb}
\DefineJournalWordException{Stream}{Stream}
\DefineJournalWordException{Streamflow}{Streamflow}
\DefineJournalWordException{Streaming}{Streaming}
\DefineJournalWordException{Streamline}{Streamline}
\DefineJournalWordException{Streamlining}{Streamlining}
\DefineJournalAbbreviation{Street}{Str}
\DefineJournalAbbreviation{Streetsville}{Streetsv}
\DefineJournalWordException{Streetwize}{Streetwize}
\DefineJournalWordException{Strength}{Strength}
\DefineJournalAbbreviation{Strengthening}{Strength}
\DefineJournalWordException{Stress}{Stress}
\DefineJournalPartialAbbreviation{Strict}{Strict}
\DefineJournalWordException{Strike}{Strike}
\DefineJournalWordException{String}{String}
\DefineJournalWordException{Stringybark}{Stringybark}
\DefineJournalWordException{Strip}{Strip}
\DefineJournalWordException{Stroke}{Stroke}
\DefineJournalPartialAbbreviation{Stroll}{Stroll}
\DefineJournalWordException{Strong}{Strong}
\DefineJournalPartialAbbreviation{Structroni}{Structron}
\DefineJournalPartialAbbreviation{Structur}{Struct}
\DefineJournalPartialAbbreviation{Struggl}{Struggl}
\DefineJournalWordException{Stubble}{Stubble}
\DefineJournalAbbreviation{Studbook}{Studb}
\DefineJournalAbbreviation{Studentship}{Studentsh}
\DefineJournalAbbreviation{Studies}{Stud}
\DefineJournalWordException{Study}{Study}
\DefineJournalAbbreviation{Studying}{Stud}
\DefineJournalWordException{Stuff}{Stuff}
\DefineJournalWordException{Sturgeon}{Sturgeon}
\DefineJournalAbbreviation{Styling}{Styl}
\DefineJournalPartialAbbreviation{Stylist}{Stylist}
\DefineJournalWordException{Stylus}{Stylus}
\DefineJournalWordException{Sub-saharan}{Sub-saharan}
\DefineJournalAbbreviation{Subaltern}{Subalt}
\DefineJournalPartialAbbreviation{Subaquati}{Subaquat}
\DefineJournalAbbreviation{Subarctic}{Subarct}
\DefineJournalAbbreviation{Subatomic}{Subat}
\DefineJournalAbbreviation{Subcellular}{Subcell}
\DefineJournalPartialAbbreviation{Subclinic}{Subclin}
\DefineJournalAbbreviation{Subcommission}{Subcomm}
\DefineJournalPartialAbbreviation{Subcommittee}{Subcomm}
\DefineJournalAbbreviation{Subcontinent}{Subcont}
\DefineJournalPartialAbbreviation{Subcontract}{Subcontract}
\DefineJournalPartialAbbreviation{Subdivis}{Subdiv}
\DefineJournalAbbreviation{Subgroup}{Subgr}
\DefineJournalWordException{Subiaco}{Subiaco}
\DefineJournalPartialAbbreviation{Subject}{Subj}
\DefineJournalWordException{Subline}{Subline}
\DefineJournalPartialAbbreviation{Submarin}{Submar}
\DefineJournalAbbreviation{Submersible}{Submers}
\DefineJournalPartialAbbreviation{Submicroscop}{Submicrosc}
\DefineJournalAbbreviation{Submission}{Submiss}
\DefineJournalPartialAbbreviation{Submitt}{Submitt}
\DefineJournalAbbreviation{Subnuclear}{Subnucl}
\DefineJournalAbbreviation{Subordinate}{Subord}
\DefineJournalAbbreviation{Subpopulation}{Subpopul}
\DefineJournalPartialAbbreviation{Subprovinc}{Subprov}
\DefineJournalPartialAbbreviation{Subscrib}{Subscr}
\DefineJournalAbbreviation{Subscription}{Subscr}
\DefineJournalWordException{Subsea}{Subsea}
\DefineJournalPartialAbbreviation{Subsecretar}{Subsecr}
\DefineJournalAbbreviation{Subsection}{Subsect}
\DefineJournalPartialAbbreviation{Subsequen}{Subseq}
\DefineJournalAbbreviation{Subseries}{Subser}
\DefineJournalPartialAbbreviation{Subsist}{Subsist}
\DefineJournalPartialAbbreviation{Substanc}{Subst}
\DefineJournalPartialAbbreviation{Substant}{Subst}
\DefineJournalAbbreviation{Substitute}{Substit}
\DefineJournalAbbreviation{Substitution}{Substit}
\DefineJournalPartialAbbreviation{Substructur}{Substruct}
\DefineJournalPartialAbbreviation{Subsurfac}{Subsurf}
\DefineJournalAbbreviation{Subterranean}{Subterr}
\DefineJournalAbbreviation{Suburban}{Suburb}
\DefineJournalAbbreviation{Subvention}{Subvent}
\DefineJournalAbbreviation{Succeeding}{Succeed}
\DefineJournalWordException{Success}{Success}
\DefineJournalAbbreviation{Successful}{Success}
\DefineJournalAbbreviation{Successoral}{Successor}
\DefineJournalAbbreviation{Succulent}{Succul}
\DefineJournalAbbreviation{Sudanese}{Sudan}
\DefineJournalAbbreviation{Sudanic}{Sudan}
\DefineJournalWordException{Sudbury}{Sudbury}
\DefineJournalAbbreviation{Sudden}{Sudd}
\DefineJournalPartialAbbreviation{Suffer}{Suff}
\DefineJournalAbbreviation{Sufficiency}{Suffic}
\DefineJournalWordException{Suffolk}{Suffolk}
\DefineJournalWordException{Sugar}{Sugar}
\DefineJournalWordException{Sugarcane}{Sugarcane}
\DefineJournalPartialAbbreviation{Suggest}{Suggest}
\DefineJournalWordException{Suicide}{Suicide}
\DefineJournalAbbreviation{Suitability}{Suitabil}
\DefineJournalWordException{Suitable}{Suitable}
\DefineJournalWordException{Sulfate}{Sulfate}
\DefineJournalWordException{Sulphur}{Sulphur}
\DefineJournalAbbreviation{Sumerian}{Sumer}
\DefineJournalPartialAbbreviation{Summar}{Summ}
\DefineJournalAbbreviation{Summative}{Summ}
\DefineJournalWordException{Summer}{Summer}
\DefineJournalAbbreviation{Summerfallow}{Summerfall}
\DefineJournalWordException{Summerfruit}{Summerfruit}
\DefineJournalAbbreviation{Summerland}{Summerl}
\DefineJournalWordException{Summit}{Summit}
\DefineJournalWordException{Sunbeam}{Sunbeam}
\DefineJournalWordException{Sundargarh}{Sundargarh}
\DefineJournalWordException{Sunday}{Sunday}
\DefineJournalWordException{Sundry}{Sundry}
\DefineJournalWordException{Sunflower}{Sunflower}
\DefineJournalWordException{Sunnyvale}{Sunnyvale}
\DefineJournalAbbreviation{Sunrise}{Sunr}
\DefineJournalAbbreviation{Sunset}{Suns}
\DefineJournalWordException{Sunshine}{Sunshine}
\DefineJournalWordException{Sunspot}{Sunspot}
\DefineJournalWordException{Sunstar}{Sunstar}
\DefineJournalAbbreviation{Superannuation}{Superann}
\DefineJournalWordException{Supercars}{Supercars}
\DefineJournalAbbreviation{Supercellular}{Supercell}
\DefineJournalPartialAbbreviation{Superceramic}{Superceram}
\DefineJournalPartialAbbreviation{Supercomposit}{Supercompos}
\DefineJournalPartialAbbreviation{Supercomput}{Supercomput}
\DefineJournalPartialAbbreviation{Superconduct}{Supercond}
\DefineJournalPartialAbbreviation{Supercritical}{Supercrit}
\DefineJournalPartialAbbreviation{Superfic}{Superf}
\DefineJournalPartialAbbreviation{Superintend}{Supt}
\DefineJournalPartialAbbreviation{Superior}{Super}
\DefineJournalWordException{Superkart}{Superkart}
\DefineJournalWordException{Superman}{Superman}
\DefineJournalAbbreviation{Supermarket}{Supermark}
\DefineJournalAbbreviation{Supernatural}{Supernat}
\DefineJournalWordException{Superpack}{Superpack}
\DefineJournalWordException{Superphosphate}{Superphosphate}
\DefineJournalPartialAbbreviation{Superplastic}{Superplast}
\DefineJournalAbbreviation{Superstore}{Superst}
\DefineJournalWordException{Supertext}{Supertext}
\DefineJournalAbbreviation{Supervising}{Superv}
\DefineJournalAbbreviation{Supervision}{Superv}
\DefineJournalPartialAbbreviation{Supervisor}{Superv}
\DefineJournalPartialAbbreviation{Supplement}{Suppl}
\DefineJournalWordException{Supplier}{Supplier}
\DefineJournalWordException{Supply}{Supply}
\DefineJournalAbbreviation{Supplyship}{Supplysh}
\DefineJournalAbbreviation{Suppressant}{Suppr}
\DefineJournalAbbreviation{Suppression}{Suppr}
\DefineJournalPartialAbbreviation{Supramolecul}{Supramol}
\DefineJournalAbbreviation{Supranational}{Supranatl}
\DefineJournalWordException{Supr\^eme}{Supr\^eme}
\DefineJournalWordException{Surbiton}{Surbiton}
\DefineJournalWordException{Sureguard}{Sureguard}
\DefineJournalAbbreviation{Surface}{Surf}
\DefineJournalAbbreviation{Surfacing}{Surf}
\DefineJournalWordException{Surfactant}{Surfactant}
\DefineJournalWordException{Surfer}{Surfer}
\DefineJournalWordException{Surfing}{Surfing}
\DefineJournalWordException{Surfline}{Surfline}
\DefineJournalPartialAbbreviation{Surgeon}{Surg}
\DefineJournalAbbreviation{Surgery}{Surg}
\DefineJournalPartialAbbreviation{Surgic}{Surg}
\DefineJournalWordException{Surinam}{Surinam}
\DefineJournalWordException{Suriname}{Suriname}
\DefineJournalAbbreviation{Surname}{Surn}
\DefineJournalWordException{Surprise}{Surprise}
\DefineJournalAbbreviation{Surprising}{Surpris}
\DefineJournalAbbreviation{Surrealist}{Surreal}
\DefineJournalWordException{Surrey}{Surrey}
\DefineJournalPartialAbbreviation{Surrogat}{Surrog}
\DefineJournalAbbreviation{Surrounding}{Surround}
\DefineJournalWordException{Surtsey}{Surtsey}
\DefineJournalPartialAbbreviation{Survey}{Surv}
\DefineJournalPartialAbbreviation{Surviv}{Surviv}
\DefineJournalWordException{Suspected}{Suspected}
\DefineJournalAbbreviation{Susquehanna}{Susquehan}
\DefineJournalWordException{Sussex}{Sussex}
\DefineJournalPartialAbbreviation{Sustain}{Sustain}
\DefineJournalAbbreviation{Sutherland}{Sutherl}
\DefineJournalWordException{Sutton}{Sutton}
\DefineJournalAbbreviation{Swansea}{Swans}
\DefineJournalWordException{Swartklip}{Swartklip}
\DefineJournalAbbreviation{Swaziland}{Swazil}
\DefineJournalWordException{Swearing}{Swearing}
\DefineJournalWordException{Sweater}{Sweater}
\DefineJournalAbbreviation{Sweden}{Swed}
\DefineJournalAbbreviation{Swedish}{Swed}
\DefineJournalAbbreviation{Sweepstake}{Sweepst}
\DefineJournalPartialAbbreviation{Sweeten}{Sweeten}
\DefineJournalPartialAbbreviation{Swim}{Swim}
\DefineJournalWordException{Swimwear}{Swimwear}
\DefineJournalWordException{Swindon}{Swindon}
\DefineJournalAbbreviation{Swinger}{Swing}
\DefineJournalAbbreviation{Swinging}{Swing}
\DefineJournalWordException{Swinny}{Swinny}
\DefineJournalWordException{Swiss}{Swiss}
\DefineJournalPartialAbbreviation{Switch}{Switch}
\DefineJournalAbbreviation{Switchboard}{Switchb}
\DefineJournalAbbreviation{Switchgear}{Switchg}
\DefineJournalAbbreviation{Switzerland}{Switz}
\DefineJournalWordException{Swizzle}{Swizzle}
\DefineJournalWordException{Swords}{Swords}
\DefineJournalWordException{Sycamore}{Sycamore}
\DefineJournalWordException{Sydenham}{Sydenham}
\DefineJournalAbbreviation{Sydney}{Syd}
\DefineJournalWordException{Syllabic}{Syllabic}
\DefineJournalWordException{Syllabus}{Syllabus}
\DefineJournalWordException{Sylloge}{Sylloge}
\DefineJournalPartialAbbreviation{Sylvicult}{Sylvic}
\DefineJournalAbbreviation{Symphony}{Symph}
\DefineJournalAbbreviation{Synagogue}{Synag}
\DefineJournalWordException{Synaptic}{Synaptic}
\DefineJournalAbbreviation{Synchronize}{Synchron}
\DefineJournalWordException{Synchrotron}{Synchrotron}
\DefineJournalPartialAbbreviation{Syndic}{Synd}
\DefineJournalPartialAbbreviation{Syndromolog}{Syndromol}
\DefineJournalPartialAbbreviation{Synerg}{Synerg}
\DefineJournalWordException{Synfuel}{Synfuel}
\DefineJournalAbbreviation{Synonym}{Synon}
\DefineJournalAbbreviation{Synopsis}{Synop}
\DefineJournalPartialAbbreviation{System}{Syst}
\DefineJournalWordException{Tabernacle}{Tabernacle}
\DefineJournalWordException{Table}{Table}
\DefineJournalWordException{Tablelands}{Tablelands}
\DefineJournalWordException{Tabletop}{Tabletop}
\DefineJournalAbbreviation{Tableware}{Tablew}
\DefineJournalWordException{Tablistic}{Tablistic}
\DefineJournalWordException{Tabloid}{Tabloid}
\DefineJournalPartialAbbreviation{Tabulation}{Tabul}
\DefineJournalAbbreviation{Tackle}{Tack}
\DefineJournalWordException{Tactical}{Tactical}
\DefineJournalWordException{Tactics}{Tactics}
\DefineJournalWordException{Tailing}{Tailing}
\DefineJournalWordException{Taipei}{Taipei}
\DefineJournalAbbreviation{Taiwanese}{Taiwan}
\DefineJournalWordException{Takeaway}{Takeaway}
\DefineJournalWordException{Takeover}{Takeover}
\DefineJournalAbbreviation{Taking}{Tak}
\DefineJournalWordException{Takoma Park}{Takoma Park}
\DefineJournalPartialAbbreviation{Talent}{Talent}
\DefineJournalAbbreviation{Talking}{Talk}
\DefineJournalAbbreviation{Tallahassee}{Tallahass}
\DefineJournalWordException{Tamarillo}{Tamarillo}
\DefineJournalWordException{Tamil-Nadu}{Tamil-Nadu}
\DefineJournalWordException{Tamworth}{Tamworth}
\DefineJournalPartialAbbreviation{Tanaidac}{Tanaidac}
\DefineJournalWordException{Tandem}{Tandem}
\DefineJournalAbbreviation{Tanganyka}{Tangan}
\DefineJournalPartialAbbreviation{Tangl}{Tangl}
\DefineJournalWordException{Tanker}{Tanker}
\DefineJournalWordException{Tankerton}{Tankerton}
\DefineJournalAbbreviation{Tanzania}{Tanzan}
\DefineJournalWordException{Tapestry}{Tapestry}
\DefineJournalAbbreviation{Taphonomy}{Taphon}
\DefineJournalWordException{Taranaki}{Taranaki}
\DefineJournalWordException{Tarantula}{Tarantula}
\DefineJournalWordException{Target}{Target}
\DefineJournalAbbreviation{Targeted}{Target}
\DefineJournalAbbreviation{Targeting}{Target}
\DefineJournalAbbreviation{Targumic}{Targum}
\DefineJournalWordException{Tariff}{Tariff}
\DefineJournalWordException{Tarlton}{Tarlton}
\DefineJournalWordException{Tartan}{Tartan}
\DefineJournalAbbreviation{Tartogenic}{Tartog}
\DefineJournalWordException{Tartrate}{Tartrate}
\DefineJournalPartialAbbreviation{Tasman}{Tasman}
\DefineJournalPartialAbbreviation{Tast}{Tast}
\DefineJournalWordException{Tattle}{Tattle}
\DefineJournalWordException{Tattler}{Tattler}
\DefineJournalWordException{Tattoo}{Tattoo}
\DefineJournalWordException{Tatura}{Tatura}
\DefineJournalWordException{Tavistock}{Tavistock}
\DefineJournalAbbreviation{Taxation}{Tax}
\DefineJournalWordException{Taxicab}{Taxicab}
\DefineJournalAbbreviation{Taxing}{Tax}
\DefineJournalAbbreviation{Taxpayer}{Taxpay}
\DefineJournalWordException{Tayside}{Tayside}
\DefineJournalPartialAbbreviation{Teacher}{Teach}
\DefineJournalAbbreviation{Teaching}{Teach}
\DefineJournalWordException{Teamwork}{Teamwork}
\DefineJournalWordException{Teaneek}{Teaneek}
\DefineJournalPartialAbbreviation{Technobiolog}{Technobiol}
\DefineJournalAbbreviation{Technocracy}{Technocr}
\DefineJournalPartialAbbreviation{Technocrat}{Technocr}
\DefineJournalWordException{Technoflow}{Technoflow}
\DefineJournalPartialAbbreviation{Technogen}{Technog}
\DefineJournalWordException{Techsource}{Techsource}
\DefineJournalWordException{Tecorian}{Tecorian}
\DefineJournalPartialAbbreviation{Tectonophysi}{Tectonophys}
\DefineJournalAbbreviation{Teddington}{Teddingt}
\DefineJournalWordException{Teenage}{Teenage}
\DefineJournalWordException{Teenager}{Teenager}
\DefineJournalWordException{Teesside}{Teesside}
\DefineJournalWordException{Tehran}{Tehran}
\DefineJournalAbbreviation{Telebook}{Teleb}
\DefineJournalWordException{Telecaster}{Telecaster}
\DefineJournalAbbreviation{Telecomeuropa}{Telecomeur}
\DefineJournalPartialAbbreviation{Telecommunication}{Telecommun}
\DefineJournalWordException{Telecommunity}{Telecommunity}
\DefineJournalPartialAbbreviation{Telecommut}{Telecommut}
\DefineJournalAbbreviation{Telegram}{Telegr}
\DefineJournalAbbreviation{Telemanagement}{Telemanag}
\DefineJournalWordException{Telemedia}{Telemedia}
\DefineJournalPartialAbbreviation{Telemetr}{Telem}
\DefineJournalPartialAbbreviation{Telephon}{Teleph}
\DefineJournalWordException{Teleplan}{Teleplan}
\DefineJournalAbbreviation{Teleprinter}{Telepr}
\DefineJournalPartialAbbreviation{Telepublish}{Telepubl}
\DefineJournalPartialAbbreviation{Telescop}{Telesc}
\DefineJournalWordException{Telestar}{Telestar}
\DefineJournalWordException{Teletext}{Teletext}
\DefineJournalPartialAbbreviation{Televis}{Telev}
\DefineJournalAbbreviation{Teleworking}{Telework}
\DefineJournalWordException{Telidon}{Telidon}
\DefineJournalWordException{Tellurium}{Tellurium}
\DefineJournalWordException{Temiscamingue}{Temiscamingue}
\DefineJournalAbbreviation{Temperance}{Temper}
\DefineJournalPartialAbbreviation{Temperat}{Temp}
\DefineJournalWordException{Tempest}{Tempest}
\DefineJournalWordException{Templar}{Templar}
\DefineJournalWordException{Template}{Template}
\DefineJournalAbbreviation{Temporary}{Tempor}
\DefineJournalWordException{Temptation}{Temptation}
\DefineJournalWordException{Tenancy}{Tenancy}
\DefineJournalWordException{Tenant}{Tenant}
\DefineJournalWordException{Tender}{Tender}
\DefineJournalAbbreviation{Tennessee}{Tenn}
\DefineJournalWordException{Tennis}{Tennis}
\DefineJournalWordException{Tennister}{Tennister}
\DefineJournalWordException{Tenpin}{Tenpin}
\DefineJournalPartialAbbreviation{Tension}{Tens}
\DefineJournalWordException{Tensor}{Tensor}
\DefineJournalWordException{Tenure}{Tenure}
\DefineJournalPartialAbbreviation{Teratolog}{Teratol}
\DefineJournalWordException{Terenure}{Terenure}
\DefineJournalPartialAbbreviation{Termin}{Termin}
\DefineJournalPartialAbbreviation{Termit}{Termit}
\DefineJournalWordException{Terpenoid}{Terpenoid}
\DefineJournalWordException{Terrace}{Terrace}
\DefineJournalWordException{Terrain}{Terrain}
\DefineJournalWordException{Terramycine}{Terramycine}
\DefineJournalPartialAbbreviation{Terrestr}{Terr}
\DefineJournalPartialAbbreviation{Territ}{Territ}
\DefineJournalPartialAbbreviation{Terror}{Terror}
\DefineJournalWordException{Tertian}{Tertian}
\DefineJournalAbbreviation{Tertiary}{Tert}
\DefineJournalWordException{Terzaghi}{Terzaghi}
\DefineJournalAbbreviation{Testament}{Testam}
\DefineJournalAbbreviation{Tested}{Test}
\DefineJournalPartialAbbreviation{Testicul}{Testic}
\DefineJournalWordException{Testimony}{Testimony}
\DefineJournalAbbreviation{Testing}{Test}
\DefineJournalWordException{Tetrahedron}{Tetrahedron}
\DefineJournalPartialAbbreviation{Tetrapeptid}{Tetrapept}
\DefineJournalAbbreviation{Texas}{Tex}
\DefineJournalPartialAbbreviation{Textbook}{Textb}
\DefineJournalAbbreviation{T\^extil}{Text}
\DefineJournalPartialAbbreviation{Textile}{Text}
\DefineJournalWordException{Textrina}{Textrina}
\DefineJournalWordException{Textual}{Textual}
\DefineJournalWordException{Texture}{Texture}
\DefineJournalAbbreviation{Thailand}{Thail}
\DefineJournalAbbreviation{Thamesville}{Thamesv}
\DefineJournalWordException{The Hague}{The Hague}
\DefineJournalPartialAbbreviation{Theatr}{Theatr}
\DefineJournalWordException{Theatre}{Theatre}
\DefineJournalPartialAbbreviation{Theatrescript}{Theatrescr}
\DefineJournalPartialAbbreviation{Themati}{Themat}
\DefineJournalPartialAbbreviation{Theolog}{Theol}
\DefineJournalAbbreviation{Theometry}{Theom}
\DefineJournalPartialAbbreviation{Theoret}{Theor}
\DefineJournalPartialAbbreviation{Theori}{Theor}
\DefineJournalWordException{Theory}{Theory}
\DefineJournalPartialAbbreviation{Therap}{Ther}
\DefineJournalWordException{Therefrom}{Therefrom}
\DefineJournalPartialAbbreviation{Thermal}{Therm}
\DefineJournalPartialAbbreviation{Thermionic}{Thermion}
\DefineJournalPartialAbbreviation{Thermochem}{Thermochem}
\DefineJournalWordException{Thermodata}{Thermodata}
\DefineJournalPartialAbbreviation{Thermodynam}{Thermodyn}
\DefineJournalAbbreviation{Thermoelasticity}{Thermoelast}
\DefineJournalPartialAbbreviation{Thermoelectri}{Thermoelectr}
\DefineJournalPartialAbbreviation{Thermogravimetr}{Thermogravim}
\DefineJournalPartialAbbreviation{Thermoluminescen}{Thermolumin}
\DefineJournalAbbreviation{Thermonuclear}{Thermonucl}
\DefineJournalPartialAbbreviation{Thermophysic}{Thermophys}
\DefineJournalPartialAbbreviation{Thermoplastic}{Thermoplast}
\DefineJournalPartialAbbreviation{Thermotherap}{Thermother}
\DefineJournalWordException{Therpewin}{Therpewin}
\DefineJournalWordException{Thesis}{Thesis}
\DefineJournalPartialAbbreviation{Thessalonik}{Thessalon}
\DefineJournalPartialAbbreviation{Thick}{Thick}
\DefineJournalAbbreviation{Thinker}{Think}
\DefineJournalAbbreviation{Thinking}{Think}
\DefineJournalWordException{Third}{Third}
\DefineJournalAbbreviation{Thirteenth}{Thirteen}
\DefineJournalWordException{Thirties}{Thirties}
\DefineJournalWordException{Thirty}{Thirty}
\DefineJournalPartialAbbreviation{Thoracal}{Thorac}
\DefineJournalAbbreviation{Thoracic}{Thorac}
\DefineJournalWordException{Thorofare}{Thorofare}
\DefineJournalAbbreviation{Thoronto}{Thor}
\DefineJournalWordException{Thoroughbred}{Thoroughbred}
\DefineJournalWordException{Thought}{Thought}
\DefineJournalWordException{Thousand}{Thousand}
\DefineJournalWordException{Thousande}{Thousande}
\DefineJournalWordException{Thread}{Thread}
\DefineJournalPartialAbbreviation{Threat}{Threat}
\DefineJournalWordException{Threefold}{Threefold}
\DefineJournalWordException{Threepenny}{Threepenny}
\DefineJournalPartialAbbreviation{Thresh}{Thresh}
\DefineJournalPartialAbbreviation{Threshold}{Threshold}
\DefineJournalWordException{Thrift}{Thrift}
\DefineJournalWordException{Thrill}{Thrill}
\DefineJournalWordException{Thriller}{Thriller}
\DefineJournalWordException{Throat}{Throat}
\DefineJournalWordException{Thrombolysis}{Thrombolysis}
\DefineJournalAbbreviation{Thrombotic}{Thromb}
\DefineJournalWordException{Thromboxane}{Thromboxane}
\DefineJournalWordException{Through}{Through}
\DefineJournalWordException{Throughout}{Throughout}
\DefineJournalWordException{Throughput}{Throughput}
\DefineJournalWordException{Throwsters}{Throwsters}
\DefineJournalPartialAbbreviation{Thump}{Thump}
\DefineJournalWordException{Thunder}{Thunder}
\DefineJournalWordException{Thunderbird}{Thunderbird}
\DefineJournalAbbreviation{Thunderstorm}{Thunderst}
\DefineJournalAbbreviation{Thursday}{Thurs}
\DefineJournalWordException{Thymus}{Thymus}
\DefineJournalWordException{Thyristor}{Thyristor}
\DefineJournalAbbreviation{Thyroidology}{Thyroidol}
\DefineJournalAbbreviation{Tibetology}{Tibetol}
\DefineJournalAbbreviation{Ticker}{Tick}
\DefineJournalAbbreviation{Ticketing}{Ticket}
\DefineJournalWordException{Tickled}{Tickled}
\DefineJournalWordException{Tidal}{Tidal}
\DefineJournalWordException{Tidbits}{Tidbits}
\DefineJournalWordException{Tiding}{Tiding}
\DefineJournalWordException{Tightwire}{Tightwire}
\DefineJournalWordException{Tilbury}{Tilbury}
\DefineJournalWordException{Tillage}{Tillage}
\DefineJournalWordException{Timber}{Timber}
\DefineJournalWordException{Timberman}{Timberman}
\DefineJournalWordException{Timbertrader}{Timbertrader}
\DefineJournalWordException{Time}{Time}
\DefineJournalAbbreviation{Timekeeping}{Timekeep}
\DefineJournalWordException{Timely}{Timely}
\DefineJournalWordException{Timepiece}{Timepiece}
\DefineJournalPartialAbbreviation{Timeshar}{Timeshar}
\DefineJournalWordException{Timetable}{Timetable}
\DefineJournalWordException{Timing}{Timing}
\DefineJournalWordException{Timmins}{Timmins}
\DefineJournalWordException{Tinnitus}{Tinnitus}
\DefineJournalAbbreviation{Tinplate}{Tinpl}
\DefineJournalWordException{Tipperary}{Tipperary}
\DefineJournalWordException{Title}{Title}
\DefineJournalWordException{Titmouse}{Titmouse}
\DefineJournalPartialAbbreviation{Titrimetr}{Titrim}
\DefineJournalAbbreviation{Tobacco}{Tob}
\DefineJournalAbbreviation{Tobacconist}{Tob}
\DefineJournalPartialAbbreviation{Tocolog}{Tocol}
\DefineJournalWordException{Today}{Today}
\DefineJournalWordException{Toddler}{Toddler}
\DefineJournalWordException{Together}{Together}
\DefineJournalPartialAbbreviation{Toilet}{Toilet}
\DefineJournalPartialAbbreviation{Toleran}{Toler}
\DefineJournalWordException{Tomato}{Tomato}
\DefineJournalPartialAbbreviation{Tomograph}{Tomogr}
\DefineJournalWordException{Tomorrow}{Tomorrow}
\DefineJournalAbbreviation{Tonbridge}{Tonbr}
\DefineJournalWordException{Tongue}{Tongue}
\DefineJournalWordException{Tonnage}{Tonnage}
\DefineJournalAbbreviation{Tooling}{Tool}
\DefineJournalAbbreviation{Toolmaker}{Toolmak}
\DefineJournalAbbreviation{Toolmaking}{Toolmak}
\DefineJournalWordException{Toowoomba}{Toowoomba}
\DefineJournalPartialAbbreviation{Topic}{Top}
\DefineJournalAbbreviation{Topmagazine}{Topmag}
\DefineJournalPartialAbbreviation{Topolog}{Topol}
\DefineJournalPartialAbbreviation{Toponym}{Topon}
\DefineJournalPartialAbbreviation{Toracic}{Torac}
\DefineJournalWordException{Torch}{Torch}
\DefineJournalAbbreviation{Toronto}{Tor}
\DefineJournalWordException{Torque}{Torque}
\DefineJournalWordException{Tortoise}{Tortoise}
\DefineJournalPartialAbbreviation{Total}{Total}
\DefineJournalWordException{Touch}{Touch}
\DefineJournalAbbreviation{Touchpaper}{Touchpap}
\DefineJournalWordException{Tought}{Tought}
\DefineJournalWordException{Tourguide}{Tourguide}
\DefineJournalPartialAbbreviation{Touris}{Tour}
\DefineJournalWordException{Tournament}{Tournament}
\DefineJournalWordException{Towage}{Towage}
\DefineJournalWordException{Towards}{Towards}
\DefineJournalWordException{Tower}{Tower}
\DefineJournalWordException{Town}{Town}
\DefineJournalAbbreviation{Towncrier}{Towncr}
\DefineJournalWordException{Towner}{Towner}
\DefineJournalAbbreviation{Township}{Townsh}
\DefineJournalWordException{Townsite}{Townsite}
\DefineJournalAbbreviation{Townsman}{Townsm}
\DefineJournalAbbreviation{Townsville}{Townsv}
\DefineJournalAbbreviation{Toxicant}{Toxic}
\DefineJournalAbbreviation{Toxicity}{Toxic}
\DefineJournalPartialAbbreviation{Toxicokineti}{Toxicokinet}
\DefineJournalPartialAbbreviation{Toxicolog}{Toxicol}
\DefineJournalWordException{Tracing}{Tracing}
\DefineJournalWordException{Track}{Track}
\DefineJournalAbbreviation{Tracking}{Track}
\DefineJournalWordException{Trackside}{Trackside}
\DefineJournalAbbreviation{Traction}{Tract}
\DefineJournalWordException{Tractionel}{Tractionel}
\DefineJournalAbbreviation{Tractor}{Tract}
\DefineJournalWordException{Trade}{Trade}
\DefineJournalAbbreviation{Tradejournal}{Tradej}
\DefineJournalAbbreviation{Tradeletter}{Tradelett}
\DefineJournalWordException{Tradelink}{Tradelink}
\DefineJournalWordException{Trademark}{Trademark}
\DefineJournalAbbreviation{Tradenames}{Traden}
\DefineJournalWordException{Tradeport}{Tradeport}
\DefineJournalWordException{Trader}{Trader}
\DefineJournalWordException{Tradeshow}{Tradeshow}
\DefineJournalWordException{Tradesman}{Tradesman}
\DefineJournalWordException{Trading}{Trading}
\DefineJournalWordException{Traffic}{Traffic}
\DefineJournalPartialAbbreviation{Traffick}{Traffick}
\DefineJournalWordException{Traider}{Traider}
\DefineJournalPartialAbbreviation{Trailblaz}{Trailblaz}
\DefineJournalWordException{Trailer}{Trailer}
\DefineJournalWordException{Trailerboat}{Trailerboat}
\DefineJournalAbbreviation{Trailering}{Trailer}
\DefineJournalAbbreviation{Trailway}{Trailw}
\DefineJournalAbbreviation{Traineeship}{Traineesh}
\DefineJournalAbbreviation{Trainer}{Train}
\DefineJournalWordException{Trainerlink}{Trainerlink}
\DefineJournalAbbreviation{Training}{Train}
\DefineJournalAbbreviation{Tramping}{Tramp}
\DefineJournalAbbreviation{Tramway}{Tramw}
\DefineJournalAbbreviation{Transatlantic}{Transatl}
\DefineJournalWordException{Transatom}{Transatom}
\DefineJournalAbbreviation{Transborder}{Transbord}
\DefineJournalAbbreviation{Transboundary}{Transbound}
\DefineJournalWordException{Transceiver}{Transceiver}
\DefineJournalAbbreviation{Transcellular}{Transcell}
\DefineJournalAbbreviation{Transcendental}{Transcend}
\DefineJournalAbbreviation{Transcriber}{Transcr}
\DefineJournalPartialAbbreviation{Transcript}{Transcr}
\DefineJournalPartialAbbreviation{Transcultur}{Transcult}
\DefineJournalPartialAbbreviation{Transdisciplin}{Transdiscipl}
\DefineJournalWordException{Transducer}{Transducer}
\DefineJournalAbbreviation{Transduction}{Transduct}
\DefineJournalWordException{Transect}{Transect}
\DefineJournalAbbreviation{Transfer}{Transf}
\DefineJournalWordException{Transferase}{Transferase}
\DefineJournalAbbreviation{Transfusion}{Transfus}
\DefineJournalWordException{Transistor}{Transistor}
\DefineJournalWordException{Transit}{Transit}
\DefineJournalAbbreviation{Transitoire}{Transit}
\DefineJournalAbbreviation{Transkeian}{Transkei}
\DefineJournalPartialAbbreviation{Translat}{Transl}
\DefineJournalPartialAbbreviation{Translocation}{Translocat}
\DefineJournalPartialAbbreviation{Transmi}{Transm}
\DefineJournalAbbreviation{Transmutation}{Transmutat}
\DefineJournalAbbreviation{Transnational}{Transnatl}
\DefineJournalAbbreviation{Transparency}{Transpar}
\DefineJournalAbbreviation{Transpersonal}{Transpers}
\DefineJournalAbbreviation{Transplant}{Transpl}
\DefineJournalAbbreviation{Transplantation}{Transplant}
\DefineJournalPartialAbbreviation{Transport}{Transp}
\DefineJournalAbbreviation{Transputer}{Transput}
\DefineJournalAbbreviation{Transworld}{Transw}
\DefineJournalAbbreviation{Transylvanian}{Transylv}
\DefineJournalAbbreviation{Trapper}{Trapp}
\DefineJournalAbbreviation{Trapping}{Trapp}
\DefineJournalPartialAbbreviation{Trasmissi}{Trasm}
\DefineJournalWordException{Trasylol}{Trasylol}
\DefineJournalWordException{Trauma}{Trauma}
\DefineJournalAbbreviation{Traumatic}{Trauma}
\DefineJournalWordException{Travel}{Travel}
\DefineJournalPartialAbbreviation{Travel}{Travel}
\DefineJournalAbbreviation{Traveletter}{Travelett}
\DefineJournalWordException{Traveltrade}{Traveltrade}
\DefineJournalPartialAbbreviation{Trawl}{Trawl}
\DefineJournalWordException{Treasure}{Treasure}
\DefineJournalAbbreviation{Treasurer}{Treas}
\DefineJournalAbbreviation{Treasury}{Treas}
\DefineJournalAbbreviation{Treated}{Treat}
\DefineJournalAbbreviation{Treater}{Treat}
\DefineJournalAbbreviation{Treating}{Treat}
\DefineJournalWordException{Treatise}{Treatise}
\DefineJournalPartialAbbreviation{Treatment}{Treat}
\DefineJournalWordException{Treaty}{Treaty}
\DefineJournalWordException{Trefoil}{Trefoil}
\DefineJournalWordException{Trench}{Trench}
\DefineJournalWordException{Trend}{Trend}
\DefineJournalWordException{Trendicator}{Trendicator}
\DefineJournalWordException{Trends}{Trends}
\DefineJournalWordException{Trendshop}{Trendshop}
\DefineJournalWordException{Trenton}{Trenton}
\DefineJournalWordException{Tressure}{Tressure}
\DefineJournalAbbreviation{Tri-athlete}{Tri-athl}
\DefineJournalWordException{Tri-state}{Tri-state}
\DefineJournalWordException{Triangle}{Triangle}
\DefineJournalWordException{Tribal}{Tribal}
\DefineJournalPartialAbbreviation{Tribolog}{Tribol}
\DefineJournalWordException{Trichogramma}{Trichogramma}
\DefineJournalWordException{Trick}{Trick}
\DefineJournalWordException{Trickle}{Trickle}
\DefineJournalAbbreviation{Tricycling}{Tricycl}
\DefineJournalAbbreviation{Triennial}{Trienn}
\DefineJournalWordException{Trinity}{Trinity}
\DefineJournalPartialAbbreviation{Tripartit}{Tripart}
\DefineJournalWordException{Triplet}{Triplet}
\DefineJournalWordException{Tripura}{Tripura}
\DefineJournalAbbreviation{Triquarterly}{Triq}
\DefineJournalWordException{Triticale}{Triticale}
\DefineJournalWordException{Triumph}{Triumph}
\DefineJournalPartialAbbreviation{Triumph}{Triumph}
\DefineJournalWordException{Triune}{Triune}
\DefineJournalPartialAbbreviation{Troglodyt}{Troglod}
\DefineJournalWordException{Troller}{Troller}
\DefineJournalAbbreviation{Trolleybus}{Trolleyb}
\DefineJournalWordException{Trolling}{Trolling}
\DefineJournalPartialAbbreviation{Trophoblast}{Trophobl}
\DefineJournalWordException{Trophy}{Trophy}
\DefineJournalAbbreviation{Trotskyist}{Trotsky}
\DefineJournalWordException{Trouser}{Trouser}
\DefineJournalPartialAbbreviation{Truck}{Truck}
\DefineJournalWordException{Trumpet}{Trumpet}
\DefineJournalPartialAbbreviation{Trust}{Trust}
\DefineJournalWordException{Trustee}{Trustee}
\DefineJournalAbbreviation{Trusteeship}{Trusteesh}
\DefineJournalAbbreviation{Tubercle}{Tuber}
\DefineJournalPartialAbbreviation{Tuberculolog}{Tuberculol}
\DefineJournalPartialAbbreviation{Tuberculos}{Tuberc}
\DefineJournalWordException{Tubing}{Tubing}
\DefineJournalAbbreviation{Tubular}{Tubul}
\DefineJournalWordException{Tucson}{Tucson}
\DefineJournalWordException{Tuesday}{Tuesday}
\DefineJournalAbbreviation{Tuition}{Tuit}
\DefineJournalWordException{Tulane}{Tulane}
\DefineJournalWordException{Tullamore}{Tullamore}
\DefineJournalWordException{Tullow}{Tullow}
\DefineJournalWordException{Tulsa}{Tulsa}
\DefineJournalWordException{Tumbler}{Tumbler}
\DefineJournalWordException{Tumour}{Tumour}
\DefineJournalWordException{Tungsten}{Tungsten}
\DefineJournalWordException{Tuning}{Tuning}
\DefineJournalPartialAbbreviation{Tunisia}{Tunis}
\DefineJournalAbbreviation{Tunnel}{Tunn}
\DefineJournalAbbreviation{Tunnelling}{Tunn}
\DefineJournalPartialAbbreviation{Turbid}{Turbid}
\DefineJournalWordException{Turbine}{Turbine}
\DefineJournalAbbreviation{Turbomachinery}{Turbomach}
\DefineJournalAbbreviation{Turbotville}{Turbotv}
\DefineJournalPartialAbbreviation{Turbulen}{Turbul}
\DefineJournalAbbreviation{Turcological}{Turcol}
\DefineJournalWordException{Turfgrass}{Turfgrass}
\DefineJournalAbbreviation{Turkey}{Turk}
\DefineJournalAbbreviation{Turner}{Turn}
\DefineJournalAbbreviation{Turning}{Turn}
\DefineJournalWordException{Turnover}{Turnover}
\DefineJournalWordException{Turntable}{Turntable}
\DefineJournalAbbreviation{Turtle}{Turt}
\DefineJournalWordException{Tussock}{Tussock}
\DefineJournalAbbreviation{Tutorial}{Tutor}
\DefineJournalWordException{Tweedsmuir}{Tweedsmuir}
\DefineJournalWordException{Twelfth}{Twelfth}
\DefineJournalWordException{Twenty}{Twenty}
\DefineJournalWordException{Twickenham}{Twickenham}
\DefineJournalWordException{Twilight}{Twilight}
\DefineJournalPartialAbbreviation{Twist}{Twist}
\DefineJournalAbbreviation{Typereader}{Typeread}
\DefineJournalAbbreviation{Typesetting}{Typeset}
\DefineJournalAbbreviation{Typewriter}{Typewrit}
\DefineJournalAbbreviation{Typical}{Typ}
\DefineJournalWordException{Typing}{Typing}
\DefineJournalWordException{Typist}{Typist}
\DefineJournalPartialAbbreviation{Typograph}{Typogr}
\DefineJournalAbbreviation{Typological}{Typol}
\DefineJournalWordException{Udder}{Udder}
\DefineJournalWordException{Uganda}{Uganda}
\DefineJournalAbbreviation{Ulsterman}{Ulsterm}
\DefineJournalPartialAbbreviation{Ultim}{Ultim}
\DefineJournalPartialAbbreviation{Ultrafiltrati}{Ultrafiltr}
\DefineJournalAbbreviation{Ultrahigh}{Ultrah}
\DefineJournalWordException{Ultralight}{Ultralight}
\DefineJournalPartialAbbreviation{Ultramolecul}{Ultramol}
\DefineJournalAbbreviation{Ultranutrition}{Ultranutr}
\DefineJournalAbbreviation{Ultraprecision}{Ultraprecis}
\DefineJournalAbbreviation{Ultrapurification}{Ultrapurif}
\DefineJournalWordException{Ultrasound}{Ultrasound}
\DefineJournalPartialAbbreviation{Ultrastructur}{Ultrastruct}
\DefineJournalAbbreviation{Ultraviolet}{Ultrav}
\DefineJournalAbbreviation{Umpire}{Ump}
\DefineJournalWordException{Uncanny}{Uncanny}
\DefineJournalPartialAbbreviation{Uncaptiv}{Uncaptiv}
\DefineJournalAbbreviation{Uncensored}{Uncens}
\DefineJournalAbbreviation{Uncertainty}{Uncertain}
\DefineJournalPartialAbbreviation{Unclassifi}{Unclassif}
\DefineJournalWordException{Uncommon}{Uncommon}
\DefineJournalAbbreviation{Unconventional}{Unconv}
\DefineJournalAbbreviation{Uncooked}{Uncook}
\DefineJournalWordException{Undercar}{Undercar}
\DefineJournalAbbreviation{Undercurrent}{Undercurr}
\DefineJournalAbbreviation{Underemployed}{Underempl}
\DefineJournalAbbreviation{Undergarment}{Undergarm}
\DefineJournalAbbreviation{Undergraduate}{Undergrad}
\DefineJournalAbbreviation{Underground}{Undergr}
\DefineJournalWordException{Underlying}{Underlying}
\DefineJournalWordException{Undersea}{Undersea}
\DefineJournalAbbreviation{Understanding}{Underst}
\DefineJournalAbbreviation{Undertaking}{Undert}
\DefineJournalPartialAbbreviation{Underutilis}{Underutil}
\DefineJournalAbbreviation{Underwater}{Underw}
%\DefineJournalPartialWordException{Underwear}{Underwear-}
\DefineJournalPartialAbbreviation{Underwrit}{Underwrit}
\DefineJournalPartialAbbreviation{Unemploy}{Unempl}
\DefineJournalPartialAbbreviation{Unexamin}{Unexam}
\DefineJournalWordException{Unfair}{Unfair}
\DefineJournalPartialAbbreviation{Unfill}{Unfill}
%\DefineJournalPartialWordException{Ungulat}{Ungulat-}
\DefineJournalAbbreviation{Unicorn}{Unic}
\DefineJournalAbbreviation{Uniform}{Unif}
\DefineJournalWordException{Unilife}{Unilife}
\DefineJournalPartialAbbreviation{Unionist}{Union}
\DefineJournalAbbreviation{Uniscience}{Unisci}
\DefineJournalPartialAbbreviation{Unishipp}{Unishipp}
\DefineJournalWordException{Unison}{Unison}
\DefineJournalAbbreviation{Unitarian}{Unit}
\DefineJournalWordException{United}{United}
\DefineJournalAbbreviation{United Arab Republic}{U A R}
\DefineJournalAbbreviation{United Kingdom}{U K}
\DefineJournalAbbreviation{United Nations}{U N}
\DefineJournalAbbreviation{United States}{U S}
\DefineJournalAbbreviation{United States of America}{U S A}
\DefineJournalAbbreviation{Unitholder}{Unithold}
\DefineJournalWordException{Uniting}{Uniting}
\DefineJournalWordException{Unitised}{Unitised}
\DefineJournalWordException{Univers}{Univers}
\DefineJournalAbbreviation{Universal}{Univers}
\DefineJournalWordException{Universalist}{Universalist}
\DefineJournalWordException{Universe}{Universe}
\DefineJournalPartialAbbreviation{Universit}{Univ}
\DefineJournalAbbreviation{Unknown}{Unkn}
\DefineJournalAbbreviation{Unlimited}{Unltd}
\DefineJournalWordException{Unlisted}{Unlisted}
\DefineJournalWordException{Unload}{Unload}
\DefineJournalAbbreviation{Unmasking}{Unmask}
\DefineJournalAbbreviation{Unmuzzle}{Unmuzz}
\DefineJournalAbbreviation{Unofficial}{Unoff}
\DefineJournalPartialAbbreviation{Unorgani}{Unorgan}
\DefineJournalWordException{Unpaid}{Unpaid}
\DefineJournalPartialAbbreviation{Unplug}{Unplug}
\DefineJournalPartialAbbreviation{Unpubli}{Unpubl}
\DefineJournalWordException{Unquoted}{Unquoted}
\DefineJournalPartialAbbreviation{Unreach}{Unreach}
\DefineJournalWordException{Unreal}{Unreal}
\DefineJournalAbbreviation{Unrelated}{Unrelat}
\DefineJournalAbbreviation{Unreported}{Unreport}
\DefineJournalAbbreviation{Unrepresented}{Unrepresent}
\DefineJournalAbbreviation{Unscathed}{Unscath}
\DefineJournalPartialAbbreviation{Unschedul}{Unsched}
\DefineJournalPartialAbbreviation{Unspeak}{Unspeak}
\DefineJournalAbbreviation{Unsuccessful}{Unsuccess}
\DefineJournalPartialAbbreviation{Untitl}{Untitl}
\DefineJournalWordException{Unusual}{Unusual}
\DefineJournalAbbreviation{Upcoming}{Upcom}
\DefineJournalPartialAbbreviation{Updat}{Updat}
\DefineJournalWordException{Update}{Update}
\DefineJournalPartialAbbreviation{Upgrad}{Upgrad}
\DefineJournalAbbreviation{Upgrading}{Upgrad}
\DefineJournalWordException{Upholstery}{Upholstery}
\DefineJournalWordException{Upkeep}{Upkeep}
\DefineJournalAbbreviation{Upland}{Upl}
\DefineJournalWordException{Uplook}{Uplook}
\DefineJournalAbbreviation{Upper}{Up}
\DefineJournalWordException{Upper-Volta}{Upper-Volta}
\DefineJournalAbbreviation{Uprating}{Uprat}
\DefineJournalWordException{Uprooted}{Uprooted}
\DefineJournalWordException{Upstairs}{Upstairs}
\DefineJournalWordException{Upstate}{Upstate}
\DefineJournalAbbreviation{Uptown}{Upt}
\DefineJournalWordException{Uptrends}{Uptrends}
\DefineJournalWordException{Uranium}{Uranium}
\DefineJournalWordException{Urban}{Urban}
\DefineJournalWordException{Urbana}{Urbana}
\DefineJournalWordException{Urbana-Champaign}{Urbana-Champaign}
\DefineJournalPartialAbbreviation{Urem}{Urem}
\DefineJournalPartialAbbreviation{Urin}{Urin}
\DefineJournalAbbreviation{Urodynamic}{Urodyn}
\DefineJournalAbbreviation{Urogenital}{Urogenit}
\DefineJournalWordException{Uruwan}{Uruwan}
\DefineJournalWordException{Usage}{Usage}
\DefineJournalWordException{Useful}{Useful}
\DefineJournalPartialAbbreviation{Useful}{Useful}
\DefineJournalWordException{Using}{Using}
\DefineJournalPartialAbbreviation{Utili}{Util}
\DefineJournalWordException{Uttar Pradesh}{Uttar Pradesh}
\DefineJournalWordException{Uxbridge}{Uxbridge}
\DefineJournalPartialAbbreviation{Vacanc}{Vacanc}
\DefineJournalWordException{Vacancy}{Vacancy}
\DefineJournalPartialAbbreviation{Vacation}{Vacat}
\DefineJournalWordException{Vacationland}{Vacationland}
\DefineJournalAbbreviation{Vaccinology}{Vaccinol}
\DefineJournalAbbreviation{Vacuum}{Vac}
\DefineJournalPartialAbbreviation{Vacuumtechni}{Vacuumtech}
\DefineJournalPartialAbbreviation{Valley}{Val}
\DefineJournalWordException{Valley-Field}{Valley-Field}
\DefineJournalAbbreviation{Valorisation}{Valoris}
\DefineJournalAbbreviation{Valuable}{Valuab}
\DefineJournalAbbreviation{Valuation}{Valuat}
\DefineJournalWordException{Value}{Value}
\DefineJournalWordException{Valueless}{Valueless}
\DefineJournalWordException{Valuer}{Valuer}
\DefineJournalWordException{Vampire}{Vampire}
\DefineJournalAbbreviation{Vandalism}{Vandal}
\DefineJournalWordException{Vanguard}{Vanguard}
\DefineJournalPartialAbbreviation{Vanguard}{Vanguard}
\DefineJournalAbbreviation{Vanishing}{Vanish}
\DefineJournalWordException{Vantage}{Vantage}
\DefineJournalPartialAbbreviation{Vapor}{Vap}
\DefineJournalAbbreviation{Vapour}{Vap}
\DefineJournalPartialAbbreviation{Variab}{Var}
\DefineJournalAbbreviation{Variance}{Var}
\DefineJournalPartialAbbreviation{Variant}{Var}
\DefineJournalPartialAbbreviation{Variation}{Var}
\DefineJournalPartialAbbreviation{Variet}{Var}
\DefineJournalAbbreviation{Various}{Var}
\DefineJournalPartialAbbreviation{Varnish}{Varn}
\DefineJournalPartialAbbreviation{Vascul}{Vasc}
\DefineJournalPartialAbbreviation{Vasoactive}{Vasoact}
\DefineJournalWordException{Vaughan}{Vaughan}
\DefineJournalWordException{Vauxhall}{Vauxhall}
\DefineJournalWordException{Vector}{Vector}
\DefineJournalPartialAbbreviation{Vegeta}{Veg}
\DefineJournalPartialAbbreviation{Vehic}{Veh}
\DefineJournalPartialAbbreviation{Velocimetr}{Velocim}
\DefineJournalAbbreviation{Velvet}{Velv}
\DefineJournalAbbreviation{Vending}{Vend}
\DefineJournalAbbreviation{Vendor}{Vend}
\DefineJournalWordException{Veneer}{Veneer}
\DefineJournalAbbreviation{Venereal}{Vener}
\DefineJournalPartialAbbreviation{Venereolog}{Venereol}
\DefineJournalAbbreviation{Venomous}{Venom}
\DefineJournalPartialAbbreviation{Ventil}{Vent}
\DefineJournalPartialAbbreviation{Ventur}{Ventur}
\DefineJournalWordException{Venue}{Venue}
\DefineJournalWordException{Verbal}{Verbal}
\DefineJournalAbbreviation{Verbatim}{Verbat}
\DefineJournalWordException{Verdict}{Verdict}
\DefineJournalWordException{Verify}{Verify}
\DefineJournalAbbreviation{Verifying}{Verif}
\DefineJournalWordException{Vermilion}{Vermilion}
\DefineJournalWordException{Vermillion}{Vermillion}
\DefineJournalWordException{Vermin}{Vermin}
\DefineJournalAbbreviation{Vermont}{Vt}
\DefineJournalAbbreviation{Vernacular}{Vernac}
\DefineJournalWordException{Vernon}{Vernon}
\DefineJournalAbbreviation{Vertical}{Vert}
\DefineJournalPartialAbbreviation{Vessel}{Vessel}
\DefineJournalAbbreviation{Vestibular}{Vestib}
\DefineJournalWordException{Veteran}{Veteran}
\DefineJournalPartialAbbreviation{Veterinar}{Vet}
\DefineJournalPartialAbbreviation{Vexillolog}{Vexillol}
\DefineJournalPartialAbbreviation{Vibration}{Vib}
\DefineJournalAbbreviation{Vibrotechni}{Vibrotech}
\DefineJournalAbbreviation{Vicinity}{Vicin}
\DefineJournalAbbreviation{Vicksburg}{Vicksbg}
\DefineJournalPartialAbbreviation{Victim}{Vict}
\DefineJournalAbbreviation{Victimization}{Victim}
\DefineJournalWordException{Victor}{Victor}
\DefineJournalAbbreviation{Victoria}{Vic}
\DefineJournalAbbreviation{Victoria Island}{Vic Isl}
\DefineJournalAbbreviation{Victorian}{Vic}
\DefineJournalAbbreviation{Victory}{Vic}
\DefineJournalPartialAbbreviation{Victuall}{Victual}
\DefineJournalWordException{Videodisc}{Videodisc}
\DefineJournalWordException{Videofile}{Videofile}
\DefineJournalPartialAbbreviation{Videograph}{Videogr}
\DefineJournalWordException{Videoplay}{Videoplay}
\DefineJournalPartialAbbreviation{Videoscop}{Videoscop}
\DefineJournalWordException{Videotape}{Videotape}
\DefineJournalWordException{Videotext}{Videotext}
\DefineJournalWordException{Videovue}{Videovue}
\DefineJournalWordException{Videoworld}{Videoworld}
\DefineJournalWordException{Vienna}{Vienna}
\DefineJournalAbbreviation{Viewdata}{Viewd}
%\DefineJournalPartialWordException{Viewer}{Viewer-}
\DefineJournalAbbreviation{Viewfinder}{Viewfind}
\DefineJournalWordException{Viewing}{Viewing}
\DefineJournalAbbreviation{Viewpoint}{Viewp}
\DefineJournalAbbreviation{Viewprint}{Viewpr}
\DefineJournalAbbreviation{Viewsweekly}{Viewswkl}
\DefineJournalWordException{Vignette}{Vignette}
\DefineJournalWordException{Village}{Village}
\DefineJournalWordException{Villanova}{Villanova}
\DefineJournalAbbreviation{Vincentian}{Vincent}
\DefineJournalAbbreviation{Vinegar}{Vineg}
\DefineJournalAbbreviation{Vinemaking}{Vinemak}
\DefineJournalWordException{Vineyard}{Vineyard}
\DefineJournalPartialAbbreviation{Vinicultur}{Vinic}
\DefineJournalWordException{Vinyl}{Vinyl}
\DefineJournalPartialAbbreviation{Violati}{Viol}
\DefineJournalWordException{Viral}{Viral}
\DefineJournalAbbreviation{Virgin-Islands}{Virg-Isl}
\DefineJournalAbbreviation{Virginia}{Va}
\DefineJournalWordException{Virtuae}{Virtuae}
\DefineJournalWordException{Virtual}{Virtual}
\DefineJournalAbbreviation{Virtualization}{Virtualiz}
\DefineJournalWordException{Virtuoso}{Virtuoso}
\DefineJournalAbbreviation{Visability}{Visabil}
\DefineJournalAbbreviation{Visceral}{Visc}
\DefineJournalWordException{Viscora}{Viscora}
\DefineJournalWordException{Viscous}{Viscous}
\DefineJournalAbbreviation{Vision}{Vis}
\DefineJournalAbbreviation{Visionary}{Vision}
\DefineJournalPartialAbbreviation{Visit}{Visit}
\DefineJournalPartialAbbreviation{Visual}{Vis}
\DefineJournalAbbreviation{Vitamin}{Vitam}
\DefineJournalPartialAbbreviation{Viticultur}{Vitic}
\DefineJournalPartialAbbreviation{Vitreoretin}{Vitreoretin}
\DefineJournalWordException{Vitreoretina}{Vitreoretina}
\DefineJournalAbbreviation{Viverrid}{Viver}
\DefineJournalAbbreviation{Vivisection}{Vivisect}
\DefineJournalPartialAbbreviation{Vocabular}{Vocab}
\DefineJournalPartialAbbreviation{Vocation}{Vocat}
\DefineJournalWordException{Voice}{Voice}
\DefineJournalAbbreviation{Volcanic}{Volcan}
\DefineJournalWordException{Volcano}{Volcano}
\DefineJournalPartialAbbreviation{Volcanolog}{Volcanol}
\DefineJournalAbbreviation{Volleyball}{Volleyb}
\DefineJournalAbbreviation{Voltage}{Volt}
\DefineJournalAbbreviation{Volusia}{Volus}
\DefineJournalWordException{Vortex}{Vortex}
\DefineJournalWordException{Voter}{Voter}
\DefineJournalWordException{Waferboard}{Waferboard}
\DefineJournalWordException{Waffenmarkt}{Waffenmarkt}
\DefineJournalAbbreviation{Wage-earner}{Wage-earn}
\DefineJournalWordException{Waikato}{Waikato}
\DefineJournalPartialAbbreviation{Wait}{Wait}
\DefineJournalPartialAbbreviation{Waiv}{Waiv}
\DefineJournalAbbreviation{Wakefield}{Wakef}
\DefineJournalWordException{Walden}{Walden}
\DefineJournalPartialAbbreviation{Waldens}{Waldens}
\DefineJournalAbbreviation{Walker}{Walk}
\DefineJournalAbbreviation{Walking}{Walk}
\DefineJournalAbbreviation{Walkway}{Walkw}
\DefineJournalAbbreviation{Wallchart}{Wallch}
\DefineJournalAbbreviation{Wallcovering}{Wallcover}
\DefineJournalWordException{Wallend}{Wallend}
\DefineJournalWordException{Wallingford}{Wallingford}
\DefineJournalAbbreviation{Wallpaper}{Wallpap}
\DefineJournalAbbreviation{Wallstreet}{Wallstr}
\DefineJournalWordException{Walnut}{Walnut}
\DefineJournalAbbreviation{Waltham}{Walth}
\DefineJournalAbbreviation{Walton}{Walt}
\DefineJournalWordException{Wanamaker}{Wanamaker}
\DefineJournalPartialAbbreviation{Wander}{Wander}
\DefineJournalWordException{Wandle}{Wandle}
\DefineJournalWordException{Wangaratta}{Wangaratta}
\DefineJournalWordException{Wantage}{Wantage}
\DefineJournalWordException{Wanted}{Wanted}
\DefineJournalAbbreviation{Warbird}{Warb}
\DefineJournalWordException{Warbler}{Warbler}
\DefineJournalAbbreviation{Warden}{Ward}
\DefineJournalAbbreviation{Warehouse}{Wareh}
\DefineJournalAbbreviation{Warehousing}{Warehous}
\DefineJournalPartialAbbreviation{Warfare}{Warf}
\DefineJournalAbbreviation{Wargame}{Warg}
\DefineJournalWordException{Warkworth}{Warkworth}
\DefineJournalAbbreviation{Warminster}{Warminst}
\DefineJournalPartialAbbreviation{Warn}{Warn}
\DefineJournalWordException{Warrant}{Warrant}
\DefineJournalWordException{Warrior}{Warrior}
\DefineJournalPartialAbbreviation{Warship}{Warsh}
\DefineJournalWordException{Warwick}{Warwick}
\DefineJournalAbbreviation{Warwickshire}{Warwicks}
\DefineJournalWordException{Wasaga-Beach}{Wasaga-Beach}
\DefineJournalWordException{Washing}{Washing}
\DefineJournalAbbreviation{Washington}{Wash}
\DefineJournalWordException{Waste}{Waste}
\DefineJournalWordException{Wastewater}{Wastewater}
\DefineJournalPartialAbbreviation{Watch}{Watch}
\DefineJournalAbbreviation{Watchbird}{Watchb}
\DefineJournalWordException{Watchman}{Watchman}
\DefineJournalWordException{Water}{Water}
\DefineJournalWordException{Waterbed}{Waterbed}
\DefineJournalWordException{Waterbird}{Waterbird}
\DefineJournalWordException{Waterborne}{Waterborne}
\DefineJournalWordException{Waterbury}{Waterbury}
\DefineJournalWordException{Watercraft}{Watercraft}
\DefineJournalWordException{Waterdown}{Waterdown}
\DefineJournalAbbreviation{Waterford}{Waterf}
\DefineJournalWordException{Waterfowl}{Waterfowl}
\DefineJournalAbbreviation{Waterfront}{Waterfr}
\DefineJournalWordException{Waterhouse}{Waterhouse}
\DefineJournalWordException{Waterloo}{Waterloo}
\DefineJournalWordException{Watermill}{Watermill}
\DefineJournalWordException{Waterpolo}{Waterpolo}
\DefineJournalWordException{Watershed}{Watershed}
\DefineJournalWordException{Waterski}{Waterski}
\DefineJournalPartialAbbreviation{Waterway}{Waterw}
\DefineJournalWordException{Waterwork}{Waterwork}
\DefineJournalWordException{Waterworld}{Waterworld}
\DefineJournalWordException{Watford}{Watford}
\DefineJournalWordException{Wattle}{Wattle}
\DefineJournalPartialAbbreviation{Wavefunction}{Wavefunct}
\DefineJournalAbbreviation{Wavelength}{Wavel}
\DefineJournalWordException{Waverton}{Waverton}
\DefineJournalWordException{Way}{Way}
\DefineJournalWordException{Waybill}{Waybill}
\DefineJournalWordException{Weald}{Weald}
\DefineJournalWordException{Wealth}{Wealth}
\DefineJournalWordException{Wealthline}{Wealthline}
\DefineJournalWordException{Wealthy}{Wealthy}
\DefineJournalAbbreviation{Weanling}{Weanl}
\DefineJournalWordException{Weapon}{Weapon}
\DefineJournalAbbreviation{Weaponry}{Weapon}
\DefineJournalPartialAbbreviation{Weather}{Weather}
\DefineJournalPartialAbbreviation{Weav}{Weav}
\DefineJournalPartialAbbreviation{Wedd}{Wedd}
\DefineJournalWordException{Wednesday}{Wednesday}
\DefineJournalWordException{Week}{Week}
\DefineJournalAbbreviation{Weekblad}{Weekbl}
\DefineJournalPartialAbbreviation{Weekend}{Weekend}
\DefineJournalAbbreviation{Weekly}{Wkly}
\DefineJournalAbbreviation{Weighing}{Weigh}
\DefineJournalPartialAbbreviation{Weight}{Weight}
\DefineJournalPartialAbbreviation{Weightlift}{Weightlift}
\DefineJournalWordException{Welcome}{Welcome}
\DefineJournalAbbreviation{Welder}{Weld}
\DefineJournalAbbreviation{Welding}{Weld}
\DefineJournalAbbreviation{Welfare}{Welf}
\DefineJournalWordException{Welland}{Welland}
\DefineJournalWordException{Wellbeing}{Wellbeing}
\DefineJournalWordException{Wellesley}{Wellesley}
\DefineJournalAbbreviation{Wellingborough}{Wellingb}
\DefineJournalAbbreviation{Wellington}{Wellingt}
\DefineJournalWordException{Wellness}{Wellness}
\DefineJournalWordException{Wentworth}{Wentworth}
\DefineJournalAbbreviation{Wesleyan}{Wesley}
\DefineJournalWordException{Wessex}{Wessex}
\DefineJournalWordException{West}{West}
\DefineJournalWordException{West Indian}{West Indian}
\DefineJournalAbbreviation{West Virginia}{W Va}
\DefineJournalWordException{Westbury}{Westbury}
\DefineJournalAbbreviation{Westchester}{Westchest}
\DefineJournalWordException{Westcoast}{Westcoast}
\DefineJournalPartialAbbreviation{Western}{West}
\DefineJournalWordException{Westfield}{Westfield}
\DefineJournalWordException{Westmeath}{Westmeath}
\DefineJournalAbbreviation{Westminster}{Westminst}
\DefineJournalAbbreviation{Westmorland}{Westmorl}
\DefineJournalAbbreviation{Westmount}{Westmt}
\DefineJournalAbbreviation{Weston}{West}
\DefineJournalAbbreviation{Weston-Super-Mare}{West-Super-Mare}
\DefineJournalWordException{Westside}{Westside}
\DefineJournalAbbreviation{Westville}{Westv}
\DefineJournalPartialAbbreviation{Westward}{Westw}
\DefineJournalWordException{Westwater}{Westwater}
\DefineJournalWordException{Wetaskiwin}{Wetaskiwin}
\DefineJournalWordException{Wether}{Wether}
\DefineJournalPartialAbbreviation{Wetland}{Wetl}
\DefineJournalWordException{Wexford}{Wexford}
\DefineJournalAbbreviation{Weybridge}{Weybr}
\DefineJournalWordException{Weyerhaeuser}{Weyerhaeuser}
\DefineJournalAbbreviation{Whaling}{Whal}
\DefineJournalAbbreviation{Wharton}{Whart}
\DefineJournalAbbreviation{Wheatgrower}{Wheatgrow}
\DefineJournalWordException{Wheaton}{Wheaton}
\DefineJournalPartialAbbreviation{Wheel}{Wheel}
\DefineJournalWordException{Wheelchair}{Wheelchair}
\DefineJournalWordException{Wheelspin}{Wheelspin}
\DefineJournalWordException{Whippet}{Whippet}
\DefineJournalWordException{Whiskey}{Whiskey}
\DefineJournalAbbreviation{Whisper}{Whisp}
\DefineJournalWordException{Whistle}{Whistle}
\DefineJournalWordException{Whitakers}{Whitakers}
\DefineJournalWordException{White}{White}
\DefineJournalWordException{White-Plains}{White-Plains}
\DefineJournalWordException{Whitebread}{Whitebread}
\DefineJournalWordException{Whitecourt}{Whitecourt}
\DefineJournalWordException{Whitehaven}{Whitehaven}
\DefineJournalWordException{Whitehorse}{Whitehorse}
\DefineJournalWordException{Whitespruce}{Whitespruce}
\DefineJournalWordException{Whitetail}{Whitetail}
\DefineJournalWordException{Whitford}{Whitford}
\DefineJournalWordException{Whitsunday}{Whitsunday}
\DefineJournalAbbreviation{Wholeness}{Wholen}
\DefineJournalPartialAbbreviation{Wholesal}{Wholes}
\DefineJournalPartialAbbreviation{Wholistic}{Wholist}
\DefineJournalWordException{Wiccan}{Wiccan}
\DefineJournalWordException{Wichita}{Wichita}
\DefineJournalWordException{Wicked}{Wicked}
\DefineJournalWordException{Wicker}{Wicker}
\DefineJournalPartialAbbreviation{Wicker}{Wicker}
\DefineJournalWordException{Wicket}{Wicket}
\DefineJournalWordException{Wiggins}{Wiggins}
\DefineJournalAbbreviation{Wildbiologie}{Wildbiol}
\DefineJournalWordException{Wildbird}{Wildbird}
\DefineJournalWordException{Wilderness}{Wilderness}
\DefineJournalWordException{Wildfire}{Wildfire}
\DefineJournalWordException{Wildfowl}{Wildfowl}
\DefineJournalWordException{Wildland}{Wildland}
\DefineJournalAbbreviation{Wildlife}{Wildl}
\DefineJournalWordException{Wildnecote}{Wildnecote}
\DefineJournalAbbreviation{Williamsburg}{Williamsbg}
\DefineJournalWordException{Willmore}{Willmore}
\DefineJournalWordException{Willoughby}{Willoughby}
\DefineJournalAbbreviation{Willow Grove}{Will Grove}
\DefineJournalWordException{Willowdale}{Willowdale}
\DefineJournalAbbreviation{Wiltshire}{Wilts}
\DefineJournalWordException{Wimborne}{Wimborne}
\DefineJournalWordException{Winchelsea}{Winchelsea}
\DefineJournalAbbreviation{Winchester}{Winch}
\DefineJournalWordException{Winchmore}{Winchmore}
\DefineJournalPartialAbbreviation{Wind}{Wind}
\DefineJournalAbbreviation{Windfall}{Windf}
\DefineJournalAbbreviation{Windletter}{Windl}
\DefineJournalWordException{Windmill}{Windmill}
\DefineJournalWordException{Window}{Window}
\DefineJournalWordException{Windsor}{Windsor}
\DefineJournalWordException{Windsport}{Windsport}
\DefineJournalPartialAbbreviation{Windsurf}{Windsurf}
\DefineJournalWordException{Wineglass}{Wineglass}
\DefineJournalPartialAbbreviation{Winemak}{Winemak}
\DefineJournalPartialAbbreviation{Winer}{Winer}
\DefineJournalWordException{Winery}{Winery}
\DefineJournalAbbreviation{Winesburg}{Winesbg}
\DefineJournalWordException{Winfield}{Winfield}
\DefineJournalWordException{Wingecarribee}{Wingecarribee}
\DefineJournalWordException{Wingspan}{Wingspan}
\DefineJournalAbbreviation{Winner}{Win}
\DefineJournalAbbreviation{Winning}{Win}
\DefineJournalAbbreviation{Winnipeg}{Winn}
\DefineJournalAbbreviation{Winston}{Winst}
\DefineJournalAbbreviation{Winston-Salem}{Winston-Sal}
\DefineJournalWordException{Winter}{Winter}
\DefineJournalAbbreviation{Wireless}{Wirel}
\DefineJournalWordException{Wiring}{Wiring}
\DefineJournalAbbreviation{Wisconsin}{Wis}
\DefineJournalWordException{Wisdom}{Wisdom}
\DefineJournalPartialAbbreviation{Witch}{Witch}
\DefineJournalWordException{Witchblade}{Witchblade}
\DefineJournalWordException{Witham}{Witham}
\DefineJournalPartialAbbreviation{Withhold}{Withhold}
\DefineJournalWordException{Without}{Without}
\DefineJournalWordException{Witlin}{Witlin}
\DefineJournalPartialAbbreviation{Witness}{Witn}
\DefineJournalWordException{Wiveliscombe}{Wiveliscombe}
\DefineJournalWordException{Wokingham}{Wokingham}
\DefineJournalPartialAbbreviation{Wolfkeep}{Wolfkeep}
\DefineJournalAbbreviation{Wolfville}{Wolfv}
\DefineJournalWordException{Wollongong}{Wollongong}
\DefineJournalAbbreviation{Wolverhampton}{Wolverh}
\DefineJournalAbbreviation{Wolverine}{Wolver}
\DefineJournalWordException{Wolves}{Wolves}
\DefineJournalWordException{Woman}{Woman}
\DefineJournalWordException{Womanly}{Womanly}
\DefineJournalWordException{Wombat}{Wombat}
\DefineJournalWordException{Women}{Women}
\DefineJournalWordException{Wonder}{Wonder}
\DefineJournalWordException{Wonderful}{Wonderful}
\DefineJournalAbbreviation{Woodbrooker}{Woodbrook}
\DefineJournalAbbreviation{Woodcarver}{Woodcarv}
\DefineJournalWordException{Woodcock}{Woodcock}
\DefineJournalWordException{Woodcraft}{Woodcraft}
\DefineJournalWordException{Wooden}{Wooden}
\DefineJournalWordException{Woodfield}{Woodfield}
\DefineJournalAbbreviation{Woodland}{Woodl}
\DefineJournalWordException{Woodpulp}{Woodpulp}
\DefineJournalWordException{Woods-Hole}{Woods-Hole}
\DefineJournalWordException{Woodstock}{Woodstock}
\DefineJournalAbbreviation{Woodturner}{Woodturn}
\DefineJournalWordException{Woodwind}{Woodwind}
\DefineJournalPartialAbbreviation{Woodwork}{Woodwork}
\DefineJournalAbbreviation{Woolgrower}{Woolgrow}
\DefineJournalAbbreviation{Woolhandler}{Woolhandl}
\DefineJournalAbbreviation{Woollen}{Wool}
\DefineJournalAbbreviation{Worcester}{Worcest}
\DefineJournalAbbreviation{Worcestershire}{Worcs}
\DefineJournalWordException{Wordperfect}{Wordperfect}
\DefineJournalWordException{Wordsearch}{Wordsearch}
\DefineJournalPartialAbbreviation{Work}{Work}
\DefineJournalWordException{Workboard}{Workboard}
\DefineJournalAbbreviation{Workbook}{Workb}
\DefineJournalWordException{Workbox}{Workbox}
\DefineJournalWordException{Workbridge}{Workbridge}
\DefineJournalWordException{Workforce}{Workforce}
\DefineJournalAbbreviation{Workgroup}{Workgr}
\DefineJournalAbbreviation{Workhouse}{Workh}
\DefineJournalWordException{Worklife}{Worklife}
\DefineJournalPartialAbbreviation{Workload}{Workload}
\DefineJournalAbbreviation{Workman}{Workm}
\DefineJournalWordException{Workout}{Workout}
\DefineJournalAbbreviation{Workpaper}{Workp}
\DefineJournalWordException{Workplace}{Workplace}
\DefineJournalWordException{Worksafe}{Worksafe}
\DefineJournalAbbreviation{Worksetting}{Worksett}
\DefineJournalAbbreviation{Worksheet}{Worksh}
\DefineJournalWordException{Workshop}{Workshop}
\DefineJournalWordException{Worksite}{Worksite}
\DefineJournalAbbreviation{Workstation}{Workstn}
\DefineJournalWordException{World}{World}
\DefineJournalWordException{Worldover}{Worldover}
\DefineJournalWordException{Worldport}{Worldport}
\DefineJournalAbbreviation{Worldtrade}{Worldtr}
\DefineJournalAbbreviation{Worldwide}{Worldw}
\DefineJournalAbbreviation{Worship}{Worsh}
\DefineJournalAbbreviation{Worshipful}{Worshipf}
\DefineJournalWordException{Worthing}{Worthing}
\DefineJournalAbbreviation{Worthwhile}{Worthw}
\DefineJournalWordException{Wound}{Wound}
\DefineJournalAbbreviation{Wrapping}{Wrap}
\DefineJournalPartialAbbreviation{Wreck}{Wreck}
\DefineJournalPartialAbbreviation{Wrestl}{Wrestl}
\DefineJournalPartialAbbreviation{Writer}{Writ}
\DefineJournalAbbreviation{Writing}{Writ}
\DefineJournalAbbreviation{Written}{Writ}
\DefineJournalWordException{Wrongful}{Wrongful}
\DefineJournalWordException{Wrought}{Wrought}
\DefineJournalWordException{Wycliffe}{Wycliffe}
\DefineJournalAbbreviation{Wyoming}{Wyo}
\DefineJournalPartialAbbreviation{Xenobiochemi}{Xenobiochem}
\DefineJournalAbbreviation{Xenophobia}{Xenophob}
\DefineJournalWordException{Xeranthemum}{Xeranthemum}
\DefineJournalPartialAbbreviation{Xerograph}{Xerogr}
\DefineJournalWordException{Xodic}{Xodic}
\DefineJournalAbbreviation{Yachting}{Yacht}
\DefineJournalAbbreviation{Yachtsman}{Yachtsm}
\DefineJournalWordException{Yancey}{Yancey}
\DefineJournalAbbreviation{Yankee}{Yank}
\DefineJournalWordException{Yardbird}{Yardbird}
\DefineJournalWordException{Yarmouth}{Yarmouth}
\DefineJournalAbbreviation{Year book}{Year b}
\DefineJournalWordException{Year-end}{Year-end}
\DefineJournalPartialAbbreviation{Yearbook}{Yearb}
\DefineJournalAbbreviation{Yearling}{Yearl}
\DefineJournalAbbreviation{Yearly}{Yrly}
\DefineJournalWordException{Yellow}{Yellow}
\DefineJournalWordException{Yellowhead}{Yellowhead}
\DefineJournalWordException{Yellowknife}{Yellowknife}
\DefineJournalWordException{Yemen}{Yemen}
\DefineJournalWordException{Yenching}{Yenching}
\DefineJournalPartialAbbreviation{Yeoman}{Yeom}
\DefineJournalWordException{Yesterday}{Yesterday}
\DefineJournalAbbreviation{Yesteryear}{Yestery}
\DefineJournalAbbreviation{Yidise}{Yid}
\DefineJournalPartialAbbreviation{Yodel}{Yodel}
\DefineJournalWordException{Yogurt}{Yogurt}
\DefineJournalPartialAbbreviation{Yonker}{Yonk}
\DefineJournalWordException{Yorker}{Yorker}
\DefineJournalAbbreviation{Yorkshire}{Yorks}
\DefineJournalWordException{Yoruba}{Yoruba}
%\DefineJournalPartialWordException{Young}{Young-}
\DefineJournalAbbreviation{Yourself}{Yours}
\DefineJournalWordException{Youth}{Youth}
\DefineJournalPartialAbbreviation{Yugoslav}{Yugosl}
\DefineJournalWordException{Yukon}{Yukon}
\DefineJournalPartialAbbreviation{Zair}{Zair}
%\DefineJournalPartialWordException{Zambez}{Zambez-}
\DefineJournalPartialAbbreviation{Zambi}{Zamb}
\DefineJournalWordException{Zaria}{Zaria}
\DefineJournalPartialAbbreviation{Zellkultur}{Zellkult}
\DefineJournalAbbreviation{Zetetic}{Zetet}
\DefineJournalAbbreviation{Zionism}{Zion}
\DefineJournalPartialAbbreviation{Zionist}{Zion}
\DefineJournalWordException{Zoning}{Zoning}
\DefineJournalWordException{Zoonoses}{Zoonoses}
\DefineJournalWordException{Zoonosis}{Zoonosis}
\DefineJournalWordException{Zoonotic}{Zoonotic}
\DefineJournalWordException{Zootomy}{Zootomy}
